Distributed Model Predictive Control for Dynamic Cooperation of Multi-Agent Systems

We propose a distributed model predictive control (MPC) framework for coordinating heterogeneous, nonlinear multi-agent systems under individual and coupling constraints. The cooperative task is encoded as a shared objective function minimized collectively by the agents. Each agent optimizes an artificial reference as an intermediate step towards the cooperative objective, along with a control input to track it. We establish recursive feasibility, asymptotic stability, and transient performance bounds under suitable assumptions. The solution to the cooperative task is not predetermined but emerges from the optimized interactions of the agents. We demonstrate the framework on numerical examples inspired by satellite constellation control, collision-free narrow-passage traversal, and coordinated quadrotor flight.

==> plotdata/narrow_path/position_A1.tex <==
x y
-20.0 0.0
-20.0 0.0
-19.750000000001222 -9.030126646436543e-11
-19.250000000003308 -1.7100626470423208e-10
-18.500000000005603 -1.7542384211921558e-10
-17.50000000003069 -1.5547924059333695e-10
-16.500000000030976 -1.9931359340752408e-10
-15.500000000078895 -1.4625706201698563e-10
-14.500000000124414 -1.1011605516308975e-10
-13.500000000178856 -7.924130795977646e-11
-12.500000000178934 -9.593675853736272e-11
-11.500000000179039 -7.769682119906918e-11
-10.500000000179195 1.619163136901136e-10
-9.500000000179464 1.0872294731179011e-10
-8.500000000189758 1.1211531703025912e-10
-7.500000000226342 1.2095127677191897e-10
-6.5000000002269385 1.0542244854860883e-10
-5.500000000229165 9.78394310013897e-11
-4.50000000023537 9.431350145305828e-11
-3.500000000235624 8.455183775346597e-11
-2.5000000002585923 8.529488226827198e-11
-1.5000000002619884 7.486172792781076e-11
-0.5000000002639416 7.359962639341688e-11
0.4999999997359441 7.156515380302153e-10
1.2705706037889937 3.013622267566962e-06
1.8096811908949462 0.055971519964106486
2.147658835693563 0.1401673248097131
2.3710856654423083 0.1486933147984427
2.491287157618368 0.14780848142456374
2.588022152690803 0.14836519819450086
2.686318070228135 0.1492650149471809
2.787343816869084 0.1497594164145652
2.8890210318606813 0.14993353400344114
2.990606659763125 0.14998159676064524
3.0920997832704313 0.14999560666437473
3.193577226190228 0.1500007947813841
3.295061189132099 0.1500014491027317
3.3965506546709974 0.14999889176048098
3.4980466581553147 0.14999851548971802
3.599562474702728 0.15001128109177297
3.7011016163093964 0.15003497329456508
3.8026229453163207 0.15002000766215595
3.9040843606861957 0.14995315688879787
4.005690318852573 0.15008417251322204
4.107174062471284 0.14999640010666404
4.208719201165157 0.1500325827865619
4.310255795947204 0.15003703388221107
4.411794862575588 0.15004227749612797
4.5133336442861145 0.15005097309395143
4.614875250148352 0.15006102805809873
4.716416763235876 0.15007253667375514
4.817957434226835 0.15008591859181292
4.919496481569505 0.1501014417130908
5.021032558265617 0.15011937089275385
5.122564167273997 0.15014001684992395
5.2240897325176165 0.15016372703307157
5.325607336647563 0.15019088377572504
5.427114869088109 0.15022190801743535
5.528609947506983 0.1502572609611056
5.630089846382352 0.1502974516389477
5.731551409938845 0.15034303778998165
5.832991284415867 0.15039462875825904
5.934405500749698 0.15045289171417142
6.035789821665423 0.15051854806667708
6.1371393765012225 0.15059238507850314
6.238448931530491 0.1506752601473471
6.33971239340447 0.15076810249142653
6.4409234522298195 0.15087191975991343
6.542074839787824 0.15098780032228887
6.643159848780633 0.15111692275162947
6.74416928678111 0.15126055469979932
6.845093009532716 0.15142006142210312
6.945920267508409 0.15159691172885487
7.046639401978965 0.15179268183730066
7.14723747286293 0.1520090628009313
7.247700871579156 0.15224785972955596
7.348014753257039 0.15251101092532104
7.4481628094002925 0.1528005772863839
7.548126684674166 0.15311875033434075
7.647889177637017 0.15346787691082275
7.747431030846783 0.15385043931573567
7.846730870918792 0.15426907010444407
7.945765882216775 0.1547265641201226
8.044511740858477 0.15522589091416367
8.142942659753496 0.15577018119754132
8.241031410561558 0.15636272811093005
8.338749016795456 0.15700700721678157
8.436064874634983 0.15770666915511355
8.532946945391926 0.15846554595614815
8.62936164684773 0.15928765501353104
8.725274257920168 0.16017720818026238
8.820648250355653 0.1611386104423017
8.915443911190179 0.16217644149611282
9.009621037738729 0.1632954877026762
9.103139502925739 0.16450075309003886
9.195956268024192 0.16579742407751824
9.288028342042445 0.16719091224077381
9.379311222612849 0.16868683775347842
9.469760177835397 0.17029105452901133
9.55932995563461 0.17200964936080404
9.647974965273821 0.17384897071873268
9.735649436066439 0.17581563547635082
9.82230759777377 0.17791656394264305
9.907903651773092 0.18015900757398007
9.992391504744978 0.18255077246993778
10.075723021928122 0.18510196210225344
10.157852433102132 0.18781864427804024
10.238728806665259 0.1907102086857162
10.31829667662326 0.19378526906962001
10.3964896244811 0.19705351137419846
10.473220851341836 0.20052650561025104
10.548367577276311 0.20421543992855468
10.621739296525789 0.20812270247616327
10.692988230902563 0.21224723085891545
10.761366266281247 0.21657772000492714
10.82468977667614 0.22100859313043553
11.138013287060048 0.19078920815463046
11.701336797416491 0.13286534895425367
12.514660307767826 0.0929511779583212
13.514660307767 0.06129821849208633
14.51466030776137 0.037468909697317754
15.51466030771296 0.020289516858135903
16.514660307712802 0.008930338561752571
17.51466030766595 0.0024255471665006745
18.514660307600437 0.00016612309639585376
19.290926153014748 -9.678490565495634e-05
19.81719200491975 -3.748010434317939e-05
20.093457865438396 -4.924073255002659e-06
20.119723778695416 8.272502339812249e-07
20.028568686480753 5.289445543510407e-07
20.001017885177827 1.0154770729853269e-07
19.99858960906709 -2.537826421233902e-09
19.999537325325463 -6.793193729759395e-09
19.999952051499864 -1.8305189308787106e-09
20.000013870382695 -1.6034654160002049e-10
20.000006781664766 -3.1558865798420044e-09
20.00000101664362 -8.604939372158782e-09
19.99999973432443 -1.4601696435301292e-08
19.99999970349886 -1.7973786681224624e-08
19.9999998999637 -6.5025369255788945e-09
19.999999988767975 -8.069399315413506e-10
20.000000001893024 1.3698012168994467e-10
20.00000000084066 7.09139413856974e-11
19.99999999974991 -1.33234256960435e-11
19.999999999640337 -3.94660970570726e-11
19.999999999729642 -4.111636031645105e-11
19.999999999577092 -5.3604121141859196e-11
19.999999989829867 -1.1798127474982323e-09
19.999999990558326 -1.522783898977309e-09
19.999999985033583 -3.4053970476843887e-09
19.999999944637402 -8.174761256807273e-09
19.999999973045586 -4.032294026456995e-09
19.999999959298908 -4.253716573421329e-09
19.99999989313495 -9.848731524764176e-09
19.999999878539178 -1.106154737251508e-08
19.999999897869614 -9.262891703665233e-09
19.99999991094102 -8.094098169486585e-09
19.99999992974873 -6.348379960607886e-09
19.999999962284587 -3.168147355570028e-09
19.999999953072663 -3.9406446716849786e-09
19.999999973012827 -1.7965258169994058e-09


==> plotdata/narrow_path/position_A2.tex <==
x y
20.0 0.0
20.0 0.0
19.750000000395872 2.3791524306204792e-11
19.250000000792543 1.8447243732566676e-11
18.500000001264898 -3.774691670344055e-11
17.66308509568119 -1.305835162224156e-10
16.83582471378449 -1.6886447795627646e-10
16.00794537137769 -1.1316955705886755e-10
15.180103916173842 -1.1415468570419307e-10
14.352260019237516 -1.4215681409801562e-10
13.52441630051958 -1.6396917157379676e-10
12.6965726756069 -1.491398393671517e-10
11.868728983366172 -1.2628365020361798e-10
11.040885244190855 -1.1595466253844222e-10
10.21304150493823 -1.0795128679852439e-10
9.385197872576962 -9.527603705983267e-11
8.557354212162958 -9.499676045798822e-11
7.729510591172112 -9.023978786437681e-11
6.901667003279826 -8.454328903617636e-11
6.073823408852499 -7.687331327055347e-11
5.245979793284437 -7.403555546403595e-11
4.418136217877439 -6.436959298916634e-11
3.5902935979706645 -3.4927671865858656e-11
2.9581481657581867 -6.948076003432391e-10
2.576002733124113 -3.0632936113828e-06
2.4438573003379487 -0.05608208781857016
2.5617118665327414 -0.14012139584418273
2.776699370524707 -0.14873836090523412
2.9030038788197983 -0.1478437915498583
3.001497955612218 -0.1483771372842577
3.099372062891963 -0.14926859433061124
3.1998977038931873 -0.1497620576275346
3.3013674499612704 -0.14993659582649727
3.402896275608713 -0.14998521413250668
3.5043738707638674 -0.14999997874874105
3.605843750393367 -0.15000614003319448
3.707323129230932 -0.1500079369933467
3.8088102203392578 -0.15000666961075107
3.9103021362964725 -0.1500078435595683
4.011803639535434 -0.15002276778623783
4.113317000721722 -0.1500494105285354
4.21483177382949 -0.15003690713547144
4.316371560529103 -0.14997093043815127
4.4178307864374045 -0.15010942783187484
4.519395693047378 -0.1500229380679425
4.620896878915269 -0.15006501353518734
4.722419183109935 -0.15007489348492567
4.823942390131598 -0.15008638426072657
4.925460585076859 -0.150102291658098
5.026978869665398 -0.15012053823775803
5.1284940144512445 -0.1501413271416042
5.230004668633243 -0.15016520608757372
5.3315095716185965 -0.15019257348369633
5.433006875314076 -0.15022383451231364
5.534494512502449 -0.15025945268697746
5.63597027336135 -0.15029994058139684
5.7374315474030775 -0.15034585874834538
5.838875461226058 -0.1503978199649253
5.940298791320842 -0.15045649199285924
6.0416978983971505 -0.15052260567559642
6.143068628079823 -0.15059695680038845
6.244406529042246 -0.15068040966569315
6.345706445035724 -0.1507739044239495
6.446962822975751 -0.1508784543657284
6.548169370318172 -0.1509951580088968
6.64931930535414 -0.15112520477849012
6.750404858203031 -0.15126987729396288
6.85141788830354 -0.15143055939757477
6.952349148568356 -0.1516087387586886
7.053189757979374 -0.15180601869167443
7.153928223088895 -0.15202411572138028
7.254551881324171 -0.152264869990291
7.355047248108423 -0.15253025228350545
7.455399708977803 -0.15282236908784932
7.55559313749216 -0.1531434698600632
7.65561044702581 -0.15349594735791997
7.7554330671463845 -0.15388235795837385
7.855040645189783 -0.15430541041924808
7.954410465803753 -0.1547679735747947
8.053520546166272 -0.15527310610137512
8.152346499488674 -0.15582403216674656
8.250861414883692 -0.1564241559818279
8.349036477843192 -0.15707707382822833
8.44684090214786 -0.1577865851665262
8.544241879844188 -0.15855667804939758
8.641204541941327 -0.15939152801584702
8.737691647145057 -0.1602955143642515
8.833663603238861 -0.1612732090444033
8.9290785837835 -0.1623293781628771
9.023892348378494 -0.1634689794010324
9.118058542701986 -0.16469716384085026
9.211527959284416 -0.16601926155903643
9.304247109146175 -0.16744074377066387
9.396160606461137 -0.16896724749662204
9.487211598023343 -0.17060456740069527
9.57733879335587 -0.17235858188469186
9.666478955486161 -0.17423527373996017
9.754565267513435 -0.17624066519756365
9.841528193792733 -0.17838079530982512
9.927294876118449 -0.18066164996904815
10.011788902942909 -0.18308910767856995
10.094929902886586 -0.18566883663524206
10.176633109345264 -0.18840619264855585
10.256808532595699 -0.19130606578619946
10.335360059707728 -0.19437286718729416
10.412185431717706 -0.19761195808477433
10.487167763687324 -0.20102291955726853
10.560178987552431 -0.20460630611108982
10.631070944425023 -0.20835879996675707
10.69966855059907 -0.21227393897655744
10.765757052868734 -0.21634134730516275
10.829057570559266 -0.22054209924613016
10.889178738276959 -0.22483656134110266
10.945531294485974 -0.229163452076271
10.997092597347107 -0.23342114003669137
11.04145968049496 -0.23735575857841348
10.835826763686503 -0.20759212323720153
10.380193847007158 -0.1738036574350176
9.674560930329378 -0.1612365858057312
8.83252253997218 -0.1551985316189186
8.005600323256754 -0.1480291008328935
7.17770872985373 -0.14118803572042918
6.349875306592462 -0.13443144921034306
5.522038157738924 -0.12780068262660563
4.694200994803746 -0.1212910954535712
3.866363530057181 -0.11490547637107618
3.038526830506988 -0.10864553698620136
2.21068956219652 -0.10251327346712094
1.3828513840425922 -0.09651075554853428
0.5550130082029182 -0.09064017092202376
-0.2728255655993528 -0.0849038364239599
-1.1006643107914589 -0.0793042075433561
-1.9285033580451518 -0.07384389556808249
-2.7563423598939547 -0.06852568282284272
-3.584181605230125 -0.0633525449628487
-4.4120213672387685 -0.05832767617403156
-5.239861044255754 -0.05345451053979497
-6.067700796350551 -0.048736761677942136
-6.895541122513404 -0.04417846289479396
-7.723383060310928 -0.03978398522621068
-8.551223645019654 -0.03555820166861276
-9.379064555925384 -0.031506438871688636
-10.206905639446264 -0.027634609717920117
-11.034746959334894 -0.023949371989277518
-11.862588397610601 -0.02045826733332129
-12.69042992161249 -0.01716994669093716
-13.518271368795228 -0.014094477454951237
-14.346112456211088 -0.011243783970451532
-15.173953228242627 -0.008632311306647239
-16.00179312410784 -0.006278075131914002
-16.82963173165029 -0.0042044269952555835
-17.657463966419265 -0.0024432810711239317
-18.485260311417882 -0.0010414887887413293
-19.26558897066092 -0.00016242505075370062
-19.795917654731316 1.3477837047998209e-05
-20.076246368733422 1.3263565443566439e-05
-20.106576560564587 2.970664950058266e-06
-20.025837852137176 7.241526267520726e-08
-20.001183686748032 -1.4301840953190315e-07
-19.998885535290146 -4.18258390699755e-08
-19.999654817771226 -3.374262230737557e-09


==> plotdata/quadrotor/A1_x1_phase1.tex <==
0 -1.5
1 -1.5
2 -1.5
3 -1.5
4 -1.4982770723171797
5 -1.492931091019829
6 -1.4825495939780815
7 -1.4663232776343826
8 -1.4439747482330005
9 -1.4158807437671102
10 -1.3828033237816244
11 -1.345647569843869
12 -1.3053109156008724
13 -1.262754398029557
14 -1.2191684820731705
15 -1.1760530537483873
16 -1.1351097026242452
17 -1.0980414723640797
18 -1.0662853624972635
19 -1.0407475587416366
20 -1.0215842447482972
21 -1.0082968950360378
22 -1.0000561790859732
23 -0.9958844059526654
24 -0.9946840129257841
25 -0.995211363577267
26 -0.9960198202389569
27 -0.9955392280572903
28 -0.9921624619836243
29 -0.9843225808548742
30 -0.970535296071677
31 -0.9494880968085745
32 -0.9200809146474693
33 -0.8814852101719683
34 -0.8331802163339422
35 -0.774995243666864
36 -0.7071748466267831
37 -0.6303906381289075
38 -0.5457339453778802
39 -0.4546987379191218
40 -0.3591254248438971
41 -0.26119734171731035
42 -0.1634251860697592
43 -0.06865068340628261
44 0.019983747847656427
45 0.09946121419950728
46 0.16691538759931776
47 0.21972461573687324
48 0.2555833505520554
49 0.2726747339955043
50 0.27025393472914944
51 0.24869420877961426
52 0.2090978654010871
53 0.1526138283835104
54 0.08128101614611803
55 -0.002244496433243967
56 -0.09472590103226476
57 -0.19143583585981433
58 -0.2875791095479533
59 -0.3787712110774216
60 -0.46116656634723957
61 -0.5314555649319186
62 -0.5868269923617043
63 -0.6269800812461533
64 -0.6543682751909526
65 -0.6726478695115324
66 -0.6854266580082243
67 -0.6959275303014164
68 -0.7070247022553757
69 -0.7212915224257536
70 -0.7406325943254802
71 -0.766307687524967
72 -0.798717774457698
73 -0.8373783945689676
74 -0.8809936768652741
75 -0.9274761644664841
76 -0.9741166558056823
77 -1.0179231827885213
78 -1.0558831063676732
79 -1.0851462567135324
80 -1.103090395036025
81 -1.1074411081637745
82 -1.0963230229217318
83 -1.0683755365970469
84 -1.022808852332051
85 -0.9594665005230391
86 -0.8788740502649803
87 -0.7821923685775165
88 -0.6711413413637121
89 -0.5480490597897375
90 -0.41637211450085565
91 -0.2809126336768485
92 -0.14639993775656865
93 -0.017085501625028504
94 0.10332845983673342
95 0.2116510555650421
96 0.30514119261760464
97 0.38144363508958595
98 0.4385318649720997
99 0.4746568334640471
100 0.4883164928782111
101 0.4782320845280248
102 0.44332268691911736
103 0.38268278537331085
104 0.2984290611864458
105 0.19663939348245207
106 0.08382960930449347
107 -0.03405839049315945
108 -0.15185380146813376
109 -0.26511986451132735
110 -0.3700613659062243
111 -0.4634354369580124
112 -0.5424756833447746
113 -0.6048254999648978
114 -0.6484752545304457
115 -0.6772530991854042
116 -0.6968119905499965
117 -0.7127439569849492
118 -0.7300348633190765
119 -0.752966181158011
120 -0.7851644718725688
121 -0.8285204018915469
122 -0.8830297365088527
123 -0.9471645955439384
124 -1.0181223710655511
125 -1.0914701878823971
126 -1.1627102740927837
127 -1.2277489821464547
128 -1.2829990848719535
129 -1.32536415542646
130 -1.3521877615909303
131 -1.3611960979858662
132 -1.350446845559903
133 -1.3182859061784564
134 -1.2633064945119918
135 -1.1843115106360165
136 -1.080277654837383
137 -0.9525707364913404
138 -0.8069948649592121
139 -0.6498826595154348
140 -0.4869210572555075
141 -0.32309430485780655
142 -0.1628835369674558
143 -0.010210137471776987
144 0.13153408112032017
145 0.25943245028951456
146 0.37098665970778494
147 0.4640621384697956
148 0.5368403806224984
149 0.5877835569563092
150 0.6155967187655957
151 0.6191916358209691
152 0.5976539030953552
153 0.5502128063546978
154 0.47621474129515606
155 0.380029159364701
156 0.26827069289261185
157 0.1474584895584463
158 0.023395569102780192
159 -0.09891869056382915
160 -0.21522443758897322
161 -0.3219029305031124
162 -0.41587718661839485
163 -0.4945210626496984
164 -0.5558681928377541
165 -0.6023427321114843
166 -0.6391867372354865
167 -0.6719282899921448
168 -0.7056252868567943
169 -0.7447007547996404
170 -0.792962299453863
171 -0.8536717445674533
172 -0.9275086218278039
173 -1.0103973989973085
174 -1.0972721351239791
175 -1.1832806960586395
176 -1.2641070880235907
177 -1.3360111442701623
178 -1.395775788670625
179 -1.4406378764513386
180 -1.468218088805361
181 -1.4764586026364352
182 -1.4635598996041181
183 -1.4279238061590807
184 -1.3681408905889059
185 -1.282988175653598
186 -1.1714394597305207
187 -1.0330312436383071
188 -0.8729213076894105
189 -0.6973066228135607
190 -0.5119177679776269
191 -0.3216134976804622
192 -0.13025355843607841
193 0.05918860425861336
194 0.24423304444203528
195 0.4226693102008888
196 0.5924066225722499
197 0.7514887653512247
198 0.8980934497575211
199 1.030514635999857
200 1.1470483142248018
201 1.2460619654886051
202 1.326069478032314
203 1.3857340116443901
204 1.4238620032726579
205 1.4393816457775033
206 1.431347384581318
207 1.3997925863715714
208 1.346405758416234
209 1.2734588663417314
210 1.1832504984319252
211 1.0780080993555183
212 0.9599678362221362
213 0.8314997476876428
214 0.694932358157485
215 0.54878637752846
216 0.39066659114405977
217 0.21831505276567562
218 0.03389954723367236
219 -0.15773971318151586
220 -0.3515248716346282
221 -0.5430457196784684
222 -0.7282518648530133
223 -0.9035909696601445
224 -1.0659988233523832
225 -1.2128603499520916
226 -1.3419550538616705
227 -1.4514005993582004
228 -1.539598669862044
229 -1.6051908078910448
230 -1.6470258370779234
231 -1.6641363113708096
232 -1.655708526880948
233 -1.6210541960521807
234 -1.5595815515187337
235 -1.470780819925755
236 -1.3542172008265225
237 -1.2095244287945088
238 -1.0421334784639513
239 -0.8589943654212786
240 -0.6666974283390109
241 -0.4710227831624912
242 -0.275515287111264
243 -0.08074923192584779
244 0.1144968655964396
245 0.30980717097157984
246 0.5025934428117937
247 0.6894117878391878
248 0.8669040159894814
249 1.032060947773644
250 1.1822632318374964
251 1.3152522864914367
252 1.4290868436637751
253 1.5221017552482587
254 1.5928695800752932
255 1.6401685523608769
256 1.6629552227388882
257 1.6603404152128114
258 1.631569440504872
259 1.5760028245710045
260 1.4930988957326345
261 1.3823986902661218
262 1.2435130492351092
263 1.0807385403896448
264 0.9008436556263314
265 0.7105318411313907
266 0.5157760099942862
267 0.32092966753048624
268 0.12651913106441393
269 -0.06767174755497574
270 -0.2625464956472261
271 -0.45537500442918477
272 -0.6426000354819655
273 -0.8207608371534441
274 -0.986758734899896
275 -1.1379004753394664
276 -1.2718733661839554
277 -1.3867010655366279
278 -1.4806984449910903
279 -1.5524302430479797
280 -1.6006750816425308
281 -1.6243942876512434
282 -1.6227052576013168
283 -1.5948584070753462
284 -1.540217884898062
285 -1.4582444595105948
286 -1.3484816346780581
287 -1.2105434449329657
288 -1.0483940327438375
289 -0.8687493455099388
290 -0.6783425225216545
291 -0.4831940981972671
292 -0.2880902388748444
293 -0.09301077508576172
294 0.10163262396396933
295 0.2966917098878177
296 0.48978764313955414
297 0.677463757727621
298 0.8562748186354432
299 1.023109020607591
300 1.1752516666055868
301 1.310366617359052
302 1.4264546103580675
303 1.5218090519237841
304 1.594975221583218
305 1.6447144932716156
306 1.6699734190045987
307 1.6698570756695925
308 1.6436059258841544
309 1.590575918243935
310 1.5102212051398847
311 1.4020793721218663
312 1.26575910029173
313 1.1048646574078367
314 0.9260543639003262
315 0.7360963327472018
316 0.5410694397813052
317 0.34605890403178585
318 0.15105826331628638
319 -0.04314616446526895
320 -0.238137735853881
321 -0.43137189458818115
322 -0.6193164040072744
323 -0.7984840872718219
324 -0.9657355682905021
325 -1.1183365696676448
326 -1.2539367333367488
327 -1.3705269765967703
328 -1.4663942914035981
329 -1.5400801116831224
330 -1.5903437335276984
331 -1.6161307189376835
332 -1.616545510529954
333 -1.5908281115516538
334 -1.538333926260791
335 -1.4585165222193952
336 -1.350913022796086
337 -1.2151314644701945
338 -1.0546454162608343
339 -0.8760911769710725
340 -0.6862469812124413
341 -0.49120870299920855
342 -0.2961847983995568
343 -0.10116843242051055
344 0.09300795643593351
345 0.28802021776914843
346 0.4813464975345314
347 0.6694540164932588
348 0.8488481080752208
349 1.0163804216723504
350 1.1693080102804785


==> plotdata/quadrotor/A1_x1_phase2.tex <==
350 1.1693080102804785
351 1.3052725386937234
352 1.4222577166435022
353 1.5185442519473427
354 1.5944749718825741
355 1.6486704646556434
356 1.6793603397496095
357 1.6848230831556168
358 1.6635168842030696
359 1.6157037754002446
360 1.5447953392039697
361 1.4555476305348218
362 1.3526903987791288
363 1.2403418134359185
364 1.121878950391689
365 0.9999930330249133
366 0.876794018134857
367 0.7539134622228361
368 0.6325927437273402
369 0.5137549449482094
370 0.3980639271844798
371 0.28597462972667553
372 0.17777548462815151
373 0.0736241190470816
374 -0.026422519452824006
375 -0.12238260592579639
376 -0.2143298005444394
377 -0.3023753346561839
378 -0.3866552987834706
379 -0.4673213760102911
380 -0.5445324921285877
381 -0.6184488574653451
382 -0.6892285916617629
383 -0.7570251701266206
384 -0.8219857049496533
385 -0.8842500390642005
386 -0.9439503344176139
387 -1.001211057002022
388 -1.056149191184989
389 -1.1088746220064423
390 -1.1594905947344565
391 -1.2080942046500753
392 -1.2547769031554161
393 -1.2996142912924649
394 -1.3426600806000473
395 -1.383954280260285
396 -1.423531602457347
397 -1.4614290828322725
398 -1.497689861474899
399 -1.5323630598263567
400 -1.5654934178143818
401 -1.5971120716713496
402 -1.6272476200195636
403 -1.655938374185112
404 -1.683239895994887
405 -1.7092265731052483
406 -1.7339890006043261
407 -1.7576290453548358
408 -1.780254335087816
409 -1.8019715056383048
410 -1.8228801603704545
411 -1.8430687118023832
412 -1.862612767842579
413 -1.8815739006611085
414 -1.9000008376858757
415 -1.9179316475313535
416 -1.9353953045823813
417 -1.9524137580149818
418 -1.9690044093316221
419 -1.9851789126385586
420 -2.0009446126389725
421 -2.0163072330945013
422 -2.0312718895120194
423 -2.0458432530428374
424 -2.060020986004775
425 -2.0737975429881357
426 -2.0871616381364184
427 -2.100102028550562
428 -2.112609986898021
429 -2.1246803300277337
430 -2.136311737162212
431 -2.1475065089539505
432 -2.1582699989323415
433 -2.1686099942574564
434 -2.1785359951168366
435 -2.188058759696889
436 -2.1971902983639
437 -2.2059428794799762
438 -2.214328681712732
439 -2.2223595997750656
440 -2.230046953094461
441 -2.2374015371649008
442 -2.2444337980342075
443 -2.251153583004376
444 -2.2575700503245195
445 -2.2636917077870446
446 -2.2695262956635323
447 -2.2750809644725294
448 -2.280362260464094
449 -2.285376151694121
450 -2.290128097850088
451 -2.294622977472955
452 -2.298865081071311
453 -2.3028583088728594
454 -2.306606208394238
455 -2.310111934927506
456 -2.313378277512908
457 -2.3164076912710927
458 -2.319202283665699
459 -2.3217638901490525
460 -2.324093984507989
461 -2.326193822685946
462 -2.328064448686198
463 -2.329706753352372
464 -2.331121415359953
465 -2.332308944220298
466 -2.333269673029853
467 -2.3340037537359026
468 -2.334511130446393
469 -2.3347915679953837
470 -2.3348447260676797
471 -2.334670100204753
472 -2.3342670517078825
473 -2.3336347226833496
474 -2.3327721580455982
475 -2.3316783967497887
476 -2.330352331231515
477 -2.3287927331034517
478 -2.3269983188815524
479 -2.324967451290873
480 -2.3226984039507417
481 -2.320189159808653
482 -2.317437892191807
483 -2.3144427307936235
484 -2.3112016723280706
485 -2.307712497083267
486 -2.303972872748619
487 -2.299980302399148
488 -2.2957321257542818
489 -2.291225628859173
490 -2.2864578897565724
491 -2.281425847379454
492 -2.2761262683141497
493 -2.2705557053122907
494 -2.264710499922214
495 -2.258586818778275
496 -2.2521806548285648
497 -2.245487772032695
498 -2.2385037122926184
499 -2.231223791651278
500 -2.223643186610386
501 -2.2157567925847768
502 -2.207559302633756
503 -2.1990452185747666
504 -2.1902088168353355
505 -2.1810452676432424
506 -2.1715486628306815
507 -2.161709940493619
508 -2.1515161414339605
509 -2.140950694133742
510 -2.1299940960073758
511 -2.118625156106611
512 -2.1068223062801184
513 -2.094564932645607
514 -2.081835238260251
515 -2.0686197607916856
516 -2.054910293971008
517 -2.0407065068844883
518 -2.0260148290525666
519 -2.010841874247562
520 -1.9952177411602492
521 -1.9792050705422883
522 -1.9628716900774381
523 -1.9462695249794821
524 -1.929421055122521
525 -1.9123275063320115
526 -1.8949685490320354
527 -1.8773119979924857
528 -1.8593231983410776
529 -1.8409757758654037
530 -1.8222575279592883
531 -1.8031731213263837
532 -1.7837495460242343
533 -1.7640313908513465
534 -1.7440757120720933
535 -1.7239434553042856
536 -1.7036978074454057
537 -1.6834031771503493
538 -1.663118740950556
539 -1.6428967020128171
540 -1.6227798888498863
541 -1.6027997498293718
542 -1.5829779546277367
543 -1.5633268610762854
544 -1.5438515216953064
545 -1.524554111234696
546 -1.5054333625741378
547 -1.486487020482023
548 -1.467712555377468
549 -1.4491083112439638
550 -1.4306726982699145
551 -1.4124043113425686
552 -1.3943016814234213
553 -1.3763622238350226
554 -1.3585828422750714
555 -1.3409599525822027
556 -1.3234901773951306
557 -1.3061691613037998
558 -1.288994012023408
559 -1.2719587058933859
560 -1.2550560772951387
561 -1.238279069521492
562 -1.2216208208131702
563 -1.2050743393198042
564 -1.1886317300333502
565 -1.1722863839765256
566 -1.1560313798890427
567 -1.1398591833204361
568 -1.123761992780087
569 -1.1077322851256126
570 -1.091762919582508
571 -1.0758464116956514
572 -1.0599758080629158
573 -1.044144316116083
574 -1.0283453234134592
575 -1.0125723362615435
576 -0.9968187321316567
577 -0.981078459669053
578 -0.9653456090558248
579 -0.9496143679034799
580 -0.9338792423596807
581 -0.9181350543452533
582 -0.9023764236430983
583 -0.8865983601259996
584 -0.8707960081304279
585 -0.8549649137460085
586 -0.8391006981266592
587 -0.8231992743815556
588 -0.8072566422017958
589 -0.7912689929635627
590 -0.7752328107473787
591 -0.7591445466842788
592 -0.7430007844970467
593 -0.7267982305497809
594 -0.7105340449848561
595 -0.6942051729485571
596 -0.6778090291936923
597 -0.6613433813899303
598 -0.6448057468134579
599 -0.6281937282834192
600 -0.6115052404281045
601 -0.5947383205480771
602 -0.5778911666209182
603 -0.5609618373016984
604 -0.5439486077224671
605 -0.5268499966869957
606 -0.5096643066046304
607 -0.4923901093052639
608 -0.475026278108986
609 -0.45757153779801757
610 -0.44002479200215944
611 -0.4223850590981567
612 -0.40465149812515766
613 -0.38682310522711666
614 -0.3688989499631202
615 -0.35087821957379073
616 -0.3327601955339021
617 -0.3145442359667953
618 -0.2962298174763548
619 -0.27781642468988765
620 -0.25930355413676687
621 -0.24069073967726992
622 -0.22197753308363788
623 -0.20316353344475815
624 -0.18424837013200013
625 -0.16523170038939358
626 -0.1461131519521846
627 -0.1268924458952974
628 -0.10756935180997558
629 -0.08814371680849421
630 -0.0686154099061567
631 -0.048984228500874756
632 -0.029250025126234598
633 -0.009412936810235258
634 0.010527252845386529
635 0.030570450019121436
636 0.05071698951610784
637 0.07096683643259101
638 0.09131979077749716
639 0.11177575063471269
640 0.1323350739342977
641 0.15299793888155755
642 0.17376453956933308
643 0.194634630202346
644 0.215607875323965
645 0.23668418634546293
646 0.2578633689398237
647 0.2791453514853408
648 0.3005303767475592
649 0.3220183511941257
650 0.34360923128045984
651 0.3653027131315522
652 0.3870985160639682
653 0.4089965007397297
654 0.43099652442438113
655 0.453098448764594
656 0.4753021394452831
657 0.4976075308867785
658 0.5200142774592168
659 0.5425223388762833
660 0.5651315007684381
661 0.5878416661876296
662 0.6106526772336687
663 0.6335643091703125
664 0.6565763239713017
665 0.6796885062791765
666 0.7029006435797926
667 0.7262125767202392
668 0.749623781994588
669 0.7731340669199159
670 0.7967435775698861
671 0.8204521018887787
672 0.8442591423746115
673 0.8681640959802037
674 0.8921672657681344
675 0.9162683509155213
676 0.94046697006554
677 0.9647631804020921
678 0.9891566684359199
679 1.0136473448592287
680 1.0382349920324165
681 1.0629194725407853
682 1.0877005287562598
683 1.1125780125568183
684 1.1375513119013698
685 1.1626202290838334
686 1.1877846154166651
687 1.2130442907863335
688 1.238399185178862
689 1.2638492411218476
690 1.2893941670660707
691 1.315033639622109
692 1.3407672479454726
693 1.3665943440207544
694 1.3925150252643341
695 1.4185291934273494
696 1.4446367369639752
697 1.470837114568997
698 1.4971301538490631
699 1.5235155978803447
700 1.549993301531154


==> plotdata/quadrotor/A1_x2_phase1.tex <==
0 0.0
1 0.0
2 0.0
3 0.0
4 0.0006965796287211108
5 0.002961724890186292
6 0.007577303494566402
7 0.015151488485977905
8 0.026101351252102185
9 0.04067496723958497
10 0.05896998829929048
11 0.0809285182648421
12 0.10636718230001417
13 0.13496001872527963
14 0.1662288452872244
15 0.1993508826705403
16 0.23309739227751694
17 0.26588720639214725
18 0.29588367729799675
19 0.32111230372090244
20 0.3394820056006251
21 0.34896324414605234
22 0.3478913681360732
23 0.33513374229408394
24 0.31010415125392476
25 0.27267476220693765
26 0.22314823951036403
27 0.16223196801060674
28 0.09099070593133113
29 0.010776135684618285
30 -0.07686042598489105
31 -0.17019699339620947
32 -0.26737002018481526
33 -0.36640916297121373
34 -0.4652832726398451
35 -0.5619357184483382
36 -0.6543280117800824
37 -0.7404885995552675
38 -0.8185440391157286
39 -0.8867225224912033
40 -0.9433999228429235
41 -0.9871305432376104
42 -1.0166814177995356
43 -1.0310798008719064
44 -1.0296795372103487
45 -1.012217418570267
46 -0.9789179260168696
47 -0.9305511849570018
48 -0.8684697074206572
49 -0.7946333226322126
50 -0.7115615316498105
51 -0.6221548082786128
52 -0.5292455281249376
53 -0.4349683809921866
54 -0.3397751510091117
55 -0.24346300809176552
56 -0.1457479911001085
57 -0.04659782531524845
58 0.05357103881730475
59 0.15393566555512833
60 0.2532901273793141
61 0.3499874663005158
62 0.44202611943014114
63 0.5274062503502036
64 0.6045454164426869
65 0.6720122039236537
66 0.7283313604024985
67 0.7720248825666115
68 0.8017393485559619
69 0.816423879640793
70 0.815354431193695
71 0.7981776499818599
72 0.7647578070641742
73 0.715157158116388
74 0.6496755778594483
75 0.5689036220072249
76 0.47381617440520957
77 0.36576330548971997
78 0.24641878944437873
79 0.11770956638865926
80 -0.018217628751862835
81 -0.15903413075513526
82 -0.3022668834908134
83 -0.445368962022768
84 -0.5857833159134742
85 -0.7210162280777768
86 -0.8486939171267645
87 -0.9665742942215527
88 -1.0725264245125479
89 -1.164569507095825
90 -1.2408689166301479
91 -1.2997395252314456
92 -1.3396796852540864
93 -1.359407146662465
94 -1.3579334522978332
95 -1.3346508510506583
96 -1.289470055284401
97 -1.2229375829179976
98 -1.1363210812948246
99 -1.0316613041838902
100 -0.9117421776352674
101 -0.7799209591426499
102 -0.6396804582981346
103 -0.4940073253814845
104 -0.3444353851303606
105 -0.19210222690963766
106 -0.038321211150490586
107 0.11511876994832865
108 0.2658140826839038
109 0.4108874043968706
110 0.5473018024234417
111 0.6724883272305229
112 0.785383318797156
113 0.8856349998120944
114 0.9727493799809112
115 1.045904540151442
116 1.103926019413755
117 1.1454505039449545
118 1.1691313426079186
119 1.1738860898859502
120 1.1589745007118843
121 1.1240786728639571
122 1.0691704250908696
123 0.9945083594488581
124 0.9006829000668083
125 0.7886603368548648
126 0.6598487432626073
127 0.5160488941768662
128 0.35938939833544636
129 0.19228153332576928
130 0.01734533632586266
131 -0.16263989728797906
132 -0.34476501363218665
133 -0.526060069425699
134 -0.7035315459718074
135 -0.8740332272919853
136 -1.034411917843911
137 -1.1818113020556262
138 -1.3137389018648704
139 -1.428055773936602
140 -1.522927827774262
141 -1.5967521549766286
142 -1.6481497835785033
143 -1.6759368347024488
144 -1.6790967087734714
145 -1.6567561653769607
146 -1.6081656575845427
147 -1.5326835013471818
148 -1.4310400725316939
149 -1.305308620318033
150 -1.158647209792783
151 -0.9950343051113558
152 -0.8187811488870108
153 -0.6338899660577774
154 -0.44309220087310297
155 -0.24887721045149847
156 -0.05398647644453858
157 0.13897737520247094
158 0.3267137839696569
159 0.5058549887241532
160 0.6733319439891347
161 0.826453550539509
162 0.9637695280138724
163 1.085084637448159
164 1.1895431089652957
165 1.27605388535604
166 1.3433155083583292
167 1.389917469550051
168 1.4145109801601423
169 1.416058638911545
170 1.3939302529174205
171 1.3480062014607506
172 1.2785606698862113
173 1.186270672402006
174 1.0722721394547794
175 0.9382096677741376
176 0.7862994196456377
177 0.6192589319275774
178 0.4402329831599937
179 0.2526863558044542
180 0.060137217766029066
181 -0.13437844183520636
182 -0.3290619844071804
183 -0.5222165196469409
184 -0.7106500525798561
185 -0.8910281848123917
186 -1.0602878062328789
187 -1.215730432880168
188 -1.3550031979177906
189 -1.4760672107632042
190 -1.5771624470422168
191 -1.6567715633520115
192 -1.7135865372493968
193 -1.7464757302700233
194 -1.754460342007908
195 -1.736697366176034
196 -1.6924693151511006
197 -1.6211701789542745
198 -1.52229105330439
199 -1.395403742404564
200 -1.242906547603443
201 -1.0704580848822156
202 -0.884764253236139
203 -0.6921118209457029
204 -0.4975703467717061
205 -0.3032235618366321
206 -0.10932419977569477
207 0.08530837279149178
208 0.27909006841778433
209 0.46868568274949246
210 0.6505567175121868
211 0.8214439255636483
212 0.9784867555266805
213 1.119221364198096
214 1.241542933218235
215 1.3436605030045208
216 1.4240529823832877
217 1.4814287368576775
218 1.5146933092024812
219 1.522919472596764
220 1.5053212973104635
221 1.461232298312785
222 1.390087534528247
223 1.291408504096485
224 1.1647926162047655
225 1.0116212080609501
226 0.8381529791165627
227 0.6512980293130978
228 0.45739533574568136
229 0.261957478915127
230 0.06666912214070028
231 -0.1275908959018888
232 -0.322788445457442
233 -0.5175213526417063
234 -0.7084893535157145
235 -0.8921491465305198
236 -1.0652254625139599
237 -1.224835295368064
238 -1.3684867341237723
239 -1.4940409353192319
240 -1.5996677790410034
241 -1.683803496895838
242 -1.7451133049587728
243 -1.7824598666294826
244 -1.7948752239680106
245 -1.781536314869935
246 -1.7417437058477223
247 -1.6749034384723034
248 -1.580511242211062
249 -1.4581388820812082
250 -1.3084325680368596
251 -1.1375337168382216
252 -0.9524280202581865
253 -0.7595766553174695
254 -0.5646199543210043
255 -0.369681756934475
256 -0.17608985617752368
257 0.01883431195701793
258 0.21362273613411195
259 0.40490788369352754
260 0.5890813741529379
261 0.7628098385800165
262 0.9231619406890408
263 1.067607773101289
264 1.1939809001570885
265 1.300432660598805
266 1.385388156183979
267 1.4475076914710712
268 1.4856524919775165
269 1.4988554253542419
270 1.4862956325473327
271 1.4472768446121003
272 1.3812088898261128
273 1.2875916079382634
274 1.1660013925448325
275 1.0168955314175814
276 0.8463850804011813
277 0.6614719453182818
278 0.46864288891661876
279 0.2735628017555157
280 0.07851344295954851
281 -0.11518074410733825
282 -0.31019874077641113
283 -0.5051803083075634
284 -0.6967807255348942
285 -0.8813873686274484
286 -1.0556547532026126
287 -1.2166380719417176
288 -1.3617943501316114
289 -1.48894323788906
290 -1.5962219902165509
291 -1.6820424545759438
292 -1.7450526807666362
293 -1.784103645622227
294 -1.7982192718335845
295 -1.7865711101494635
296 -1.7484562318650054
297 -1.6832787866847938
298 -1.5905338945731637
299 -1.4697938523086709
300 -1.3213780332352456
301 -1.1513774776414265
302 -0.9668108515942901
303 -0.7741900847719636
304 -0.5792062516482634
305 -0.3842225777648429
306 -0.19057416383696735
307 0.004410295341012255
308 0.19939515028099752
309 0.3910359223447121
310 0.5757108699837673
311 0.7500630265099654
312 0.9111364186238745
313 1.0563788838487407
314 1.183604776027741
315 1.2909492218705918
316 1.3768241887176476
317 1.4398789021575147
318 1.4789655078938062
319 1.493109108004225
320 1.481482373864523
321 1.44338374284007
322 1.378218491482552
323 1.2854826266559192
324 1.1647495984950773
325 1.0163340433359345
326 0.846327007630776
327 0.6617481949440659
328 0.46911072347786664
329 0.27410624298519176
330 0.07910562221661932
331 -0.11456842400181677
332 -0.30956634895135415
333 -0.5045638968499493
334 -0.6962197765661344
335 -0.8809130335460558
336 -1.055286784569577
337 -1.2163850425253315
338 -1.3616555936137371
339 -1.488912768678228
340 -1.5962916773100215
341 -1.682204105138989
342 -1.745299076655182
343 -1.784428371171664
344 -1.7986166877139376
345 -1.7870364157240348
346 -1.7489854031247334
347 -1.683868385742954
348 -1.5911810216740756
349 -1.4704964868559978
350 -1.3221207590427606


==> plotdata/quadrotor/A1_x2_phase2.tex <==
350 -1.3221207590427606
351 -1.1521430350654736
352 -0.9675834334049727
353 -0.7749559193992261
354 -0.5804355166375816
355 -0.38948477825479233
356 -0.20682755447894716
357 -0.036517432781556
358 0.11797654928015991
359 0.2536889713774171
360 0.368086918159669
361 0.45901010022939304
362 0.5246345345628037
363 0.566106122399467
364 0.5866815469962265
365 0.590227675738565
366 0.5803663768435404
367 0.5601688663266828
368 0.5321270913184721
369 0.4982258988373127
370 0.4600355229600705
371 0.4187961319089661
372 0.37548652053100073
373 0.33087791043377196
374 0.2855760190407835
375 0.24005441430275495
376 0.19467982074719814
377 0.1497343079835897
378 0.10543157701186495
379 0.06192982892858134
380 0.019343289662187867
381 -0.022248592454487105
382 -0.06279436213605596
383 -0.10226477205907022
384 -0.14064794942500383
385 -0.17794558218359272
386 -0.21416973165961903
387 -0.24934034296645538
388 -0.2834831793141195
389 -0.31662818543448523
390 -0.34880817337771375
391 -0.3800577483731954
392 -0.41041247591006874
393 -0.4399057498610935
394 -0.46856310855994676
395 -0.49640183237787316
396 -0.5234332333996752
397 -0.5496675270957394
398 -0.5751170726734876
399 -0.5997967015701507
400 -0.623718145294686
401 -0.6468832866993038
402 -0.669291515119808
403 -0.6909486411589231
404 -0.7118730042716596
405 -0.7320969975625954
406 -0.7516654419667347
407 -0.7706323365367435
408 -0.7890572065674681
409 -0.8070005434666971
410 -0.8245196257681873
411 -0.8416656215687158
412 -0.8584824825334629
413 -0.8750056307211443
414 -0.8912625830365785
415 -0.9072744251129834
416 -0.9230564637883666
417 -0.9386195011284624
418 -0.9539717012815941
419 -0.9691166271302007
420 -0.9840541796781989
421 -0.9987832302253767
422 -1.0133024514492597
423 -1.0276106514514556
424 -1.041705559576125
425 -1.0555820965210578
426 -1.069232091556196
427 -1.0826455428863
428 -1.0958122659151024
429 -1.1087230629584517
430 -1.1213706285571752
431 -1.133749916202733
432 -1.145858083756729
433 -1.157694278425792
434 -1.169259155919278
435 -1.180554631521696
436 -1.191584294000873
437 -1.2023521875849499
438 -1.212862513172526
439 -1.2231194966721253
440 -1.2331270620615897
441 -1.2428889793410447
442 -1.252409208700783
443 -1.261691553741227
444 -1.270739521652885
445 -1.27955635853797
446 -1.2881448749194562
447 -1.2965076735855563
448 -1.3046471343280075
449 -1.312565391762485
450 -1.3202644311886202
451 -1.327745893811859
452 -1.3350109903864285
453 -1.3420609141511861
454 -1.3488968220888315
455 -1.3555196810163255
456 -1.3619303155708489
457 -1.368129388736575
458 -1.374117368276235
459 -1.3798946086524746
460 -1.3854610550988473
461 -1.390816777376248
462 -1.3959616109850705
463 -1.4008956211039096
464 -1.4056188870594983
465 -1.4101311741102454
466 -1.4144322694490907
467 -1.4185220678433133
468 -1.4224004623659046
469 -1.426067344219723
470 -1.4295224397755655
471 -1.4327653702508152
472 -1.435795656077738
473 -1.438612808530915
474 -1.4412162972500797
475 -1.4436055189676686
476 -1.4457798187264832
477 -1.4477385119273136
478 -1.4494809233140897
479 -1.4510063317704036
480 -1.4523139690971023
481 -1.4534029772902204
482 -1.4542725061947712
483 -1.4549216542883223
484 -1.455349524319143
485 -1.4555551225997356
486 -1.4555374318694771
487 -1.4552954278380568
488 -1.4548279966311284
489 -1.4541339976128995
490 -1.4532122520231867
491 -1.4520615517246351
492 -1.450680639793609
493 -1.4490681731245152
494 -1.447222719552417
495 -1.4451427783072868
496 -1.4428267852212944
497 -1.4402730813760074
498 -1.4374799108483145
499 -1.4344454165756104
500 -1.431167678673052
501 -1.4276446233224362
502 -1.4238740645158732
503 -1.4198536975964797
504 -1.4155811673831171
505 -1.4110777616011805
506 -1.4063846455834874
507 -1.4015453466361394
508 -1.3965947485623975
509 -1.3915547172546923
510 -1.3864333038182939
511 -1.3812258701355473
512 -1.37591641587863
513 -1.3704792977051872
514 -1.3648807455711123
515 -1.3590813810821698
516 -1.353039744397968
517 -1.3467095445560933
518 -1.3400472715679959
519 -1.3330334717758925
520 -1.3257177641149018
521 -1.3181566887609446
522 -1.3104139656316014
523 -1.302525043772653
524 -1.2944822784969958
525 -1.2862371461716382
526 -1.277737059855488
527 -1.2689289801382202
528 -1.2597559738335615
529 -1.2501530456419672
530 -1.240052751512763
531 -1.2293973714326416
532 -1.2181458124180315
533 -1.2062774514395471
534 -1.1937766797210505
535 -1.1806382146235566
536 -1.1668622765250443
537 -1.152452533796914
538 -1.1374058528427453
539 -1.1217138560828508
540 -1.1053702044354972
541 -1.0883785221305988
542 -1.0707541459836571
543 -1.0525209661287276
544 -1.0337132050862947
545 -1.0143706889968873
546 -0.9945324877155506
547 -0.9742374055572488
548 -0.9535241616988
549 -0.9324330275184199
550 -0.9110052013934167
551 -0.889283030064588
552 -0.867309822050585
553 -0.8451285408410912
554 -0.822782044697533
555 -0.8003130108545008
556 -0.7777642560369372
557 -0.7551768739934784
558 -0.7325926018313718
559 -0.7100481458680848
560 -0.6875769876322182
561 -0.6652105255295431
562 -0.6429778484805189
563 -0.6209051613941928
564 -0.5990147888926102
565 -0.5773276570807985
566 -0.5558612059620128
567 -0.5346293965598596
568 -0.513642964292137
569 -0.4929101474437591
570 -0.47243688611453843
571 -0.45222631089730025
572 -0.432279701956878
573 -0.4125963398957797
574 -0.3931736720377797
575 -0.3740074455742778
576 -0.3550916749172254
577 -0.3364194224293809
578 -0.31798259685608765
579 -0.2997721031691582
580 -0.28177816498800884
581 -0.2639904772554097
582 -0.24639791942080244
583 -0.2289891430981461
584 -0.2117524869692989
585 -0.19467632552652425
586 -0.17774886794751255
587 -0.16095845821902055
588 -0.14429341424000508
589 -0.12774222013930114
590 -0.11129367466328698
591 -0.09493664505639368
592 -0.0786602376876471
593 -0.06245384790799907
594 -0.04630747028914459
595 -0.030211137554904097
596 -0.014155529348932345
597 0.0018681072012640063
598 0.017868475230249137
599 0.03385392117378323
600 0.049832252784877275
601 0.06581088523756151
602 0.08179681745677986
603 0.09779689667134293
604 0.11381751944763355
605 0.12986460525617816
606 0.14594400006915226
607 0.16206106650022414
608 0.1782206613546007
609 0.19442753307540508
610 0.21068605323123646
611 0.2270002841772706
612 0.24337396792854796
613 0.2598107993260331
614 0.27631421679274254
615 0.2928873819056565
616 0.30953321061722766
617 0.32625439625372493
618 0.343053381134852
619 0.35993246338687224
620 0.3768938014349584
621 0.3939393987637181
622 0.4110711296242917
623 0.42829071907848654
624 0.44559976590197853
625 0.46299975395718235
626 0.4804921025314615
627 0.4980780659804107
628 0.5157587806526327
629 0.5335352468350683
630 0.55140837500718
631 0.5693790806039153
632 0.5874481739639309
633 0.605616158702699
634 0.6238838078993674
635 0.6422515668260788
636 0.6607202311792179
637 0.6792902215354429
638 0.6979617720551695
639 0.7167351762264609
640 0.7356111137248246
641 0.7545900717530384
642 0.7736725274583337
643 0.7928585338156534
644 0.8121480394380727
645 0.8315411984435769
646 0.8510380487382313
647 0.8706387244159906
648 0.89034362964693
649 0.9101528453197635
650 0.9300664860298098
651 0.9500844154889488
652 0.9702065067381946
653 0.9904327516517589
654 1.0107631291378796
655 1.0311976156836438
656 1.051736180155912
657 1.0723788466096855
658 1.0931253755288646
659 1.1139758004351452
660 1.134929988964178
661 1.1559879123318597
662 1.1771494799883753
663 1.1984145348687063
664 1.2197829031808805
665 1.2412544278975495
666 1.2628289507181631
667 1.2845063593572854
668 1.3062862000428483
669 1.3281683233482005
670 1.3501528918413412
671 1.372239731768735
672 1.394428401784519
673 1.4167183598702706
674 1.4391099050703398
675 1.461602772311584
676 1.4841966196423984
677 1.5068915120376127
678 1.5296871669260137
679 1.5525835100678833
680 1.5755803465777596
681 1.59867755346164
682 1.621874894861622
683 1.6451722363867645
684 1.6685690083698057
685 1.6920650279333302
686 1.7156601571454648
687 1.739354226923999
688 1.763147171301939
689 1.7870389348815812
690 1.8110292424148282
691 1.835117788038365
692 1.8593041831026713
693 1.8835878148133827
694 1.9079687706792514
695 1.9324469527757442
696 1.957022249790031
697 1.981694146267246
698 2.006462472993047
699 2.031326981058269
700 2.05628752628365


==> plotdata/quadrotor/A1_x3_phase1.tex <==
0 0.0
1 0.0
2 -1.545430450278218e-15
3 -5.31130694980675e-15
4 -3.417710559006082e-14
5 -1.183053655040567e-13
6 2.202504845172371e-13
7 8.718359367776434e-14
8 -1.1376855013622843e-12
9 -3.9476510949043585e-12
10 -8.824461161793805e-12
11 -1.6328662866271772e-11
12 -2.6911770589777012e-11
13 -4.093793748438657e-11
14 -5.890555598853099e-11
15 -8.133449469482913e-11
16 -9.716247362234755e-11
17 -1.083761347331347e-10
18 -1.1606926975105127e-10
19 -1.1555156831377646e-10
20 -1.1666065447002438e-10
21 -1.1849598635649272e-10
22 -1.2310632513390373e-10
23 -1.2878393462756322e-10
24 -1.355366663347013e-10
25 -1.4184651675464012e-10
26 -1.4534828451928663e-10
27 -1.4618228405538505e-10
28 -1.446271546967637e-10
29 -1.3976993784581284e-10
30 -1.3245026408981177e-10
31 -1.235584257130995e-10
32 -1.1373449737561714e-10
33 -1.0346603573907486e-10
34 -9.318059213114792e-11
35 -8.31436075543479e-11
36 -7.3603239059139e-11
37 -6.45503739349351e-11
38 -5.5712376934025066e-11
39 -4.651266038990796e-11
40 -3.645286739129003e-11
41 -2.45919906660674e-11
42 -9.04377017718613e-12
43 1.2663363690990117e-11
44 4.507501927264461e-11
45 9.310584303534601e-11
46 1.6349073206356485e-10
47 2.649327157655535e-10
48 4.0753901586754194e-10
49 6.021801546296503e-10
50 8.606915891107295e-10
51 1.1953357059724115e-09
52 1.621148744135326e-09
53 2.154458158543094e-09
54 2.8088792447533713e-09
55 3.5874503190314052e-09
56 4.4839484125702724e-09
57 5.480478648678402e-09
58 6.539832160257222e-09
59 7.60102588870382e-09
60 8.56506199298224e-09
61 9.355563399537918e-09
62 9.928758188948455e-09
63 1.0251474567013479e-08
64 1.0342630840654015e-08
65 1.0224619497734017e-08
66 9.932325042427699e-09
67 9.488298342574815e-09
68 8.915221929584057e-09
69 8.234842461263278e-09
70 7.468940612653804e-09
71 6.637051210844909e-09
72 5.753796745722191e-09
73 4.832158371215208e-09
74 3.8833584348196915e-09
75 2.922164838992111e-09
76 1.957507080874174e-09
77 9.670083400692505e-10
78 5.4205884225755776e-12
79 -8.693646513790917e-10
80 -1.5685202825466053e-09
81 -1.9207604395887657e-09
82 -1.6142484504655282e-09
83 -9.693865266057212e-11
84 3.6160569649723697e-09
85 1.1244931474863062e-08
86 2.4968681504589098e-08
87 4.833745737897745e-08
88 8.688577013415968e-08
89 1.4894335192749966e-07
90 2.468614646566892e-07
91 3.985592745259226e-07
92 6.296270171901598e-07
93 9.757409907962257e-07
94 1.4857421542835426e-06
95 2.2244377256441798e-06
96 3.2753505844240754e-06
97 4.744448684004255e-06
98 6.7621359210789945e-06
99 9.482015513295752e-06
100 1.3078691757737463e-05
101 1.7737942983444557e-05
102 2.36322795413102e-05
103 3.09019395037602e-05
104 3.963995555329448e-05
105 4.988003548612953e-05
106 6.157856198651504e-05
107 7.455494178405079e-05
108 8.844391768983332e-05
109 0.00010264594107493257
110 0.00011625953909387482
111 0.00012803890881448517
112 0.0001373032415291498
113 0.00014316739437170164
114 0.00014584786519691314
115 0.0001456368849468782
116 0.0001428322514648351
117 0.00013772519556470197
118 0.0001306124556424494
119 0.0001217737925573027
120 0.0001114356710274046
121 9.977687552519056e-05
122 8.689993933131757e-05
123 7.280950308922852e-05
124 5.741225709860144e-05
125 4.053276808626562e-05
126 2.1944807604050843e-05
127 1.4378028792273724e-06
128 -2.1034057133100106e-05
129 -4.4971279452372525e-05
130 -6.892694361155789e-05
131 -8.943947684652881e-05
132 -9.939519923783262e-05
133 -8.549564526488121e-05
134 -2.4018563302181456e-05
135 0.0001239901842634519
136 0.00041593378023389274
137 0.0009305390316283283
138 0.0017634993852472295
139 0.002983169917029205
140 0.0046211895990256125
141 0.006717439866199708
142 0.009319573256504902
143 0.012484879330893416
144 0.016282219134862944
145 0.020792106671257908
146 0.02611244298991668
147 0.032350493885070455
148 0.03960928347290779
149 0.047904778732826676
150 0.05717453056190812
151 0.06733761816849244
152 0.07828398882655202
153 0.0898659953521239
154 0.10188638796019593
155 0.11409198043167207
156 0.12616436637769274
157 0.1377082713127573
158 0.1482405584856747
159 0.15718366574815856
160 0.16385332921840418
161 0.16744221877829418
162 0.16775397831554598
163 0.16445218015528654
164 0.1577741606515691
165 0.1485687449815426
166 0.13757327893414423
167 0.12541798998799583
168 0.11263164371561966
169 0.09964716743209577
170 0.08681260761423364
171 0.07439837951995552
172 0.06261281944775651
173 0.051608911982596
174 0.0414896332052458
175 0.03231684748435751
176 0.024110474705997004
177 0.016855661925201215
178 0.010513344011523491
179 0.005024881276008381
180 0.0003219578873624824
181 -0.003643577643532161
182 -0.006912211125649163
183 -0.009546242136038656
184 -0.011630085819941582
185 -0.013267690777071448
186 -0.014571380324320964
187 -0.015651949298366424
188 -0.01661969717628431
189 -0.017561041869538645
190 -0.018517762646843267
191 -0.019524040221876565
192 -0.020596505269373396
193 -0.02172801435501421
194 -0.022885599135769406
195 -0.02401003902168217
196 -0.025012077285209044
197 -0.025772184852363607
198 -0.026147048112905583
199 -0.026046736002592608
200 -0.025433430555363394
201 -0.024253719589206184
202 -0.02244161548308485
203 -0.019922874873728555
204 -0.0166213354106003
205 -0.012467160927955002
206 -0.007407598422833062
207 -0.0014208605049540121
208 0.005467872736457356
209 0.013168264951188682
210 0.02150396235192481
211 0.02960569914290071
212 0.035622229192526715
213 0.03841527388457695
214 0.03735729161770705
215 0.03370618023626674
216 0.028493294671255498
217 0.022538432893126896
218 0.016468676170044202
219 0.010738900478172293
220 0.005656881833428535
221 0.0014061857300454025
222 -0.0019257769512647975
223 -0.0043261751726957716
224 -0.005835566270458812
225 -0.00652676782953466
226 -0.006497011074971583
227 -0.005863592078756184
228 -0.004757531094386465
229 -0.003322028152654203
230 -0.0017183135947789858
231 -0.00010837125777428684
232 0.0013955423128284743
233 0.0027299830980245386
234 0.0038584789967103395
235 0.004747725397641477
236 0.005361324229841978
237 0.0056603313846912435
238 0.005597381571744807
239 0.005137615425022326
240 0.004278368196049282
241 0.0030121413001943497
242 0.001336675685363571
243 -0.0007374776102132936
244 -0.00318297841878236
245 -0.005952477849486289
246 -0.008971432940795596
247 -0.012134040933640285
248 -0.015305344949120269
249 -0.01839458799054907
250 -0.021350366100080953
251 -0.02408949987211798
252 -0.026497511845680152
253 -0.02843170801636374
254 -0.029726920380220085
255 -0.030204251410765905
256 -0.02968386332582812
257 -0.028002810216984312
258 -0.025036354098398366
259 -0.02072304662204861
260 -0.0150941529587331
261 -0.00889216989956687
262 -0.0038734807850173934
263 -0.001126953098569947
264 -0.0012849652349359016
265 -0.00315022046972373
266 -0.005801080240597105
267 -0.008564632759601877
268 -0.010983934248541561
269 -0.012783465866200942
270 -0.013831187743505136
271 -0.014105262840348753
272 -0.013658037821407855
273 -0.012589609034862592
274 -0.011024026737054006
275 -0.009087538231166682
276 -0.006902263824971444
277 -0.004584091700071968
278 -0.002239511904257996
279 3.1796859625557537e-05
280 0.0021259498329744206
281 0.003947300488817583
282 0.005454095265236035
283 0.006653140401030003
284 0.007574315951956538
285 0.008243849151764394
286 0.008675925711887661
287 0.008871551094388714
288 0.008811599560053836
289 0.008477191440461995
290 0.007869373423441654
291 0.006972249452711868
292 0.005763848372504757
293 0.004225289520839283
294 0.0023459408665802367
295 0.0001290757929140276
296 -0.002398701855296652
297 -0.005180652142993252
298 -0.008129011838435089
299 -0.011195434162093077
300 -0.014363244558303413
301 -0.017573711181704282
302 -0.020724171034109066
303 -0.023669021355823355
304 -0.026223770682059836
305 -0.028172681689606283
306 -0.029281249591306194
307 -0.029314903856095777
308 -0.02806248074812171
309 -0.025365577206433135
310 -0.021154430493151754
311 -0.01607542353020228
312 -0.01180564286875365
313 -0.009383675952133193
314 -0.009428939986045626
315 -0.010770818384955477
316 -0.012548173510870505
317 -0.01417287262727116
318 -0.015286041040124236
319 -0.015712908203066395
320 -0.015416008070882004
321 -0.014455029435320392
322 -0.012946411599161205
323 -0.011034757064402443
324 -0.00886881451712832
325 -0.006580981343184946
326 -0.004283329984547127
327 -0.00206851754528074
328 -9.924533236533185e-06
329 0.0018323188521939039
330 0.0033974423151258907
331 0.004633557022473036
332 0.0055409813648989534
333 0.006165172408082512
334 0.0065699053043262136
335 0.00680977983468661
336 0.006921302092775738
337 0.006921505451306401
338 0.006800867657603469
339 0.006543650292048743
340 0.0061476595308985055
341 0.005587578559662725
342 0.004826137171791286
343 0.0038236765267780216
344 0.002543851426613798
345 0.0009600863402706313
346 -0.0009340343441858784
347 -0.0031166812637689776
348 -0.0055353920980411924
349 -0.008175787322914806
350 -0.011052099831133278


==> plotdata/quadrotor/A1_x3_phase2.tex <==
350 -0.011052099831133278
351 -0.014131684274310006
352 -0.017557843020602065
353 -0.02104967834312672
354 -0.02327798707083464
355 -0.024341573177573784
356 -0.02465368944194144
357 -0.024558363038158153
358 -0.024258801076739597
359 -0.023859831789256394
360 -0.023412620067368235
361 -0.022945187373305538
362 -0.02247391155763551
363 -0.02200564041868685
364 -0.021544114416095092
365 -0.021090533265806614
366 -0.020645649743313472
367 -0.02020973448184051
368 -0.019782817576276795
369 -0.019364818218547058
370 -0.018955603292370102
371 -0.018555015297514844
372 -0.018162886076370517
373 -0.01777904380074193
374 -0.017403321178849823
375 -0.017035542688170077
376 -0.016675542556165712
377 -0.01632315571626794
378 -0.015978221500064338
379 -0.01564058269015549
380 -0.015310085197599216
381 -0.014986578161856846
382 -0.014669913965132595
383 -0.014359948433010005
384 -0.014056539055008789
385 -0.013759547192560907
386 -0.013468837217162749
387 -0.013184276781670883
388 -0.012905735730804961
389 -0.01263308614437847
390 -0.012366203499566875
391 -0.012105372781850069
392 -0.011851241666360828
393 -0.011604324283187169
394 -0.011364861719220553
395 -0.01113282473695731
396 -0.010908029780403145
397 -0.010690162233512678
398 -0.010479205935956125
399 -0.010275513216821134
400 -0.0100792517871273
401 -0.009890266849809608
402 -0.00970809751319582
403 -0.009532133287441177
404 -0.00936171869626821
405 -0.009196255682388747
406 -0.009035251369810766
407 -0.008878341483375754
408 -0.008725299502994461
409 -0.008576003650830897
410 -0.008430380986726311
411 -0.00828842566176449
412 -0.008150146029629723
413 -0.008015535063452485
414 -0.00788459696940815
415 -0.007757328566449789
416 -0.007633670603924965
417 -0.007513645564099629
418 -0.007397291879233751
419 -0.007284573274154546
420 -0.007175420788363972
421 -0.007069735307350747
422 -0.006967271833507922
423 -0.006867666036699642
424 -0.006770671949096265
425 -0.006676169423744817
426 -0.006584086147455498
427 -0.006494369415700277
428 -0.006406954045690708
429 -0.006321766292052928
430 -0.0062387187609907226
431 -0.006157713115315102
432 -0.006078661999686198
433 -0.006001503149449353
434 -0.0059261472042014185
435 -0.005852547273055629
436 -0.005780658539653805
437 -0.0057104470559191
438 -0.00564188703105714
439 -0.005574947257334055
440 -0.005509591221654133
441 -0.005445786853923096
442 -0.005383501308317513
443 -0.005322693782318812
444 -0.00526332720423644
445 -0.0052053611630552945
446 -0.005148759191472917
447 -0.00509348420717408
448 -0.005039502325520719
449 -0.004986790276235504
450 -0.004935310795817526
451 -0.004885029710861702
452 -0.004835917244663304
453 -0.004787940319371615
454 -0.004741071477371184
455 -0.004695276371262346
456 -0.004650528231677528
457 -0.004606799317020099
458 -0.004564066878090044
459 -0.004522298791138153
460 -0.004481465683371644
461 -0.004441535716222147
462 -0.004402488800665777
463 -0.004364297085656853
464 -0.004326934386213279
465 -0.004290370885043133
466 -0.00425458017972437
467 -0.00421953786287625
468 -0.004185215020511144
469 -0.0041515905995189685
470 -0.004118647418229593
471 -0.004086363538782351
472 -0.0040547142391464215
473 -0.0040236744084203736
474 -0.00399322806559857
475 -0.003963353144765034
476 -0.003934024546265609
477 -0.0039052268389682407
478 -0.0038769454647464394
479 -0.0038491665006408675
480 -0.0038218767120849454
481 -0.003795061884214063
482 -0.0037687041683553157
483 -0.003742791513935649
484 -0.0037173150505868005
485 -0.0036922570772770723
486 -0.0036676073473541734
487 -0.003643359054612531
488 -0.0036194986988958102
489 -0.003596015959113664
490 -0.0035729029371014817
491 -0.0035501539699178937
492 -0.0035277615162726057
493 -0.0035057171813118277
494 -0.0034840136942398963
495 -0.0034626433814434754
496 -0.003441600514616363
497 -0.0034208808985325785
498 -0.003400481003547439
499 -0.0033803980896119925
500 -0.003360627457626818
501 -0.003341163591285624
502 -0.003322076307020282
503 -0.0033209989868223707
504 -0.003355448088828055
505 -0.003436030303608799
506 -0.0035672658101839547
507 -0.003749857474060918
508 -0.003982794670988523
509 -0.004263994229686955
510 -0.004590148420476031
511 -0.004956257765038957
512 -0.005354810332912733
513 -0.0057763068375144035
514 -0.00621018339725839
515 -0.006644349866310545
516 -0.007067521281364929
517 -0.00747931863041649
518 -0.00797017531870628
519 -0.008576512771433642
520 -0.00931433003803479
521 -0.010189104665110695
522 -0.011203446590446182
523 -0.012351453198164785
524 -0.013632982385979164
525 -0.015029637449032839
526 -0.016508254157237213
527 -0.01803740276724349
528 -0.019617161117655314
529 -0.02119588062399705
530 -0.02269899410560929
531 -0.024062550628322354
532 -0.025222896473971086
533 -0.02614009225782932
534 -0.026803178384256
535 -0.027240225626901177
536 -0.02754411602552566
537 -0.027830941938809077
538 -0.028219931517670948
539 -0.02880532619300054
540 -0.029563050693040344
541 -0.030272399867763304
542 -0.030811820706353608
543 -0.03099689832648001
544 -0.030845968873787214
545 -0.03046179918814772
546 -0.029942900667927957
547 -0.02935465186383619
548 -0.028737758636495695
549 -0.02811323438006368
550 -0.027490773827519955
551 -0.02687572289743096
552 -0.026270720528960227
553 -0.025676809065056025
554 -0.02509452885011235
555 -0.024523940977621422
556 -0.02396480229074033
557 -0.023416928749990577
558 -0.02288023627335543
559 -0.022354544475016006
560 -0.021839617029244165
561 -0.02133521376129471
562 -0.02084105379402853
563 -0.02035701866105577
564 -0.019882956596796453
565 -0.019418654834032992
566 -0.018963852788391626
567 -0.018518395900024825
568 -0.018082148790887476
569 -0.017654916599879732
570 -0.017236582974107684
571 -0.016827003025979698
572 -0.01642606632696208
573 -0.01603361353675135
574 -0.015649490639888335
575 -0.01527358341264487
576 -0.014905753253186108
577 -0.014545859703511016
578 -0.01419382606878488
579 -0.013849528941978766
580 -0.013512801591769685
581 -0.013183500753424672
582 -0.012861476830603045
583 -0.012546636275775399
584 -0.012238841085476758
585 -0.011938013925785865
586 -0.011643967169192606
587 -0.011356579203228207
588 -0.011075746444935064
589 -0.010801339201714825
590 -0.010533217223868989
591 -0.010271262165674786
592 -0.010015352986287225
593 -0.009765366829336429
594 -0.009521226840883237
595 -0.00928284824372021
596 -0.009050058834533303
597 -0.008822714215578214
598 -0.008600747806818115
599 -0.00838403855399526
600 -0.008172494252655106
601 -0.007965963511441349
602 -0.007764331027883111
603 -0.007567493478011597
604 -0.0073753256528559545
605 -0.007187774431458648
606 -0.007004748502474065
607 -0.006826118164997929
608 -0.006651797174856786
609 -0.006481698545957604
610 -0.006315749130409865
611 -0.006153832351494393
612 -0.005995832386336751
613 -0.005841673488599966
614 -0.005691272464437508
615 -0.005544543758274999
616 -0.0054014024152505575
617 -0.0052617629129180265
618 -0.005125542260433165
619 -0.004992659849976371
620 -0.004863037701368798
621 -0.004736599625933798
622 -0.00461326777368296
623 -0.00449300385544937
624 -0.004375687260926345
625 -0.004261246174251153
626 -0.004149615137414701
627 -0.004040703955290971
628 -0.00393446579084907
629 -0.0038308653988459542
630 -0.003729844176030465
631 -0.003631324802083015
632 -0.0035352457478518757
633 -0.003441543981106163
634 -0.0033501466577022174
635 -0.0032609921180649223
636 -0.003174109734721586
637 -0.0030894382901598518
638 -0.0030068628739153926
639 -0.0029263544035810422
640 -0.002847778625180047
641 -0.002771090839830726
642 -0.002696322104306464
643 -0.0026234287032540216
644 -0.002552351971627013
645 -0.0024830808915334525
646 -0.002415494975502123
647 -0.002349543101912558
648 -0.0022852360003608324
649 -0.0022225419286804322
650 -0.0021614682287251314
651 -0.0021019505077785623
652 -0.0020438986798592593
653 -0.0019872886562033497
654 -0.001932086413155083
655 -0.0018782542230523448
656 -0.0018257763027587019
657 -0.0017745793118502512
658 -0.0017246231391280617
659 -0.0016758555897232617
660 -0.00162827498653359
661 -0.0015818789972568015
662 -0.0015366335899603182
663 -0.0014925152749429864
664 -0.0014494894275207976
665 -0.0014075229342047342
666 -0.0013665893459030617
667 -0.001326680238594584
668 -0.0012877449621822956
669 -0.0012498078204066744
670 -0.0012128567897243328
671 -0.001176831841776898
672 -0.0011416776787415335
673 -0.0011074190142433946
674 -0.0010740129255539632
675 -0.0010414548178284677
676 -0.00100978276080412
677 -0.0009788884257382329
678 -0.0009487744605363985
679 -0.0009193931099841143
680 -0.0008907746237569979
681 -0.000862844877978608
682 -0.000835603958622715
683 -0.0008090908698444247
684 -0.0007832612714025872
685 -0.0007580986943715658
686 -0.0007335658544810939
687 -0.0007096222769466697
688 -0.0006862590520513646
689 -0.0006635203329944974
690 -0.0006413670185282288
691 -0.0006198034522088465
692 -0.0005987755276873138
693 -0.0005782229365886081
694 -0.0005581781600569568
695 -0.0005386591791008645
696 -0.0005196802823649985
697 -0.0005011669028650561
698 -0.00048311232243789144
699 -0.0004654851338360352
700 -0.00044827042356030506


==> plotdata/quadrotor/A2_x1_phase1.tex <==
0 -0.5
1 -0.5
2 -0.5
3 -0.5
4 -0.500051584915063
5 -0.5003515774626136
6 -0.5012400723582063
7 -0.5031584695950346
8 -0.5065982670312758
9 -0.5118984140473473
10 -0.5192810160335739
11 -0.5289171770889195
12 -0.5409612343774357
13 -0.555520042140115
14 -0.5729830780913476
15 -0.5936921744731635
16 -0.6176803802089982
17 -0.6445704874108178
18 -0.6735991035601437
19 -0.7037175783100688
20 -0.7338621942417392
21 -0.762971641732669
22 -0.7897707132119101
23 -0.8127297243792706
24 -0.8301586893319739
25 -0.8403997263911095
26 -0.8419677910791619
27 -0.8336488175621389
28 -0.814554349574979
29 -0.7841338025819717
30 -0.7421457158002074
31 -0.6886931670843711
32 -0.6242358331984268
33 -0.5496231817046126
34 -0.4660259788275853
35 -0.3749097047292545
36 -0.2779970624117186
37 -0.17719873372777062
38 -0.07460448656567925
39 0.0275896963395722
40 0.1271243402348657
41 0.2217169193063763
42 0.3091172652855158
43 0.3871732234707413
44 0.453933773324957
45 0.5077641584181818
46 0.5472444908170445
47 0.5713624222706363
48 0.5797121221039203
49 0.5726794918367243
50 0.5515110791352389
51 0.5182603420786571
52 0.4754877142629294
53 0.4257204543557529
54 0.3706155001983086
55 0.31101923953042643
56 0.24709477141250702
57 0.17864310554863294
58 0.10543538478878522
59 0.02727158502785368
60 -0.05616066787440553
61 -0.1453607736185946
62 -0.2399543997830552
63 -0.33854381747392603
64 -0.43887688383570767
65 -0.5384526909789575
66 -0.6352926675041561
67 -0.728121389729546
68 -0.8160495112474546
69 -0.8980789611208146
70 -0.9729027373750202
71 -1.03888592206389
72 -1.094227324323804
73 -1.137115542048718
74 -1.1658549864635386
75 -1.1790100142634048
76 -1.1755051993657573
77 -1.1546791717034242
78 -1.1163132264323223
79 -1.0606015080629128
80 -0.9880752989756912
81 -0.899620835391374
82 -0.7964608216919016
83 -0.6801799171505452
84 -0.552641771719734
85 -0.4159407981536031
86 -0.27235690522152
87 -0.12431139869538968
88 0.025621232311543923
89 0.17475501447487507
90 0.320317921227337
91 0.4594881864958258
92 0.5894092999080278
93 0.7072649046596599
94 0.8105035041415019
95 0.8968806193057851
96 0.9644457166005982
97 1.0115108286356322
98 1.036621597912183
99 1.039172930704463
100 1.019622802251353
101 0.9794388940438034
102 0.9207921600837922
103 0.8460183259333942
104 0.756800254205741
105 0.6542791425358674
106 0.5392179518225334
107 0.41234293222294627
108 0.2747310589898011
109 0.1280041762115561
110 -0.02555143500956894
111 -0.18276987829882171
112 -0.33948160012102535
113 -0.4925573011427377
114 -0.6392311001592521
115 -0.777012871364031
116 -0.9042554591921794
117 -1.02046597977944
118 -1.1259265706861932
119 -1.220748154028937
120 -1.304459684395891
121 -1.3759618318264912
122 -1.4337386189764818
123 -1.4760710038354574
124 -1.5012206367378729
125 -1.5076280313579233
126 -1.4940612971453986
127 -1.4597086064650402
128 -1.4042436744978488
129 -1.3278140243680119
130 -1.2309652652344667
131 -1.1146683135947222
132 -0.9803302973269253
133 -0.8298149078988416
134 -0.6653330935187848
135 -0.48937491126161164
136 -0.3046739671732066
137 -0.1142996273983432
138 0.07773969898246519
139 0.2672177292211401
140 0.4502498026490318
141 0.6233796099201376
142 0.7835882087600055
143 0.9282623756674735
144 1.0551438281787062
145 1.1622869935800357
146 1.2480217367864685
147 1.3109234470705107
148 1.349780014962076
149 1.363564638146786
150 1.351417716796412
151 1.3126337793831762
152 1.2466602685385877
153 1.1540439186957108
154 1.036489274307049
155 0.8963083106857958
156 0.7362313152957533
157 0.5597346662883199
158 0.37168735511642714
159 0.17765848197657053
160 -0.01760026911901766
161 -0.2129555966620755
162 -0.40651507860761643
163 -0.5949808176198427
164 -0.7749753950488387
165 -0.9434257793780795
166 -1.0976368319097363
167 -1.2363984388369629
168 -1.3601385133349353
169 -1.4693403718193352
170 -1.563750195518781
171 -1.6420305207472197
172 -1.7023859237152292
173 -1.7430425821843591
174 -1.7623963124718764
175 -1.7590473088331158
176 -1.7317974534859502
177 -1.6796360608259535
178 -1.602045290076053
179 -1.499548983434231
180 -1.3735743593582876
181 -1.2264113619851156
182 -1.061198370953273
183 -0.8819217056433086
184 -0.6932090712270222
185 -0.4998228337924162
186 -0.3054531595865769
187 -0.11095992455590536
188 0.08309530199716225
189 0.2736227769499962
190 0.4570522672765817
191 0.630004568564257
192 0.7894760882346883
193 0.9328656515298273
194 1.0579462326860147
195 1.1628158441236272
196 1.2458586452791274
197 1.3057100653449067
198 1.3412240307881724
199 1.3514417759255832
200 1.3355626477944598
201 1.2929172113441803
202 1.2229452184644471
203 1.1251762574483346
204 0.9992154287768839
205 0.8465153063118912
206 0.6733937360381268
207 0.486818347155232
208 0.293187225013657
209 0.09808233161089594
210 -0.09674645839324769
211 -0.2917391107758276
212 -0.48666006235148307
213 -0.6794377938467717
214 -0.866740872635282
215 -1.0451887858846816
216 -1.211718066176849
217 -1.3636587012367603
218 -1.499236220697208
219 -1.6174623636932723
220 -1.7167706034014547
221 -1.7955616676206936
222 -1.8523755197724812
223 -1.8859327560355106
224 -1.8951318695697852
225 -1.8790317762673363
226 -1.8368307537842423
227 -1.7678462928055767
228 -1.6715007649822864
229 -1.5480716530327339
230 -1.399876601552708
231 -1.2310015181206215
232 -1.0470087556944172
233 -0.8539823116741128
234 -0.6574596988890908
235 -0.46133587421760913
236 -0.26645599641649864
237 -0.07070235375860964
238 0.1250939051320281
239 0.31937750437020895
240 0.5090201315882507
241 0.690758648921433
242 0.8616075231381839
243 1.018945748809296
244 1.1604877664126885
245 1.2842351733121946
246 1.3884566428723077
247 1.471649793281132
248 1.5325082720543486
249 1.5698918894915805
250 1.5828041619099944
251 1.5703766478837382
252 1.5318553209575834
253 1.4665888812588699
254 1.3740198132905137
255 1.2536761881092549
256 1.1058022332556072
257 0.9363997936526838
258 0.7524561259004464
259 0.5604756837954925
260 0.3661525749467849
261 0.17191267587138975
262 -0.02164109667546632
263 -0.21602569451078005
264 -0.41018432384963166
265 -0.6008729296467329
266 -0.7845072103288201
267 -0.9577472630488006
268 -1.1176500507774054
269 -1.2616793494528804
270 -1.3876698787163848
271 -1.493781449778162
272 -1.5784526009195479
273 -1.6403587930975256
274 -1.6783784333326612
275 -1.691562186776373
276 -1.679106114550499
277 -1.6403291831915163
278 -1.574652577440765
279 -1.4815805260925439
280 -1.360694150306456
281 -1.2120941899871285
282 -1.0418098772370803
283 -0.8568373992533386
284 -0.6636682015114646
285 -0.467961355317674
286 -0.27242193218055155
287 -0.07732895635362558
288 0.11804364196758121
289 0.3133935961495691
290 0.5058005467112592
291 0.6917522524389121
292 0.8679042088468877
293 1.0312831364134234
294 1.179309205525841
295 1.3097635545738133
296 1.420743296365265
297 1.5106184608533966
298 1.5779936337857927
299 1.6216759055182794
300 1.6406467862041443
301 1.634038246446315
302 1.6011118219407485
303 1.54124026270766
304 1.4538915916474278
305 1.3386144046581436
306 1.1950256740857688
307 1.0286255037797125
308 0.846406891320957
309 0.6550143476365715
310 0.46030246194228297
311 0.26555240058292073
312 0.07141231231317924
313 -0.1231414845686972
314 -0.31792615139851454
315 -0.5099121079157539
316 -0.6955095718366734
317 -0.8713059864109998
318 -1.0342696517197618
319 -1.1817755525527236
320 -1.3115749577605118
321 -1.4217516449500915
322 -1.510676709140957
323 -1.5769677099060249
324 -1.6194515133413385
325 -1.6371338218780804
326 -1.629171949385292
327 -1.5948514378691203
328 -1.533567047376167
329 -1.4448060582891329
330 -1.3281344445521421
331 -1.1831859965180478
332 -1.015655021710894
333 -0.8325608325822526
334 -0.6405165223901281
335 -0.4453247546699342
336 -0.2501702750900395
337 -0.05503654930287569
338 0.14000237105197993
339 0.3351184821136454
340 0.52742746555888
341 0.7134022554039935
342 0.8896633106499814
343 1.0531988363133065
344 1.2013951957107258
345 1.3320077805876507
346 1.4431173090182343
347 1.5330859622314401
348 1.6005177008389972
349 1.6442236891207571
350 1.6631925630782831


==> plotdata/quadrotor/A2_x1_phase2.tex <==
350 1.6631925630782831
351 1.6565648353617195
352 1.623610747203182
353 1.5637111548863438
354 1.4797295039890248
355 1.3785501863444536
356 1.2674161638372745
357 1.1529076524523791
358 1.0407523561025267
359 0.9358699409660088
360 0.8424695550222413
361 0.7626946053361842
362 0.6960788964423714
363 0.6408097349229263
364 0.594715674409184
365 0.5557541298308216
366 0.5221804067049959
367 0.4925670686499697
368 0.46576839663808667
369 0.4408727975133743
370 0.41715882419765254
371 0.3940585393574048
372 0.37112839030189054
373 0.34802625970382023
374 0.3244932935327186
375 0.3003392724325088
376 0.2754312784507741
377 0.24968302624095928
378 0.2230472655871051
379 0.19550885645799593
380 0.1670787799367123
381 0.1377888182795133
382 0.1076871836708655
383 0.07683465791379672
384 0.04530121989636247
385 0.01316317015108899
386 -0.019499326335515217
387 -0.052604254795759545
388 -0.08606946122494391
389 -0.11981403144276292
390 -0.15375937876843354
391 -0.18783010983645004
392 -0.22195465069196835
393 -0.2560209089078048
394 -0.28986296091633285
395 -0.32329979589226143
396 -0.35616643355961913
397 -0.38832923892901233
398 -0.4196902429351904
399 -0.45018606976373576
400 -0.47976292509364765
401 -0.5083650709639099
402 -0.5359502903141227
403 -0.5625067274814837
404 -0.5880622842193716
405 -0.6126851162481395
406 -0.6364792175424437
407 -0.6595750745670795
408 -0.6821183131033958
409 -0.7042565790831393
410 -0.7261274908331653
411 -0.7478490216702683
412 -0.769514297737966
413 -0.7911892642053011
414 -0.8129140358931338
415 -0.8347065957435116
416 -0.8565667617826158
417 -0.8784802411550071
418 -0.9004246700066411
419 -0.9223693029127683
420 -0.9442773006586926
421 -0.9661103732085793
422 -0.9878310745964087
423 -1.0094023841182578
424 -1.03076344176424
425 -1.0518214863848272
426 -1.0724754256785276
427 -1.092634207146104
428 -1.1122263721866685
429 -1.1312017592446066
430 -1.1495301013250867
431 -1.1671981951306516
432 -1.184206976280794
433 -1.20056820091869
434 -1.2163013410618477
435 -1.231430984874434
436 -1.2459857659938407
437 -1.2599965597309373
438 -1.2734952430086763
439 -1.2865136569301183
440 -1.2990827264028884
441 -1.3112324235044863
442 -1.322991162316975
443 -1.3343861322303407
444 -1.3454428608510145
445 -1.3561848308648106
446 -1.366633099060246
447 -1.3768067408607176
448 -1.3867233509100234
449 -1.3963987162019946
450 -1.4058470817787818
451 -1.4150813250885503
452 -1.4241133547061429
453 -1.4329530027658013
454 -1.4416096664706606
455 -1.4500910796723399
456 -1.4584035860633509
457 -1.4665522850537314
458 -1.4745416006359333
459 -1.4823750087409737
460 -1.4900553056289854
461 -1.497583454619125
462 -1.5049618569950727
463 -1.5121923366246357
464 -1.5192765408142326
465 -1.5262156174089367
466 -1.5330101722458316
467 -1.5396605962090022
468 -1.5461662788062487
469 -1.5525275428377967
470 -1.55874437559497
471 -1.5648169146818356
472 -1.5707450582869533
473 -1.5765284527897092
474 -1.582166726723354
475 -1.5876595834323943
476 -1.5930066054442338
477 -1.5982074980352392
478 -1.60326206331797
479 -1.6081701442208902
480 -1.612931466031423
481 -1.6175458710972417
482 -1.6220132696340863
483 -1.626333652752824
484 -1.6305071122844994
485 -1.6345340321994763
486 -1.6384147703913527
487 -1.64214956733319
488 -1.6457389998110021
489 -1.6491837096896929
490 -1.6524845001026047
491 -1.6556423013454031
492 -1.6586581904756048
493 -1.6615334143040061
494 -1.6642693782110667
495 -1.666867642290502
496 -1.6693299260646477
497 -1.671658114478941
498 -1.6738542627700916
499 -1.6759205764140852
500 -1.6778594540483847
501 -1.6796734951212604
502 -1.6813654975593568
503 -1.6829384489982426
504 -1.684395513935366
505 -1.6857378046249645
506 -1.6869657741347002
507 -1.6880815258675768
508 -1.6890898540488226
509 -1.6899982280486296
510 -1.6908162120351298
511 -1.6915544619960696
512 -1.692223446152698
513 -1.6928302308525642
514 -1.6933773849928246
515 -1.6938653200965672
516 -1.6942944491144545
517 -1.6946662684555256
518 -1.694983593961957
519 -1.6952504972050675
520 -1.695455449904027
521 -1.69558177994399
522 -1.6956197266446134
523 -1.6955733561697122
524 -1.6954619925269496
525 -1.6953170031328457
526 -1.695176564005681
527 -1.6950805834862948
528 -1.6950658847841067
529 -1.695161647084275
530 -1.695385500835607
531 -1.6957417208041157
532 -1.6962206634794166
533 -1.6968007366516316
534 -1.6974426666920426
535 -1.6980952731312748
536 -1.6987017004422358
537 -1.6992057320967207
538 -1.699565363555591
539 -1.6997515510080712
540 -1.699743049858654
541 -1.6995230936166428
542 -1.6990798066469013
543 -1.6984068559554817
544 -1.697505694341157
545 -1.69638125848592
546 -1.695039309010115
547 -1.6934853978588653
548 -1.691724396453056
549 -1.6897606915379761
550 -1.6875981477909747
551 -1.685240243477078
552 -1.6826901234979605
553 -1.679950439902699
554 -1.6770235073615312
555 -1.673911396054181
556 -1.670616143818613
557 -1.6671393739825702
558 -1.663481910698321
559 -1.6596445881855972
560 -1.6556282709876193
561 -1.6514335546456995
562 -1.64706077822736
563 -1.6425098248284256
564 -1.6377798191254878
565 -1.6328698006900955
566 -1.627779068901151
567 -1.622506600317364
568 -1.6170511312837839
569 -1.611411219961252
570 -1.6055852805126767
571 -1.5995712728250335
572 -1.59336848768775
573 -1.5869760692359227
574 -1.5803926990681103
575 -1.5736171880660046
576 -1.5666486656247707
577 -1.5594859745049658
578 -1.5521281520488825
579 -1.5445742791579953
580 -1.536823647701309
581 -1.528875522967225
582 -1.5207298594561938
583 -1.5123861443443056
584 -1.5038439731281592
585 -1.4951030973913984
586 -1.4861636739289708
587 -1.4770263174946803
588 -1.4676910037294046
589 -1.4581578729980413
590 -1.4484275476630741
591 -1.438500713660922
592 -1.4283775341645104
593 -1.418058944057949
594 -1.4075457117544263
595 -1.396839009400788
596 -1.3859395858641288
597 -1.374848460686489
598 -1.3635668778319885
599 -1.3520960414458023
600 -1.3404371772045574
601 -1.3285917274491916
602 -1.3165614577470313
603 -1.3043474953330187
604 -1.2919507640810086
605 -1.2793721859255185
606 -1.266612974242017
607 -1.2536742465065795
608 -1.2405575157067048
609 -1.2272647538623873
610 -1.2137976731095266
611 -1.2001577728675614
612 -1.186346264718892
613 -1.172364151675233
614 -1.158213017272159
615 -1.1438944174807284
616 -1.1294098095410616
617 -1.1147605937688407
618 -1.0999481158741817
619 -1.0849737092454543
620 -1.0698386982407393
621 -1.0545443961175656
622 -1.0390921059316456
623 -1.0234831181510253
624 -1.0077187134215806
625 -0.9917999529758265
626 -0.9757281455954299
627 -0.9595046325552301
628 -0.9431306946495702
629 -0.9266072278841678
630 -0.9099356291988424
631 -0.8931171489563655
632 -0.8761529676501126
633 -0.8590442143154522
634 -0.8417918543814449
635 -0.8243972585279844
636 -0.8068611551161985
637 -0.7891846745560229
638 -0.7713691694850304
639 -0.7534155774326874
640 -0.735324584714829
641 -0.7170970419736782
642 -0.698733658327029
643 -0.6802355364868812
644 -0.6616037965430112
645 -0.6428392639857832
646 -0.623942921445185
647 -0.6049155327974866
648 -0.585757636401281
649 -0.56647002466916
650 -0.5470534669104151
651 -0.5275088884540986
652 -0.5078371676175412
653 -0.4880390928036663
654 -0.46811545779286207
655 -0.44806681206646887
656 -0.4278938907433518
657 -0.40759731782789616
658 -0.38717789673440306
659 -0.36663633505344695
660 -0.34597336575115184
661 -0.32518957586701447
662 -0.304285548225198
663 -0.28326193678223843
664 -0.26211941587663623
665 -0.24085864418985192
666 -0.21948017258689848
667 -0.19798450570483456
668 -0.1763725240373965
669 -0.15464485650436807
670 -0.13280156263786053
671 -0.11084322493215322
672 -0.08877074751528663
673 -0.06658513273074458
674 -0.04428629064473303
675 -0.021874873747594475
676 0.0006484649436381204
677 0.02328354961895316
678 0.04602975319728781
679 0.06888673780005566
680 0.09185412094625477
681 0.11493143791988611
682 0.13811816411955452
683 0.16141392254016051
684 0.18481781720287443
685 0.20832940868919728
686 0.2319483694328348
687 0.25567429501581
688 0.279506932055935
689 0.30344609430823477
690 0.32749128881585166
691 0.35164198588146367
692 0.3758976652897145
693 0.40025744166480787
694 0.4247213115307417
695 0.44928903454755964
696 0.47396026641415856
697 0.4987343091244368
698 0.5236108280363584
699 0.54858937755286
700 0.5736696773368632


==> plotdata/quadrotor/A2_x2_phase1.tex <==
0 0.0
1 0.0
2 0.0
3 0.0
4 0.000715821695541621
5 0.002925915571731008
6 0.0071920120894816315
7 0.01380070916430956
8 0.022779954522081536
9 0.03379892916780422
10 0.04630172675961962
11 0.05962892524112336
12 0.07307780659677396
13 0.08586496730255572
14 0.09679090479069595
15 0.10435232009720535
16 0.10690177908222318
17 0.10283049666076333
18 0.09075775421111404
19 0.06978641764878399
20 0.03959596166115602
21 0.00036601012699097324
22 -0.0474911688960023
23 -0.10340149641004823
24 -0.1666272996653797
25 -0.23620730427393005
26 -0.3109009744777781
27 -0.3892148810056706
28 -0.46946108246940105
29 -0.5498398556776762
30 -0.6285220863341775
31 -0.7036683166778176
32 -0.7734695814536033
33 -0.8362129885609079
34 -0.8903196557464592
35 -0.9343711588762009
36 -0.9671325820874058
37 -0.9876051327062279
38 -0.9950590369845589
39 -0.989063263266266
40 -0.9695061547920707
41 -0.9366035297205952
42 -0.890910068102942
43 -0.8333258553780641
44 -0.7650885101012004
45 -0.6877639758542646
46 -0.6032932673429284
47 -0.5139549170579887
48 -0.4223410043855677
49 -0.3312886781290886
50 -0.24376554238354942
51 -0.16261235035557992
52 -0.0900426068804427
53 -0.027049027806346507
54 0.02702750971790352
55 0.07317396936600842
56 0.11217953781201392
57 0.14457275976484654
58 0.1708209888156951
59 0.19151537749531156
60 0.20747201682010916
61 0.21952620885102384
62 0.228539602668129
63 0.23511442530558582
64 0.2389440577391595
65 0.2389662596146412
66 0.23353325209186984
67 0.22067302248128404
68 0.19845762140805184
69 0.16529297906265156
70 0.1200325686887195
71 0.062009201603515196
72 -0.00883444671495151
73 -0.09192850789905957
74 -0.1860795310092689
75 -0.28952753185773883
76 -0.4000539216252631
77 -0.5151218566826758
78 -0.6320037534421246
79 -0.7479104253660628
80 -0.8601001664867134
81 -0.9659300509875959
82 -1.0629073299575265
83 -1.1487551207920224
84 -1.2214439543911202
85 -1.2792278484220465
86 -1.320666652308452
87 -1.3446592057482905
88 -1.3504804711637484
89 -1.3378075160199892
90 -1.3067497133670976
91 -1.2578436590650135
92 -1.1920171741594736
93 -1.1105768695288776
94 -1.0152085496384777
95 -0.908014787299818
96 -0.7915628362123347
97 -0.6688310927754442
98 -0.5431882867015126
99 -0.4183368270021931
100 -0.29817421226425045
101 -0.1862881417814235
102 -0.0857919591072799
103 0.001544008298199312
104 0.07586460728898292
105 0.13802507006666304
106 0.18921452389167298
107 0.23104759756774285
108 0.2658570890794466
109 0.2967944755250543
110 0.3274226270372893
111 0.36019968443625755
112 0.39463000357568967
113 0.4279784248270371
114 0.4565765533911774
115 0.47680242398753314
116 0.4853780149238058
117 0.4794291271056895
118 0.45647343906504395
119 0.41439394974721283
120 0.35140714529073536
121 0.2671031278137385
122 0.16237639784455707
123 0.03913415229223187
124 -0.09992401358399104
125 -0.25149004534184294
126 -0.41183033332196917
127 -0.5769230230032729
128 -0.7423310360333093
129 -0.9038232437447979
130 -1.0576301498760285
131 -1.2004801219487407
132 -1.329557097256659
133 -1.4424396608380978
134 -1.5370467878365448
135 -1.61158844992301
136 -1.6645245163313696
137 -1.6945295373503688
138 -1.7004617236311435
139 -1.6814995025215085
140 -1.637698659955332
141 -1.5698555100558398
142 -1.4793578369315372
143 -1.3681010420542383
144 -1.2384513419947112
145 -1.0932858363458806
146 -0.9361270224125507
147 -0.7714067953812852
148 -0.6039576553542751
149 -0.43824820023420596
150 -0.2781980951523265
151 -0.12723293731091057
152 0.011659605110976579
153 0.13590581299800908
154 0.2436410515586455
155 0.3344776766130848
156 0.4092490980587268
157 0.470010222593918
158 0.5203181806415511
159 0.5648767170017187
160 0.6081782466844384
161 0.6511754242005354
162 0.6912019998700792
163 0.7247490746049096
164 0.7483842083560074
165 0.759030067704526
166 0.7540272638418039
167 0.7311125944252895
168 0.6883708975889993
169 0.6241819344874565
170 0.5371738854543948
171 0.42618449462838914
172 0.29023970848898917
173 0.13088645847813418
174 -0.04646478717965849
175 -0.23540653939281916
176 -0.42992715576911833
177 -0.6247572636009816
178 -0.8159204872711026
179 -0.9996389380110181
180 -1.172547256135113
181 -1.3317236533575172
182 -1.474655819032376
183 -1.599193206923686
184 -1.7035054244650758
185 -1.7860388142482804
186 -1.8454760010175961
187 -1.8807009629647664
188 -1.8907677528726023
189 -1.874873079033251
190 -1.832331451266463
191 -1.7625565058947648
192 -1.6650501329766283
193 -1.5393913404703008
194 -1.387845503934974
195 -1.215954084749816
196 -1.0304381413783958
197 -0.8376366423642885
198 -0.6425230995600997
199 -0.4475129610874379
200 -0.25621902896219895
201 -0.07225330444817063
202 0.1011144627749562
203 0.26102262413269695
204 0.4050013896439666
205 0.5309309061227095
206 0.6369979656604949
207 0.7216566807593948
208 0.78544892371389
209 0.8325151474965908
210 0.8684112801573952
211 0.8963597288459566
212 0.9167323157296712
213 0.9285184454190588
214 0.9292782519150838
215 0.9163709038172204
216 0.887351280493304
217 0.840074543575626
218 0.7727002255120774
219 0.683665199176138
220 0.5716449421063172
221 0.4355127786343863
222 0.2763041851488114
223 0.0992601561256673
224 -0.08925661187321621
225 -0.28323076431775945
226 -0.47778081680780693
227 -0.6714032830583978
228 -0.8607547601506159
229 -1.0422501297773732
230 -1.212573154211519
231 -1.3688156788625934
232 -1.5084925912528067
233 -1.6294926683448026
234 -1.7300274889476623
235 -1.8085905692500652
236 -1.8639190311735592
237 -1.8949533326837409
238 -1.900800865715313
239 -1.8807024589268746
240 -1.8340101889047746
241 -1.7601791642707367
242 -1.6587525303757882
243 -1.5293425765132482
244 -1.3738675370082798
245 -1.198673681835308
246 -1.0106236534574622
247 -0.8159795024477564
248 -0.6201777075766528
249 -0.4247951476292997
250 -0.22937545257476077
251 -0.03381168188160677
252 0.16085113997346429
253 0.3514726211228245
254 0.5345972016276092
255 0.7070057151459141
256 0.8658530695281516
257 1.008670981432627
258 1.1333326784000959
259 1.2380091319802502
260 1.3211299810360746
261 1.381350525673442
262 1.4175203911928496
263 1.4286570110232408
264 1.413923249046111
265 1.3726073147567825
266 1.3041041325489007
267 1.207900053254954
268 1.0835595244830944
269 0.9323185115682605
270 0.7604377058689313
271 0.5748848475119703
272 0.3820742978399038
273 0.1876021657601227
274 -0.006379381004010615
275 -0.19926089620218115
276 -0.3938824165872698
277 -0.5879624532866086
278 -0.7778984105236904
279 -0.9600387271412718
280 -1.1310689814780561
281 -1.2880974420533464
282 -1.4286424930142285
283 -1.5505905893324745
284 -1.6521484492156588
285 -1.7317975393003506
286 -1.7882529332888213
287 -1.8204268053510837
288 -1.8273984667744498
289 -1.8083884380526762
290 -1.7627366895865126
291 -1.689884308646993
292 -1.5893582038609515
293 -1.4607589353396595
294 -1.305987161088808
295 -1.131406621405218
296 -0.9439095899281167
297 -0.7497914498702294
298 -0.5545255815391408
299 -0.3593034180765469
300 -0.1646863985421485
301 0.03050249158682672
302 0.2247602410429673
303 0.4147935599308886
304 0.5970920967232257
305 0.768416540892625
306 0.9259173088184656
307 1.0671326977495594
308 1.1899517134406772
309 1.2925699957382417
310 1.3734476997160119
311 1.4312723770043507
312 1.4649269212056608
313 1.4734615374049962
314 1.456069438611462
315 1.4120658726363131
316 1.3408700385818895
317 1.241989471277124
318 1.1150067869781586
319 0.9615961417967387
320 0.7880865372351428
321 0.6013989044042182
322 0.40787539384192334
323 0.21304197773432626
324 0.018181092316686243
325 -0.17536035958008064
326 -0.3702534036367616
327 -0.5644202274563423
328 -0.754359417525156
329 -0.9364793373738718
330 -1.1075063814680939
331 -1.2645765585230162
332 -1.4052248715392333
333 -1.5273448210646172
334 -1.6291423121612663
335 -1.709092513462387
336 -1.765901022460918
337 -1.7984685457710607
338 -1.8058621828973926
339 -1.7872913083737172
340 -1.7420857558916725
341 -1.6696777901881883
342 -1.5695865442517114
343 -1.4414051613433667
344 -1.2869952926899029
345 -1.112715878332398
346 -0.9254669993903649
347 -0.7315563737942632
348 -0.5364724249231199
349 -0.3414013940135582
350 -0.14763964156018983


==> plotdata/quadrotor/A2_x2_phase2.tex <==
350 -0.14763964156018983
351 0.047426325078603004
352 0.24173887120929505
353 0.43181503701504453
354 0.6135926788742279
355 0.7832199730684903
356 0.9372710911953988
357 1.0727713413508484
358 1.1871632361744975
359 1.2782577468009604
360 1.346247575673074
361 1.3936721887850536
362 1.4239666486551947
363 1.440493318072059
364 1.4461433670888886
365 1.4432587913741646
366 1.4336859074084694
367 1.4188647889230817
368 1.3999160226045892
369 1.3777133828996018
370 1.3529411586218216
371 1.3261380809313086
372 1.2977309270562267
373 1.268060140626715
374 1.2373993672620938
375 1.2059703082811997
376 1.1739544315499482
377 1.1415011150704066
378 1.108734666581263
379 1.075759444596675
380 1.0426637701451802
381 1.0095228356200114
382 0.976401097377604
383 0.9433540958664722
384 0.9104298683704297
385 0.8776700494283639
386 0.8451107619282424
387 0.8127833555600743
388 0.780714987269233
389 0.7489291097592208
390 0.7174458950592207
391 0.6862825855425908
392 0.6554538145134448
393 0.6249768958944993
394 0.5948794619601836
395 0.5651986929857751
396 0.5359753214233515
397 0.5072471939430502
398 0.47904534217223194
399 0.4513910853446976
400 0.42430436460277693
401 0.3978090890874334
402 0.3719265071716611
403 0.34666633033743954
404 0.3220212557955119
405 0.2979668252162055
406 0.2744638907227053
407 0.25146314255715163
408 0.2289092656077059
409 0.20674605513167832
410 0.18492080773806363
411 0.1633871798503931
412 0.14210620700615076
413 0.12104788089318266
414 0.10019057702789219
415 0.07951909486273098
416 0.059024289346124276
417 0.03870145283212898
418 0.018548310768028757
419 -0.0014321805488927697
420 -0.021233044153439865
421 -0.040846807737935906
422 -0.06026615705257857
423 -0.0794843705754883
424 -0.09848714113857496
425 -0.11724940378070553
426 -0.1357410481803159
427 -0.15393271443471276
428 -0.17179971496756757
429 -0.18932358455684864
430 -0.20649237675208862
431 -0.2233009841220982
432 -0.2397498319500942
433 -0.25584376386199303
434 -0.2715907630150636
435 -0.2870014817786598
436 -0.30208887885823316
437 -0.31686664822612726
438 -0.3313488378892397
439 -0.3455492119894531
440 -0.359480397397656
441 -0.37315451298598135
442 -0.3865831943383662
443 -0.39977727443212857
444 -0.41274655643801333
445 -0.4254999107684729
446 -0.43804520597847807
447 -0.4503896280846234
448 -0.4625394894449314
449 -0.4745002777365899
450 -0.48627670358824115
451 -0.4978728213526736
452 -0.5092920344006239
453 -0.5205370120923658
454 -0.5316103896724572
455 -0.5425143538295942
456 -0.5532505574068871
457 -0.563820432601114
458 -0.5742251335880443
459 -0.5844655176689656
460 -0.5945418162120226
461 -0.6044541425576602
462 -0.6142024484272082
463 -0.6237869007257104
464 -0.6332074848504279
465 -0.6424641621728785
466 -0.6515568380519101
467 -0.660485530378853
468 -0.6692500576681828
469 -0.6778503862217407
470 -0.6862864039001134
471 -0.6945579640138044
472 -0.7026648199532992
473 -0.7106067344082244
474 -0.7183835723599723
475 -0.7259952867749695
476 -0.7334416975364996
477 -0.7407227468411891
478 -0.7478385854639598
479 -0.7547894026946665
480 -0.7615752035578792
481 -0.7681960872590355
482 -0.7746522153614344
483 -0.7809437920090206
484 -0.7870711337620492
485 -0.7930347891447272
486 -0.7988352244900891
487 -0.8044727918891248
488 -0.8099480455674636
489 -0.8152614560326356
490 -0.8204136623429269
491 -0.8254054130859049
492 -0.8302375531016628
493 -0.8349110053529949
494 -0.8394267762582446
495 -0.8437859438119789
496 -0.8479896489216698
497 -0.8520390981729956
498 -0.8559355626063672
499 -0.8596803171528882
500 -0.8632747387613429
501 -0.8667203175302555
502 -0.8700186372375266
503 -0.8731713648929255
504 -0.8761802737874991
505 -0.8790503366431618
506 -0.8817893483844728
507 -0.884405621902228
508 -0.8869065024615951
509 -0.8892977054330506
510 -0.8915831724965709
511 -0.8937651773444063
512 -0.8958445830909716
513 -0.8978211513936009
514 -0.8996939019389906
515 -0.9014614823998159
516 -0.9031224449024849
517 -0.9046754858185909
518 -0.906119684334083
519 -0.9074547123863707
520 -0.908637778291117
521 -0.9096020699317994
522 -0.9102839437369923
523 -0.9106404772126394
524 -0.9106548756577926
525 -0.910333357243771
526 -0.9097015117929548
527 -0.9087997783641845
528 -0.9076798368952033
529 -0.9064008561423024
530 -0.905025447329664
531 -0.9036144854324342
532 -0.9022210185148205
533 -0.900881156008596
534 -0.8996181091778838
535 -0.898439305749854
536 -0.8973416298481485
537 -0.8963166844613687
538 -0.8953619967579329
539 -0.8944822105331078
540 -0.8936858768963369
541 -0.8929806529256132
542 -0.8923700102624446
543 -0.8918507262304722
544 -0.8914115685022304
545 -0.8910372923268658
546 -0.8907110241359275
547 -0.8904158251929575
548 -0.8901352911357536
549 -0.8898536783821646
550 -0.8895557482542497
551 -0.889226555437618
552 -0.8888512903583745
553 -0.888415058588907
554 -0.887902956184933
555 -0.8873001646310127
556 -0.8865921651198756
557 -0.8857646152646981
558 -0.8848031498763855
559 -0.8836941455010883
560 -0.8824248412893885
561 -0.880983236238863
562 -0.8793581121792721
563 -0.8775389757588621
564 -0.8755158554833078
565 -0.8732799344002248
566 -0.8708234977089647
567 -0.8681395744171786
568 -0.8652219132733198
569 -0.8620651814434963
570 -0.858664986823443
571 -0.855017436844854
572 -0.8511201773102955
573 -0.8469715724742252
574 -0.84257046472783
575 -0.8379164059587465
576 -0.833009555473949
577 -0.8278504961327227
578 -0.8224403419891062
579 -0.8167804885944643
580 -0.8108727717355877
581 -0.8047193808603923
582 -0.7983229369758996
583 -0.791686003550225
584 -0.7848112831424925
585 -0.7777017297725054
586 -0.7703605124326125
587 -0.762791048470535
588 -0.7549964923675354
589 -0.7469800341475059
590 -0.7387451029762966
591 -0.730294956125316
592 -0.7216326924541107
593 -0.7127615495439817
594 -0.7036847438304665
595 -0.6944053743647922
596 -0.6849264266624562
597 -0.6752510119245706
598 -0.6653820749464785
599 -0.6553223709914552
600 -0.6450747056430596
601 -0.6346418022894151
602 -0.624026560076773
603 -0.6132312415863567
604 -0.6022580084958536
605 -0.591109052578788
606 -0.579786366883293
607 -0.5682919196364471
608 -0.5566279065878957
609 -0.544796451622474
610 -0.5327995056715014
611 -0.5206389099367436
612 -0.5083164370186666
613 -0.49583359360914814
614 -0.48319196892675165
615 -0.47039312066321354
616 -0.45743854491477703
617 -0.44432967892237596
618 -0.43106788321136635
619 -0.41765446238350046
620 -0.40409066818393835
621 -0.39037770041536335
622 -0.37651671257212166
623 -0.3625088127824662
624 -0.3483550712316253
625 -0.3340565037227908
626 -0.319614057585108
627 -0.3050287051859096
628 -0.29030139422871765
629 -0.275432976066475
630 -0.2604243936124113
631 -0.245276472268813
632 -0.2299900275238046
633 -0.21456598290101672
634 -0.19900499431406216
635 -0.18330803760137848
636 -0.16747558890409955
637 -0.15150842220101177
638 -0.13540747070261733
639 -0.11917342440414032
640 -0.10280661968381959
641 -0.08630754937138546
642 -0.06967661932564082
643 -0.05291463025657396
644 -0.03602242300830581
645 -0.019000571475458337
646 -0.0018497353529697523
647 0.015429553571519095
648 0.03283702653781115
649 0.05037215270050871
650 0.06803444398145259
651 0.08582323838679444
652 0.10373792874822745
653 0.12177797102502565
654 0.13994280550106217
655 0.15823205049997222
656 0.1766452280675468
657 0.1951819233531508
658 0.21384151749600405
659 0.23262353412807188
660 0.2515274666264132
661 0.2705529218170697
662 0.2896994924031018
663 0.30896669926440123
664 0.32835403909181404
665 0.34786101712882483
666 0.36748723419608725
667 0.38723232723813716
668 0.40709558136442814
669 0.42707651142789127
670 0.4471751557628875
671 0.467391067924344
672 0.48772349260684333
673 0.5081715766991476
674 0.5287354765742005
675 0.5494146594513423
676 0.5702085869644862
677 0.591117161880793
678 0.6121398574821274
679 0.6332764183426702
680 0.654526536397151
681 0.6758898355055605
682 0.6973658787790838
683 0.7189543601631087
684 0.7406544848487987
685 0.7624658830582891
686 0.7843882843388521
687 0.8064213459944056
688 0.8285648603491711
689 0.8508186787314211
690 0.8731823665452433
691 0.8956554489614
692 0.9182374565214647
693 0.9409275798428081
694 0.9637258309448149
695 0.986631997213969
696 1.0096457737846678
697 1.0327665212860913
698 1.0559939378530114
699 1.0793276113416015
700 1.1027672828745476


==> plotdata/quadrotor/A2_x3_phase1.tex <==
0 0.0
1 0.0
2 2.522426711948356e-15
3 3.630873379734112e-14
4 4.7251091928046665e-15
5 -1.5830892152735033e-13
6 -5.158184990250447e-13
7 -1.1179146497397597e-12
8 -2.0252244326002254e-12
9 -3.3427838275201792e-12
10 -5.186340246154941e-12
11 -7.732072759836227e-12
12 -1.0723084642449975e-11
13 -1.3367049689350096e-11
14 -1.5884467075011343e-11
15 -1.8387318334589508e-11
16 -2.0813484269410763e-11
17 -2.3042989738542018e-11
18 -2.498188322874739e-11
19 -2.7248887590758383e-11
20 -2.936580756340845e-11
21 -3.12861203610737e-11
22 -3.3207445682137406e-11
23 -3.518573876704068e-11
24 -3.727937070152621e-11
25 -3.9378189597982784e-11
26 -4.113246632186929e-11
27 -4.2317740422959106e-11
28 -4.3050203402117405e-11
29 -4.347418425254546e-11
30 -4.364828498637507e-11
31 -4.3704133645405815e-11
32 -4.358094329859341e-11
33 -4.3221852763508647e-11
34 -4.2908645525585595e-11
35 -4.2843861791652666e-11
36 -4.336657255521458e-11
37 -4.478781789885033e-11
38 -4.73451322591245e-11
39 -5.172870132241768e-11
40 -5.927352830781272e-11
41 -7.17035497643792e-11
42 -9.163077407947638e-11
43 -1.229929402768448e-10
44 -1.73784258095111e-10
45 -2.538688015363277e-10
46 -3.7623435034106476e-10
47 -5.57381838461879e-10
48 -8.168017551213325e-10
49 -1.176613242392932e-09
50 -1.6613821607336377e-09
51 -2.296850354355229e-09
52 -3.1110100273679112e-09
53 -4.1305642461964e-09
54 -5.374288800652494e-09
55 -6.848875244713782e-09
56 -8.546066574410816e-09
57 -1.0435860211543969e-08
58 -1.2456415010575485e-08
59 -1.4509230634729421e-08
60 -1.6451159297048437e-08
61 -1.8220745392483198e-08
62 -1.9761671676832297e-08
63 -2.1016785041183542e-08
64 -2.195769900126266e-08
65 -2.2542774065215104e-08
66 -2.2720339103443627e-08
67 -2.2505669416972304e-08
68 -2.1937722003428923e-08
69 -2.1052969376711425e-08
70 -1.9885041577794034e-08
71 -1.8473957226206045e-08
72 -1.685370730086789e-08
73 -1.5054847839479642e-08
74 -1.31080645893178e-08
75 -1.1046296251038265e-08
76 -8.905711101903087e-09
77 -6.812229589314718e-09
78 -4.9289544179487235e-09
79 -3.4435168139168654e-09
80 -2.5588814978050397e-09
81 -2.7580187911269225e-09
82 -4.87317389996634e-09
83 -1.0266823871063489e-08
84 -2.1279512534277965e-08
85 -4.1564700126173206e-08
86 -7.555724119256981e-08
87 -1.2991814484664136e-07
88 -2.1451539980787975e-07
89 -3.4354224668575746e-07
90 -5.374320150330903e-07
91 -8.249581848218668e-07
92 -1.2466157096469034e-06
93 -1.85804747353302e-06
94 -2.734260929209143e-06
95 -3.974514968856369e-06
96 -5.705917916660753e-06
97 -8.087530408129597e-06
98 -1.1314501283639092e-05
99 -1.561831453546603e-05
100 -2.125193521813174e-05
101 -2.8475093197499754e-05
102 -3.749855293696314e-05
103 -4.846168041646949e-05
104 -6.143166931117606e-05
105 -7.643243070061702e-05
106 -9.338628181710718e-05
107 -0.00011192939159487382
108 -0.00013135319533990496
109 -0.00015056649776418852
110 -0.00016804156334165654
111 -0.00018173055934257222
112 -0.00019085310309929326
113 -0.0001957241586545244
114 -0.0001967084105329242
115 -0.0001941571379488316
116 -0.00018847250964070027
117 -0.00018011037884217983
118 -0.00016953178932137546
119 -0.00015716115858984024
120 -0.00014336870183951687
121 -0.00012846294647976818
122 -0.00011267589452755187
123 -9.617112773559808e-05
124 -7.907493909051764e-05
125 -6.148416075909322e-05
126 -4.347059026317265e-05
127 -2.5225721964314795e-05
128 -7.211814843159878e-06
129 1.0051338808381198e-05
130 2.4446271950058257e-05
131 3.098579644838399e-05
132 2.0415952665224817e-05
133 -2.4225758388762813e-05
134 -0.00013263916327828083
135 -0.00035210427466271456
136 -0.0007564388709266902
137 -0.0014515778292598649
138 -0.0025737710687175233
139 -0.004204435819827292
140 -0.006366215356318339
141 -0.00909890828924434
142 -0.012457568515155143
143 -0.016513304997842457
144 -0.021353140138292766
145 -0.027076904726873786
146 -0.03379958544341594
147 -0.041635308198170906
148 -0.05067601333672619
149 -0.06091393104306401
150 -0.07225926429305322
151 -0.08460279677023723
152 -0.09779440305911831
153 -0.11163083939763543
154 -0.12583639343824005
155 -0.140045097202014
156 -0.15378932492832065
157 -0.1664829841341491
158 -0.17739905125646807
159 -0.1856431772989366
160 -0.19012118204033723
161 -0.18953554214616325
162 -0.18455827891917523
163 -0.17620968356768468
164 -0.16540311523666443
165 -0.1529384787463448
166 -0.1394089211837391
167 -0.12531384809136364
168 -0.11107040602479719
169 -0.0970187062614152
170 -0.08342651815169144
171 -0.0704976843897731
172 -0.05838487628537576
173 -0.04719875890532744
174 -0.03701211696729302
175 -0.02785984284900623
176 -0.01974591056591036
177 -0.012658464328995239
178 -0.006573218646154257
179 -0.0014625031711700456
180 0.0027074054094341484
181 0.005972773731485365
182 0.008369415911291048
183 0.009940679333348315
184 0.01073561711742928
185 0.010794108398771152
186 0.010146776725968008
187 0.008805200148919393
188 0.006757065571564972
189 0.003968838993412638
190 0.0004204090304908469
191 -0.003908647073225938
192 -0.009065148177067446
193 -0.015120036451972789
194 -0.022166303817760035
195 -0.030316172766975263
196 -0.03969124455701449
197 -0.05040704547923065
198 -0.06254424761922389
199 -0.07607839755576953
200 -0.09089031019733176
201 -0.1067948829346868
202 -0.12352791444874886
203 -0.14073097852217678
204 -0.1579305216432381
205 -0.17451740447973935
206 -0.1897262169249034
207 -0.20262264956950052
208 -0.21208816061982763
209 -0.21679245382872506
210 -0.21514034226265236
211 -0.2052328701825366
212 -0.18778486224579713
213 -0.16555752077809233
214 -0.1410393912366389
215 -0.11606393560068701
216 -0.09175246270211534
217 -0.06892303198991363
218 -0.04814214342564628
219 -0.02976598206183193
220 -0.013975397087904344
221 -0.0008053712467755974
222 0.009816747048145457
223 0.01803111049498524
224 0.024018643999136512
225 0.027993974403862844
226 0.03019783008285915
227 0.030883702597735933
228 0.030350658560001003
229 0.028933736079903967
230 0.026977348907100088
231 0.024782709036525397
232 0.022564876616663204
233 0.02046711117575572
234 0.01858596042932074
235 0.016984442545015493
236 0.01570434169798369
237 0.014759623784525375
238 0.014130965669593628
239 0.013763946459933516
240 0.013597680161850626
241 0.013573212496580408
242 0.013612078224520185
243 0.01361379314900739
244 0.01345519649749262
245 0.012991251559222287
246 0.012061396981715612
247 0.010501477987087995
248 0.008166623984952204
249 0.004998269716968028
250 0.0010085279618191629
251 -0.003751402200077772
252 -0.009181040867894369
253 -0.015117561975045646
254 -0.021318367939615616
255 -0.027441496829088568
256 -0.03302720263345443
257 -0.037477274863633156
258 -0.04003586539762386
259 -0.03976706914290311
260 -0.035521752705951315
261 -0.025900821204448782
262 -0.012180187874600602
263 0.002249980321562886
264 0.014184191757145219
265 0.022867934321765128
266 0.02858244729787128
267 0.0316972269432187
268 0.032639024123442786
269 0.03186655393630742
270 0.029847290080647307
271 0.027041044684177555
272 0.023872822752611184
273 0.02070374506822632
274 0.017812382667758524
275 0.015387339274132432
276 0.013509574714176364
277 0.012110406814314256
278 0.011030010194292379
279 0.010094136070934163
280 0.009181954897308333
281 0.00827089690869994
282 0.007398226622079661
283 0.0066184383077414685
284 0.005982203574101149
285 0.005525985064143695
286 0.00527523546290409
287 0.005234920558153892
288 0.0053832295047017515
289 0.00566924416844377
290 0.006040953170877181
291 0.006452567873815176
292 0.0068421173146274205
293 0.007127704010370462
294 0.007205536530903312
295 0.006949288590374737
296 0.006215028643640153
297 0.00485173384225818
298 0.002722904922501245
299 -0.0002274332771820503
300 -0.003990933656237985
301 -0.008526646865117121
302 -0.01375048086072869
303 -0.019521317398744416
304 -0.025622264732670826
305 -0.031739238038018015
306 -0.03744020658440193
307 -0.04215172615648974
308 -0.04513664032757169
309 -0.04546836934253208
310 -0.041994642125143526
311 -0.03329831084835347
312 -0.0206211761762296
313 -0.007304842004428273
314 0.003503560153424616
315 0.011111448784245902
316 0.015859323620655195
317 0.018168217160860853
318 0.01850507750207159
319 0.01735542695096538
320 0.01519946706956076
321 0.01249632321681369
322 0.009658326510488171
323 0.007024304243515226
324 0.004843353594020976
325 0.0032699455862353318
326 0.0023488848210040324
327 0.001975044667344557
328 0.0019536391151108584
329 0.0020780739321759664
330 0.00219857002756668
331 0.002267774797930228
332 0.002302525872849744
333 0.002341741335731451
334 0.0024253852680712444
335 0.002583866843339396
336 0.002841291366894967
337 0.0032055360439482063
338 0.0036615018821805406
339 0.0041682821536123595
340 0.004686551754464922
341 0.005185189441986516
342 0.005618083189700424
343 0.005919577384481197
344 0.006001465510504705
345 0.005751942201827653
346 0.005038959837706166
347 0.0037199706002654406
348 0.001662880213628671
349 -0.0011887075141330007
350 -0.004832010544315101


==> plotdata/quadrotor/A2_x3_phase2.tex <==
350 -0.004832010544315101
351 -0.0092367702429597
352 -0.014088565630635607
353 -0.01617656752266001
354 -0.017053969501540745
355 -0.017405145318776055
356 -0.017561437239729905
357 -0.01764370062048608
358 -0.017694973030591633
359 -0.017731164984101114
360 -0.017756706594882894
361 -0.017768099245730983
362 -0.0177720467950654
363 -0.017773630324036848
364 -0.017774740231115978
365 -0.017775344339346223
366 -0.017775620593038
367 -0.01777575266362766
368 -0.01777581886311886
369 -0.017775852309709614
370 -0.017775869067329222
371 -0.01777587735932276
372 -0.01777588141072153
373 -0.017775883361720427
374 -0.01777588427345392
375 -0.017775884655946428
376 -0.01777588472831236
377 -0.017775884609039356
378 -0.017775884353722075
379 -0.017775883996068557
380 -0.01777588353983162
381 -0.017775882956080825
382 -0.017775882266642624
383 -0.017775881452492044
384 -0.017775880505182504
385 -0.01777587941897799
386 -0.017775878195637
387 -0.017775876814159507
388 -0.01777587526610024
389 -0.017775873524515224
390 -0.017775871126681306
391 -0.017749528560305955
392 -0.017661229499465015
393 -0.01748462863882459
394 -0.017198057413071833
395 -0.016785334986889097
396 -0.016232804718225153
397 -0.01552643240692991
398 -0.014648262630940287
399 -0.013569315660973599
400 -0.012249238151007508
401 -0.010636973177944643
402 -0.008671856386026383
403 -0.00628840529549627
404 -0.003422880241817027
405 -2.228402459147818e-05
406 0.003947379987853862
407 0.008491351044988852
408 0.013580726889792942
409 0.019153519861821962
410 0.02512135359962219
411 0.031373871861014674
412 0.037791329823899766
413 0.044256620523679055
414 0.050659497062339964
415 0.0569061420898441
416 0.06291951612353307
417 0.06863862938754858
418 0.07402057225152377
419 0.0790414620315575
420 0.08368985891927108
421 0.08796792434098157
422 0.09187708702183046
423 0.09542509779974115
424 0.09862919531923693
425 0.10151518092091319
426 0.1041118574015116
427 0.10644955993116755
428 0.10855755648670448
429 0.11046775705423513
430 0.11220672012284184
431 0.11379722375555652
432 0.11526014747455883
433 0.11662145775255744
434 0.11790088365396738
435 0.11911974305703527
436 0.12029836149518995
437 0.12145640853997783
438 0.12261267898166692
439 0.1237835943624621
440 0.12498358785724395
441 0.12622385320366056
442 0.12751227589851385
443 0.1288542451337659
444 0.13025342616873967
445 0.13171170713963884
446 0.13322907214606516
447 0.1348047852652713
448 0.1364374414933747
449 0.1381245390356514
450 0.13986328182408447
451 0.14165052992226188
452 0.14348326782599177
453 0.14535842709726157
454 0.14727287677857817
455 0.14922360735106321
456 0.15120730366233798
457 0.15322118764299503
458 0.15526175781501764
459 0.1573270377390063
460 0.1594118383453994
461 0.16151289245264638
462 0.163625616562802
463 0.16574610171662402
464 0.16787066060218506
465 0.1699960628226684
466 0.17212050058494988
467 0.17423946416779632
468 0.17634975220086874
469 0.1784473001329214
470 0.18052860981313743
471 0.18259064451218096
472 0.18463047851780776
473 0.18664510457224529
474 0.18863178000500597
475 0.19058756755275158
476 0.19250981188591285
477 0.19439609474888433
478 0.19624416305822498
479 0.19805199775124663
480 0.1998176515135364
481 0.20153917600852672
482 0.20321464198141032
483 0.20484173575533327
484 0.20641807964749714
485 0.2079414711716179
486 0.20940930162204424
487 0.21082039314608286
488 0.21217470019200382
489 0.21347123313541402
490 0.21470870092398997
491 0.21588693204488704
492 0.21700662557202247
493 0.21806835828170906
494 0.21907230778385298
495 0.22001836152966156
496 0.22090634324036643
497 0.22173624052035412
498 0.22250820532685156
499 0.2232225013413293
500 0.22387952059609523
501 0.22447987875539985
502 0.22502465820160036
503 0.22552429128423238
504 0.225987258098399
505 0.22641342017020186
506 0.2267954497826282
507 0.22712212179435348
508 0.22738151986838917
509 0.22756461087271623
510 0.227668521872694
511 0.22770469989760606
512 0.22769507244384288
513 0.22765877370147217
514 0.22760816754639987
515 0.22755017463077332
516 0.22748842691308963
517 0.22742474073850957
518 0.22763362596494296
519 0.22835517206905118
520 0.22967485468524262
521 0.23158887808493747
522 0.23406178606889483
523 0.2370485797310124
524 0.24049650935801814
525 0.24434678494276094
526 0.2485322464064246
527 0.2529724496063512
528 0.2575655100340499
529 0.26218583864607525
530 0.26669933346037
531 0.27101721502956433
532 0.2751011111999552
533 0.27897416042495665
534 0.2826617411043715
535 0.28619550382908937
536 0.2896334295694204
537 0.2930021828160923
538 0.29630885136006563
539 0.29953369400159474
540 0.3026350529561508
541 0.30552825801549865
542 0.3081955162440421
543 0.3105304315379068
544 0.3126023390529963
545 0.31454100957292946
546 0.31645226772048224
547 0.31839754540696247
548 0.3204065022138592
549 0.322488127320318
550 0.3246410357994506
551 0.32686890283203207
552 0.32916943558333045
553 0.33153390240030467
554 0.333949432094391
555 0.33640362654271855
556 0.33888876149188424
557 0.3413980658719913
558 0.34391931924669106
559 0.34643758481546305
560 0.3489371475613042
561 0.35140764593120816
562 0.35385061368111065
563 0.3562532228068266
564 0.3586083279147797
565 0.36091965653828
566 0.3631906226130829
567 0.36541785687723394
568 0.36759538263498504
569 0.36972743622781706
570 0.37180064113085354
571 0.3738099541429076
572 0.37575719100779087
573 0.3776376230770603
574 0.3794506842193438
575 0.38120007683867224
576 0.3828830780890706
577 0.38449994059049164
578 0.38605072298476595
579 0.3875374837245335
580 0.38895649849466507
581 0.3903108579702919
582 0.39160310979411983
583 0.3928364672579018
584 0.39400908422528164
585 0.39512231808111364
586 0.39617960259177293
587 0.39717995224494607
588 0.3981277295908807
589 0.39902506497751766
590 0.3998812351815473
591 0.40068956525987853
592 0.40145047046044857
593 0.40216006725032966
594 0.402831623971291
595 0.4034690534305766
596 0.4040648778106704
597 0.40462912824341235
598 0.4051669660471197
599 0.4056661548970817
600 0.40613133919552363
601 0.40656416240917076
602 0.40697683722439937
603 0.4073717405159009
604 0.40773571019376414
605 0.40808378100458603
606 0.4084149171711573
607 0.4087090021118378
608 0.40896077605004605
609 0.40917774768213466
610 0.40939524180591746
611 0.40961573501911336
612 0.4098014450418206
613 0.40995513542090956
614 0.41008618172540473
615 0.4102017003402954
616 0.41030692986198475
617 0.41040419581332555
618 0.4104948651640815
619 0.4105799416369154
620 0.4106601763019425
621 0.41073588356884544
622 0.4108074447106573
623 0.41090709212169974
624 0.41099314461737235
625 0.41106089817774344
626 0.4111146612452223
627 0.4112110001920643
628 0.4112988692058251
629 0.41135929860993636
630 0.411398867375117
631 0.41146915653634575
632 0.41154300109473096
633 0.4116293388718631
634 0.41172511580316645
635 0.4118142016708434
636 0.4118836943673224
637 0.41195497003390075
638 0.4119987301147156
639 0.41202695880360146
640 0.4120513089217102
641 0.4120805649109812
642 0.4121210286707613
643 0.41216798243279457
644 0.4122049587434961
645 0.4122395969723865
646 0.4122604898337949
647 0.4122850269926896
648 0.41231324532723984
649 0.41235321633011246
650 0.41238688682432184
651 0.41241414532166054
652 0.41243172554192276
653 0.4124569906026206
654 0.41246540879978233
655 0.4124854594645851
656 0.41251877946240295
657 0.412540392098332
658 0.41254649142068983
659 0.4125436921746787
660 0.4125370182701129
661 0.4125287417404479
662 0.4125202153926592
663 0.41251083075517087
664 0.4125008780480036
665 0.4124897323688568
666 0.41247826541796334
667 0.41246525956798646
668 0.41245269303145277
669 0.4124346180747083
670 0.4124150706143028
671 0.4123981136591441
672 0.4123852126447971
673 0.41237078521339265
674 0.41235820393484884
675 0.4123508093939814
676 0.41235297087395667
677 0.4123487188496654
678 0.4123534430038221
679 0.4123581569238822
680 0.4123544289929088
681 0.4123501591275194
682 0.4123468160682832
683 0.4123456032835253
684 0.41234413849404944
685 0.41234362101120486
686 0.4123348663127894
687 0.4123221095599102
688 0.4123103019405593
689 0.4123075670347869
690 0.41231056553744405
691 0.41231307424939306
692 0.41231803923105353
693 0.412341849916286
694 0.4123674863493735
695 0.4123914448140199
696 0.4123958410396389
697 0.4123963978629293
698 0.41239431243874775
699 0.41239209445481984
700 0.41239035897455945


==> plotdata/quadrotor/A3_x1_phase1.tex <==
0 0.5
1 0.5
2 0.5
3 0.5
4 0.4988051729340516
5 0.49493239806004025
6 0.48705098548761827
7 0.4741121913873786
8 0.4553684242731025
9 0.43042677305510274
10 0.39918447809677754
11 0.36176313556327044
12 0.3184526878552416
13 0.26971246272991156
14 0.21604695499399962
15 0.1583606475373165
16 0.09809712261283177
17 0.03721099989033205
18 -0.02204118267348222
19 -0.07731336496111846
20 -0.12631998998430605
21 -0.16693821105635154
22 -0.19729104002561032
23 -0.21583538252642906
24 -0.2214343648384912
25 -0.21341416341043049
26 -0.1915984652100391
27 -0.1563684083027469
28 -0.10860212581598055
29 -0.04959726647427097
30 0.01901319886136818
31 0.09530561806983014
32 0.17714507387364004
33 0.26224407826086316
34 0.34824017778096544
35 0.4327407691771143
36 0.5133881486475489
37 0.5879151316119706
38 0.65418434722431
39 0.7102404526275731
40 0.754359628641612
41 0.7851034282776933
42 0.8013929658334673
43 0.8025799608957337
44 0.7884715610435954
45 0.7593616059879916
46 0.7162861568740005
47 0.6609851555547525
48 0.5958624530303263
49 0.5239503957725107
50 0.44881508077146187
51 0.3743287241876958
52 0.30436248111039826
53 0.24241394420202822
54 0.19009689096457522
55 0.14814190461505602
56 0.11638684622137285
57 0.09331747427503606
58 0.07573795056176617
59 0.05999375576865376
60 0.04259586684812458
61 0.02043643781002211
62 -0.009093502796195405
63 -0.047971502856998485
64 -0.09764787403707378
65 -0.15835758707732855
66 -0.22756807188351108
67 -0.30076468169007875
68 -0.37327815816522436
69 -0.4408305093819885
70 -0.4996557696528767
71 -0.5464879549473329
72 -0.5785134203562455
73 -0.5933210612902655
74 -0.5888588584517354
75 -0.5633903906777117
76 -0.5154577280468501
77 -0.44538427745947323
78 -0.35496604766348067
79 -0.2468439773319121
80 -0.12414294298636556
81 0.009691816021645025
82 0.1510556063466325
83 0.29627467285281484
84 0.4414848689331317
85 0.5826769700703055
86 0.7161817194900657
87 0.8387742948540591
88 0.9476379201396801
89 1.040336249958042
90 1.11476857861283
91 1.1691279796850416
92 1.2018634808056707
93 1.2116485360690372
94 1.1973512905272359
95 1.1584089653281167
96 1.0957018266180252
97 1.011510793344291
98 0.9099048515382064
99 0.7968132062863212
100 0.6780713949432351
101 0.5588954542722242
102 0.4438075634882318
103 0.33669200558599754
104 0.2408788379442916
105 0.15922762802018278
106 0.0942032383093987
107 0.04489788789875983
108 0.006419045072928023
109 -0.026801351207428416
110 -0.05996113949665368
111 -0.09762483849410392
112 -0.14371161838369
113 -0.2015512668700451
114 -0.27266843790645595
115 -0.35318624575846513
116 -0.43803148112354107
117 -0.522278121806718
118 -0.6015301379512983
119 -0.6719785349719579
120 -0.7303544300845782
121 -0.7738647993981402
122 -0.8001264391520652
123 -0.8071061849747231
124 -0.7930709054278648
125 -0.7565454859705143
126 -0.696277349749005
127 -0.6112072181452936
128 -0.5004466725892591
129 -0.36494886742976523
130 -0.2101954884154868
131 -0.042711008857156146
132 0.13137504769585354
133 0.3066717415776986
134 0.4785378215332994
135 0.6430037340432494
136 0.796681569918195
137 0.9366841095997175
138 1.0605539607573218
139 1.1662069693756203
140 1.2518818326836156
141 1.3160599449227264
142 1.357427713139854
143 1.374849241948682
144 1.3673458604147937
145 1.3340794278656927
146 1.2743401707505941
147 1.188208589933179
148 1.081404291529948
149 0.9605943357445133
150 0.8319429013733898
151 0.7008685386847177
152 0.5721015640604126
153 0.44971512223701227
154 0.3371900843885394
155 0.23748895625551805
156 0.15313033545736646
157 0.08367696601992025
158 0.024453381051686617
159 -0.029978262436612287
160 -0.08473039282484718
161 -0.1443103014186566
162 -0.21258316822270626
163 -0.29280898150923645
164 -0.38229001618397696
165 -0.47627870104072023
166 -0.5699144045280772
167 -0.6587887167718305
168 -0.7390545450132193
169 -0.8073967439407641
170 -0.8609695414401675
171 -0.8973351487031261
172 -0.9144038363824465
173 -0.9103836781279043
174 -0.8837444135837584
175 -0.8331887544062939
176 -0.7576227773972646
177 -0.6561300905349086
178 -0.5279556429382202
179 -0.37431031021719197
180 -0.2012048130787797
181 -0.01530851935148253
182 0.17725313490662947
183 0.3711457439564402
184 0.5617978439546875
185 0.7452918277898121
186 0.9182931959399098
187 1.0779605351566464
188 1.2218662997815055
189 1.3479300482248076
190 1.4543643678716633
191 1.5396296536362677
192 1.6023976261155628
193 1.6415201563098036
194 1.6560042427531696
195 1.6449915667088684
196 1.6077442297197935
197 1.5436322600857915
198 1.452121462531594
199 1.337054669583336
200 1.2045565024839278
201 1.061012210566966
202 0.912263598476416
203 0.7634380879246578
204 0.6189718596509628
205 0.4826571343649495
206 0.3577200704567427
207 0.24686586689714918
208 0.14651461831241963
209 0.051510666877333064
210 -0.04324204674823098
211 -0.14230254420256394
212 -0.24958720240331483
213 -0.3626851497004231
214 -0.47729337613504685
215 -0.5889765737833715
216 -0.6936928387729069
217 -0.7879041080146726
218 -0.868557700307768
219 -0.9330335505102322
220 -0.9790941153752986
221 -1.0048340013978077
222 -1.0086357012722251
223 -0.9891278706903832
224 -0.9451460566916099
225 -0.8756935633523226
226 -0.7799239563345001
227 -0.6571613342280229
228 -0.5075350444956541
229 -0.33702414472828646
230 -0.15258305879746775
231 0.039317974134213035
232 0.2330380342295151
233 0.4270725520378572
234 0.6183695846900451
235 0.8033715319514274
236 0.9786896576306483
237 1.1412912907105355
238 1.2885114391656982
239 1.4180498407336086
240 1.5279378019289365
241 1.6165123718315775
242 1.682379676108917
243 1.7243735484895677
244 1.741502130591471
245 1.7329140760328394
246 1.697894306700943
247 1.6358450514961165
248 1.5462544247493062
249 1.4286878208115648
250 1.2827850701442338
251 1.1144499161621348
252 0.930741524163607
253 0.7382612309161614
254 0.542786867104609
255 0.34743014529736416
256 0.1521380309605314
257 -0.043233586281598874
258 -0.23862286377615544
259 -0.431104949744493
260 -0.6171523533249885
261 -0.7933958671711445
262 -0.9568332621774768
263 -1.104852834673725
264 -1.235206275251392
265 -1.3459673089779731
266 -1.4354897728004816
267 -1.5023698673664803
268 -1.5454126182814516
269 -1.5636012654334062
270 -1.5560760588654607
271 -1.5221086796057202
272 -1.461080355185819
273 -1.3724650246685584
274 -1.255815067064976
275 -1.1107485123254357
276 -0.9432427662244149
277 -0.7603889619542663
278 -0.5688148221550617
279 -0.3743246969569561
280 -0.17976399158626818
281 0.014770882789643475
282 0.2094322615853035
283 0.4039068116245608
284 0.5951600714563362
285 0.7796296158931835
286 0.9539365591031377
287 1.115083606251935
288 1.2604798066476919
289 1.3879105107105103
290 1.4954923931314508
291 1.5816277663247997
292 1.6449626220060691
293 1.684349918148136
294 1.6988177173139327
295 1.6875422526679524
296 1.649825422776547
297 1.5850758168933412
298 1.4927928915005104
299 1.3725539861389746
300 1.2245057609463386
301 1.0547060311341014
302 0.8701797071158917
303 0.6774515285968019
304 0.4822217158953104
305 0.28703080881499843
306 0.09231124857895959
307 -0.10285208426151071
308 -0.29790156745763996
309 -0.4897468721617846
310 -0.6748398082059035
311 -0.8498351083657415
312 -1.0117671389609642
313 -1.158064354264965
314 -1.2865173325512023
315 -1.3952366752939085
316 -1.4826108385838639
317 -1.547267584392167
318 -1.5880397483709923
319 -1.6039354715815637
320 -1.5941126767905807
321 -1.5578567590557861
322 -1.4945617282774
323 -1.4037139946671209
324 -1.2848779527914815
325 -1.1380059672101568
326 -0.9691281890471193
327 -0.7852966650273974
328 -0.5930780825669935
329 -0.39821865783397803
330 -0.2033369185480178
331 -0.00920347724238435
332 0.1857064923794181
333 0.38058595983065163
334 0.5722501005524125
335 0.7571079471501728
336 0.9317911607251317
337 1.093320938302003
338 1.239122441299842
339 1.3669906169420503
340 1.4750441564630241
341 1.561681462273713
342 1.625540808117471
343 1.6654658205854935
344 1.6804750956409518
345 1.669736076202358
346 1.6325422406339567
347 1.568294573204277
348 1.4764860047047446
349 1.3566876369154903
350 1.2090120564481721


==> plotdata/quadrotor/A3_x1_phase2.tex <==
350 1.2090120564481721
351 1.0395161826903832
352 0.8552363747797932
353 0.6627132384350224
354 0.4681473874207527
355 0.27702358118524495
356 0.09408450703169624
357 -0.07660032499266745
358 -0.23154835654096026
359 -0.3677825806328779
360 -0.48276005296476343
361 -0.5761755785911634
362 -0.6502009328812867
363 -0.7080451718296557
364 -0.7529389358931403
365 -0.7876935578415148
366 -0.8145957056529541
367 -0.8354451839802274
368 -0.8516358699656882
369 -0.8642384132687465
370 -0.8740715633392121
371 -0.8817601868953863
372 -0.8877815384831992
373 -0.8925019020734263
374 -0.8962054449517468
375 -0.8991166736040621
376 -0.9014175392936383
377 -0.9032601777243146
378 -0.9047759258141089
379 -0.9060814503919269
380 -0.9072826137562607
381 -0.9084766924860016
382 -0.9097534088375056
383 -0.9111952381146999
384 -0.9128773106946872
385 -0.9148671347539954
386 -0.9172242986569051
387 -0.9200002463935795
388 -0.9232381908910481
389 -0.9269731831174799
390 -0.9312323179969825
391 -0.9360350695606454
392 -0.9413937562990212
393 -0.94736222743474
394 -0.9540375680185904
395 -0.9615123094709624
396 -0.9698462229981942
397 -0.9790639529886164
398 -0.9891589152502469
399 -1.0001017082180652
400 -1.0118237301222577
401 -1.0242125300623683
402 -1.0371333463427677
403 -1.050451707882816
404 -1.0640460552088347
405 -1.0778124739083292
406 -1.0916649658587543
407 -1.1055333846363251
408 -1.1193614684152082
409 -1.133104884487315
410 -1.1467291173803005
411 -1.1602089220928222
412 -1.1735278007399406
413 -1.1866759295950735
414 -1.1996488862347383
415 -1.2124485085221766
416 -1.2250803155489232
417 -1.237552878378896
418 -1.2498766487538717
419 -1.2620609235529314
420 -1.2741138120786806
421 -1.28604352445791
422 -1.2978582042747424
423 -1.3095660360679042
424 -1.3211724392180435
425 -1.3326785308938653
426 -1.3440804049337418
427 -1.3553705253096846
428 -1.366539588371437
429 -1.3775782894660387
430 -1.3884779466737178
431 -1.3992321976334234
432 -1.4098358992371491
433 -1.4202851021389613
434 -1.4305768084465964
435 -1.4407105929652833
436 -1.4506869386846797
437 -1.4605076027141537
438 -1.4701750409650616
439 -1.4796917850508915
440 -1.4890601247525923
441 -1.4982821381818037
442 -1.5073602929390792
443 -1.5162960767825546
444 -1.525090652310173
445 -1.5337449732313686
446 -1.5422585887948346
447 -1.5506316492393657
448 -1.5588636322675382
449 -1.5669541819433495
450 -1.5749027659790311
451 -1.582708448435222
452 -1.5903703192093632
453 -1.5978874026894565
454 -1.605259090067822
455 -1.612484989770284
456 -1.6195646173812241
457 -1.6264976319174487
458 -1.6332835486104385
459 -1.6399221905592516
460 -1.6464131470725285
461 -1.6527563288895089
462 -1.6589513190844323
463 -1.664998045927411
464 -1.670896472159817
465 -1.6766466059724516
466 -1.6822486209047374
467 -1.6877029118312237
468 -1.6930098847683266
469 -1.698170052821175
470 -1.7031839442673329
471 -1.708052121844454
472 -1.712775137140198
473 -1.7173536293015215
474 -1.721788355841723
475 -1.7260801667877583
476 -1.7302298777245804
477 -1.7342384349679107
478 -1.7381069087522973
479 -1.7418364306031229
480 -1.7454281187555234
481 -1.7488831532191713
482 -1.752202731673342
483 -1.7553881230970463
484 -1.7584406589302861
485 -1.7613617375150845
486 -1.7641528272254494
487 -1.7668154952154769
488 -1.7693513827728147
489 -1.7717622221790479
490 -1.7740498375677638
491 -1.776216130752293
492 -1.7782631009259828
493 -1.7801928505010445
494 -1.782007609088503
495 -1.783709736750362
496 -1.7853017214651576
497 -1.7867861778670229
498 -1.788165845888946
499 -1.789443595070882
500 -1.790622440681646
501 -1.791705539162602
502 -1.7926962388988121
503 -1.7935980992713387
504 -1.7944148215950784
505 -1.7951503606993067
506 -1.79580948968852
507 -1.796397906454759
508 -1.7969218341538775
509 -1.7973872545110765
510 -1.7977983287913488
511 -1.798158042581385
512 -1.798469140166229
513 -1.7987346642236757
514 -1.7989581566208577
515 -1.7991436398034755
516 -1.7992954977923856
517 -1.7994182801194143
518 -1.7995165064209964
519 -1.7995944648591828
520 -1.7996559854328258
521 -1.7997071528163866
522 -1.7997581821783009
523 -1.7998235059168617
524 -1.799920638281598
525 -1.800067919867915
526 -1.8002813923579035
527 -1.8005716799910598
528 -1.8009413353022268
529 -1.8013826537526332
530 -1.8018781058312185
531 -1.8024017365334577
532 -1.8029192797987208
533 -1.8033918128401136
534 -1.803785080072405
535 -1.8040744366630106
536 -1.8042404157177525
537 -1.8042653599560445
538 -1.8041306913853996
539 -1.803817554458838
540 -1.8033078769105597
541 -1.802587564186197
542 -1.8016476234012764
543 -1.8004820772811754
544 -1.799087104631195
545 -1.7974602607124295
546 -1.7955993344275185
547 -1.7935024552182437
548 -1.7911681861209314
549 -1.7885957645634216
550 -1.7857850972380724
551 -1.7827365202468375
552 -1.7794506456321062
553 -1.7759281440154175
554 -1.7721698857850166
555 -1.7681770733307796
556 -1.763951433731297
557 -1.7594944941785822
558 -1.7548072322155372
559 -1.7498911849431145
560 -1.7447482942914168
561 -1.7393805340483806
562 -1.7337901506768825
563 -1.7279789789118232
564 -1.7219484988250344
565 -1.7157005846750073
566 -1.709237194617219
567 -1.702559903917999
568 -1.6956700103330455
569 -1.6885690986935982
570 -1.6812588718751431
571 -1.673740470905987
572 -1.6660159969761066
573 -1.658087370506835
574 -1.649956403425887
575 -1.6416249395054048
576 -1.6330948046903246
577 -1.624367725155254
578 -1.6154454094422823
579 -1.6063294929666543
580 -1.5970216152126018
581 -1.5875234831569174
582 -1.5778372518448263
583 -1.5679647188342918
584 -1.5579074375024917
585 -1.547667109449091
586 -1.5372454159371913
587 -1.5266442929334858
588 -1.5158653602273062
589 -1.5049097777894282
590 -1.4937794018391881
591 -1.4824760300915545
592 -1.4710010447275357
593 -1.4593559157139016
594 -1.4475421956867431
595 -1.4355612092248922
596 -1.4234141164117036
597 -1.4111025535422579
598 -1.398627725020078
599 -1.3859909035613633
600 -1.3731935389686467
601 -1.3602372707371118
602 -1.3471237059534396
603 -1.3338540586661367
604 -1.3204293426963714
605 -1.306850392686079
606 -1.293118234070922
607 -1.2792338280586737
608 -1.2651984396700082
609 -1.2510135352539111
610 -1.2366804047008966
611 -1.2222001774714888
612 -1.2075738025799765
613 -1.1928019603215485
614 -1.1778856973631133
615 -1.16282604826503
616 -1.1476239801803643
617 -1.1322804154934767
618 -1.1167962211303502
619 -1.1011722410654872
620 -1.0854093009306436
621 -1.069508209741698
622 -1.0534697624276015
623 -1.03729473737742
624 -1.0209839020562932
625 -1.0045378999012489
626 -0.9879574665790711
627 -0.9712433849743516
628 -0.9543964056976542
629 -0.9374171208306841
630 -0.9203063383000809
631 -0.9030647284291975
632 -0.8856929526084091
633 -0.8681915952830941
634 -0.8505612589319747
635 -0.8328028770365137
636 -0.814916757999291
637 -0.7969035659905135
638 -0.7787641931337941
639 -0.7604992116564885
640 -0.7421088674275458
641 -0.7235935830565607
642 -0.7049536576910733
643 -0.6861898121937623
644 -0.667302780025363
645 -0.648293048787387
646 -0.6291612929580384
647 -0.609907943904016
648 -0.5905331847526257
649 -0.5710374590006264
650 -0.5514211385419188
651 -0.5316848756179462
652 -0.5118293158121906
653 -0.49185495608191165
654 -0.47176222470399665
655 -0.45155146361385834
656 -0.4312232084362602
657 -0.41077788945137517
658 -0.39021605509994833
659 -0.369538128434845
660 -0.34874453720095705
661 -0.32783564418327155
662 -0.30681185035953557
663 -0.2856735790119849
664 -0.26442129121836094
665 -0.24305541878771292
666 -0.2215763944411442
667 -0.19998451726320152
668 -0.1782805431317636
669 -0.15646490976269256
670 -0.13453755416410743
671 -0.11249886593856909
672 -0.09034959665066107
673 -0.06809058955205345
674 -0.04572158606857958
675 -0.023243108114950593
676 -0.0006556870436712874
677 0.022040602238131896
678 0.04484531012017121
679 0.06775821558711131
680 0.09077904672031926
681 0.1139074177594532
682 0.13714284085339748
683 0.1604850254648545
684 0.18393321779496147
685 0.20748707097809557
686 0.23114632500097632
687 0.2549106684563318
688 0.27877996308276204
689 0.3027540407251872
690 0.32683253495265785
691 0.35101502320337735
692 0.37530099879427414
693 0.3996896571585942
694 0.4241810858549244
695 0.44877513115053635
696 0.4734714960897988
697 0.49826948160305345
698 0.5231687505032668
699 0.5481690010531766
700 0.573269993126489


==> plotdata/quadrotor/A3_x2_phase1.tex <==
0 0.0
1 0.0
2 0.0
3 0.0
4 0.00031215833459599787
5 0.0011425047536333022
6 0.0024636724970430526
7 0.004021835421128739
8 0.005383185525486052
9 0.006002799003069796
10 0.00527680221862359
11 0.0025835725717803307
12 -0.0027007337989380436
13 -0.011223499022283322
14 -0.024153568498900806
15 -0.04281384250903998
16 -0.06834907302852637
17 -0.10149138127723228
18 -0.142525138924764
19 -0.1912895205121432
20 -0.2472174283471275
21 -0.30933980886055545
22 -0.37633340774376445
23 -0.4465457201174257
24 -0.5181001461836561
25 -0.5889632528372052
26 -0.6570278987749872
27 -0.7201898468783051
28 -0.7764423485797702
29 -0.8239617918511315
30 -0.8611557885405685
31 -0.8866935444491647
32 -0.8995482820801488
33 -0.899028975542121
34 -0.8847895007367012
35 -0.8568264762528348
36 -0.8154910718966565
37 -0.7614580424097501
38 -0.6957015640259722
39 -0.6194735810351365
40 -0.5342642217678268
41 -0.44175659013657553
42 -0.34380896145893014
43 -0.24241198612460477
44 -0.13961185742897736
45 -0.037449322363439036
46 0.062087940386961984
47 0.15714307546703
48 0.24609340359643533
49 0.32764361855103147
50 0.4008685587142612
51 0.4652231507188441
52 0.5206106186728845
53 0.5674620545639171
54 0.6063929844829061
55 0.6376551486792138
56 0.6610305282549851
57 0.6759259537861835
58 0.6815010655599288
59 0.6769053883931943
60 0.6613414180882808
61 0.6340864965080907
62 0.5945174093177359
63 0.5421236544347441
64 0.4760194943754628
65 0.39551294443951984
66 0.3007238573505657
67 0.1928283863049896
68 0.07374990660929565
69 -0.054199066829668296
70 -0.18850048675546563
71 -0.3264720383834987
72 -0.46530278810476133
73 -0.602113218402676
74 -0.734020495492964
75 -0.8581736202560412
76 -0.9718375531846672
77 -1.0724702830994128
78 -1.15781454175974
79 -1.2259643859089169
80 -1.2753932279260516
81 -1.3049748743053688
82 -1.3140224205700755
83 -1.302312573055503
84 -1.270070295947473
85 -1.217939917844808
86 -1.1469742857249083
87 -1.0585808686014575
88 -0.9544745984515762
89 -0.836654123270731
90 -0.7073846464649778
91 -0.5691781843208836
92 -0.4247784300642832
93 -0.2770636598106716
94 -0.12890037035094015
95 0.0169127993417435
96 0.1576692138694067
97 0.29086375061623804
98 0.41436419397503244
99 0.5265402544123419
100 0.626346140582558
101 0.7133856145624119
102 0.7880202325960206
103 0.8514013211504722
104 0.9048787715899375
105 0.9489534528852406
106 0.9829729637836103
107 1.0053100807385444
108 1.0139508437593385
109 1.0069639053972912
110 0.9826157850223974
111 0.9393903037161266
112 0.8760715889752881
113 0.7920109277881195
114 0.6871002175256055
115 0.5619034893696704
116 0.41808532226988915
117 0.2586805423063283
118 0.08757397199891062
119 -0.09120734591307023
120 -0.27382807751899435
121 -0.45667662348501104
122 -0.6361857701930878
123 -0.8087344333068294
124 -0.9710231148289605
125 -1.1201550737389485
126 -1.2536219205928503
127 -1.3692615461890485
128 -1.4652122113532724
129 -1.53987095491637
130 -1.591857565468069
131 -1.6199858051264244
132 -1.6232421893207256
133 -1.6012751512286656
134 -1.5544107939514
135 -1.4835113617416167
136 -1.3899109813377624
137 -1.2753607301437335
138 -1.1419621505740563
139 -0.9921339183618241
140 -0.8285892063704523
141 -0.654330640470951
142 -0.4726406536049613
143 -0.28697249158777266
144 -0.10079588910815929
145 0.08246702516461452
146 0.2594729497873337
147 0.42707087564262425
148 0.5824956477232398
149 0.7235308093551118
150 0.8486348867947051
151 0.9571026409085647
152 1.0492791636841865
153 1.1265643496709765
154 1.1907379621274592
155 1.242575093825147
156 1.2805736505704386
157 1.3026651656610915
158 1.3067878613531985
159 1.2910690483147187
160 1.2538705368573881
161 1.1937871646396516
162 1.1096275173119452
163 1.000389661564
164 0.8656597426288174
165 0.7075831966342117
166 0.5314571202831909
167 0.34366883058749065
168 0.15025415876901993
169 -0.043752319421512476
170 -0.23800049890898708
171 -0.4319197470897922
172 -0.6224473052565448
173 -0.8060592450823508
174 -0.9794243529135122
175 -1.1395869460600259
176 -1.2839922215992061
177 -1.4104549346162085
178 -1.5171124077354325
179 -1.6023761824628517
180 -1.6649009356248472
181 -1.7035461495301443
182 -1.7173440455393838
183 -1.7054804857320274
184 -1.6672818787451353
185 -1.6021869895398715
186 -1.5097222964688017
187 -1.3894892436869632
188 -1.2438853944024908
189 -1.0773188039471513
190 -0.8952384196163756
191 -0.7035508203760915
192 -0.5079254431450483
193 -0.31231007424666457
194 -0.11709469723461949
195 0.07854038585121212
196 0.27395566935134236
197 0.4662297004936534
198 0.6519626481185116
199 0.8279337139111165
200 0.991277690853102
201 1.139507333992817
202 1.2704779188142339
203 1.382305068857947
204 1.4733329853491604
205 1.5421186800418332
206 1.5874120529520375
207 1.6081320076653824
208 1.6033484138720808
209 1.5722708300222363
210 1.5142354838148495
211 1.4286932341048895
212 1.3151832280620188
213 1.1733209873993011
214 1.008251281468984
215 0.8269221198708767
216 0.636023048328569
217 0.4414736001350859
218 0.24686604531393183
219 0.052504094069229734
220 -0.1421446778616626
221 -0.33682155585785
222 -0.5287465021194465
223 -0.7144019941280193
224 -0.8903821810519524
225 -1.0536406113732044
226 -1.2015324128875844
227 -1.3317918660198036
228 -1.4424884096261361
229 -1.531971475726587
230 -1.5988132877033405
231 -1.6417736895296562
232 -1.6597792672063303
233 -1.6519167724828392
234 -1.6174197600416937
235 -1.5556534485864144
236 -1.466109521555043
237 -1.348400148012603
238 -1.2024799614860302
239 -1.0344232776040616
240 -0.8513188413948005
241 -0.6597606369614868
242 -0.4655148033657708
243 -0.27114843325326143
244 -0.07679579661517152
245 0.11776603261988944
246 0.3112570026460042
247 0.5004053988206408
248 0.681636289673486
249 0.8516244921722904
250 1.0074450543039843
251 1.1465854683734247
252 1.266910540527702
253 1.3666174498260912
254 1.444189950467319
255 1.4983534897241262
256 1.5280368344410677
257 1.5323380731557652
258 1.5104962762722498
259 1.4618685893023449
260 1.3859115146382004
261 1.282165225799123
262 1.15024177977306
263 0.9927732437374377
264 0.8162594747659045
265 0.6275497275143664
266 0.4328563974792206
267 0.23757103757361805
268 0.04229557512372481
269 -0.15275067806932466
270 -0.3480301867826928
271 -0.5418668281870902
272 -0.7309602159103588
273 -0.9118397068679444
274 -1.0813139623791677
275 -1.2365784571425298
276 -1.3752115329561103
277 -1.4951370601433136
278 -1.5945813368176804
279 -1.6720319780920683
280 -1.7262016474753197
281 -1.755995345749956
282 -1.7604822828638567
283 -1.7388720435337082
284 -1.6904938781842016
285 -1.6147787683234003
286 -1.5112439811734948
287 -1.3794796931869753
288 -1.2222388061684515
289 -1.0460466642824393
290 -0.857758131620215
291 -0.6635912865113875
292 -0.4689455612751958
293 -0.27422987904594653
294 -0.08027274071887497
295 0.11453430396950506
296 0.3078314763353486
297 0.49610080994708294
298 0.6758096593861705
299 0.8437582995590654
300 0.997154989346732
301 1.1336017814764434
302 1.251054587460204
303 1.3477768494226845
304 1.4222963972059888
305 1.47336602526067
306 1.4999290925066424
307 1.501090387887709
308 1.476091525650351
309 1.424290088868866
310 1.345141913271709
311 1.2381863301869345
312 1.103033836590958
313 0.9430148072419924
314 0.764745893658339
315 0.5750219544953068
316 0.37996419432231643
317 0.1848747356545679
318 -0.010212105045249498
319 -0.20445644689869566
320 -0.3995496303323187
321 -0.5930106863507932
322 -0.7813138398029436
323 -0.9609588958876504
324 -1.1287880747636365
325 -1.2820483616063665
326 -1.4183718161166854
327 -1.535733305785868
328 -1.6324056775936562
329 -1.7069182497558069
330 -1.758020139471815
331 -1.784648284768419
332 -1.7858999584735384
333 -1.7610090743164317
334 -1.7093258213110694
335 -1.6302992741977573
336 -1.52346245233679
337 -1.388419707664807
338 -1.2285208458293542
339 -1.0503862696026431
340 -0.8608124570472279
341 -0.6659222955248691
342 -0.47101817007871216
343 -0.2761040149670211
344 -0.08203890815051587
345 0.1128873463450509
346 0.30615837830504306
347 0.49423595451828845
348 0.6736166624165274
349 0.8411433315701329
350 0.9940654708581259


==> plotdata/quadrotor/A3_x2_phase2.tex <==
350 0.9940654708581259
351 1.1300189638631821
352 1.2469840698010817
353 1.34323996352017
354 1.4189046758630888
355 1.4736661879088315
356 1.5093423618963373
357 1.5289915714292845
358 1.535887076140809
359 1.5329699911058632
360 1.5226715702453046
361 1.5069136970977173
362 1.4871745468307835
363 1.464567989231262
364 1.4399178628166818
365 1.413822186745095
366 1.3867066098778873
367 1.3588679987389811
368 1.330509199280425
369 1.3017663212353354
370 1.2727296123192962
371 1.243458717391502
372 1.2139937495221227
373 1.1843630337615012
374 1.1545884502017538
375 1.1246889237977165
376 1.0946828482262285
377 1.0645887930115419
378 1.0344264416786675
379 1.0042167674738376
380 0.9739820201684211
381 0.9437453685145923
382 0.9135306179692868
383 0.8833618850740917
384 0.8532632404558051
385 0.8232583714633543
386 0.7933703105163785
387 0.7636211990983786
388 0.7340320952837263
389 0.704622801269103
390 0.6754117870607883
391 0.6464161529932032
392 0.6176515542138863
393 0.5891332835995501
394 0.560883568001833
395 0.532934093503011
396 0.5053240156138975
397 0.4780913700135621
398 0.45126898984022296
399 0.42488124021510015
400 0.3989680762470687
401 0.3735950793091561
402 0.3488332445978145
403 0.3247374766577523
404 0.30133439990721494
405 0.27861849442133413
406 0.25655349402620775
407 0.23507838175067358
408 0.21411503371204268
409 0.19357740365603263
410 0.1733807537281814
411 0.15344826930667196
412 0.13371494170740025
413 0.11413028804609064
414 0.09465818456474834
415 0.07527424803430122
416 0.055964750567446736
417 0.03672412174088971
418 0.017552025932136374
419 -0.001545448883572248
420 -0.020557383741330346
421 -0.03947120417949844
422 -0.05827425701382815
423 -0.07695432813045969
424 -0.09549931710663422
425 -0.11389524460577641
426 -0.13212477216811955
427 -0.1501678779736717
428 -0.16800442283196892
429 -0.1856157234287459
430 -0.20298578773755713
431 -0.2201020882212761
432 -0.23695547657483654
433 -0.2535399308533285
434 -0.2698518979835311
435 -0.2858901875312093
436 -0.30165645119734624
437 -0.31715364614960223
438 -0.3323855927999884
439 -0.3473565346470426
440 -0.3620703194531382
441 -0.3765312251099685
442 -0.3907442216506715
443 -0.40471392502980813
444 -0.4184448941051381
445 -0.43194157721313714
446 -0.44520777078509444
447 -0.45824756533900846
448 -0.4710645920779172
449 -0.4836623034271155
450 -0.49604399575503055
451 -0.508212462653767
452 -0.5201702442512124
453 -0.5319195665039382
454 -0.5434629244258009
455 -0.554802832237689
456 -0.5659413685012948
457 -0.5768806217366543
458 -0.5876223916916534
459 -0.5981684281885027
460 -0.6085198089485446
461 -0.6186776624309681
462 -0.6286428538271408
463 -0.6384168267439456
464 -0.6480007374677769
465 -0.657395730674609
466 -0.6666029310937468
467 -0.675623665114922
468 -0.6844590898556586
469 -0.6931104146822167
470 -0.7015787137297802
471 -0.7098649903742457
472 -0.7179700993554573
473 -0.7258949130129294
474 -0.7336404160726575
475 -0.7412076762953779
476 -0.7485974982945953
477 -0.7558108020806077
478 -0.7628487364651554
479 -0.7697124444252084
480 -0.7764029269693736
481 -0.7829211748092197
482 -0.7892681131536584
483 -0.7954446855662963
484 -0.8014518509604902
485 -0.8072905794068478
486 -0.8129618380874168
487 -0.8184666913629296
488 -0.8238062381157065
489 -0.8289816802375423
490 -0.8339942546789357
491 -0.8388451629792162
492 -0.8435355990153468
493 -0.8480667728886492
494 -0.8524399776262732
495 -0.8566566131669296
496 -0.860718133770961
497 -0.8646260297542473
498 -0.8683818419364145
499 -0.8719871658519268
500 -0.8754436549946392
501 -0.8787530312978201
502 -0.8819170901698056
503 -0.8849377044567229
504 -0.8878168381456395
505 -0.8905595015015065
506 -0.8931732987026342
507 -0.8956662211829834
508 -0.8980452410841065
509 -0.9003156379082197
510 -0.9024810964533339
511 -0.9045439251411604
512 -0.9065053107734884
513 -0.9083656055604411
514 -0.9101245352065104
515 -0.9117814403391286
516 -0.9133354647163332
517 -0.914785804258483
518 -0.9161319323715835
519 -0.9173738281486497
520 -0.9184950065337845
521 -0.9194596481107992
522 -0.9202292947193479
523 -0.9207778699433536
524 -0.9210969594998479
525 -0.9211939887078527
526 -0.9210890189740432
527 -0.920811892195012
528 -0.9203992670200453
529 -0.9198920156926029
530 -0.9193273109621554
531 -0.9187284207963726
532 -0.9181070937742029
533 -0.9174682332686149
534 -0.9168218570621113
535 -0.9161806714479015
536 -0.9155603331236434
537 -0.9149774841558426
538 -0.9144484066876967
539 -0.9139865061711715
540 -0.913598287588589
541 -0.9132809263737846
542 -0.9130251370985825
543 -0.9128189026498909
544 -0.9126496971665767
545 -0.9125052811200265
546 -0.9123736469430188
547 -0.9122428090635487
548 -0.9121005491268991
549 -0.9119342810600531
550 -0.9117309494302386
551 -0.9114769495762953
552 -0.9111581554345194
553 -0.9107598884088246
554 -0.9102671532566693
555 -0.9096648627689866
556 -0.9089382277052378
557 -0.9080725175102872
558 -0.9070529690138129
559 -0.9058657372759055
560 -0.9044979774674828
561 -0.9029376749298134
562 -0.9011737752626596
563 -0.8991959872459049
564 -0.89699479502855
565 -0.8945620344788595
566 -0.8918906378986949
567 -0.8889743443125885
568 -0.8858076029288967
569 -0.8823861136312905
570 -0.8787066263353855
571 -0.8747664047831814
572 -0.8705640891566606
573 -0.8660989903726226
574 -0.8613711076019794
575 -0.8563810819977449
576 -0.851130077922116
577 -0.8456197818920133
578 -0.83985237326367
579 -0.8338302520804501
580 -0.8275563225845773
581 -0.8210337872221032
582 -0.8142660985034638
583 -0.8072567942186426
584 -0.8000093946761712
585 -0.7925275878220921
586 -0.7848151357642942
587 -0.7768760271605981
588 -0.7687141109794668
589 -0.7603330411633453
590 -0.7517367869402809
591 -0.742929117596619
592 -0.7339136739939592
593 -0.7246939521568521
594 -0.7152735643439605
595 -0.7056557442372816
596 -0.6958437529975908
597 -0.6858410418387283
598 -0.6756505947044307
599 -0.6652752712542421
600 -0.6547180872715727
601 -0.6439819335766522
602 -0.6330696438159618
603 -0.6219836492379088
604 -0.6107262829824546
605 -0.5992997773209167
606 -0.5877062071284407
607 -0.5759476501055949
608 -0.5640262922827165
609 -0.5519441041638915
610 -0.5397029638348629
611 -0.527304672368236
612 -0.5147509941539659
613 -0.5020434171429776
614 -0.4891834122723826
615 -0.47617242512210195
616 -0.4630118531965984
617 -0.4497030404885634
618 -0.43624725310265394
619 -0.4226456949165586
620 -0.40889951147698206
621 -0.39500979444143347
622 -0.3809775867707601
623 -0.36680388302871836
624 -0.35248963742876405
625 -0.33803578700550296
626 -0.3234431330864875
627 -0.30871250823800117
628 -0.2938447293217175
629 -0.2788406153121281
630 -0.2637009514050532
631 -0.24842640659666249
632 -0.23301766462996654
633 -0.2174754620104342
634 -0.20180041062587836
635 -0.18599338638301693
636 -0.17005476228463143
637 -0.15398518488841068
638 -0.1377854760544428
639 -0.12145624484539089
640 -0.10499770383012362
641 -0.08841023908976799
642 -0.07169414254153209
643 -0.054850110625959875
644 -0.037878867684344536
645 -0.020780901608546423
646 -0.003556823426953265
647 0.013792939679101363
648 0.03126822263380585
649 0.04886858970187863
650 0.06659369811169849
651 0.08444294348988626
652 0.10241574074049699
653 0.12051162176515598
654 0.13873018352765187
655 0.15707108257485763
656 0.17553384496059551
657 0.1941180836422515
658 0.21282326622645864
659 0.2316490191147404
660 0.2505949607617798
661 0.2696607552870105
662 0.28884602936742954
663 0.30815038230556385
664 0.32757337687975213
665 0.3471146040509622
666 0.36677365617498514
667 0.38655024486866185
668 0.40644365844097824
669 0.4264534830850921
670 0.44657976609674704
671 0.46682213452443805
672 0.48717988000456713
673 0.5076522081845234
674 0.5282393459376185
675 0.5489407968440451
676 0.5697560540108635
677 0.5906850356287847
678 0.611727301277698
679 0.6328826319984303
680 0.6541507533511082
681 0.6755312967258585
682 0.6970237958323889
683 0.7186279652027387
684 0.7403430839073877
685 0.7621688098959584
686 0.7841048812013988
687 0.8061509873008076
688 0.8283069767588507
689 0.8505726715385075
690 0.8729477071895616
691 0.8954316660230703
692 0.9180240518067417
693 0.9407240902534546
694 0.9635318392172957
695 0.986447130106874
696 1.0094696650228943
697 1.0325987678446735
698 1.0558341004122693
699 1.079175352844907
700 1.1026222757680875


==> plotdata/quadrotor/A3_x3_phase1.tex <==
0 0.0
1 0.0
2 1.8118839761882557e-14
3 1.0853540288735531e-14
4 -4.709121981250065e-14
5 -1.8232526599604173e-13
6 -4.3325343312972115e-13
7 -8.666489748065943e-13
8 -1.5558576649254976e-12
9 -2.5780622081583718e-12
10 -4.037019607494586e-12
11 -6.030020927028091e-12
12 -8.022933428719626e-12
13 -1.0157439334079754e-11
14 -1.2498162504925858e-11
15 -1.5045849011130488e-11
16 -1.7697701082397547e-11
17 -2.040842161932233e-11
18 -2.3148452044097215e-11
19 -2.567242418649585e-11
20 -2.8135360707892692e-11
21 -3.062956110966298e-11
22 -3.299447826066172e-11
23 -3.5060008229947936e-11
24 -3.678620075220353e-11
25 -3.828358074997597e-11
26 -3.934312431397304e-11
27 -4.010454190961356e-11
28 -4.048803958767168e-11
29 -4.059119262933565e-11
30 -4.032859379776712e-11
31 -3.976683871087518e-11
32 -3.885702426487116e-11
33 -3.7539713559908724e-11
34 -3.583449981192645e-11
35 -3.368590739682988e-11
36 -3.1067752814806246e-11
37 -2.7788082945789956e-11
38 -2.349089811559681e-11
39 -1.7618280168107976e-11
40 -9.44689659831967e-12
41 2.0417445512066327e-12
42 1.8501058463016297e-11
43 4.24222790229578e-11
44 7.46123340888971e-11
45 1.1569751379170156e-10
46 1.673176797112319e-10
47 2.319906933223592e-10
48 3.1259089539048545e-10
49 4.1316440047012294e-10
50 5.386517543115587e-10
51 6.948129893658006e-10
52 8.885636049171808e-10
53 1.1290663159968518e-09
54 1.4279350502022227e-09
55 1.7967721710476782e-09
56 2.24710740681644e-09
57 2.790843858235803e-09
58 3.437866133992884e-09
59 4.194224292319859e-09
60 5.059746772673179e-09
61 6.0264064671855526e-09
62 7.071178735884587e-09
63 8.149759551656645e-09
64 9.189932796971336e-09
65 1.0083621067025209e-08
66 1.0690311000871592e-08
67 1.0983944811471251e-08
68 1.1005238746975015e-08
69 1.0797329998979426e-08
70 1.0398450100979067e-08
71 9.842427921569201e-09
72 9.160480232139894e-09
73 8.381864162743118e-09
74 7.529540528850026e-09
75 6.619583992062422e-09
76 5.660864115242253e-09
77 4.654602374642996e-09
78 3.5893636862738324e-09
79 2.4424411293466667e-09
80 1.2269027394040724e-09
81 -3.8616825293042834e-11
82 -1.3919058794442617e-09
83 -2.9688449565412568e-09
84 -5.051613563011865e-09
85 -8.282078489685314e-09
86 -1.4229916942554152e-08
87 -2.5396153038315102e-08
88 -4.5693078032371656e-08
89 -8.11544121503971e-08
90 -1.4066631624842786e-07
91 -2.371508549181556e-07
92 -3.8911657959772586e-07
93 -6.223292991691665e-07
94 -9.723283364770907e-07
95 -1.4869087297242347e-06
96 -2.2276088529338267e-06
97 -3.2719558682892115e-06
98 -4.712565180007289e-06
99 -6.654181642282708e-06
100 -9.207395582411237e-06
101 -1.2477144091267434e-05
102 -1.65477993835772e-05
103 -2.1472756647611395e-05
104 -2.7264108339650766e-05
105 -3.3883124178490936e-05
106 -4.121220119211345e-05
107 -4.921808463818068e-05
108 -5.77856389928222e-05
109 -6.668651834383256e-05
110 -7.555696538112501e-05
111 -8.386850115842394e-05
112 -9.089155812448625e-05
113 -9.566087809535163e-05
114 -9.828793001990022e-05
115 -9.897311558004773e-05
116 -9.789928719083462e-05
117 -9.522021985688411e-05
118 -9.10810554456276e-05
119 -8.561351606010346e-05
120 -7.893108688826088e-05
121 -7.112667931647107e-05
122 -6.226220039653893e-05
123 -5.23631114109335e-05
124 -4.14138434727462e-05
125 -2.944802642737439e-05
126 -1.661906033019629e-05
127 -3.3190990459352564e-06
128 9.509441096398116e-06
129 1.963935655892263e-05
130 2.2961577313918075e-05
131 1.1952304427573844e-05
132 -2.6678073952606176e-05
133 -0.00011548705191589899
134 -0.00029192615887028593
135 -0.0006138396729481777
136 -0.0011667587958221937
137 -0.002066007648811503
138 -0.003443312081095318
139 -0.005392070550474682
140 -0.007946772096329033
141 -0.011151188137175298
142 -0.015054728831614617
143 -0.019713827536720623
144 -0.025192256836527194
145 -0.03155647321121328
146 -0.0388759334355126
147 -0.04721996648752795
148 -0.056639808334336225
149 -0.0670850356275902
150 -0.07843572942831546
151 -0.09052648540030533
152 -0.10313963870811835
153 -0.11599706661158801
154 -0.12873826671129168
155 -0.14089667183388618
156 -0.15188386512755148
157 -0.16147899010739974
158 -0.16966947813562913
159 -0.17634185389325543
160 -0.1812707377660191
161 -0.18408268897270247
162 -0.18424613610906818
163 -0.1810608086240949
164 -0.17435979153269707
165 -0.16489788863353033
166 -0.1534322305563886
167 -0.14062095317913964
168 -0.12702673468984044
169 -0.11311760777149125
170 -0.09927343569981233
171 -0.08579386255441725
172 -0.07291143251165867
173 -0.060800038457006225
174 -0.04958220429296857
175 -0.03933804803584599
176 -0.03011305848715732
177 -0.021927582349158085
178 -0.01478203524091853
179 -0.008665468871325058
180 -0.0035550856184267624
181 0.0005729056557492495
182 0.0037242752913310795
183 0.005907959748832732
184 0.007143628877341969
185 0.007454233886871877
186 0.0068625761046869314
187 0.00539116021215558
188 0.0030550604123604015
189 -0.00014709158499922378
190 -0.0042256541580398595
191 -0.009181231138146239
192 -0.015038412022418242
193 -0.021846926426963193
194 -0.029678343890316927
195 -0.03861942054255942
196 -0.04876974379492939
197 -0.06022944623940264
198 -0.07307848658382686
199 -0.08727961641315461
200 -0.10269146668487256
201 -0.11911161183090502
202 -0.136256527152272
203 -0.15373982912525141
204 -0.17104619529849216
205 -0.1874992905865473
206 -0.20225894554914783
207 -0.21557535459825208
208 -0.2277018308650233
209 -0.23855614008486775
210 -0.2477122282296067
211 -0.2543709740921991
212 -0.2573463629141595
213 -0.25504072935948924
214 -0.2461423560914887
215 -0.23211154276914633
216 -0.21449207441747734
217 -0.1945722288083454
218 -0.17342205979115566
219 -0.15191632081065745
220 -0.1307456970601136
221 -0.11043597553697929
222 -0.09137508184562115
223 -0.07383431274471487
224 -0.057985649759397295
225 -0.043912164002381966
226 -0.03161861767816536
227 -0.02105179780353247
228 -0.012134705795718003
229 -0.004775427075333483
230 0.0011423743319338119
231 0.005758096777286408
232 0.009217830688543349
233 0.011648354117417034
234 0.013142465137972322
235 0.013754491017577456
236 0.013507496200166075
237 0.012408072002298683
238 0.01045471760934642
239 0.007638210774375881
240 0.003952096872632864
241 -0.0006082461540451124
242 -0.006077040013408937
243 -0.012520611368680936
244 -0.020033193507239942
245 -0.02872936584270963
246 -0.038740617347773156
247 -0.050202213104116905
248 -0.06323077938027834
249 -0.07782499709016921
250 -0.09387567370366943
251 -0.11120565082038703
252 -0.1295471446649024
253 -0.14851452920949013
254 -0.1675741841232469
255 -0.186006099814697
256 -0.2028939292941037
257 -0.21837783098907518
258 -0.2325618869182187
259 -0.24516075729460995
260 -0.25546336162566846
261 -0.2622873057866314
262 -0.26394582407979544
263 -0.2582071304717927
264 -0.2429674056967803
265 -0.2206147789258657
266 -0.19387705413761816
267 -0.16496600805249195
268 -0.1356492482631554
269 -0.10730374605764646
270 -0.08095427624174777
271 -0.05731643628900879
272 -0.03684463846837609
273 -0.01977163727931009
274 -0.006140368754100657
275 0.004179602566634171
276 0.011486644687959497
277 0.016244307990075993
278 0.019022529445230016
279 0.020410607856768303
280 0.02094377718581407
281 0.0210191321975923
282 0.02088229410342688
283 0.020665182996763315
284 0.020423156153459902
285 0.02015802824331127
286 0.019837019505243362
287 0.01941195810383481
288 0.018829262655518045
289 0.0180308099050165
290 0.01696413386262479
291 0.015581071915147654
292 0.01380539108793377
293 0.011529296757726628
294 0.00861561634894323
295 0.004903727338384506
296 0.0002110093167609836
297 -0.005655549693598685
298 -0.01287874943133113
299 -0.021532985297943487
300 -0.03159533697757753
301 -0.042985257420163965
302 -0.05554167644013139
303 -0.06899413092653679
304 -0.08293061685750351
305 -0.09675586294859621
306 -0.10967897073951428
307 -0.12196161522406054
308 -0.13382162501818864
309 -0.1450750184821424
310 -0.15509376264447458
311 -0.16275389199705967
312 -0.16639509853164672
313 -0.1637729947180296
314 -0.15272584183849636
315 -0.13553941154909788
316 -0.11479989124226755
317 -0.09254726694417197
318 -0.07035922077443205
319 -0.049416014750103696
320 -0.030549719550321697
321 -0.014296349528800482
322 -0.0009513089133873203
323 0.009386449132511273
324 0.016779655270771986
325 0.02143551860046374
326 0.023701190390106736
327 0.024063433382218752
328 0.023093415878685672
329 0.02136390022189318
330 0.019380455772185383
331 0.017501811322178974
332 0.01593065606420165
333 0.014754833965642106
334 0.013987137382063771
335 0.013590279165895447
336 0.01349711384952431
337 0.01363044080147459
338 0.013913282298330176
339 0.014269302403697713
340 0.014632376203082805
341 0.014944491706885376
342 0.015122129340348142
343 0.015051216045670014
344 0.014587967650904464
345 0.013562930527981118
346 0.011781287111094243
347 0.009032549986584565
348 0.005107926950028892
349 -9.979226412297395e-05
350 -0.006611008721036242


==> plotdata/quadrotor/A3_x3_phase2.tex <==
350 -0.006611008721036242
351 -0.014398297417084906
352 -0.02412090614679023
353 -0.03268481089841233
354 -0.03823024832913864
355 -0.041318045614749374
356 -0.04285291363360228
357 -0.04359535709252967
358 -0.04395639760109597
359 -0.044133131764621775
360 -0.04421997702713554
361 -0.044263109963066954
362 -0.04428517059651632
363 -0.044296613856797035
364 -0.04430183239505846
365 -0.04430438360026387
366 -0.044305633060986976
367 -0.04430620926695176
368 -0.04430644333686695
369 -0.04430650476215153
370 -0.04430647802691098
371 -0.04430640535675542
372 -0.04430630791933983
373 -0.04430619627431461
374 -0.04430607553322572
375 -0.044305948203816226
376 -0.04430581531336399
377 -0.044305677633747424
378 -0.044305535479489996
379 -0.04430538908056229
380 -0.04430523845932356
381 -0.044305083622080486
382 -0.044304924736241216
383 -0.04430476181842634
384 -0.04430459488471501
385 -0.0443044239240473
386 -0.044304248963960784
387 -0.044304070067047154
388 -0.0443038872517521
389 -0.044303700527046595
390 -0.044303510391839364
391 -0.0443338972162372
392 -0.0444276890428147
393 -0.04460890180098336
394 -0.04489272348025869
395 -0.04529395740978217
396 -0.04582708686687902
397 -0.04650767507361042
398 -0.047371418709799586
399 -0.048486170493273854
400 -0.049942231697956745
401 -0.05184042391088067
402 -0.054284145913528065
403 -0.0573727403472936
404 -0.06119366593159069
405 -0.0658109022279332
406 -0.07125824516933939
407 -0.07752991661038985
408 -0.08457443857323457
409 -0.09230032693819949
410 -0.10058734282243872
411 -0.10929231686596821
412 -0.11826538073117697
413 -0.12735986137357
414 -0.13643773865392894
415 -0.1453817130319614
416 -0.15409087597144716
417 -0.1624897047285017
418 -0.17052698263014424
419 -0.17817127421039058
420 -0.18540191027001424
421 -0.19220788235170738
422 -0.19855076389377146
423 -0.20437464734498234
424 -0.20964272884848054
425 -0.21434816627318476
426 -0.21850985901913011
427 -0.2221657175530978
428 -0.22536220803537638
429 -0.22815374851835754
430 -0.23058749109036353
431 -0.23270661315042374
432 -0.23455191998948802
433 -0.2361735068684252
434 -0.23761070522867192
435 -0.23889684891513266
436 -0.24006220694640834
437 -0.24113461027791455
438 -0.2421318852385326
439 -0.2430758605942681
440 -0.24398239453933301
441 -0.24486355522478748
442 -0.2457289480432476
443 -0.24658338782995992
444 -0.24743441322387982
445 -0.2482844121444959
446 -0.2491396375210667
447 -0.24999952768079434
448 -0.25086806575325216
449 -0.2517485046051695
450 -0.25263874772040024
451 -0.2535374726903765
452 -0.2544499851229199
453 -0.2553756533095079
454 -0.25631381136038434
455 -0.2572650723979432
456 -0.25822957256735124
457 -0.25920646325143
458 -0.2601886459072892
459 -0.2611726135293997
460 -0.26216097454411963
461 -0.2631558041331908
462 -0.2641562561939743
463 -0.26516148698447584
464 -0.2661697284842126
465 -0.267181438570313
466 -0.26819192940047987
467 -0.2692028361282276
468 -0.27021109083558
469 -0.27121587704842387
470 -0.27221433935977135
471 -0.27320433119833437
472 -0.274185040777333
473 -0.27515499150709605
474 -0.2761099693353233
475 -0.2770493775715874
476 -0.27797415354838806
477 -0.2788835880859053
478 -0.27977523248265396
479 -0.280648114606426
480 -0.2815000643389489
481 -0.2823283972792936
482 -0.2831327190682875
483 -0.2839118119306063
484 -0.28466423969345933
485 -0.2853889162889107
486 -0.28608481224005533
487 -0.2867505891983296
488 -0.2873861426929394
489 -0.28799067398226336
490 -0.2885637655982537
491 -0.2891051691740161
492 -0.28961453454966685
493 -0.29009150991414423
494 -0.2905358126653345
495 -0.29094728146780685
496 -0.29132595976629644
497 -0.2916720849942447
498 -0.2919859597666263
499 -0.29226809382783037
500 -0.29251868695508354
501 -0.2927380407175075
502 -0.2929267840652145
503 -0.29308606266948245
504 -0.29321068064495753
505 -0.2932911494024375
506 -0.2933187347301299
507 -0.2932922781664617
508 -0.2932267362444086
509 -0.2931382574983856
510 -0.2930379353878865
511 -0.29293209536198533
512 -0.2928239796462553
513 -0.2927150807073893
514 -0.29260603310729705
515 -0.2924970315155379
516 -0.29238805714078864
517 -0.2922790487801523
518 -0.29229799901536585
519 -0.29263132676303755
520 -0.29337329647681115
521 -0.29454873002529663
522 -0.29613749543422824
523 -0.29809235295518444
524 -0.3003364634825634
525 -0.3027783627741038
526 -0.3053204404782825
527 -0.3078581741142084
528 -0.31030468371458914
529 -0.3126409060714303
530 -0.31485196044673375
531 -0.316937804068922
532 -0.3189246747343604
533 -0.3208583148468444
534 -0.3227607191720065
535 -0.3246361274185193
536 -0.32644239694319677
537 -0.32808303350796547
538 -0.329475424818806
539 -0.3305631922092008
540 -0.33136948742931127
541 -0.33204103046874056
542 -0.3327181289349379
543 -0.3334732862983754
544 -0.3343403489601839
545 -0.33533066252175203
546 -0.3364435327753478
547 -0.33766833191131
548 -0.3389956933679084
549 -0.3404167726343218
550 -0.3419208425312714
551 -0.34350427657000676
552 -0.3451585667349312
553 -0.3468754191290177
554 -0.34863254875847033
555 -0.3504237483421145
556 -0.35224566672601854
557 -0.3540886986251282
558 -0.35594076791146995
559 -0.3577937577934911
560 -0.3596391056160507
561 -0.361472972212959
562 -0.36329802181573095
563 -0.3651037303270517
564 -0.36688362950737935
565 -0.3686379177595021
566 -0.3703686542457849
567 -0.372068936353238
568 -0.37373195337791343
569 -0.37536290720685167
570 -0.37694869225094724
571 -0.3784861371469322
572 -0.3799774121920173
573 -0.3814190642854384
574 -0.38281097629116995
575 -0.38415697714410096
576 -0.38545376426261185
577 -0.3867004100592234
578 -0.38790052197754293
579 -0.3890527458875778
580 -0.3901519310750302
581 -0.3912015463346651
582 -0.39220475067844723
583 -0.3931616874908762
584 -0.39407258073061296
585 -0.3949402351550113
586 -0.3957637429461431
587 -0.39654468554918765
588 -0.39728327363427834
589 -0.3979810328399517
590 -0.3986494498386993
591 -0.3992815521065465
592 -0.39987427811588894
593 -0.4004284026515317
594 -0.40095807361117647
595 -0.40146366110825515
596 -0.4019379659756887
597 -0.402389324719719
598 -0.4028261089002623
599 -0.4032291339763597
600 -0.40360410072442027
601 -0.4039503288897181
602 -0.4042833628656446
603 -0.40460386803328946
604 -0.4049018634081052
605 -0.4051944051543174
606 -0.4054760275339504
607 -0.40571959891242937
608 -0.405923163415615
609 -0.40609551085549955
610 -0.40627462927389857
611 -0.40646331315186146
612 -0.4066188220361553
613 -0.4067441791175574
614 -0.4068493070791867
615 -0.40694153289061286
616 -0.40702618716794475
617 -0.40710539908567467
618 -0.4071803860745564
619 -0.4072520253115984
620 -0.4073210012571477
621 -0.4073875383764558
622 -0.4074516989973081
623 -0.40754980801805013
624 -0.40763442389122767
625 -0.40770041172710486
626 -0.40775246883984584
627 -0.40784640761464874
628 -0.4079329657281593
629 -0.40799426456271054
630 -0.4080365678362981
631 -0.4081150378992205
632 -0.4081970314600761
633 -0.4082905420935373
634 -0.40839512384254556
635 -0.40849198849307955
636 -0.40857350941622705
637 -0.40865998064149894
638 -0.4087162551912746
639 -0.40876022159907344
640 -0.4087952282547809
641 -0.40883094850175666
642 -0.40888013299911086
643 -0.40893803169171516
644 -0.40898547486820774
645 -0.40902910201045656
646 -0.4090553908773812
647 -0.4090861552262693
648 -0.40912466355033106
649 -0.40917553923521194
650 -0.40922421210553434
651 -0.4092709333838912
652 -0.40930605532294073
653 -0.4093468148391047
654 -0.4093702131355882
655 -0.4093999901754658
656 -0.4094434764270257
657 -0.4094723341969678
658 -0.40948278099813595
659 -0.40948241598940155
660 -0.4094761245715804
661 -0.4094694966757425
662 -0.40946375062669116
663 -0.40945727781216096
664 -0.4094496950058302
665 -0.4094409613118746
666 -0.40943229962032135
667 -0.4094220605643942
668 -0.4094133901099038
669 -0.4094031943937915
670 -0.4093927843155403
671 -0.40938388636411227
672 -0.40937672547261544
673 -0.40936884391230643
674 -0.4093620542632305
675 -0.4093615439781989
676 -0.4093782057435786
677 -0.4093868962725573
678 -0.4094047549405356
679 -0.4094187245481491
680 -0.4094259174337001
681 -0.409428864494304
682 -0.4094299118539302
683 -0.40943745998479225
684 -0.40944537985952384
685 -0.4094569900834486
686 -0.40946031916189873
687 -0.40945710932251556
688 -0.4094541595685097
689 -0.4094616368131434
690 -0.4094742007745757
691 -0.4094869012734011
692 -0.409501057584674
693 -0.4095304518272815
694 -0.40956198977222713
695 -0.4095929159550196
696 -0.4096080574320258
697 -0.4096201294315215
698 -0.40962633346236244
699 -0.40962830157519464
700 -0.40962816447356903


==> plotdata/quadrotor/A4_x1_phase1.tex <==
0 1.5
1 1.5
2 1.5
3 1.5
4 1.4980720471294269
5 1.4919744382918967
6 1.47987352094078
7 1.460509409826998
8 1.4331699590193512
9 1.3977083598878939
10 1.3543981187477434
11 1.3037983304014256
12 1.2466505554002691
13 1.18388491243923
14 1.1166868223720376
15 1.0467530793277318
16 0.9762773520066411
17 0.9078017720376373
18 0.8439414954985905
19 0.7871302720795651
20 0.7394415533232888
21 0.702482982575357
22 0.677347327697088
23 0.6645668311394577
24 0.6641014279683428
25 0.6753354475406753
26 0.697158497558602
27 0.7280065985634818
28 0.7659705681371567
29 0.8089117543067381
30 0.8545788480431048
31 0.9006696988689881
32 0.9449410644981718
33 0.9853073449035237
34 1.0199039501591616
35 1.04716328176023
36 1.0658769522733789
37 1.0752349595116641
38 1.0748494991657198
39 1.0647567277256256
40 1.0454095089237663
41 1.0176707165426793
42 0.9827805619067461
43 0.9423010325540414
44 0.8980489322523573
45 0.851979998897102
46 0.8061761456951038
47 0.7626550252981883
48 0.7231332883412249
49 0.6887933232662442
50 0.6601060489173898
51 0.6367884751659113
52 0.617888638093189
53 0.6020314943751112
54 0.5858873538038736
55 0.5657726216261807
56 0.5388317768544001
57 0.5038235946657079
58 0.4613263363590234
59 0.412484901715889
60 0.35857414499941476
61 0.3016072036018358
62 0.2438622098881901
63 0.18761806241599138
64 0.13508567962755325
65 0.08842567383755935
66 0.04962351251579138
67 0.020731764080007258
68 0.0037463979598343286
69 0.00048519294836884934
70 0.012374694774529937
71 0.040206920915711444
72 0.08392818562927862
73 0.14288216209137708
74 0.21580369987652565
75 0.3007820114603462
76 0.3953812324057354
77 0.49674276235930503
78 0.6017875639543919
79 0.7073672318867157
80 0.8103488240172508
81 0.9077107632625293
82 0.9966655747386928
83 1.0747418434980596
84 1.1398182278037097
85 1.1902276592995356
86 1.2248294013137488
87 1.2430556998509787
88 1.2449371663531283
89 1.231059407013796
90 1.2025171088965878
91 1.1608818447416507
92 1.1081572982670174
93 1.046723837972439
94 0.979284953562041
95 0.9087902984008587
96 0.838399488366881
97 0.7712921633303191
98 0.7104030956548654
99 0.6580949912127924
100 0.615836280604662
101 0.5839779007523264
102 0.5616109969123723
103 0.546415174917964
104 0.5339673746964047
105 0.5196599301417536
106 0.49930681456446735
107 0.4696682164824396
108 0.42871825081045833
109 0.3742050100443701
110 0.30518398805527125
111 0.22580985682316873
112 0.14131084327835
113 0.056699793539352436
114 -0.02356804473913389
115 -0.09562788262837481
116 -0.15615432666579132
117 -0.20229421572361042
118 -0.23159875377976114
119 -0.241969279955216
120 -0.23161384741108051
121 -0.1990104406423161
122 -0.1428763620327853
123 -0.06214655412772835
124 0.042813019691485266
125 0.16855221822866556
126 0.3094803916975288
127 0.4595244529001372
128 0.6130980828586126
129 0.7653091608263536
130 0.9119411572549017
131 1.0493816275766965
132 1.174538163185559
133 1.2847603535850112
134 1.3777728852468527
135 1.451619257580556
136 1.5046144584718328
137 1.5352971883981044
138 1.5423856948536885
139 1.5258450876710747
140 1.4868963974930887
141 1.427774822421422
142 1.3515887296815436
143 1.2620862927396292
144 1.1636016599624692
145 1.0612220099451033
146 0.9597520891203969
147 0.8634446497235895
148 0.7759799430318529
149 0.7004974129095779
150 0.6396501373394551
151 0.5941635103807162
152 0.5605074093716631
153 0.5338111438289673
154 0.5092067936801958
155 0.48211227428738535
156 0.44847629943610906
157 0.4047970623819239
158 0.3480797806489425
159 0.2759185159807246
160 0.19218439754320948
161 0.10218356911298293
162 0.01109545383302453
163 -0.07645377164516884
164 -0.15645792578733184
165 -0.2254880360452013
166 -0.28061951870830637
167 -0.31936022250455104
168 -0.3395883666180924
169 -0.3394983537025136
170 -0.31755393557672273
171 -0.2724470071469447
172 -0.20306239621497255
173 -0.10844712101061614
174 0.01221804946489892
175 0.15406074136976566
176 0.31047900780625215
177 0.47510315627687316
178 0.6422881809179308
179 0.8071581492353829
180 0.9655270009061495
181 1.113793786486431
182 1.2488586183802919
183 1.368050316659831
184 1.4690579715213745
185 1.5498717902062482
186 1.6087348389216176
187 1.6441051677558898
188 1.6546308942395758
189 1.6391447043856824
190 1.5967399320762867
191 1.5267989878102655
192 1.4291624206456324
193 1.3076858094998536
194 1.1674037959199939
195 1.0131723353847513
196 0.8493696805792136
197 0.6798610482550673
198 0.5080953171224464
199 0.33718973577235023
200 0.1699961726974482
201 0.00919808126257704
202 -0.14353398218966293
203 -0.289265543502797
204 -0.4298521040808738
205 -0.5668438697679645
206 -0.7006557086374676
207 -0.8287828221165234
208 -0.9480487368656019
209 -1.0553601964804629
210 -1.1479291466210628
211 -1.223315467622938
212 -1.2794129641352945
213 -1.3144202744369506
214 -1.326805835796857
215 -1.3152798024581625
216 -1.2787673118876033
217 -1.2163777042150068
218 -1.1273937026120122
219 -1.0112590450235257
220 -0.8675448062225343
221 -0.7013307805969906
222 -0.5194901119382234
223 -0.32861200948933555
224 -0.13451097463630757
225 0.05923279963462247
226 0.2537057474075941
227 0.44810316111091164
228 0.6392398051355996
229 0.8234934915028107
230 0.9974476349501078
231 1.1580662974871168
232 1.3027174616182984
233 1.4291505191587774
234 1.5354600945907295
235 1.620040301929247
236 1.6815435258713198
237 1.7188423213817297
238 1.730992666839389
239 1.7172011501461648
240 1.6767961423242537
241 1.6092098092961098
242 1.513961815084475
243 1.3906472308887572
244 1.240073973660404
245 1.0684268849885126
246 0.8826935341987172
247 0.6893241940677409
248 0.4939454799188109
249 0.29880360366813363
250 0.10382781514629585
251 -0.09151508185111035
252 -0.2863954994472547
253 -0.4776732939138764
254 -0.6618206618938851
255 -0.8355306035710365
256 -0.9958766413402338
257 -1.140323769435668
258 -1.266694604354688
259 -1.3731255989758695
260 -1.458025246743599
261 -1.5200364128540886
262 -1.558002716388143
263 -1.570939837375456
264 -1.558010978076142
265 -1.5185055445441944
266 -1.4518205652813445
267 -1.3574442404234668
268 -1.23494157041854
269 -1.0851526776792157
270 -0.9142734778418203
271 -0.729305578600138
272 -0.5367179868363102
273 -0.34215774525444864
274 -0.14752073902541624
275 0.045831828485482784
276 0.24057026756429828
277 0.4348585311488927
278 0.6252268831436765
279 0.8080443115098264
280 0.9799783357626952
281 1.1381076823848884
282 1.2799192090704792
283 1.4032693807999042
284 1.5063382892959756
285 1.5875844173874802
286 1.645703088922262
287 1.6795901954767178
288 1.6883110948725348
289 1.6710739179310006
290 1.6272076253774872
291 1.556143530291309
292 1.4574000488743168
293 1.3305697019650675
294 1.1772322004123539
295 1.0037001099502312
296 0.8168977824581195
297 0.6231727876834494
298 0.42805184270344887
299 0.2329383863860261
300 0.038630591855904506
301 -0.15648354597686703
302 -0.35083406111170656
303 -0.5410849687059696
304 -0.7236927532741313
305 -0.8953907778016605
306 -1.0533075195983082
307 -1.1949645744410555
308 -1.3182388655309507
309 -1.4213178007755203
310 -1.502656745920352
311 -1.5609409761268518
312 -1.5950525329640237
313 -1.604041606866773
314 -1.5871019172140732
315 -1.5435495605417702
316 -1.4728046503183225
317 -1.3743755850077801
318 -1.2478457259804734
319 -1.0947912653938652
320 -0.9215250898126112
321 -0.7349763063686579
322 -0.5415003853111282
323 -0.3466355815299274
324 -0.1517442411006514
325 0.04182666221533163
326 0.2367481803057366
327 0.43099974586445006
328 0.6210918624134332
329 0.8034305952393402
330 0.974734958066007
331 1.1321329769069532
332 1.2731523276007246
333 1.3956795013763914
334 1.4979133533362226
335 1.5783230833157864
336 1.6356084796433752
337 1.6686659400308645
338 1.6765591506265567
339 1.6584942407252392
340 1.6137981834823254
341 1.5419007113297802
342 1.4423189159800307
343 1.3146441250243306
344 1.1606465553508376
345 0.9866704131375021
346 0.7996248869460075
347 0.6058325142875591
348 0.4107967153678288
349 0.21576479031937945
350 0.022070434359461738


==> plotdata/quadrotor/A4_x1_phase2.tex <==
350 0.022070434359461738
351 -0.17296126282836236
352 -0.36727930336066594
353 -0.5573945854531113
354 -0.7406971081118484
355 -0.9136348344302778
356 -1.0727057292069513
357 -1.2147516558845883
358 -1.3370156768445391
359 -1.4371227122768382
360 -1.5133049250970088
361 -1.5672816482649985
362 -1.602694203108396
363 -1.623567532975569
364 -1.6335410143182658
365 -1.6356267689297426
366 -1.6322118218157204
367 -1.6251435798638567
368 -1.6158289014941356
369 -1.6053226077471476
370 -1.5944003009538692
371 -1.5836172091508556
372 -1.5733553802340707
373 -1.5638615338664175
374 -1.5552780920186324
375 -1.5476687278764016
376 -1.5410388710632017
377 -1.5353525019449439
378 -1.5305453368650193
379 -1.5265354137224159
380 -1.5232316839465254
381 -1.520540464235422
382 -1.5183702780065227
383 -1.5166353398932544
384 -1.5152579664223904
385 -1.5141699401435158
386 -1.5133131875248904
387 -1.5126398394934961
388 -1.5121118731563123
389 -1.5117004389538613
390 -1.5113849931157635
391 -1.5111523142675691
392 -1.5109954691733267
393 -1.5109122695724857
394 -1.510903461221498
395 -1.510971592395325
396 -1.511120346262248
397 -1.5113542789226406
398 -1.5116785257056824
399 -1.5120988232067172
400 -1.5126551346878505
401 -1.5134238349323479
402 -1.5144885316860077
403 -1.5159158967067643
404 -1.5177458397620966
405 -1.5199900904184234
406 -1.5226348155737683
407 -1.5256462218967073
408 -1.5289780791101666
409 -1.5325782325100217
410 -1.536394872090322
411 -1.5403810406701135
412 -1.5444979640903465
413 -1.5487154459648553
414 -1.5530121944492632
415 -1.5573738540055133
416 -1.5617915952988428
417 -1.5662612473639987
418 -1.5707819403115433
419 -1.575352783695346
420 -1.5799729324105751
421 -1.5846426963470097
422 -1.5893627536103871
423 -1.594135880732812
424 -1.5989945669391405
425 -1.6040071631941608
426 -1.6092494152477719
427 -1.6147845191907146
428 -1.620655559456566
429 -1.6268851914781965
430 -1.6334791501030173
431 -1.6404299043134076
432 -1.647720544436549
433 -1.6553278100114863
434 -1.6632242549221452
435 -1.6713791546330965
436 -1.6797620863540224
437 -1.6883409945853411
438 -1.697083614160786
439 -1.7059581455053605
440 -1.7149327615497567
441 -1.723977455088269
442 -1.733064576292278
443 -1.742168414430136
444 -1.7512650197906348
445 -1.7603325031899584
446 -1.7693523181825979
447 -1.7783077523353268
448 -1.7871836751009442
449 -1.7959663422454246
450 -1.8046433718139003
451 -1.8132037753049757
452 -1.8216370292985027
453 -1.8299344454194932
454 -1.8380878794527669
455 -1.8460907939812299
456 -1.8539377740084417
457 -1.861624731938631
458 -1.8691482078485668
459 -1.876505369808671
460 -1.8836933641045692
461 -1.8907112273333742
462 -1.8975565528964375
463 -1.9042282396529697
464 -1.9107251709744553
465 -1.9170468189585936
466 -1.923193228136201
467 -1.9291649232964627
468 -1.9349634127301383
469 -1.9405893512750152
470 -1.9460436865098627
471 -1.9513272273312388
472 -1.956441046925937
473 -1.9613866075967008
474 -1.9661655802040798
475 -1.9707796795778167
476 -1.975230651900552
477 -1.9795203551804421
478 -1.9836508245099886
479 -1.9876242646443456
480 -1.9914430125346667
481 -1.9951094789754984
482 -1.998626088546426
483 -2.0019953237945143
484 -2.0052197895141
485 -2.008302068217755
486 -2.0112448650773747
487 -2.0140510922490407
488 -2.0167235991752253
489 -2.019265298109798
490 -2.021679168615981
491 -2.0239682887994395
492 -2.02613579603294
493 -2.0281848689915574
494 -2.030118727648055
495 -2.0319406419969823
496 -2.0336539249115826
497 -2.0352619383365664
498 -2.0367680992422774
499 -2.038175883619114
500 -2.0394887927738914
501 -2.040710372332016
502 -2.0418441427141967
503 -2.0428935703725153
504 -2.0438621560895287
505 -2.044755049167052
506 -2.0455797837197274
507 -2.0463459716538264
508 -2.0470650550834173
509 -2.047750395264012
510 -2.048418154654163
511 -2.0490860495665055
512 -2.0497718964116283
513 -2.0504944308320385
514 -2.051272224664018
515 -2.0521195909016225
516 -2.0530432404263586
517 -2.0540380432436836
518 -2.0550890852572468
519 -2.0561787177730966
520 -2.057278377730047
521 -2.0583320030822425
522 -2.0592775195464212
523 -2.0600608545253154
524 -2.06064246577869
525 -2.060988552575831
526 -2.0610808821073316
527 -2.060912237708356
528 -2.0604805592778486
529 -2.0597844030402532
530 -2.058821509808958
531 -2.057588929041857
532 -2.0560850955621226
533 -2.054310799837989
534 -2.0522725698362327
535 -2.0499815107301576
536 -2.0474493219278527
537 -2.044685884704924
538 -2.0416956797748615
539 -2.0384789469361126
540 -2.035036716481208
541 -2.031372494058674
542 -2.027490275984043
543 -2.023392422957113
544 -2.019079417463732
545 -2.014550648473528
546 -2.009803660944881
547 -2.0048348682455215
548 -1.9996400770222724
549 -1.9942151540652582
550 -1.9885562354003192
551 -1.98265956293982
552 -1.9765215861056433
553 -1.9701388801934459
554 -1.9635082461701765
555 -1.9566269358684734
556 -1.9494930946355942
557 -1.9421053388428744
558 -1.934462257664441
559 -1.926563659858706
560 -1.9184106257246143
561 -1.9100048109229184
562 -1.901348097798603
563 -1.8924429204903037
564 -1.8832923521447882
565 -1.8739001865192115
566 -1.8642704823731149
567 -1.85440797354751
568 -1.844317330406658
569 -1.8340036094992294
570 -1.8234722795717335
571 -1.812729273573844
572 -1.8017795875732066
573 -1.790628485550898
574 -1.7792818379827768
575 -1.7677454306507792
576 -1.756024673185833
577 -1.7441255509072222
578 -1.732053759370651
579 -1.7198144451586386
580 -1.7074129445286734
581 -1.694854804310375
582 -1.6821443169071812
583 -1.6692859911768854
584 -1.6562840815405222
585 -1.6431429713076302
586 -1.62986618897104
587 -1.616457250423735
588 -1.6029196555595155
589 -1.5892570508301667
590 -1.5754725800184224
591 -1.5615686312698775
592 -1.547548014806723
593 -1.5334125575821125
594 -1.5191645978857875
595 -1.504805422791337
596 -1.490337267836465
597 -1.4757622683445972
598 -1.4610817393762132
599 -1.4462966984599497
600 -1.4314084499081976
601 -1.416417613192513
602 -1.4013249582558622
603 -1.386130880478003
604 -1.3708361836308958
605 -1.3554421100063845
606 -1.3399486961402765
607 -1.324356485131348
608 -1.3086660334545555
609 -1.2928768501284984
610 -1.2769886702111133
611 -1.261001553372008
612 -1.2449161761114507
613 -1.2287329491633665
614 -1.2124514000226543
615 -1.19607120725424
616 -1.179592216257549
617 -1.163014340623815
618 -1.1463375024259437
619 -1.129561594790064
620 -1.1126864708996098
621 -1.0957119481756052
622 -1.0786378107354095
623 -1.061463815140341
624 -1.0441897013138133
625 -1.0268155366217604
626 -1.0093407853045833
627 -0.9917649839846171
628 -0.9740877719297898
629 -0.9563093011190095
630 -0.9384290840493461
631 -0.9204466029282883
632 -0.9023614986727216
633 -0.8841740324466797
634 -0.8658837379567375
635 -0.847490554640859
636 -0.8289939711502251
637 -0.810393819077223
638 -0.7916900575103342
639 -0.7728826598556553
640 -0.7539709676542408
641 -0.734954500231929
642 -0.7158328170373276
643 -0.6966059949453101
644 -0.6772742779324846
645 -0.6578375562268988
646 -0.6382958218826498
647 -0.6186489695328223
648 -0.598896544179875
649 -0.5790384996809907
650 -0.5590746607844179
651 -0.5390052082883521
652 -0.5188301787677191
653 -0.4985494561594736
654 -0.47816298660043144
655 -0.45767072206829107
656 -0.43707265301087106
657 -0.41636868781172043
658 -0.39555908467848483
659 -0.374643789892157
660 -0.3536227779581142
661 -0.3324959842098319
662 -0.31126337455438535
663 -0.2899250628908906
664 -0.2684811827107099
665 -0.24693183540947017
666 -0.22527712928814247
667 -0.20351713404165211
668 -0.18165229654445808
669 -0.1596827149832423
670 -0.1376081020920607
671 -0.11542859928541596
672 -0.09314465963403702
673 -0.07075686106625102
674 -0.04826475172436943
675 -0.02566858147402526
676 -0.0029686574244593283
677 0.019835163181516822
678 0.04274255441106932
679 0.06575351795605987
680 0.08886786043468758
681 0.11208547542916966
682 0.13540617199151664
683 0.1588298488032809
684 0.18235583475809597
685 0.2059839871059352
686 0.22971419403506732
687 0.2535463292293763
688 0.27748040899169624
689 0.3015164127845461
690 0.32565405800393504
691 0.34989300878631174
692 0.37423287553971984
693 0.3986729250471912
694 0.4232132977943829
695 0.44785393532415185
696 0.4725947205602107
697 0.4974350557752579
698 0.5223747572428019
699 0.5474135764280788
700 0.5725513670046487


==> plotdata/quadrotor/A4_x2_phase1.tex <==
0 0.0
1 0.0
2 0.0
3 0.0
4 -0.00027751133004694993
5 -0.0013315549528138293
6 -0.0037832534205044493
7 -0.008306279850509522
8 -0.01557597137114146
9 -0.026189229881033376
10 -0.04064770107859758
11 -0.059352085571252766
12 -0.08261209534923727
13 -0.1106555385922068
14 -0.14398722432290476
15 -0.1829878441783756
16 -0.2276177980509547
17 -0.2772618814840555
18 -0.3308326619101977
19 -0.3868802983274693
20 -0.44370150280629894
21 -0.49940067193446663
22 -0.5519726025660978
23 -0.5993659120598919
24 -0.6395941732025461
25 -0.6708240299307463
26 -0.6914422801689926
27 -0.700132749185551
28 -0.6959357343440619
29 -0.6782658372851283
30 -0.6468984553874495
31 -0.6019932159673049
32 -0.5440610567958688
33 -0.4739559629905216
34 -0.3928385125269061
35 -0.302138907471869
36 -0.20350200416530187
37 -0.09874151343934867
38 0.010170440020653579
39 0.12114987825537062
40 0.23204329647490846
41 0.3406348622828083
42 0.444690304606316
43 0.5420080774856926
44 0.630463072961181
45 0.7080538705121645
46 0.7730065858473786
47 0.8237947613596888
48 0.8592094573684401
49 0.8784547701832583
50 0.8812733466136713
51 0.8680778641464602
52 0.8398986751422661
53 0.7981731878384082
54 0.7439916623054837
55 0.678462717331855
56 0.6029563050258746
57 0.5190611675408577
58 0.4283760269313427
59 0.33227598877480363
60 0.23190929212986278
61 0.12848593076008097
62 0.023135475290060478
63 -0.08320189474051067
64 -0.1900800880200727
65 -0.2970740179845735
66 -0.4034706950838774
67 -0.5081866154194794
68 -0.6098192842918083
69 -0.7067383122572892
70 -0.7971489324793299
71 -0.8791385171393429
72 -0.9507569568750373
73 -1.0101072511431919
74 -1.0554288794900295
75 -1.085180757477054
76 -1.0981214605114287
77 -1.0933879593313145
78 -1.0705483052716547
79 -1.0296022971645549
80 -0.9709479982589335
81 -0.8953763094919525
82 -0.8040125934802873
83 -0.6982991557767826
84 -0.5799576113125742
85 -0.4509344457004083
86 -0.3133299598767707
87 -0.16933825007963116
88 -0.021242854380780857
89 0.12865374173135535
90 0.27807033605505127
91 0.4247379403679006
92 0.5664202813459345
93 0.7009222530798827
94 0.8260684133189297
95 0.939727936503322
96 1.0399169149178173
97 1.124843326108015
98 1.1929432259862132
99 1.2429571805060198
100 1.2740317833160861
101 1.2858245799852563
102 1.2784213370471411
103 1.2521178044135026
104 1.206738651415337
105 1.1422679671257816
106 1.059360798184203
107 0.9593833987010937
108 0.8436954550835126
109 0.7132068388599226
110 0.5685416424841313
111 0.41095379840002233
112 0.24308730585428445
113 0.06846023911030005
114 -0.10965030153789057
115 -0.288157593212759
116 -0.46401641105203617
117 -0.6341725337921813
118 -0.795409380471921
119 -0.9447349470935426
120 -1.0794958874797147
121 -1.1973821294736846
122 -1.2963970344237599
123 -1.3748196114044793
124 -1.4311688117329249
125 -1.46417303685586
126 -1.4727460008907254
127 -1.4564274514900082
128 -1.4155273696880097
129 -1.350959123950512
130 -1.2640818956327164
131 -1.1566250065050334
132 -1.0305842955064577
133 -0.8881938859079651
134 -0.7318900170221097
135 -0.5642563888039892
136 -0.3879612272641057
137 -0.20571433063396877
138 -0.020259594309651435
139 0.165694682564206
140 0.3495137822996706
141 0.528600687468954
142 0.7004145211314694
143 0.8625021214899149
144 1.012481309826713
145 1.1480592910741898
146 1.2671201965785732
147 1.3677493127644316
148 1.4482490419280574
149 1.507195797036726
150 1.5435192567708613
151 1.5565810574023675
152 1.5461038651896066
153 1.5119466614004202
154 1.453422032920749
155 1.3700352258416257
156 1.2623045339881835
157 1.1323111604828384
158 0.9830381000479022
159 0.8173046469605756
160 0.6377477475261342
161 0.44795417800363235
162 0.2529696138525859
163 0.05737859928084954
164 -0.13835053503057396
165 -0.3335372449205577
166 -0.5250962934372166
167 -0.7095141972083864
168 -0.8834819379488443
169 -1.0440633311172611
170 -1.1887092694535208
171 -1.315225349568858
172 -1.4217316408009981
173 -1.5066228376681923
174 -1.5685305240791374
175 -1.6062904530776034
176 -1.6189167210094377
177 -1.6055813996451467
178 -1.5655928821923508
179 -1.4983834860559642
180 -1.404173462843468
181 -1.2849793620847125
182 -1.1438792055112246
183 -0.9844680255958487
184 -0.8106123356174062
185 -0.6262989798314678
186 -0.435462007414335
187 -0.24164733774611774
188 -0.04729037389576879
189 0.14722461745010107
190 0.34002634244252394
191 0.5277597278319955
192 0.706919972775811
193 0.8742842186372132
194 1.0270222178772364
195 1.1627026348693676
196 1.2792530644148843
197 1.3749121156897959
198 1.44819137482213
199 1.4978390510550315
200 1.5228059741144138
201 1.5222120261342538
202 1.4953173358325131
203 1.4414980873217575
204 1.3602248942594146
205 1.2510499185152404
206 1.1135966614809958
207 0.9517741867037407
208 0.7723073734923378
209 0.5819566637155038
210 0.3867751009777502
211 0.19158017540197586
212 -0.0032594514739752722
213 -0.19770646844693365
214 -0.3929251388250944
215 -0.5862426912155724
216 -0.7740970245246738
217 -0.9530022466745549
218 -1.1198287208485658
219 -1.2718520258988142
220 -1.4067295331775043
221 -1.5224568574411106
222 -1.6173234097807763
223 -1.6898722601469738
224 -1.738864201629032
225 -1.7632454180416874
226 -1.762120944248194
227 -1.734731159888129
228 -1.6804319438484547
229 -1.5986768425864115
230 -1.4890012963025574
231 -1.3510092476019966
232 -1.1888867731436583
233 -1.0094093452749036
234 -0.8193278032152839
235 -0.6246725210880198
236 -0.42994707054435005
237 -0.23516717442142446
238 -0.04083268030809223
239 0.15398095153642338
240 0.3465515635470986
241 0.5333182019956202
242 0.7108076272878735
243 0.8759053747689496
244 1.0259045705490761
245 1.158483873735684
246 1.271665074735459
247 1.3637682348168565
248 1.4333698997266024
249 1.4792649954567971
250 1.500433822433323
251 1.4960134192338514
252 1.4652730323448988
253 1.4075937740775877
254 1.3224512189347153
255 1.2094011256175374
256 1.0680675098717916
257 0.9033168523291568
258 0.7220329910044622
259 0.5309013096613842
260 0.33584757614320737
261 0.14078727655679701
262 -0.05427725376717768
263 -0.2490130012452922
264 -0.44408122992218535
265 -0.6367032384070717
266 -0.8233387762466517
267 -1.0005595779819885
268 -1.1652988575577143
269 -1.3148917022287245
270 -1.4470495739792344
271 -1.5598169280978091
272 -1.65152694332974
273 -1.7207611146989505
274 -1.7663137914743132
275 -1.787160934347928
276 -1.7824336732707768
277 -1.7513949771398176
278 -1.6934198335300994
279 -1.607978389300676
280 -1.4946218130351714
281 -1.352970027417329
282 -1.1880069072113137
283 -1.0066373293634099
284 -0.8155415859275189
285 -0.6206362515953829
286 -0.42570548974192635
287 -0.23076048045872527
288 -0.036073232043788483
289 0.15888113560557768
290 0.35128729459503294
291 0.5375992451273481
292 0.7143917525585386
293 0.8786038202735004
294 1.02757755164805
295 1.1590322191022566
296 1.2710211690251747
297 1.361887600367555
298 1.4302235893085735
299 1.4748340031513272
300 1.4947049635834686
301 1.4889767386186477
302 1.4569204895358447
303 1.3979185546028514
304 1.3114475981816178
305 1.19706447730355
306 1.0543943083624028
307 0.8886326328898735
308 0.7067180012583081
309 0.5153095085654283
310 0.3202882138964944
311 0.12526446372696753
312 -0.06976119889119164
313 -0.2645682341216522
314 -0.45959568427041475
315 -0.6520098178041922
316 -0.8382711433258716
317 -1.014968825495874
318 -1.1790571784772832
319 -1.3278918134991038
320 -1.4592027528459226
321 -1.5710510033469074
322 -1.6617843433900783
323 -1.729996893487507
324 -1.7744935237954225
325 -1.7942590818518416
326 -1.7884318526967662
327 -1.7562808740164277
328 -1.6971863174796946
329 -1.610622850521053
330 -1.496145554701362
331 -1.3533777838864696
332 -1.1875540771301956
333 -1.005620001106772
334 -0.8142327211340332
335 -0.6192700627048187
336 -0.4242977235533171
337 -0.22931958033816957
338 -0.034534777190437155
339 0.16044796987999613
340 0.3527821663632088
341 0.5389264342082243
342 0.7154711582839536
343 0.8793728291173222
344 1.0279897408637417
345 1.1590547367192214
346 1.2706319220752935
347 1.3610722979590526
348 1.4289735129111085
349 1.4731439416640675
350 1.4925717709594855


==> plotdata/quadrotor/A4_x2_phase2.tex <==
350 1.4925717709594855
351 1.4863984446814669
352 1.4538957509827537
353 1.39444632137001
354 1.3095396742596404
355 1.205832188441609
356 1.0906791418956505
357 0.9708467108071459
358 0.8522458551253111
359 0.7399585918641077
360 0.6383337710371687
361 0.5510883249366043
362 0.47915530378810456
363 0.42129186336530633
364 0.37535568897496063
365 0.33910813832027875
366 0.31056070022559445
367 0.28806702229801073
368 0.27030595277430713
369 0.2562300674916618
370 0.2450111808533381
371 0.23599314600971186
372 0.22865393539029877
373 0.22257655875407512
374 0.217426301051777
375 0.21293313726324628
376 0.2088781056760303
377 0.2050827196551951
378 0.2014011304764717
379 0.1977141924069064
380 0.19392439051092422
381 0.18995227477234133
382 0.18573359109595405
383 0.18121701009397262
384 0.17636187523478297
385 0.17113694210721436
386 0.16551878442374215
387 0.1594908371979058
388 0.15304236593104864
389 0.14616775367831356
390 0.13886575443630905
391 0.13113879316399565
392 0.12299242578738617
393 0.11443676304767993
394 0.10548981448494991
395 0.09617751952993886
396 0.08653123842918106
397 0.07658393770977448
398 0.06636807237758358
399 0.05591319056921987
400 0.045233485617762414
401 0.03433264562805701
402 0.023212856486319995
403 0.011879803685428986
404 0.0003424825635862522
405 -0.011387442651869388
406 -0.02329595319491095
407 -0.03536754856078729
408 -0.04758708857956377
409 -0.05993974412865696
410 -0.0724117453111837
411 -0.0849904175702247
412 -0.09766496611169834
413 -0.11042526275902133
414 -0.12326228631060127
415 -0.13616776881538883
416 -0.1491338072168606
417 -0.16215315450689327
418 -0.1752200911928856
419 -0.18832546620710933
420 -0.20145792722555994
421 -0.2146072464620624
422 -0.22776423583688699
423 -0.24092118521596298
424 -0.25407591393365014
425 -0.26723080762008905
426 -0.28038641712874024
427 -0.29353868962728713
428 -0.3066793230614247
429 -0.3197969142174844
430 -0.3328786175584721
431 -0.34591152340839404
432 -0.35888341761036074
433 -0.37178318012546596
434 -0.384600795996657
435 -0.3973272737960416
436 -0.40995573344853226
437 -0.42247970284157627
438 -0.43489329135101246
439 -0.44719104446947255
440 -0.4593672099530042
441 -0.47141668403976816
442 -0.4833352731598543
443 -0.4951191874348205
444 -0.5067649364229739
445 -0.5182693390025428
446 -0.5296299460010934
447 -0.5408447175137334
448 -0.5519117655621281
449 -0.5628293707009264
450 -0.5735958154502888
451 -0.5842097164222743
452 -0.5946696181513177
453 -0.6049742728891525
454 -0.6151224641295717
455 -0.6251134138472165
456 -0.6349464114776253
457 -0.6446210121746987
458 -0.6541367870783256
459 -0.6634933149510769
460 -0.6726898506308545
461 -0.6817259136983862
462 -0.6906007958673472
463 -0.699314414744771
464 -0.7078665419278684
465 -0.7162570477308956
466 -0.7244858957127752
467 -0.7325532615377276
468 -0.7404594333864345
469 -0.7482045694018037
470 -0.7557888553338977
471 -0.7632124148127192
472 -0.77047536389373
473 -0.7775779017945041
474 -0.7845203479433537
475 -0.7913030793255884
476 -0.7979262898956717
477 -0.8043902975911777
478 -0.8106956246679637
479 -0.8168428595570585
480 -0.8228325857690104
481 -0.8286654105963012
482 -0.8343419117291043
483 -0.8398626610411845
484 -0.8452283367569172
485 -0.8504396531519649
486 -0.8554973488374535
487 -0.8604022619667961
488 -0.8651552825882142
489 -0.8697572913958354
490 -0.8742092475430822
491 -0.8785121861300239
492 -0.8826671952865095
493 -0.886675416645142
494 -0.890538030159307
495 -0.8942562657131166
496 -0.8978314051676292
497 -0.9012648071086262
498 -0.9045579074596035
499 -0.9077122222952507
500 -0.9107293345463676
501 -0.9136109133773711
502 -0.9163587250172287
503 -0.9189745140347242
504 -0.9214599655594935
505 -0.9237847827718568
506 -0.9258915215939518
507 -0.9277191375480717
508 -0.9292180579547958
509 -0.9303563113535047
510 -0.9311205261605041
511 -0.9315143210269562
512 -0.931556226968967
513 -0.9312771540479856
514 -0.930718073243554
515 -0.9299264038595856
516 -0.9289511808986746
517 -0.9278471510098926
518 -0.9266651216314604
519 -0.9254292064944385
520 -0.9241475077283494
521 -0.9228656654578989
522 -0.9216275144908604
523 -0.9204769555450776
524 -0.9194570306839471
525 -0.9186135672011795
526 -0.9179622674865563
527 -0.9174917855390617
528 -0.9171742761868545
529 -0.9169763410633965
530 -0.9168653364575933
531 -0.9168131907764459
532 -0.9167979545176393
533 -0.9168037464952002
534 -0.9168204635370866
535 -0.9168424730775103
536 -0.9168670866281784
537 -0.9168934407389306
538 -0.916921720900742
539 -0.9169526234465163
540 -0.9169870724893849
541 -0.9170259131730779
542 -0.9170694304590986
543 -0.9171169658529326
544 -0.9171665832588426
545 -0.9172149550218661
546 -0.9172571861264865
547 -0.9172867402320803
548 -0.917295423724303
549 -0.9172734851969284
550 -0.9172097525530596
551 -0.9170917495579403
552 -0.9169058904068
553 -0.9166376720086687
554 -0.9162719485911401
555 -0.9157932237873441
556 -0.9151859516992081
557 -0.9144346624888751
558 -0.9135238944764624
559 -0.9124390658579625
560 -0.9111665332906161
561 -0.9096934869359405
562 -0.9080079197576779
563 -0.9060988040905371
564 -0.9039562695303173
565 -0.9015715210708196
566 -0.8989370424742974
567 -0.8960466478389214
568 -0.8928951247232079
569 -0.8894783254017191
570 -0.8857931490095673
571 -0.8818375269108196
572 -0.8776100786501303
573 -0.8731102767670694
574 -0.8683385234471078
575 -0.8632958630920377
576 -0.8579838787109155
577 -0.8524048749040994
578 -0.8465614619558689
579 -0.8404565324504069
580 -0.8340934525265283
581 -0.827476077163406
582 -0.8206082712739767
583 -0.8134939995726332
584 -0.8061373199198205
585 -0.7985426501768216
586 -0.7907141090026639
587 -0.7826560971631615
588 -0.7743728438926205
589 -0.7658686848196392
590 -0.7571480129144125
591 -0.7482149721520167
592 -0.7390735333401
593 -0.7297274572385978
594 -0.7201806153229054
595 -0.7104364590241625
596 -0.700498692050673
597 -0.6903710571273312
598 -0.6800568190234082
599 -0.6695590912942073
600 -0.6588809943371035
601 -0.6480254391527966
602 -0.6369953165177059
603 -0.6257931183534369
604 -0.614421312281535
605 -0.6028824392257863
606 -0.5911785544281972
607 -0.5793118334591276
608 -0.5672844799053867
609 -0.5550984494228876
610 -0.5427555978381816
611 -0.5302577444314743
612 -0.5176067670937408
613 -0.5048042819486904
614 -0.49185170539772033
615 -0.4787504525394665
616 -0.4655019065200582
617 -0.4521073965119767
618 -0.43856818723223956
619 -0.42488548077318233
620 -0.41106041477684246
621 -0.39709406614948156
622 -0.38298745336878953
623 -0.368741541633877
624 -0.35435725050924316
625 -0.33983546653002017
626 -0.32517697325378553
627 -0.31038256119599467
628 -0.29545300026223104
629 -0.2803890711234638
630 -0.2651914917480551
631 -0.2498608782755327
632 -0.23439786461271508
633 -0.21880332033967728
634 -0.20307767640679283
635 -0.1872217623560621
636 -0.17123583327089087
637 -0.15512052819738067
638 -0.1388766388952885
639 -0.12250473879178506
640 -0.10600502152877816
641 -0.08937779742479164
642 -0.07262332575079565
643 -0.055742255753066
644 -0.03873532758675385
645 -0.02160295475009817
646 -0.0043457295097472926
647 0.013035965868823062
648 0.030541998490186493
649 0.04817194093263971
650 0.06592544043841866
651 0.08380186541494451
652 0.10180070374027936
653 0.1199216336071232
654 0.13816429029992194
655 0.15652837886470905
656 0.17501345777583624
657 0.19361921581793914
658 0.21234509941421637
659 0.2311907542308386
660 0.2501558124669053
661 0.2692399842624547
662 0.2884429765040945
663 0.3077643769682097
664 0.32720376767147036
665 0.3467607679161926
666 0.36643499670355173
667 0.38622612210881446
668 0.40613347064528804
669 0.4261566961605402
670 0.44629581547186686
671 0.4665504536306826
672 0.4869199603021657
673 0.5074035786889337
674 0.5280015154597697
675 0.548713325484688
676 0.5695385180846597
677 0.5904770254894312
678 0.6115283660157145
679 0.6326923521728889
680 0.6539686353652941
681 0.6753569307194813
682 0.6968568830640955
683 0.7184682326226733
684 0.7401901959362491
685 0.7620224858608254
686 0.7839648511196274
687 0.8060170292333232
688 0.8281789013070857
689 0.8504503172691529
690 0.8728308827029225
691 0.8953201607975134
692 0.9179176680150187
693 0.9406225964252403
694 0.9634349665386405
695 0.9863546166231761
696 1.009381322252741
697 1.0325144098860113
698 1.0557536016595443
699 1.079098569300709
700 1.1025490811989798


==> plotdata/quadrotor/A4_x3_phase1.tex <==
0 0.0
1 0.0
2 1.1155520951433575e-14
3 1.623590151211829e-14
4 -7.85149723014911e-15
5 -1.0169642905566436e-13
6 -3.5983660495730883e-13
7 -8.881428925633374e-13
8 -1.7876899960356243e-12
9 -3.2055247345397223e-12
10 -5.3061377514040944e-12
11 -8.283134178554974e-12
12 -1.1997585147582868e-11
13 -1.639607560832701e-11
14 -2.1189840992974495e-11
15 -2.6013715626049816e-11
16 -3.085261823798646e-11
17 -3.5675604692642085e-11
18 -4.024954591841379e-11
19 -4.429976385722512e-11
20 -4.774351580749681e-11
21 -5.0507757975992724e-11
22 -5.2587640908541294e-11
23 -5.4093192147774975e-11
24 -5.4801425619643856e-11
25 -5.488928422892059e-11
26 -5.43199796254612e-11
27 -5.328596230924632e-11
28 -5.180931239578968e-11
29 -5.00209118570183e-11
30 -4.797987784854741e-11
31 -4.57280080468081e-11
32 -4.336177639174821e-11
33 -4.0922998323367214e-11
34 -3.8464182949837784e-11
35 -3.6046348128593317e-11
36 -3.3810554356250586e-11
37 -3.195680164935767e-11
38 -3.06647507386515e-11
39 -3.013017391140239e-11
40 -3.0693581010154966e-11
41 -3.2683544759493096e-11
42 -3.6633203137625975e-11
43 -4.336769166002342e-11
44 -5.027157357062607e-11
45 -5.369512834363378e-11
46 -4.92277330010893e-11
47 -3.159524197826613e-11
48 5.292601912287866e-12
49 6.832248544696996e-11
50 1.6517740064614375e-10
51 3.0337291789805935e-10
52 4.907106188056787e-10
53 7.363744458643851e-10
54 1.048293594152483e-09
55 1.4297711992128372e-09
56 1.87745261115424e-09
57 2.3775519331081796e-09
58 2.9028947245990366e-09
59 3.4115218561225903e-09
60 3.849693275270738e-09
61 4.209178499081645e-09
62 4.486000548808988e-09
63 4.679750844616137e-09
64 4.7925707313822844e-09
65 4.830053637050469e-09
66 4.8011621167631806e-09
67 4.708894092431138e-09
68 4.561272604064471e-09
69 4.358712786256548e-09
70 4.1020988206241796e-09
71 3.795355940638957e-09
72 3.4416122218772227e-09
73 3.047349270701717e-09
74 2.618062691084334e-09
75 2.1641257674787093e-09
76 1.706095460463076e-09
77 1.2579275576740665e-09
78 8.441082144372567e-10
79 5.478005604686596e-10
80 5.665675217869658e-10
81 1.2090730372449355e-09
82 3.002580903910258e-09
83 6.854358680641328e-09
84 1.4278876712126025e-08
85 2.7815032250799737e-08
86 5.119674641562711e-08
87 9.020163071582488e-08
88 1.5340017837317534e-07
89 2.533032042073558e-07
90 4.0795461783815775e-07
91 6.430642749144511e-07
92 9.948693379691065e-07
93 1.5138083780463775e-06
94 2.2689053863445e-06
95 3.351426765956234e-06
96 4.878098049623248e-06
97 6.9923049947817615e-06
98 9.862760721279783e-06
99 1.3677253366566332e-05
100 1.864098591317642e-05
101 2.4954284438347684e-05
102 3.275449201833425e-05
103 4.208996143761468e-05
104 5.2920991656684186e-05
105 6.51533747997668e-05
106 7.857872996520855e-05
107 9.297802182704374e-05
108 0.00010788204764329736
109 0.000122544336867243
110 0.00013589432787330935
111 0.0001464918914604496
112 0.0001533648808193533
113 0.00015681493645850253
114 0.00015718042876873285
115 0.00015477692381152153
116 0.0001499385052815505
117 0.0001430114801778437
118 0.00013433631686190494
119 0.00012422573851450736
120 0.00011294885260229037
121 0.00010071323190366853
122 8.765005592845652e-05
123 7.383640452820469e-05
124 5.936187988018201e-05
125 4.436026144267299e-05
126 2.912607227791849e-05
127 1.4266156074196309e-05
128 1.046093193455238e-06
129 -8.06661361021814e-06
130 -8.523370309365716e-06
131 7.580334753018962e-06
132 5.457174286730645e-05
133 0.00015764558958817785
134 0.00035940812014830566
135 0.0007266896694135738
136 0.0013647557095758955
137 0.0024209573433895317
138 0.0040723009301363786
139 0.006431665437374575
140 0.009527422803438376
141 0.013404329813279645
142 0.01812109069442064
143 0.023751954088282047
144 0.030385646213244435
145 0.038117318081846194
146 0.047038532968964666
147 0.05722256719374566
148 0.06869503462102247
149 0.08135018449882211
150 0.0949767891976491
151 0.1093190904384831
152 0.12406880193840678
153 0.13885175541803085
154 0.1532102022424636
155 0.16658315199575963
156 0.1782909111929167
157 0.18790131030013735
158 0.19524985171874035
159 0.20003747735716848
160 0.20182221867245978
161 0.2000133843257637
162 0.19486849361673605
163 0.18709126618126554
164 0.17730172374456096
165 0.16603857996945276
166 0.15376426973255314
167 0.14087311936036961
168 0.12769793634877077
169 0.11451769917131113
170 0.10156242439806454
171 0.08901851092016841
172 0.07703492985542812
173 0.0657275342675121
174 0.05518701346236325
175 0.04547165284178621
176 0.03662829875214908
177 0.028701936619625182
178 0.021743511898588117
179 0.015810025431970607
180 0.010944618791293017
181 0.007220153302828859
182 0.004706072540015829
183 0.003431579426248321
184 0.0034022272321191298
185 0.004636599152247956
186 0.007169095274294471
187 0.011049867454255437
188 0.016352090258216073
189 0.023157807199122395
190 0.03149227825748345
191 0.041341357758320076
192 0.05271215893061422
193 0.06563036283586511
194 0.080139189983911
195 0.09629264013412128
196 0.11414149647444
197 0.13370867317376436
198 0.1549529994099821
199 0.1776798010827279
200 0.2015558463887899
201 0.22615648455844306
202 0.250944344437868
203 0.27524600987931513
204 0.29822447617821757
205 0.3188496582009993
206 0.3358820209907737
207 0.3485966930867576
208 0.35636539600436995
209 0.3582384322245669
210 0.3529197942298556
211 0.33931715345700647
212 0.31921158349675605
213 0.2945641105025573
214 0.26701442089703553
215 0.2379165419700486
216 0.20837218865042167
217 0.1792613855622313
218 0.15127319923706645
219 0.12493379186592946
220 0.10063097612556815
221 0.0786360876493869
222 0.059122618353792095
223 0.042182353207258425
224 0.027838012612080083
225 0.016020445145721436
226 0.006580454137607626
227 -0.0006946660215490039
228 -0.006069035306215427
229 -0.00984867591534159
230 -0.012416741408961297
231 -0.014166458641373156
232 -0.01534127148620073
233 -0.016068789572707208
234 -0.01640754245745791
235 -0.01636108776915473
236 -0.01589858417826307
237 -0.014963951195209504
238 -0.0134689977282901
239 -0.011306936876291102
240 -0.008416697558071042
241 -0.004764799229874557
242 -0.00028336011464835144
243 0.005128750140572828
244 0.011604997557014921
245 0.019304734857390798
246 0.028399211837261594
247 0.039046477786772296
248 0.05135423428019566
249 0.06528851389342569
250 0.08068609559495729
251 0.09729766971183408
252 0.1147623513504961
253 0.1325788753180726
254 0.15007233796936365
255 0.16635818279722697
256 0.1803195296117945
257 0.19132451318153385
258 0.19880287407337213
259 0.201824362531953
260 0.1990723143080008
261 0.18939353419457677
262 0.17447110191087625
263 0.1561376395286589
264 0.1358824040857854
265 0.11489483505065859
266 0.09410465931111119
267 0.07421796805022263
268 0.05575255022289011
269 0.03906964791235376
270 0.024401314250884928
271 0.01187467125665715
272 0.0015321940033598547
273 -0.006651366409384633
274 -0.012755512702636765
275 -0.01693695598266793
276 -0.019417153141272816
277 -0.020464318676758752
278 -0.02038189990359089
279 -0.019500265290790603
280 -0.018213081916964347
281 -0.016913534999938733
282 -0.01583747360187527
283 -0.015099605479902363
284 -0.014742128895329899
285 -0.01474926578578983
286 -0.015067262876125897
287 -0.01561598130798245
288 -0.01628016029517509
289 -0.016923068806629884
290 -0.017449557498959104
291 -0.017787023968729488
292 -0.017822317762985318
293 -0.01740144280533414
294 -0.016329380175299092
295 -0.014375141078958154
296 -0.0112856040249012
297 -0.00680936102870931
298 -0.0007339522982357924
299 0.007022117257343181
300 0.016420041617849667
301 0.027341632740908013
302 0.039560866389203087
303 0.052709592080795856
304 0.06624078153784271
305 0.07938569808426521
306 0.09112582334067185
307 0.10090425644040943
308 0.10819692020921233
309 0.11208738254268145
310 0.11123834445879605
311 0.10444132100197183
312 0.09329254592099243
313 0.0795129435046488
314 0.06446313409796815
315 0.04919480250095036
316 0.03449704923869808
317 0.020937546192816535
318 0.008901899513474757
319 -0.0013713452766733487
320 -0.009761018823570618
321 -0.01623754454690495
322 -0.020841263297593896
323 -0.023664626257175463
324 -0.02483891260265282
325 -0.024557511058971263
326 -0.02306435877229221
327 -0.020637881281647397
328 -0.01758072775391703
329 -0.014213794285237126
330 -0.010915437384599136
331 -0.008059305145583624
332 -0.0058599053621175515
333 -0.004410907332892795
334 -0.0037350346898174956
335 -0.0037996997324566176
336 -0.0045375976037381445
337 -0.005858283907740926
338 -0.00763909984998198
339 -0.009737932463749899
340 -0.012055563404153095
341 -0.014514525277476603
342 -0.016994401011294596
343 -0.019330655193074232
344 -0.021311750046157738
345 -0.022683133565596564
346 -0.02315818679881347
347 -0.022440863697058826
348 -0.02026293696081941
349 -0.01647529082586853
350 -0.011037278476015506


==> plotdata/quadrotor/A4_x3_phase2.tex <==
350 -0.011037278476015506
351 -0.00397745610714695
352 0.002783771830598386
353 0.009167684477755
354 0.01327705919412294
355 0.01562178170541538
356 0.016822482574110665
357 0.017406536335719168
358 0.01770744534891515
359 0.017866403633022863
360 0.01794931395243779
361 0.017989025679958883
362 0.018007722102860908
363 0.0180162021780899
364 0.018020437517731868
365 0.01802278131373862
366 0.018023872844897003
367 0.01802418255315611
368 0.018024193120965707
369 0.018024136305655844
370 0.018024028483583667
371 0.01802386704477864
372 0.018023687463467573
373 0.018023512145637827
374 0.018023338539233765
375 0.018023166051571903
376 0.01802299771199572
377 0.01802283374991245
378 0.01802267388897454
379 0.018022518133208425
380 0.018022366331344988
381 0.01802221829640486
382 0.018022074107481904
383 0.0180219338244188
384 0.018021797192075334
385 0.01802166396278377
386 0.01802153398398671
387 0.018021407217333446
388 0.018021283532318858
389 0.01802116274578585
390 0.0180210447747668
391 0.01802092978880553
392 0.018020818073099153
393 0.018020710120647303
394 0.01802060587989943
395 0.01802050568911185
396 0.01802040940525608
397 0.018020362571217762
398 0.018058358665848845
399 0.01820288969599144
400 0.018508734053154046
401 0.01902185322227995
402 0.019785663334390195
403 0.020837474184333883
404 0.022205148877807643
405 0.023902168670458475
406 0.025926029502024852
407 0.028252942496884793
408 0.0308436549444097
409 0.033646223098213336
410 0.03660456985161593
411 0.039661686346212824
412 0.04276841713611282
413 0.04588553130281394
414 0.04898366077302896
415 0.05204420228656094
416 0.05506144622917731
417 0.05801507313836217
418 0.06088857898398168
419 0.06367761631533624
420 0.06638287766212343
421 0.06900635713915379
422 0.07151657570977257
423 0.07384945229810884
424 0.07595516456614938
425 0.07780884004232043
426 0.07940662928200747
427 0.08075765457620557
428 0.0818794824056243
429 0.08279250317811275
430 0.08351797952715789
431 0.08407704498878352
432 0.08448906053905539
433 0.08477086747749597
434 0.08493903488092708
435 0.08500463082494525
436 0.08497669930062213
437 0.08486146190439836
438 0.08466087697827984
439 0.08437830857598708
440 0.08401572895687134
441 0.08357651295337269
442 0.08306403172412304
443 0.0824811420600927
444 0.08183256695714773
445 0.08112108633017151
446 0.08035155209646551
447 0.07952713127760526
448 0.07865257752719551
449 0.077733155091826
450 0.07677208106498112
451 0.07577238007042048
452 0.07473959516475659
453 0.0736766891683453
454 0.07258715794392534
455 0.07147412935809658
456 0.0703412913960016
457 0.06919155632206186
458 0.06802676303959329
459 0.06684723899075982
460 0.06565777902353512
461 0.06446142907732297
462 0.06326223149222321
463 0.06206371429969421
464 0.06086836928292116
465 0.059678565882104385
466 0.058494509375581163
467 0.05731953434160469
468 0.056154983144772165
469 0.055003460715408736
470 0.053866931141247215
471 0.052746860215366065
472 0.051644681304961984
473 0.050561532005760364
474 0.049498282356838605
475 0.04845606439208254
476 0.04743627312195241
477 0.04644010132858153
478 0.045468610834327364
479 0.04452285949076643
480 0.04360372338825091
481 0.042711752861029614
482 0.041847363905051456
483 0.041011031937214816
484 0.04020317117496324
485 0.03942319539286203
486 0.038670926247796056
487 0.03794667479361442
488 0.03725117044897228
489 0.036584301178372094
490 0.035945766538270314
491 0.035336251635412486
492 0.03475652254752285
493 0.03420695294321918
494 0.03368752097812564
495 0.03319790396232719
496 0.032737751333030383
497 0.03230669773384015
498 0.031904373151525854
499 0.0315303291919041
500 0.031183666486620052
501 0.03086315343482837
502 0.030567697920491764
503 0.030306874519797543
504 0.03009327570651041
505 0.029934889610936596
506 0.029837717408415867
507 0.02981085131072698
508 0.02987299133827989
509 0.030042969250205706
510 0.030332370600237885
511 0.030738107813922878
512 0.03124140008470327
513 0.03181675376251442
514 0.03243853312880252
515 0.0330808765575211
516 0.03372117301609122
517 0.034358264807331826
518 0.03499815095937289
519 0.0356060593262436
520 0.03617957001536669
521 0.036719051728281264
522 0.03722545767327713
523 0.03767842713271283
524 0.03809521927445863
525 0.03846107165516683
526 0.038741934294717506
527 0.03890609924045359
528 0.03899072165018017
529 0.03903258005366109
530 0.03905218718802029
531 0.03905701390466998
532 0.039006875568861385
533 0.038852555784309184
534 0.03856566484809989
535 0.03814078603119743
536 0.03757934265863481
537 0.03688327555073644
538 0.03608315335007132
539 0.03523047628235497
540 0.03436284125458838
541 0.0335026565397996
542 0.03266237827683635
543 0.03184690239240742
544 0.031055297573342897
545 0.0302840470610587
546 0.029528363301825185
547 0.02878345076194827
548 0.028045391962480997
549 0.027311227043024387
550 0.02657877509963515
551 0.02584899103645697
552 0.02512264624961802
553 0.02440027105373981
554 0.02368075453018957
555 0.022964475146826886
556 0.022252266701564313
557 0.021545340301567663
558 0.020844727886322387
559 0.02015045782391594
560 0.019461075255232742
561 0.018776633337560893
562 0.01810050643016689
563 0.01743022781059464
564 0.016766507039140136
565 0.016114397829430815
566 0.015477539239865955
567 0.014857195809388109
568 0.014252061588384808
569 0.013666747502569953
570 0.01309898729723938
571 0.012547719635074828
572 0.012014672035636515
573 0.01149752279303031
574 0.010997826812201596
575 0.010516852696164926
576 0.010054711533822997
577 0.009610796430169896
578 0.009189777551472432
579 0.00878868682122836
580 0.008404176250997366
581 0.00803591974048225
582 0.007684862292041738
583 0.007348800588866636
584 0.007028610086102387
585 0.006726409902587264
586 0.00643656887674217
587 0.0061620799076389345
588 0.00589890606287602
589 0.005648563120916154
590 0.005410411287397529
591 0.005185334948523808
592 0.004967435511046376
593 0.004763152736511011
594 0.004573435481708646
595 0.004393911575704492
596 0.0042278407132830455
597 0.0040721096040032675
598 0.003929801518612905
599 0.0037936358383998505
600 0.0036635223620768635
601 0.0035396376063531404
602 0.003425200251320114
603 0.0033157475936072944
604 0.0032134832967215367
605 0.003122095174446114
606 0.003038152826162261
607 0.00295576190003905
608 0.002875378200875523
609 0.002797422482870255
610 0.0027269809161962408
611 0.0026644137179953732
612 0.00260381763279355
613 0.0025448251006224597
614 0.002488040220654939
615 0.0024339288915918695
616 0.0023828228612099486
617 0.0023346646809028425
618 0.002289364550237755
619 0.00224682015785237
620 0.0022069771849000585
621 0.0021697529641584016
622 0.002134815641737805
623 0.002105269607855318
624 0.0020766745854777905
625 0.0020485726631475107
626 0.0020211666441511044
627 0.0019940221891585944
628 0.0019683650050241626
629 0.0019452261441868445
630 0.001924284292556301
631 0.001908875014957821
632 0.0018936318951912254
633 0.001877202112478803
634 0.0018625897594205126
635 0.0018478683679327187
636 0.0018381684717706992
637 0.0018303846841858887
638 0.0018207277070632494
639 0.0018152947427360964
640 0.0018059836231168048
641 0.0017933322252278521
642 0.0017823439005342342
643 0.0017726106347094484
644 0.0017630594903694356
645 0.0017548827237513815
646 0.0017438384421553275
647 0.0017344425827043864
648 0.0017273440224945594
649 0.0017201133348448278
650 0.0017171066797672073
651 0.0017185436729605153
652 0.0017191614273997262
653 0.0017170922341226843
654 0.00171454381456128
655 0.0017078679374299467
656 0.0017019425947280458
657 0.0016932004710277224
658 0.0016817713619346531
659 0.0016689518055030721
660 0.0016544287466863114
661 0.001641592129322277
662 0.0016301889549831432
663 0.0016190611120095917
664 0.0016077563417092597
665 0.001596534292309866
666 0.001586073224663355
667 0.001575727712961533
668 0.0015667107621984133
669 0.0015611499492165929
670 0.001557047067654736
671 0.0015523548489640745
672 0.0015455919098392513
673 0.0015399227293760958
674 0.0015336311695759838
675 0.0015287706838013938
676 0.0015312182491760166
677 0.0015321474546804677
678 0.0015349833572274472
679 0.0015345009660026323
680 0.0015357220752062867
681 0.0015324756195736443
682 0.001526284918968324
683 0.0015251650626479545
684 0.001525075855787513
685 0.0015283250047638352
686 0.0015313876828275444
687 0.0015313156947454705
688 0.001530305068067499
689 0.0015302988294621325
690 0.0015281947181626438
691 0.0015265436179747291
692 0.0015247150005197774
693 0.0015196858415235219
694 0.0015142764197370146
695 0.0015102440764676805
696 0.0015110332747991654
697 0.0015126414900364122
698 0.0015116051910963998
699 0.0015070442789750361
700 0.0014999343857586582


==> plotdata/satellite_constellation/sat_A1_dtheta.tex <==
t dtheta
0 -50.0
1 -49.99995660731687
2 -49.99980318557733
3 -49.99959153460236
4 -49.99939620381867
5 -49.99932476471908
6 -49.99947492158958
7 -49.99987177495112
8 -50.000511980222825
9 -50.00141172647155
10 -50.002767258028456
11 -50.00475130071639
12 -50.00743165041835
13 -50.01082510516981
14 -50.01495810666365
15 -50.019868718809356
16 -50.02559807363245
17 -50.03222624012841
18 -50.039841296035625
19 -50.04850048788499
20 -50.05821886399462
21 -50.06903509608669
22 -50.08100507825352
23 -50.09411246048438
24 -50.10829381794521
25 -50.123490300997155
26 -50.13957591418404
27 -50.1564623694161
28 -50.174076876543154
29 -50.192356467131795
30 -50.211285731842985
31 -50.23080190680939
32 -50.25076760343258
33 -50.271129852868015
34 -50.29185533286745
35 -50.31289256459605
36 -50.334184305814176
37 -50.355669881768506
38 -50.3772868195161
39 -50.39897312731934
40 -50.420733883425314
41 -50.442580913393314
42 -50.46440159371123
43 -50.48607797410853
44 -50.50754036568507
45 -50.528776820864834
46 -50.54979449735561
47 -50.57061371001569
48 -50.591306339272755
49 -50.61186203531733
50 -50.632293448018416
51 -50.6527306978561
52 -50.67333100396375
53 -50.69408058796121
54 -50.714997926402184
55 -50.73624370151711
56 -50.75787551823858
57 -50.77992369312228
58 -50.802448335080804
59 -50.8254659392409
60 -50.84900258261168
61 -50.87315317029663
62 -50.898007748425094
63 -50.9236290213794
64 -50.95005789431145
65 -50.977336691615164
66 -51.005572195182985
67 -51.034859997597856
68 -51.06525217895967
69 -51.09677157519701
70 -51.12941753643972
71 -51.16314991615525
72 -51.19792481860649
73 -51.23371223125059
74 -51.27048226183745
75 -51.308159677483374
76 -51.34663283917651
77 -51.38581079422896
78 -51.425612610705436
79 -51.465941684787886
80 -51.50671801902196
81 -51.547891667896565
82 -51.58937735098744
83 -51.6310422582076
84 -51.672795571586974
85 -51.71461888818733
86 -51.75644829523765
87 -51.79818182557769
88 -51.839753553864895
89 -51.88110995141282
90 -51.92220455788078
91 -51.96301209921796
92 -52.00353599570392
93 -52.04377989539568
94 -52.08377380894253
95 -52.12358365143669
96 -52.16323981983822
97 -52.20280553402478
98 -52.24239443857952
99 -52.28211570703623
100 -52.32206975726118
101 -52.36235465226418
102 -52.40306902142818
103 -52.44430407358726
104 -52.486144549636855
105 -52.52868268599401
106 -52.57201609331989
107 -52.616230354629494
108 -52.66139892732605
109 -52.707591429110664
110 -52.75486955746352
111 -52.803306276288694
112 -52.85291076059833
113 -52.903629985663095
114 -52.955419212291076
115 -53.0082323352588
116 -53.062034440043945
117 -53.116788541082656
118 -53.17244096237242
119 -53.22894410847268
120 -53.2862837999504
121 -53.34443930004336
122 -53.40335127775777
123 -53.462964241903165
124 -53.52322458843809
125 -53.58406304507394
126 -53.64538390455205
127 -53.70708288172271
128 -53.76908751221611
129 -53.831321488945775
130 -53.893686961545626
131 -53.956126827365274
132 -54.01859301057095
133 -54.08103526575498
134 -54.14339899682598
135 -54.20563997648018
136 -54.26772441936249
137 -54.329631045543834
138 -54.391349954414075
139 -54.452891804311164
140 -54.51425606579255
141 -54.57551454611832
142 -54.63677387175736
143 -54.69805237290888
144 -54.759379189672366
145 -54.82084111827286
146 -54.88245046915198
147 -54.94409826529084
148 -55.00576118221697
149 -55.06747234965132
150 -55.12923255063035
151 -55.19105421717593
152 -55.252973334244544
153 -55.31501397521844
154 -55.377162024238004
155 -55.43941965378778
156 -55.501787641498005
157 -55.56426781469965
158 -55.62686344539672
159 -55.68954975047877
160 -55.75232112760359
161 -55.815179314783805
162 -55.87811269322235
163 -55.941098460347575
164 -56.00411486991632
165 -56.06714934673636
166 -56.13018799904008
167 -56.19321689474836
168 -56.25622294604274
169 -56.31919259194572
170 -56.38211265256072
171 -56.444968538280996
172 -56.507743937045305
173 -56.57042367166787
174 -56.632994094401376
175 -56.69544459469007
176 -56.75777137766975
177 -56.81997247022544
178 -56.88204490198899
179 -56.943985754138396
180 -57.00579487813799
181 -57.06747223728428
182 -57.129019536851445
183 -57.19044202861392
184 -57.25175447339001
185 -57.31295860594848
186 -57.374054182260686
187 -57.435058087247796
188 -57.49598423161113
189 -57.5568492983678
190 -57.61767131801858
191 -57.678476550118155
192 -57.73926900243148
193 -57.80005425033166
194 -57.86086503825042
195 -57.92176163967547
196 -57.982773202088886
197 -58.04388808444292
198 -58.105081223481406
199 -58.1663915766653
200 -58.22786201152036
201 -58.28946376376021
202 -58.35118322195224
203 -58.413033215505266
204 -58.47503526309636
205 -58.5371895506289
206 -58.59949399562773
207 -58.66194327881657
208 -58.72452946354715
209 -58.78724237556966
210 -58.85006996588916
211 -58.91299858307358
212 -58.97601292731428
213 -59.03909629245865
214 -59.102232250324164
215 -59.165400793997094
216 -59.22858187963099
217 -59.29175811440786
218 -59.35491073749913
219 -59.418022549931884
220 -59.481074842647395
221 -59.54405046792783
222 -59.606936165182134
223 -59.66971787015709
224 -59.73238416123678
225 -59.79492638370953
226 -59.85736854330674
227 -59.919697295934824
228 -59.98186889183302
229 -60.04388845751321
230 -60.105760456239324
231 -60.16748541079299
232 -60.229064350882894
233 -60.29051921322724
234 -60.35187135950075
235 -60.41313037802665
236 -60.474304234728166
237 -60.5353766621789
238 -60.59635831180977
239 -60.657304572060895
240 -60.71827712915726
241 -60.77929933739649
242 -60.84039256296632
243 -60.90160745250372
244 -60.96296080867692
245 -61.02445083124067
246 -61.08608508294661
247 -61.14785777697446
248 -61.209772066684295
249 -61.271835032511945
250 -61.33404738874098
251 -61.39640585728473
252 -61.45891204830303
253 -61.521576970902494
254 -61.58439213739243
255 -61.64733056981297
256 -61.7103849911865
257 -61.77359527652665
258 -61.836952722465064
259 -61.90031604675613
260 -61.963619113917595
261 -62.026839162526144
262 -62.089885766442315
263 -62.15271805218589
264 -62.21530992879336
265 -62.277631438894375
266 -62.339665443037696
267 -62.40139796715374
268 -62.462878021525704
269 -62.52416541996129
270 -62.58527394764157
271 -62.646219074715304
272 -62.70701979356769
273 -62.767694024756324
274 -62.82826449260489
275 -62.88875541723656
276 -62.949179782476335
277 -63.00955434050297
278 -63.069900657401625
279 -63.13023323994295
280 -63.190564291517305
281 -63.250910998467376
282 -63.31128850155819
283 -63.37171013142568
284 -63.43219116360408
285 -63.49274364880166
286 -63.55341359231109
287 -63.614208935224866
288 -63.67513320918938
289 -63.736236677652826
290 -63.797542157945024
291 -63.85907099136478
292 -63.920850682720406
293 -63.982837059421804
294 -64.04496473896903
295 -64.10723274534358
296 -64.16968146217873
297 -64.23237702107699
298 -64.29525592866615
299 -64.3582668757911
300 -64.42138586084874
301 -64.48451613854058
302 -64.54762627099235
303 -64.61069523040999
304 -64.67366253848253
305 -64.73649148697767
306 -64.79924981884932
307 -64.861983058038
308 -64.9246701167448
309 -64.98732436383416
310 -65.04999210941092
311 -65.11270680157513
312 -65.17547974201311
313 -65.23832144537522
314 -65.30124430341193
315 -65.36426693494174
316 -65.4274134835945
317 -65.49066577375272
318 -65.55398278132668
319 -65.61737336486891
320 -65.68080149231248
321 -65.74420494816957
322 -65.80750052677294
323 -65.87054792049423
324 -65.93326539150081
325 -65.99565145182726
326 -66.05775998698951
327 -66.11964372845297
328 -66.18135990630518
329 -66.24296213957373
330 -66.30448333709055
331 -66.36595033882271
332 -66.42737826542849
333 -66.4887829781254
334 -66.55018496400831
335 -66.61160466268623
336 -66.67305908728346
337 -66.7345676006684
338 -66.79614878925393
339 -66.8578192912432
340 -66.91959858411695
341 -66.98150340275092
342 -67.04354642417448
343 -67.10572364892309
344 -67.16803811781342
345 -67.23048638315677
346 -67.29302954676653
347 -67.35564246911268
348 -67.4183222475467
349 -67.48103252139875
350 -67.54373603761124
351 -67.60640469880587
352 -67.66902967979814
353 -67.7316122705974
354 -67.79412549348886
355 -67.85657753475172
356 -67.918984528328
357 -67.9813448638775
358 -68.04365915509808
359 -68.10593095323527
360 -68.1681716499636
361 -68.23038508522569
362 -68.2925703230607
363 -68.35473410158846
364 -68.41688417762752
365 -68.47902672775324
366 -68.54116555711482
367 -68.60330156378167
368 -68.66543353242484
369 -68.72756313271239
370 -68.78966356898877
371 -68.85167875988796
372 -68.91358190755803
373 -68.97536535313333
374 -69.03701815753521
375 -69.09854467176532
376 -69.1599487366599
377 -69.22118863932059
378 -69.2822372583599
379 -69.34311659285119
380 -69.4038409726823
381 -69.46442003134605
382 -69.52485778858642
383 -69.58516609472187
384 -69.64538403039273
385 -69.70556486065378
386 -69.76576151664288
387 -69.82602550550303
388 -69.88637005184215
389 -69.94679603874224
390 -70.00730584196181
391 -70.06793185057045
392 -70.12868844860219
393 -70.1895784401175
394 -70.25062174825214
395 -70.31183438763128
396 -70.37322875221756
397 -70.43480899943911
398 -70.49657477457278
399 -70.55852144300589
400 -70.62064056850494
401 -70.68294159970827
402 -70.74542781649183
403 -70.80805938920352
404 -70.87078930350366
405 -70.93360159825906
406 -70.99646912295589
407 -71.05932327767154
408 -71.12213126617655
409 -71.18489902592677
410 -71.24761644824899
411 -71.3102734984018
412 -71.37285390273613
413 -71.43535176599278
414 -71.49777524784704
415 -71.56013105922453
416 -71.62241094602422
417 -71.68462287479608
418 -71.74678203768414
419 -71.80890462817004
420 -71.87101254563784
421 -71.93312132349891
422 -71.99523262291552
423 -72.05735901313977
424 -72.11951756145511
425 -72.18169986103001
426 -72.24387292409294
427 -72.3060089631646
428 -72.36809503359302
429 -72.43013940647528
430 -72.4921585495421
431 -72.55416470813375
432 -72.61615929817091
433 -72.67813914672816
434 -72.74010909212429
435 -72.80207480295496
436 -72.86403874440428
437 -72.92601696747437
438 -72.98802905165782
439 -73.05007151379147
440 -73.1121278293498
441 -73.17419012719095
442 -73.23625136743019
443 -73.29831481181151
444 -73.36039067469292
445 -73.42248465488096
446 -73.4846034106654
447 -73.54675330343287
448 -73.60893980760335
449 -73.67116785138289
450 -73.73346157756274
451 -73.79580404123494
452 -73.85816591488033
453 -73.92053627465191
454 -73.98292269660894
455 -74.04535420719733
456 -74.10779614585786
457 -74.17023503444074
458 -74.2326688758023
459 -74.29507882284796
460 -74.35743754176822
461 -74.41973332218417
462 -74.48195257733697
463 -74.54408644900585
464 -74.60613028092267
465 -74.66811392878755
466 -74.73006239867217
467 -74.79196153571633
468 -74.85378886425848
469 -74.91551778092528
470 -74.97714263765457
471 -75.03869530411677
472 -75.10020441714242
473 -75.16163567758586
474 -75.22298831927559
475 -75.28428725724883
476 -75.3454965852795
477 -75.40663574600657
478 -75.46773255575886
479 -75.52876854100884
480 -75.58979091441137
481 -75.65084372955353
482 -75.71193750797522
483 -75.77305227270999
484 -75.83419482759555
485 -75.89538020011909
486 -75.95661356573699
487 -76.0179134357066
488 -76.07932802050897
489 -76.14088665991974
490 -76.20260544879218
491 -76.26449311556657
492 -76.32655564979672
493 -76.38880786241607
494 -76.45125577863651
495 -76.5139011665712
496 -76.57674107467844
497 -76.63977219591172
498 -76.70298584416622
499 -76.7663651967133
500 -76.8298745316822
501 -76.89345502311637
502 -76.95705394680962
503 -77.02062341921383
504 -77.08409899903427
505 -77.14743901712971
506 -77.21062591046297
507 -77.27365821333267
508 -77.33655806934388
509 -77.39933910669771
510 -77.46200128025777
511 -77.5245483875636
512 -77.5869828905017
513 -77.64929536455833
514 -77.71148765035717
515 -77.77356535391037
516 -77.83551825715845
517 -77.89734032423226
518 -77.95903888224389
519 -78.02067815462993
520 -78.08223225506002
521 -78.14366444477504
522 -78.20504470348507
523 -78.26640644062402
524 -78.32777288499123
525 -78.38916693315171
526 -78.45063455024885
527 -78.51220360820983
528 -78.57387600153787
529 -78.63565187032314
530 -78.6975308201394
531 -78.75948386705208
532 -78.82149389378773
533 -78.88358526875685
534 -78.94575296709179
535 -79.00800211321514
536 -79.07034716081637
537 -79.13280613333534
538 -79.19538056922089
539 -79.25807131902152
540 -79.32085920425187
541 -79.38369118972096
542 -79.44656089086088
543 -79.5094565322514
544 -79.57236308271854
545 -79.63526944302656
546 -79.6981665789069
547 -79.76104569078642
548 -79.82389310104477
549 -79.8866848910762
550 -79.94939635897624
551 -80.01200173552735
552 -80.07448832206133
553 -80.13685560733715
554 -80.1991077264708
555 -80.2612553785258
556 -80.32330307631698
557 -80.38525673564835
558 -80.44712362344885
559 -80.50891298036461
560 -80.57063496417659
561 -80.63229849940602
562 -80.6939132183496
563 -80.75549391621006
564 -80.81708625350261
565 -80.87875195365307
566 -80.94053436483179
567 -81.00247274142227
568 -81.0646083390883
569 -81.12688456990908
570 -81.18922269553227
571 -81.25162711970847
572 -81.31410124194646
573 -81.37664766731368
574 -81.43926874375849
575 -81.50195999247693
576 -81.56474720110182
577 -81.62764713715025
578 -81.69058110744778
579 -81.7535383150085
580 -81.81655373504856
581 -81.87962871483668
582 -81.94276632925376
583 -82.00593574493891
584 -82.06910888685402
585 -82.13225986854336
586 -82.19539208890254
587 -82.25850961063388
588 -82.3215984145754
589 -82.38465913610686
590 -82.44769088043574
591 -82.51070007178255
592 -82.57369139843838
593 -82.63668210616336
594 -82.69968190470463
595 -82.76267953099526
596 -82.82566127413196
597 -82.88861232894843
598 -82.95151752427984
599 -83.0143213513573
600 -83.07695995174117
601 -83.1394172352193
602 -83.20168916523562
603 -83.26378549472118
604 -83.32570740193499
605 -83.3874496436701
606 -83.44900720051409
607 -83.51044942100852
608 -83.57186716642526
609 -83.63325593749003
610 -83.69460420780342
611 -83.75589608020121
612 -83.81716022071639
613 -83.8784125000461
614 -83.93970612576837
615 -84.00102188905257
616 -84.06239784858252
617 -84.12385937955912
618 -84.18544835328352
619 -84.24723592507128
620 -84.3092488852379
621 -84.37148054502295
622 -84.43386423868287
623 -84.49644480386145
624 -84.55919717617971
625 -84.62209345785813
626 -84.6850902721675
627 -84.74817142649252
628 -84.81130258283942
629 -84.8743901513448
630 -84.93739829045869
631 -85.00025397663879
632 -85.06289315484591
633 -85.1252922125004
634 -85.18741599759164
635 -85.24930482823937
636 -85.3110063024571
637 -85.37249814924414
638 -85.43377671809311
639 -85.49491124137157
640 -85.55596617024176
641 -85.61706161025361
642 -85.67819650677468
643 -85.73941224702506
644 -85.80078717372336
645 -85.86229257604136
646 -85.92404240131232
647 -85.98611842639815
648 -86.04850103039944
649 -86.11114000710695
650 -86.17398369507127
651 -86.23699199606145
652 -86.30010834665497
653 -86.36320541211383
654 -86.42614031669854
655 -86.48880032151479
656 -86.5510834399282
657 -86.61289923448652
658 -86.67417310242887
659 -86.73480596485987
660 -86.79468830257717
661 -86.8537313089223
662 -86.91185214887778
663 -86.96899069566808
664 -87.02509590823533
665 -87.08012549658753
666 -87.13405106634463
667 -87.186865563233
668 -87.23856249446402
669 -87.28913986399854
670 -87.33863247887516
671 -87.38708022964609
672 -87.4345091103747
673 -87.48095618476881
674 -87.52647922029718
675 -87.57114964866953
676 -87.61504985607249
677 -87.6582538895457
678 -87.70084036750582
679 -87.74290409735818
680 -87.78454389175488
681 -87.82585785084923
682 -87.86694432210389
683 -87.90789527124302
684 -87.94879941563258
685 -87.98973780077341
686 -88.03077642772382
687 -88.07197039504359
688 -88.11336422927202
689 -88.15499180618052
690 -88.1968708410275
691 -88.23896950458536
692 -88.28121262860708
693 -88.3235482088289
694 -88.36590139541347
695 -88.40818981020003
696 -88.45036850813344
697 -88.49235655183988
698 -88.53405516344348
699 -88.57537148773794
700 -88.616214348897
701 -88.65647339432054
702 -88.69603790815468
703 -88.73483163155416
704 -88.77282885365834
705 -88.80998722606945
706 -88.84625790174928
707 -88.88159494694925
708 -88.91598305094443
709 -88.9494757377236
710 -88.98209975287051
711 -89.01386884462376
712 -89.04479806644504
713 -89.07487744205571
714 -89.1040708146162
715 -89.13235763804617
716 -89.15976415221935
717 -89.18632753548597
718 -89.21209199029653
719 -89.23711178065524
720 -89.261448179649
721 -89.28516776449588
722 -89.3083288598913
723 -89.33097691397538
724 -89.35315856955786
725 -89.37491933471946
726 -89.39630340100902
727 -89.41735229902949
728 -89.43810427734536
729 -89.45859422398914
730 -89.47885166973911
731 -89.49890010442363
732 -89.51876132325192
733 -89.53845842381882
734 -89.55801797433224
735 -89.57744846862415
736 -89.59676505776521
737 -89.61599304117992
738 -89.6351647558928
739 -89.65428698606668
740 -89.673335228657
741 -89.69229099931565
742 -89.7111335732568
743 -89.72981835267151
744 -89.7482858496155
745 -89.76646261098249
746 -89.78430480247495
747 -89.80176358894884
748 -89.81879853796848
749 -89.83537457771105
750 -89.85143889958034
751 -89.86694730751508
752 -89.88187124301331
753 -89.89618422537154
754 -89.90984849023417
755 -89.92282983979362
756 -89.93509893523178
757 -89.94663251073314
758 -89.95743095417431
759 -89.96748349444618
760 -89.97676206383376
761 -89.98525466456664
762 -89.99296013122445
763 -89.99988517540818
764 -90.00604255354529
765 -90.0114523276074
766 -90.0161397457263
767 -90.0201307249595
768 -90.02345688516803
769 -90.02615328128284
770 -90.02825856202267
771 -90.02984314573125
772 -90.03096771007205
773 -90.03170099805048
774 -90.03207877270357
775 -90.03213552863583
776 -90.03192744679716
777 -90.03148056424261
778 -90.03083444144454
779 -90.0300207006407
780 -90.02906567465722
781 -90.02799067873738
782 -90.02681186292406
783 -90.02553950598264
784 -90.02418145689265
785 -90.02271557127553
786 -90.02111858023311
787 -90.01934495283928
788 -90.017306086215
789 -90.01494156703643
790 -90.01223627371999
791 -90.00917879488983
792 -90.00575006011431
793 -90.00193448691704
794 -89.99769513362581
795 -89.9929976337979
796 -89.98780891878636
797 -89.98209015219017
798 -89.97581726331993
799 -89.96897147467013
800 -89.96152337978687
801 -89.95345009601611
802 -89.94474150401552
803 -89.93539276322961
804 -89.92540133537749
805 -89.9147727395962
806 -89.90349712943318
807 -89.89156826626571
808 -89.87900027137553
809 -89.86579949665014
810 -89.85196728950805
811 -89.83751058296899
812 -89.82243852020616
813 -89.80676215831197
814 -89.79050183683039
815 -89.77368749828932
816 -89.75635033503605
817 -89.73853189779052
818 -89.72027904170997
819 -89.70163462632411
820 -89.68270123068139
821 -89.66355590447358
822 -89.64422947027471
823 -89.62472711061268
824 -89.60503704504761
825 -89.58519868228004
826 -89.56522985156437
827 -89.54515045757107
828 -89.52497400334798
829 -89.50470503149093
830 -89.48434286978802
831 -89.46388483655836
832 -89.4433213224476
833 -89.42263586276245
834 -89.40180692853367
835 -89.38080873394335
836 -89.35961167624166
837 -89.33818268393348
838 -89.31648455946107
839 -89.29447593371752
840 -89.27211439174242
841 -89.2493552474203
842 -89.22615188372293
843 -89.20246081581034
844 -89.17824119780525
845 -89.15345269253022
846 -89.12805772286815
847 -89.1020240068579
848 -89.075323914336
849 -89.04793628359616
850 -89.01984284407808
851 -88.9910279231352
852 -88.96148887468526
853 -88.93121530867498
854 -88.90021180632446
855 -88.86848503647583
856 -88.83603774564399
857 -88.80288952053596
858 -88.76905555965241
859 -88.73455711403933
860 -88.69942134303224
861 -88.66368217011431
862 -88.62738371588554
863 -88.59055106828279
864 -88.55321339071551
865 -88.51541490348355
866 -88.47719791806297
867 -88.43860754058235
868 -88.39967270335787
869 -88.36042102631089
870 -88.32088285429676
871 -88.28108936201532
872 -88.24106517830435
873 -88.2008302817779
874 -88.16039995034117
875 -88.11979041807699
876 -88.0789938175897
877 -88.03798640457728
878 -87.99676568836396
879 -87.95530564677863
880 -87.91357567027538
881 -87.87154076415861
882 -87.82916245348082
883 -87.78640281550965
884 -87.74322597156983
885 -87.69960101583068
886 -87.65550636457384
887 -87.61093641114968
888 -87.56587851396698
889 -87.52030239976415
890 -87.47418881684743
891 -87.42752762827509
892 -87.38031703574502
893 -87.332552341088
894 -87.28419813201188
895 -87.23522436536962
896 -87.185612557287
897 -87.13535644579268
898 -87.08444950164211
899 -87.03288198979268
900 -86.98065359533673
901 -86.92777052522777
902 -86.87423814222906
903 -86.8200666055709
904 -86.76527598107371
905 -86.7098927375615
906 -86.65394980406984
907 -86.59748638562083
908 -86.54054722932162
909 -86.48318130711533
910 -86.42543934833574
911 -86.3673714706031
912 -86.30902518762714
913 -86.25044373183415
914 -86.1916645316236
915 -86.13271872489085
916 -86.07363172796313
917 -86.01442292869899
918 -85.95510526018434
919 -85.89568501467876
920 -85.83612669771554
921 -85.77634633852217
922 -85.71627169588612
923 -85.65597949631815
924 -85.59565085893318
925 -85.53537819683538
926 -85.47520521540734
927 -85.41516281896529
928 -85.35525154923066
929 -85.29547508893934
930 -85.23581501096997
931 -85.17625675227492
932 -85.11671013988158
933 -85.05709065777367
934 -84.99736296076395
935 -84.93747535285718
936 -84.87739349327488
937 -84.81706803708947
938 -84.75647291156908
939 -84.69559855647725
940 -84.6344424400485
941 -84.5730002367244
942 -84.51127557635546
943 -84.44927486867392
944 -84.38702825529315
945 -84.3245262075929
946 -84.26177088419051
947 -84.19879322720574
948 -84.13563864862722
949 -84.07231786856123
950 -84.00879657040682
951 -83.94514561671794
952 -83.8813994400342
953 -83.81755914179851
954 -83.75363828985532
955 -83.68961860063631
956 -83.62557443566708
957 -83.56159105860861
958 -83.497655530068
959 -83.433772898724
960 -83.3699465631832
961 -83.30617681760204
962 -83.2424655461529
963 -83.17881653358961
964 -83.1152320412037
965 -83.05171437647914
966 -82.98826895367466
967 -82.92490139155228
968 -82.86161552592323
969 -82.79841639803973
970 -82.73530767620316
971 -82.67229301001053
972 -82.60935096857052
973 -82.54649484297435
974 -82.48377002179119
975 -82.42118831693304
976 -82.35876169929043
977 -82.29647331135436
978 -82.2343243697598
979 -82.17233964882159
980 -82.110513422105
981 -82.04879798476816
982 -81.9871319107799
983 -81.92547773932492
984 -81.86378477082356
985 -81.80200226967493
986 -81.74009828779454
987 -81.67804911467788
988 -81.61583953801507
989 -81.5534625250385
990 -81.49091867198177
991 -81.42821552991528
992 -81.3653669970109
993 -81.30239135691181
994 -81.23931050971295
995 -81.17615027853174
996 -81.11293691134993
997 -81.04969726762998
998 -80.98645926803269
999 -80.92324734032373
1000 -80.86008636322072
1001 -80.79700095998076
1002 -80.73401182078283
1003 -80.67113818764193
1004 -80.60839790433415
1005 -80.54580548899793
1006 -80.48336925104556
1007 -80.42109298250105
1008 -80.35898155011424
1009 -80.29703731809104
1010 -80.23526016281954
1011 -80.17364839855406
1012 -80.11219755713249
1013 -80.05089898021906
1014 -79.98973937627476
1015 -79.92870400596797
1016 -79.86777431846855
1017 -79.8069339569473
1018 -79.74616546458067
1019 -79.68544514624318
1020 -79.62474265386169
1021 -79.56402512421175
1022 -79.50326623977381
1023 -79.44244492028656
1024 -79.38151514243457
1025 -79.32041608855862
1026 -79.25911967120132
1027 -79.19765280414676
1028 -79.13600736504684
1029 -79.07419474600074
1030 -79.01224823321634
1031 -78.95015707901374
1032 -78.88790505188067
1033 -78.8254598537474
1034 -78.76283740538656
1035 -78.70005698474645
1036 -78.63712013609029
1037 -78.57403964663126
1038 -78.51082775382636
1039 -78.4475004238606
1040 -78.38406928261584
1041 -78.32055282509589
1042 -78.25697271703652
1043 -78.19334424239426
1044 -78.12968855305914
1045 -78.06601794544433
1046 -78.0023551928262
1047 -77.93872151243117
1048 -77.87512182525741
1049 -77.81157822237235
1050 -77.74814302277645
1051 -77.68487176458316
1052 -77.62178719347973
1053 -77.55889980250953
1054 -77.4962133329933
1055 -77.43372821671302
1056 -77.37144103419192
1057 -77.30934383954828
1058 -77.24743128407307
1059 -77.18569825845489
1060 -77.12414494718993
1061 -77.06275685495753
1062 -77.00150938602451
1063 -76.94038863587787
1064 -76.87939078106461
1065 -76.81850229667994
1066 -76.75768390292357
1067 -76.69691241279347
1068 -76.63617184314597
1069 -76.57543997292967
1070 -76.51466914594918
1071 -76.45378114194571
1072 -76.39276595520077
1073 -76.33163580293959
1074 -76.27036995606669
1075 -76.20896590630933
1076 -76.1474121590236
1077 -76.08570540029666
1078 -76.02384536048098
1079 -75.96181067421544
1080 -75.89958689330658
1081 -75.83715126083574
1082 -75.7745442852658
1083 -75.7117971389606
1084 -75.6489204245138
1085 -75.58590790556464
1086 -75.5227829672854
1087 -75.45956899016338
1088 -75.39629217094294
1089 -75.33297714778637
1090 -75.2696028362033
1091 -75.20617936457313
1092 -75.14276577355133
1093 -75.0793964224741
1094 -75.01609117180375
1095 -74.9528634701378
1096 -74.8897224189996
1097 -74.82666201325111
1098 -74.76369475835703
1099 -74.7008538924422
1100 -74.63815691400855
1101 -74.57562732126522
1102 -74.51326054068001
1103 -74.4510544732098
1104 -74.38901772051071
1105 -74.32713015616301
1106 -74.26537361538848
1107 -74.20375027079525
1108 -74.14224955058677
1109 -74.08084632680715
1110 -74.01952369374712
1111 -73.95829304008448
1112 -73.8971486810792
1113 -73.83607185092208
1114 -73.77503935632365
1115 -73.71401906679081
1116 -73.65297709491863
1117 -73.59190291655392
1118 -73.53076378965453
1119 -73.4695240821999
1120 -73.40818045794308
1121 -73.34673719365676
1122 -73.2851585018724
1123 -73.22342848498039
1124 -73.16156105102257
1125 -73.09952931932929
1126 -73.03732086295128
1127 -72.97494249806168
1128 -72.91240880729343
1129 -72.8497145654192
1130 -72.78688595385647
1131 -72.72396588172022
1132 -72.66099815782124
1133 -72.59803135931325
1134 -72.53510012636738
1135 -72.47223167053035
1136 -72.40944468246843
1137 -72.34674853330849
1138 -72.28416209800454
1139 -72.22170890199169
1140 -72.1594034152243
1141 -72.09722960318298
1142 -72.03514661977306
1143 -71.97311558098431
1144 -71.9110950955207
1145 -71.84904542668615
1146 -71.78695225937828
1147 -71.72483413192732
1148 -71.66269885002716
1149 -71.60056169442468
1150 -71.53846611892335
1151 -71.47647649525973
1152 -71.4146292031007
1153 -71.35295053889212
1154 -71.29145215561313
1155 -71.23013009612364
1156 -71.16897460784355
1157 -71.10797272897746
1158 -71.04711037539657
1159 -70.9863671801844
1160 -70.92572054881727
1161 -70.86514460254195
1162 -70.80461378406329
1163 -70.74410640989551
1164 -70.6835997157969
1165 -70.6230669871518
1166 -70.56248436067025
1167 -70.5018295319196
1168 -70.44108608901946
1169 -70.38025124117347
1170 -70.31930598330514
1171 -70.25822317219404
1172 -70.19699065820512
1173 -70.13559901503007
1174 -70.07404177981272
1175 -70.01231576353209
1176 -69.95042098040614
1177 -69.88836074853769
1178 -69.82614131363157
1179 -69.76377165164335
1180 -69.70126350817648
1181 -69.63863151795455
1182 -69.57589232553653
1183 -69.51306250292116
1184 -69.45016160794232
1185 -69.38721181186666
1186 -69.32423518643031
1187 -69.26125515047043
1188 -69.1982950299556
1189 -69.13537569423268
1190 -69.0725163215208
1191 -69.00973543261837
1192 -68.9470501263176
1193 -68.88447522739297
1194 -68.82202226856624
1195 -68.7597013475923
1196 -68.69752240389892
1197 -68.63549149399175
1198 -68.57360768895587
1199 -68.51186842411575
1200 -68.45027852013132
1201 -68.38883344567643
1202 -68.32751602799654
1203 -68.2663181299296
1204 -68.2052299833976
1205 -68.14423431766579
1206 -68.08331623269795
1207 -68.02246068334233
1208 -67.96164951281638
1209 -67.90086139590666
1210 -67.84007926467994
1211 -67.77928362791874
1212 -67.7184451149713
1213 -67.65754661400642
1214 -67.59657488211204
1215 -67.5355117260529
1216 -67.47434532495242
1217 -67.41306395196196
1218 -67.3516560425106
1219 -67.29011352513915
1220 -67.22843227312461
1221 -67.16661145152956
1222 -67.10465331731386
1223 -67.04255893461031
1224 -66.98032989611855
1225 -66.91797453765123
1226 -66.85551176703743
1227 -66.79294347547707
1228 -66.73027235618856
1229 -66.66752557411093
1230 -66.60471696629399
1231 -66.54185565544552
1232 -66.47895891354277
1233 -66.41604419411334
1234 -66.35312442407464
1235 -66.29022234780949
1236 -66.22735846786101
1237 -66.16453918951822
1238 -66.1017795389941
1239 -66.03909771003032
1240 -65.97650950601636
1241 -65.91402620591523
1242 -65.85165370803902
1243 -65.78939805791606
1244 -65.72726372576841
1245 -65.66525444159264
1246 -65.60337005285403
1247 -65.54160652950219
1248 -65.47995961867484
1249 -65.41842297310767
1250 -65.35699103192172
1251 -65.29565864511561
1252 -65.23441133995358
1253 -65.17323160103695
1254 -65.11209429764634
1255 -65.05099713205054
1256 -64.98993204560621
1257 -64.92887316456758
1258 -64.86781245360245
1259 -64.8067242492721
1260 -64.74559138087544
1261 -64.68440593044387
1262 -64.62315541237325
1263 -64.5618247991625
1264 -64.50039730415627
1265 -64.43886281709976
1266 -64.37720921417855
1267 -64.31543372072112
1268 -64.25353547589941
1269 -64.19150865553134
1270 -64.12935324343833
1271 -64.06707148541237
1272 -64.00465051611569
1273 -63.94211823725887
1274 -63.87948553492001
1275 -63.81676479240932
1276 -63.75399075499774
1277 -63.6911502524262
1278 -63.62826938135656
1279 -63.56536701604749
1280 -63.502463155914775
1281 -63.439587758901965
1282 -63.37674938303107
1283 -63.313967556210024
1284 -63.25125203337694
1285 -63.18861873312556
1286 -63.12609252508842
1287 -63.06368725023016
1288 -63.00141349598202
1289 -62.939280986086
1290 -62.87729348292679
1291 -62.81545117457338
1292 -62.75375310837627
1293 -62.69219588418511
1294 -62.63077299274284
1295 -62.56947449237117
1296 -62.508286297804666
1297 -62.447193537856634
1298 -62.386182174266665
1299 -62.325236548233214
1300 -62.26433971360134
1301 -62.203475358644866
1302 -62.14262658955683
1303 -62.0817755261052
1304 -62.02090449550866
1305 -61.959993530409
1306 -61.899024987538844
1307 -61.83798577026273
1308 -61.77686364376825
1309 -61.71564611024929
1310 -61.654321681759725
1311 -61.59289851532211
1312 -61.53137021128833
1313 -61.469704888247236
1314 -61.40790151347385
1315 -61.34596115705618
1316 -61.28387544200147
1317 -61.22164901693922
1318 -61.159288469337405
1319 -61.09679671635151
1320 -61.03417587055381
1321 -60.971435240050376
1322 -60.908586978039274
1323 -60.845644441899154
1324 -60.782622420985774
1325 -60.71953776965542
1326 -60.656408623696734
1327 -60.593253306612354
1328 -60.53008562376423
1329 -60.46692308002645
1330 -60.40379205733979
1331 -60.340712319041266
1332 -60.27769978360084
1333 -60.21477731498942
1334 -60.151961948400356
1335 -60.08927104196864
1336 -60.026709071480724
1337 -59.96429422866719
1338 -59.902045377838554
1339 -59.839953751927844
1340 -59.778019039495135
1341 -59.71623504361731
1342 -59.65459806001744
1343 -59.59309814185833
1344 -59.53172300826215
1345 -59.470468415554315
1346 -59.40931698642818
1347 -59.348246557907515
1348 -59.28723934457318
1349 -59.22627469035075
1350 -59.16530905430523
1351 -59.10434096682781
1352 -59.043388645266106
1353 -58.982385408294
1354 -58.92132358501857
1355 -58.86023458188432
1356 -58.79907944441667
1357 -58.73783225931656
1358 -58.67648216233194
1359 -58.61501521319566
1360 -58.55341445335055
1361 -58.49167266953228
1362 -58.42980350682484
1363 -58.36780641503563
1364 -58.30567246794333
1365 -58.24340450685051
1366 -58.18100780057308
1367 -58.118489828837646
1368 -58.055860024871805
1369 -57.99313035399677
1370 -57.93031505651562
1371 -57.86742959181553
1372 -57.804490584292076
1373 -57.74151543620293
1374 -57.6785219637953
1375 -57.615528154548905
1376 -57.55256970417927
1377 -57.48967158566651
1378 -57.426829207923795
1379 -57.36402126975072
1380 -57.30125950753044
1381 -57.238553581728496
1382 -57.17588755658898
1383 -57.11330757642239
1384 -57.05082747461784
1385 -56.98842616602058
1386 -56.926109372401456
1387 -56.863886399212205
1388 -56.801790816619
1389 -56.73982433650731
1390 -56.67795864024256
1391 -56.61619718093045
1392 -56.55453671564039
1393 -56.4929571613067
1394 -56.431448127767844
1395 -56.370001817902065
1396 -56.308606578003925
1397 -56.24724967713602
1398 -56.18591019305965
1399 -56.12456733834521
1400 -56.06319362501111
1401 -56.00172194225845
1402 -55.94011540037377
1403 -55.878377201925076
1404 -55.81649522082301
1405 -55.75446362242601
1406 -55.692279152804964
1407 -55.62994362260233
1408 -55.56746446088711
1409 -55.5048528014058
1410 -55.44212195105203
1411 -55.37928815036782
1412 -55.316386115264855
1413 -55.253407108792615
1414 -55.190357298650156
1415 -55.127254109036805
1416 -55.06409431627506
1417 -55.00089921215944
1418 -54.937683798963135
1419 -54.874445225479384
1420 -54.81123215962485
1421 -54.74811254527783
1422 -54.68511323217896
1423 -54.622261334746426
1424 -54.55956805826592
1425 -54.49704011096428
1426 -54.434687312661715
1427 -54.37253601300372
1428 -54.31058503209468
1429 -54.24881908116111
1430 -54.18723277275661
1431 -54.125816684373625
1432 -54.064558548790465
1433 -54.00341722623072
1434 -53.942410952559044
1435 -53.88153479980917
1436 -53.820744529759395
1437 -53.76002120373144
1438 -53.69933665732227
1439 -53.63867680258929
1440 -53.578014072613705
1441 -53.51727965363338
1442 -53.456432467099795
1443 -53.39549040372075
1444 -53.33453199558905
1445 -53.27363544578506
1446 -53.21276126168556
1447 -53.15187559477605
1448 -53.09100005505392
1449 -53.03013278003029
1450 -52.96920781593365
1451 -52.90821793773415
1452 -52.84721043458726
1453 -52.7861694764296
1454 -52.72504675899396
1455 -52.6637925469284
1456 -52.60238136522957
1457 -52.540794845078494
1458 -52.4790191233067
1459 -52.417063554701265
1460 -52.35490712175137
1461 -52.29251774803807
1462 -52.22991106818706
1463 -52.167118754916224
1464 -52.10418297308629
1465 -52.04114543412917
1466 -51.97802365482773
1467 -51.91484044617796
1468 -51.85163075150051
1469 -51.78842329133645
1470 -51.725250335067194
1471 -51.662139648035804
1472 -51.59910271088156
1473 -51.536147414174486
1474 -51.4732841961266
1475 -51.41051693873345
1476 -51.3478531954006
1477 -51.28529808727503
1478 -51.222856890284035
1479 -51.160533602397685
1480 -51.09832712339362
1481 -51.036232419958246
1482 -50.97422135665041
1483 -50.91229962066097
1484 -50.85049932238469
1485 -50.788809515334734
1486 -50.72722358866356
1487 -50.66578265235356
1488 -50.6044304460145
1489 -50.54314914634472
1490 -50.48194666445871
1491 -50.42076142477224
1492 -50.35960581197481
1493 -50.29844211938868
1494 -50.23726976656965
1495 -50.176101815086255
1496 -50.11491485191002
1497 -50.053696110264745
1498 -49.99247088755728
1499 -49.93118980032617
1500 -49.86981345381116
1501 -49.808327662255536
1502 -49.74673318471613
1503 -49.68505929487573
1504 -49.62328194897532
1505 -49.561363810589945
1506 -49.499279277415916
1507 -49.43702954070235
1508 -49.37462788517323
1509 -49.31205251659232
1510 -49.24927508980416
1511 -49.186428353395925
1512 -49.12349427296429
1513 -49.06033089203041
1514 -48.99696235658868
1515 -48.9334413209541
1516 -48.86981047421447
1517 -48.806135486798574
1518 -48.74249099120999
1519 -48.67898491762115
1520 -48.61571941064098
1521 -48.5527624049373
1522 -48.49018375545535
1523 -48.42805590755999
1524 -48.366453825928055
1525 -48.30545961521747
1526 -48.245168569202576
1527 -48.18565441752548
1528 -48.12698736706912
1529 -48.06923489159139
1530 -48.01241766215004
1531 -47.95656217187439
1532 -47.90170834887266
1533 -47.84790892008195
1534 -47.79517835452355
1535 -47.743495169093336
1536 -47.69287767602836
1537 -47.64331684127826
1538 -47.59477244179592
1539 -47.54720678897118
1540 -47.50056286814785
1541 -47.45477645055046
1542 -47.409800895509015
1543 -47.365552808292705
1544 -47.32194069624769
1545 -47.27886672707689
1546 -47.23618623195378
1547 -47.19375496346543
1548 -47.1514896949039
1549 -47.10934822164185
1550 -47.06727539434869
1551 -47.02524904298237
1552 -46.98326052759061
1553 -46.941273144882615
1554 -46.899254299216594
1555 -46.85718026424983
1556 -46.81500725187394
1557 -46.77269676649685
1558 -46.73027634189524
1559 -46.687798302099864
1560 -46.645297929116765
1561 -46.60285582052618
1562 -46.56056806455026
1563 -46.518536757468965
1564 -46.47686773004031
1565 -46.43566703422201
1566 -46.39503709464695
1567 -46.35507936292182
1568 -46.31589651076006
1569 -46.27757929839841
1570 -46.24020780975213
1571 -46.20384584101355
1572 -46.16851890132637
1573 -46.134228921894874
1574 -46.10096427242416
1575 -46.06869869939739
1576 -46.03739401884152
1577 -46.00699905767094
1578 -45.977454056174444
1579 -45.94870132148148
1580 -45.920694720644825
1581 -45.89341589411787
1582 -45.86684331980015
1583 -45.84094798485464
1584 -45.815698496519026
1585 -45.79106410224886
1586 -45.767006913609265
1587 -45.743485174420314
1588 -45.720464520771515
1589 -45.69791639658973
1590 -45.67580860775863
1591 -45.65410295821721
1592 -45.63275849667819
1593 -45.61173697042215
1594 -45.59101191432735
1595 -45.570561174356094
1596 -45.55033442817728
1597 -45.530291385362034
1598 -45.510426365127444
1599 -45.4907353379719
1600 -45.47121597572855
1601 -45.45186883922862
1602 -45.43269793168739
1603 -45.413710458336084
1604 -45.39491670366325
1605 -45.37633037051378
1606 -45.35796957955295
1607 -45.33985385915284
1608 -45.32200375302684
1609 -45.30444220376714
1610 -45.28719530701778
1611 -45.27029139717835
1612 -45.25376084096766
1613 -45.23763603602663
1614 -45.2219497149785
1615 -45.20673189921427
1616 -45.192008271427405
1617 -45.177803745298235
1618 -45.164144596522995
1619 -45.1510552092739
1620 -45.13855632557952
1621 -45.12666620445775
1622 -45.115399963244364
1623 -45.10476893237423
1624 -45.094780374064335
1625 -45.0854376107557
1626 -45.076739860760995
1627 -45.068682316442924
1628 -45.06125595409175
1629 -45.05444745966496
1630 -45.04824377749224
1631 -45.04262257613482
1632 -45.03755139943529
1633 -45.03299475144587
1634 -45.028914406392985
1635 -45.02526921125284
1636 -45.02201627872181
1637 -45.01911450460335
1638 -45.01652319793489
1639 -45.0142006582928
1640 -45.01210616748529
1641 -45.01020141768475
1642 -45.00844996846541
1643 -45.00681702296076
1644 -45.005264555396195
1645 -45.00376436132198
1646 -45.002307128609765
1647 -45.00088338392176
1648 -44.99947846057289
1649 -44.99808003150916
1650 -44.99667880086712
1651 -44.995270961711114
1652 -44.993863327838376
1653 -44.992473207952486
1654 -44.99112115847847
1655 -44.9898186532813
1656 -44.988622168705675
1657 -44.987545511258375
1658 -44.98655714681186
1659 -44.98568013890772
1660 -44.98494220584326
1661 -44.98442533771701
1662 -44.98415164544874
1663 -44.984139277226056
1664 -44.98448688208397
1665 -44.98516523660324
1666 -44.98608638766376
1667 -44.98719835774814
1668 -44.98844534894912
1669 -44.989796864839036
1670 -44.99125706654174
1671 -44.992825761120834
1672 -44.994426501044885
1673 -44.99598908591054
1674 -44.997496412014165
1675 -44.998923486819656
1676 -45.00024731878871
1677 -45.00148015846775
1678 -45.00261401230071
1679 -45.00364784119213
1680 -45.00460423162441
1681 -45.00545994099879
1682 -45.00622112808393
1683 -45.00691530358149
1684 -45.00754577994685
1685 -45.008117268713065
1686 -45.00863603102583
1687 -45.00910937413838
1688 -45.00954514815879
1689 -45.00995118001098
1690 -45.01035386948675
1691 -45.01073161781523
1692 -45.01104821404611
1693 -45.01130303875838
1694 -45.0115357182933
1695 -45.011786555726246
1696 -45.0120260944627
1697 -45.01224538744865
1698 -45.012473043100314
1699 -45.01272609953735
1700 -45.013011382539126
1701 -45.013301811171516
1702 -45.0135666260555
1703 -45.01380352988814
1704 -45.01401143093453
1705 -45.01418970198154
1706 -45.01433833876429
1707 -45.01445929286379
1708 -45.014554367252536
1709 -45.01462461937202
1710 -45.014670876321986
1711 -45.01469193724061
1712 -45.014685623763235
1713 -45.01465000509592
1714 -45.01458305740848
1715 -45.014482873635025
1716 -45.01434815183621
1717 -45.0141788581176
1718 -45.0139741054625
1719 -45.013732841629015
1720 -45.01345771469995
1721 -45.01315410286891
1722 -45.01282762585867
1723 -45.01248377587181
1724 -45.012127742803315
1725 -45.01176420354599
1726 -45.01139901692865
1727 -45.01103790600375
1728 -45.010697015725256
1729 -45.01037506799098
1730 -45.0100561656831
1731 -45.009740265634825
1732 -45.00942696047624
1733 -45.00911450459679
1734 -45.008802379138395
1735 -45.00849225025982
1736 -45.00818630322869
1737 -45.00789530052745
1738 -45.0075959327097
1739 -45.007254384588684
1740 -45.00687262391913
1741 -45.006453316169114
1742 -45.00600274345055
1743 -45.00554877346887
1744 -45.00511972582595
1745 -45.004702282032014
1746 -45.004298899967615
1747 -45.00393404753956
1748 -45.00359188948809
1749 -45.00327063323999
1750 -45.002990417478806
1751 -45.00275110140765
1752 -45.00255056733931
1753 -45.002385318314076
1754 -45.00225103097272
1755 -45.00214293144373
1756 -45.00205609776978
1757 -45.00200577173398
1758 -45.00201894018544
1759 -45.00210478833159
1760 -45.00226355710725
1761 -45.00248983016273
1762 -45.00277857693653
1763 -45.00312223192862
1764 -45.003511027725395
1765 -45.003941213181676
1766 -45.00442437384274
1767 -45.00496615802033
1768 -45.005579227583034
1769 -45.00626936600671
1770 -45.007041922878074
1771 -45.00790615210371
1772 -45.008853853202794
1773 -45.00986011565744
1774 -45.01087917828606
1775 -45.01185915942634
1776 -45.012771162912784
1777 -45.013603729697635
1778 -45.014353518238245
1779 -45.01502523703386
1780 -45.01562418755558
1781 -45.016162096943496
1782 -45.01665072012224
1783 -45.0171013606997
1784 -45.017523419811695
1785 -45.017932251553496
1786 -45.01832138238633
1787 -45.01865550906925
1788 -45.01890176201709
1789 -45.01904739793581
1790 -45.01908807014035
1791 -45.019026081217945
1792 -45.01888640278898
1793 -45.018684525835695
1794 -45.0184231770915
1795 -45.018108566033185
1796 -45.01774891890031
1797 -45.01735944213711
1798 -45.01693334391242
1799 -45.01645442637063
1800 -45.015940719454775
1801 -45.01542400035558
1802 -45.01489664344109
1803 -45.01434195211868
1804 -45.013757923845155
1805 -45.01313549648439
1806 -45.01247617438642
1807 -45.01177463689711
1808 -45.01103561237784
1809 -45.01026142146063
1810 -45.009456065571115
1811 -45.008625051939156
1812 -45.00777223349418
1813 -45.00689997871029
1814 -45.00601104964345
1815 -45.005110892678346
1816 -45.00421084438094
1817 -45.003320698234596
1818 -45.00244815697809
1819 -45.00160401347739
1820 -45.00081154413288
1821 -45.000104866175114
1822 -44.99951354476696
1823 -44.9990436671526
1824 -44.99867913040167
1825 -44.99840125222462
1826 -44.998186295583096
1827 -44.99801061644246
1828 -44.99785024629732
1829 -44.99768628675872
1830 -44.99750126190144
1831 -44.99727600361246
1832 -44.99699254166379
1833 -44.99663977652252
1834 -44.996210432688436
1835 -44.995700802116396
1836 -44.99511044724675
1837 -44.99444237664608
1838 -44.99371717346217
1839 -44.99295305115721
1840 -44.992150520440525
1841 -44.99131215340034
1842 -44.990441003768105
1843 -44.98954227847234
1844 -44.988623957377165
1845 -44.987695145476096
1846 -44.98676762333525
1847 -44.98582352210052
1848 -44.98482759880616
1849 -44.983757243474585
1850 -44.982618258435764
1851 -44.98142511807182
1852 -44.98017166294804
1853 -44.97890253462237
1854 -44.97768937559282
1855 -44.976575837870534
1856 -44.97559776463152
1857 -44.974785149462726
1858 -44.97416149812111
1859 -44.973741306656876
1860 -44.973530451821524
1861 -44.9735272708695
1862 -44.97372350248621
1863 -44.97410508701512
1864 -44.97465271288706
1865 -44.975342809192654
1866 -44.97614871450615
1867 -44.97703683792475
1868 -44.977972609249925
1869 -44.978928200741535
1870 -44.979880140848074
1871 -44.98081101311836
1872 -44.981704424247695
1873 -44.98254801465391
1874 -44.98333429130273
1875 -44.98406033171692
1876 -44.98472462903698
1877 -44.985324207944295
1878 -44.985859806492016
1879 -44.986335584230936
1880 -44.986758692244884
1881 -44.98713807984488
1882 -44.98748353674445
1883 -44.987805180630616
1884 -44.98811545175378
1885 -44.98842811267061
1886 -44.98875242959223
1887 -44.98909467710552
1888 -44.989458343275636
1889 -44.989844370505914
1890 -44.99025160196766
1891 -44.99067639497006
1892 -44.991114116777226
1893 -44.99156166167287
1894 -44.99201613700306
1895 -44.99247363094896
1896 -44.99293036874642
1897 -44.993384541243024
1898 -44.99383666134001
1899 -44.99428787605308
1900 -44.99473896845046
1901 -44.99518850631403
1902 -44.99563384328551
1903 -44.99607134176623
1904 -44.99649600115969
1905 -44.99690140365899
1906 -44.9972806355944
1907 -44.997626578875995
1908 -44.99793351016473
1909 -44.998196995766165
1910 -44.99840345864735
1911 -44.99853138991775
1912 -44.99856004924725
1913 -44.998471763346494
1914 -44.99829152633115
1915 -44.998068289784705
1916 -44.99781916194764
1917 -44.99751964239962
1918 -44.997149526726574
1919 -44.99675656046681
1920 -44.99639092292356
1921 -44.99606475993106
1922 -44.995807694126476
1923 -44.99563625632359
1924 -44.99555028098456
1925 -44.995544824234834
1926 -44.9956295680696
1927 -44.99578274047925
1928 -44.99594666210767
1929 -44.99609752376831
1930 -44.99622127233471
1931 -44.99629829202644
1932 -44.99632643759
1933 -44.99633989442261
1934 -44.996387673676224
1935 -44.99653957194569
1936 -44.99685642647221
1937 -44.997370764913306
1938 -44.99806425039355
1939 -44.998922347249206
1940 -44.999916205429045
1941 -45.00100432534057
1942 -45.002141994464736
1943 -45.00329018561043
1944 -45.004391393121175
1945 -45.00538013718567
1946 -45.00620959877534
1947 -45.00684496266947
1948 -45.007272769315925
1949 -45.00747656592947
1950 -45.007470564911415
1951 -45.00732302926622
1952 -45.00707266503304
1953 -45.006703790524185
1954 -45.00620667652282
1955 -45.00558274868281
1956 -45.00487396841036
1957 -45.00409254269427
1958 -45.00324030813279
1959 -45.00236151858715
1960 -45.00148586021688
1961 -45.00062821686008
1962 -44.99981668092138
1963 -44.99907023786914
1964 -44.99841614840956
1965 -44.9978365157477
1966 -44.99734000523465
1967 -44.996996540855186
1968 -44.99678478218618
1969 -44.996656468387776
1970 -44.99660090993343
1971 -44.99651772127245
1972 -44.99641690749635
1973 -44.99636693960748
1974 -44.996323979678515
1975 -44.996292943910206
1976 -44.996297116348494
1977 -44.9963407244796
1978 -44.99642550976153
1979 -44.99654683310908
1980 -44.99670086262091
1981 -44.99690239705542
1982 -44.99715420106107
1983 -44.99742233783891
1984 -44.997666235889
1985 -44.99785148364932
1986 -44.99795171874807
1987 -44.99794706001406
1988 -44.99779923680194
1989 -44.99748709293724
1990 -44.99702372498541
1991 -44.99643673788289
1992 -44.99575483110195
1993 -44.99499638362956
1994 -44.99417965819809
1995 -44.99332284235139
1996 -44.99244319115695
1997 -44.991555553298014
1998 -44.99067226349202
1999 -44.9897766555038
2000 -44.98883918595906


==> plotdata/satellite_constellation/sat_A1_r.tex <==
t r
0 6848.233953273979
1 6848.243232969134
2 6848.2739411959465
3 6848.330085550513
4 6848.415219619215
5 6848.532379464354
6 6848.684029396594
7 6848.872018004617
8 6849.097545218812
9 6849.361141022182
10 6849.662656187239
11 6850.001265205418
12 6850.375481358211
13 6850.783183624388
14 6851.221654921509
15 6851.68763099168
16 6852.177359036254
17 6852.68666503388
18 6853.211028510395
19 6853.745663350538
20 6854.285603244026
21 6854.825790263577
22 6855.361164925382
23 6855.886756115169
24 6856.397769336603
25 6856.889671686905
26 6857.358272118831
27 6857.799795523787
28 6858.210949313429
29 6858.58898143056
30 6858.931728791022
31 6859.237655252858
32 6859.505878410309
33 6859.736184995004
34 6859.929034395455
35 6860.085549844559
36 6860.207498937329
37 6860.297262685151
38 6860.357791725791
39 6860.392555521398
40 6860.40548118487
41 6860.400882329524
42 6860.383383429468
43 6860.35783789617
44 6860.329241477661
45 6860.302644755538
46 6860.283063135305
47 6860.275387229307
48 6860.284297213054
49 6860.314173769597
50 6860.369030221174
51 6860.452441300701
52 6860.567469630852
53 6860.716616542554
54 6860.901777378213
55 6861.124207946369
56 6861.38450232468
57 6861.682582627623
58 6862.017700649535
59 6862.388451335546
60 6862.792798146398
61 6863.228109617907
62 6863.691206479905
63 6864.17841845147
64 6864.685649777285
65 6865.208452183944
66 6865.742104007822
67 6866.2816940767
68 6866.822208838205
69 6867.358621165593
70 6867.885979278741
71 6868.399494236874
72 6868.894624401645
73 6869.367155375136
74 6869.813274077175
75 6870.229635781648
76 6870.613422747489
77 6870.962393462102
78 6871.274921838437
79 6871.550025528703
80 6871.787382916317
81 6871.987338501471
82 6872.150896594684
83 6872.279703466089
84 6872.376018253593
85 6872.442673074672
86 6872.483023074648
87 6872.500887340544
88 6872.500481606281
89 6872.486343970721
90 6872.463254914173
91 6872.436153003797
92 6872.410047831257
93 6872.389931568927
94 6872.3806908016595
95 6872.387020248818
96 6872.413339823795
97 6872.463716464256
98 6872.541792219345
99 6872.650719868904
100 6872.793107162777
101 6872.970970771216
102 6873.185700760974
103 6873.438036119957
104 6873.728051851088
105 6874.055157893171
106 6874.418109841492
107 6874.815031327479
108 6875.243447511364
109 6875.700329153514
110 6876.182146488297
111 6876.684931933512
112 6877.204350442374
113 6877.735776213295
114 6878.274374446063
115 6878.815186749828
116 6879.353218571649
117 6879.88352701453
118 6880.401307743974
119 6880.901979348007
120 6881.381263602312
121 6881.835260316649
122 6882.2605155178
123 6882.654081653709
124 6883.013568877098
125 6883.337186544626
126 6883.623774559153
127 6883.87282331324
128 6884.084482215268
129 6884.259518948133
130 6884.399318932534
131 6884.505953008616
132 6884.582068900595
133 6884.630851794183
134 6884.655963146964
135 6884.661479162863
136 6884.651819791878
137 6884.631670124659
138 6884.605902902495
139 6884.579491754109
140 6884.5574188318715
141 6884.5438439608615
142 6884.539791412419
143 6884.545329605589
144 6884.560255339348
145 6884.5830868408875
146 6884.6101697622435
147 6884.640191488205
148 6884.674225029618
149 6884.712854397473
150 6884.756348705614
151 6884.80517005067
152 6884.858933943272
153 6884.91675183388
154 6884.977608601474
155 6885.040435265306
156 6885.104129465514
157 6885.167572843101
158 6885.229651157695
159 6885.289274950408
160 6885.345397567608
161 6885.39703361683
162 6885.443276702497
163 6885.483315041009
164 6885.516445637322
165 6885.542086588245
166 6885.559787421259
167 6885.569237396081
168 6885.570270411961
169 6885.562867795384
170 6885.547158941269
171 6885.523419321207
172 6885.492065352517
173 6885.4536468621645
174 6885.408837946618
175 6885.358424838877
176 6885.303292143079
177 6885.244407044407
178 6885.182803041028
179 6885.119561592747
180 6885.055775767815
181 6884.992532141565
182 6884.930980431672
183 6884.872212556947
184 6884.817260669243
185 6884.767081715301
186 6884.722532215159
187 6884.684399052985
188 6884.653376094378
189 6884.630011335193
190 6884.614674563279
191 6884.607551127183
192 6884.608849011773
193 6884.618571676138
194 6884.636537810305
195 6884.662112382469
196 6884.6936581646705
197 6884.729893076421
198 6884.770454864878
199 6884.815661519762
200 6884.863727182791
201 6884.91369298745
202 6884.96546414504
203 6885.019211658233
204 6885.074199094642
205 6885.129460815973
206 6885.184026434606
207 6885.236938403679
208 6885.287267899194
209 6885.334131293071
210 6885.376705823686
211 6885.414243964717
212 6885.446086471237
213 6885.471674267142
214 6885.490522640359
215 6885.502230118587
216 6885.506673075858
217 6885.503796806524
218 6885.493651619609
219 6885.476381100605
220 6885.452218013407
221 6885.421666975149
222 6885.385277205309
223 6885.343666350527
224 6885.297588449314
225 6885.247858882793
226 6885.195350152896
227 6885.140984191403
228 6885.085715274178
229 6885.03051384418
230 6884.976349105387
231 6884.924171985978
232 6884.874898681193
233 6884.829385734799
234 6884.788407309956
235 6884.7526898443275
236 6884.722877311708
237 6884.69950346407
238 6884.682975618229
239 6884.673567564444
240 6884.67144084068
241 6884.67662721934
242 6884.689032958135
243 6884.708324176556
244 6884.733645606681
245 6884.764230513936
246 6884.7992120435
247 6884.837833190958
248 6884.87940840641
249 6884.923251801411
250 6884.96877126287
251 6885.015509484917
252 6885.063016207883
253 6885.1106068762065
254 6885.157699639427
255 6885.203419632261
256 6885.247107003586
257 6885.288033022761
258 6885.325479065414
259 6885.358787685618
260 6885.387373939011
261 6885.41073625736
262 6885.428464212612
263 6885.4402463333
264 6885.445875645195
265 6885.445253069559
266 6885.43838920533
267 6885.425404135543
268 6885.406525602083
269 6885.382084609551
270 6885.352510023261
271 6885.318320784433
272 6885.280116824696
273 6885.238568568044
274 6885.194390929241
275 6885.148306245861
276 6885.101118295099
277 6885.05369455632
278 6885.006813973304
279 6884.9612960334025
280 6884.91801401038
281 6884.877710314495
282 6884.840983317086
283 6884.808491875553
284 6884.780835477849
285 6884.758507040426
286 6884.741880780391
287 6884.731224066499
288 6884.726748187133
289 6884.728539990414
290 6884.736567691734
291 6884.750675662558
292 6884.770568303886
293 6884.795842898272
294 6884.825941292751
295 6884.8601962339235
296 6884.897889247837
297 6884.938319553904
298 6884.9807911433545
299 6885.024395392544
300 6885.068342045086
301 6885.112134543745
302 6885.155330330086
303 6885.1970632134535
304 6885.236733464825
305 6885.273796175526
306 6885.30762816133
307 6885.337635432998
308 6885.363291531856
309 6885.384146099907
310 6885.399832727979
311 6885.410075948463
312 6885.414695840239
313 6885.413610936599
314 6885.4068397509245
315 6885.394500776473
316 6885.376810520028
317 6885.354079566335
318 6885.326706645892
319 6885.295171805111
320 6885.2600067694575
321 6885.221778851479
322 6885.181200261645
323 6885.138940200393
324 6885.09571095467
325 6885.052352816197
326 6885.009648509382
327 6884.968348044944
328 6884.929176845927
329 6884.892822680265
330 6884.859923820763
331 6884.831043008385
332 6884.806635248755
333 6884.787129782793
334 6884.77290479038
335 6884.764156902694
336 6884.761039880533
337 6884.763634975217
338 6884.771883844583
339 6884.785626406148
340 6884.804507758372
341 6884.827951499787
342 6884.85547583097
343 6884.886624717648
344 6884.92108917885
345 6884.957884245598
346 6884.996411410386
347 6885.036476334804
348 6885.077208461545
349 6885.117181812263
350 6885.155714568196
351 6885.192246759403
352 6885.226610544926
353 6885.257753383486
354 6885.285234606159
355 6885.309158159644
356 6885.329230503544
357 6885.345099155174
358 6885.356485456517
359 6885.363189280033
360 6885.3650926416185
361 6885.3621617676
362 6885.35444783973
363 6885.3420859477055
364 6885.325292993473
365 6885.304363784501
366 6885.279665467074
367 6885.25163121283
368 6885.220753181938
369 6885.187573097108
370 6885.152672897667
371 6885.116665502271
372 6885.0800909034815
373 6885.043373783602
374 6885.007395838477
375 6884.972861297856
376 6884.940290409873
377 6884.910047330774
378 6884.882807517409
379 6884.858919300359
380 6884.839015918561
381 6884.823513619329
382 6884.8126852010055
383 6884.806713133062
384 6884.8056838687335
385 6884.809635912514
386 6884.818506425667
387 6884.832139477257
388 6884.850296434407
389 6884.872658737418
390 6884.898831583477
391 6884.928172278271
392 6884.95963626798
393 6884.99287497872
394 6885.0275728763745
395 6885.063324528559
396 6885.099541298932
397 6885.1355870031075
398 6885.170828044331
399 6885.20464558284
400 6885.236446476756
401 6885.265672145871
402 6885.291809894967
403 6885.314366905878
404 6885.332881458549
405 6885.347104965652
406 6885.356809609059
407 6885.361825735865
408 6885.362065016016
409 6885.357522835705
410 6885.348279066418
411 6885.334495603329
412 6885.31641421246
413 6885.294352339223
414 6885.268696975876
415 6885.239898184076
416 6885.208461502116
417 6885.174938525547
418 6885.139917790878
419 6885.104014043783
420 6885.067803396156
421 6885.031802114383
422 6884.996775704312
423 6884.9633793205
424 6884.9321992069235
425 6884.903742831265
426 6884.878367725868
427 6884.856466836843
428 6884.838479148515
429 6884.824869069116
430 6884.815909337853
431 6884.811722102001
432 6884.81225864939
433 6884.817469084498
434 6884.827237756304
435 6884.841347973805
436 6884.859568625683
437 6884.881703896713
438 6884.907169460323
439 6884.935417473125
440 6884.965883041863
441 6884.998035024617
442 6885.031444266386
443 6885.065815204235
444 6885.100607347519
445 6885.135209907274
446 6885.169015310464
447 6885.20142966527
448 6885.231883602697
449 6885.259842182814
450 6885.284815311777
451 6885.30636456853
452 6885.32411144957
453 6885.33774431339
454 6885.347023434469
455 6885.351785249997
456 6885.351946437542
457 6885.3475042058935
458 6885.338536355058
459 6885.32519974181
460 6885.307727541491
461 6885.286427171724
462 6885.261672607032
463 6885.233898253069
464 6885.203591520925
465 6885.171281514632
466 6885.137529459986
467 6885.10293438946
468 6885.068105584291
469 6885.033654494783
470 6885.000181523287
471 6884.968259568849
472 6884.93844493002
473 6884.911280040072
474 6884.887246659544
475 6884.866766613601
476 6884.850200379687
477 6884.837825132551
478 6884.829810767153
479 6884.8262752246865
480 6884.827295094999
481 6884.8328541596065
482 6884.842704119696
483 6884.85676588726
484 6884.874900338302
485 6884.896807538787
486 6884.922022243979
487 6884.949856677216
488 6884.97976987348
489 6885.011327468019
490 6885.04412614541
491 6885.0774702503895
492 6885.110973639032
493 6885.14410514374
494 6885.1762827130815
495 6885.206941099312
496 6885.235540778781
497 6885.261580504731
498 6885.284603917343
499 6885.304206535797
500 6885.320043328198
501 6885.331837048797
502 6885.33938007278
503 6885.342539254244
504 6885.341259186929
505 6885.335561512773
506 6885.32554714679
507 6885.311391885798
508 6885.293343966604
509 6885.2717190599205
510 6885.246897194403
511 6885.219314118141
512 6885.189453664068
513 6885.1578406380195
514 6885.1250298862815
515 6885.091597499255
516 6885.058130425242
517 6885.0251952259105
518 6884.993308832841
519 6884.962400139313
520 6884.931320525568
521 6884.902193218166
522 6884.876289557144
523 6884.854094425785
524 6884.83591506291
525 6884.822163255709
526 6884.813091564298
527 6884.80881935257
528 6884.809421587407
529 6884.8148244659815
530 6884.824964431688
531 6884.839535758517
532 6884.858248089425
533 6884.880579340118
534 6884.905895135099
535 6884.934158280417
536 6884.964840800606
537 6884.997408201949
538 6885.030611348969
539 6885.063806153627
540 6885.095901513269
541 6885.127086395735
542 6885.1575053414235
543 6885.186735074816
544 6885.214261157692
545 6885.239599398832
546 6885.262304793806
547 6885.281979649377
548 6885.29827890387
549 6885.310915991285
550 6885.319669970368
551 6885.324387266682
552 6885.324893259532
553 6885.32100068955
554 6885.3129882126805
555 6885.301055930621
556 6885.285412272404
557 6885.266330010079
558 6885.244145500765
559 6885.219248602052
560 6885.192076037229
561 6885.163103892982
562 6885.132840444751
563 6885.1017450394165
564 6885.070141858974
565 6885.0385946165015
566 6885.0078894929775
567 6884.978619367054
568 6884.951298302024
569 6884.926405331383
570 6884.9043775261935
571 6884.88560116078
572 6884.870406465455
573 6884.859061277397
574 6884.851763491129
575 6884.848642440371
576 6884.8497543278345
577 6884.855080264969
578 6884.86452680271
579 6884.877928080922
580 6884.89504880444
581 6884.915587461576
582 6884.939180825186
583 6884.965417288572
584 6884.993752223557
585 6885.023553578233
586 6885.054401724463
587 6885.085623093533
588 6885.116819481665
589 6885.147428255781
590 6885.176999055889
591 6885.205036939547
592 6885.231049897769
593 6885.254580597353
594 6885.275214785407
595 6885.292592261421
596 6885.306408477651
597 6885.316419299423
598 6885.322445680179
599 6885.324384091966
600 6885.3222023256985
601 6885.315938200829
602 6885.30570205405
603 6885.291673197377
604 6885.274094623968
605 6885.253269294068
606 6885.229565990741
607 6885.203403737867
608 6885.175243723281
609 6885.145388177247
610 6885.113004981952
611 6885.076848896082
612 6885.039323812708
613 6884.99985205272
614 6884.96011394241
615 6884.919523362309
616 6884.880032227449
617 6884.841205121065
618 6884.804707855791
619 6884.770016484259
620 6884.738729986023
621 6884.710113690015
622 6884.6874809258525
623 6884.6717712617765
624 6884.663284628396
625 6884.662249255776
626 6884.668673997247
627 6884.682465936978
628 6884.703389764773
629 6884.731087505315
630 6884.764784331515
631 6884.803078263527
632 6884.8458046254045
633 6884.891908847742
634 6884.9412169432535
635 6884.993053372143
636 6885.0462451450085
637 6885.099110036521
638 6885.151431224527
639 6885.202386840442
640 6885.251091708409
641 6885.295293239651
642 6885.331787772205
643 6885.360510913637
644 6885.379394792333
645 6885.38915087349
646 6885.388843874272
647 6885.374788594765
648 6885.342803119589
649 6885.289005130932
650 6885.20986754125
651 6885.102301039708
652 6884.963716448675
653 6884.79206138133
654 6884.585866777531
655 6884.3442791329135
656 6884.067057528137
657 6883.754575920345
658 6883.407847871909
659 6883.028507422443
660 6882.6187363404115
661 6882.18126321284
662 6881.719330045176
663 6881.2366118906
664 6880.737126214316
665 6880.225168539104
666 6879.70525614978
667 6879.182055028133
668 6878.660290530799
669 6878.1446543925895
670 6877.639749687263
671 6877.149994963817
672 6876.679515301917
673 6876.232098706225
674 6875.811121024887
675 6875.419489170625
676 6875.059590181044
677 6874.7332521307935
678 6874.441709796963
679 6874.185583914001
680 6873.9648928508595
681 6873.779032133908
682 6873.626801933372
683 6873.506415999379
684 6873.415436710948
685 6873.350902719529
686 6873.309171678235
687 6873.286279567189
688 6873.278333034632
689 6873.281368168033
690 6873.275966742841
691 6873.241791945694
692 6873.174025697649
693 6873.069316365522
694 6872.925056153928
695 6872.739130743979
696 6872.5103002173555
697 6872.238267286922
698 6871.923271749442
699 6871.56604797664
700 6871.168357607162
701 6870.733553186736
702 6870.26664619172
703 6869.775398931402
704 6869.267093313235
705 6868.757303114333
706 6868.260307599828
707 6867.779055460942
708 6867.31865827646
709 6866.882265649779
710 6866.472061588014
711 6866.088672500272
712 6865.7195997637
713 6865.355014984791
714 6864.99680949351
715 6864.6469588638365
716 6864.3075089461145
717 6863.979987195108
718 6863.665752609489
719 6863.36530992088
720 6863.078698946637
721 6862.806548862062
722 6862.549161650647
723 6862.306518594967
724 6862.078349348295
725 6861.864169396096
726 6861.663229914343
727 6861.4745159376125
728 6861.296782029184
729 6861.128622416638
730 6860.968460878821
731 6860.814564197682
732 6860.6650806940115
733 6860.518077351168
734 6860.371571013211
735 6860.223600176079
736 6860.072239148198
737 6859.91560074224
738 6859.751907958514
739 6859.579527913419
740 6859.397335717689
741 6859.204400061529
742 6858.999604920685
743 6858.782081341267
744 6858.551258969317
745 6858.306827530047
746 6858.048775341841
747 6857.777366023415
748 6857.493027714965
749 6857.196406741002
750 6856.88836165533
751 6856.569947553531
752 6856.242351624282
753 6855.906812262423
754 6855.56475014592
755 6855.217702722007
756 6854.867296909897
757 6854.515239400716
758 6854.1632483662925
759 6853.813022268604
760 6853.466247944656
761 6853.124551572593
762 6852.789469660843
763 6852.462421614907
764 6852.144684365369
765 6851.8373969144595
766 6851.541485976238
767 6851.257648144299
768 6850.986392138625
769 6850.728002652899
770 6850.482535193676
771 6850.249814996069
772 6850.029440061723
773 6849.820788264013
774 6849.623028387777
775 6849.435134915535
776 6849.255906274831
777 6849.083986250478
778 6848.917888178645
779 6848.756021457104
780 6848.596719909862
781 6848.438271526765
782 6848.278949025065
783 6848.117040676624
784 6847.950880871325
785 6847.778879851162
786 6847.599552108312
787 6847.411542918003
788 6847.213652554948
789 6847.00485774267
790 6846.784329959674
791 6846.55145029735
792 6846.305820570366
793 6846.047270494118
794 6845.7758608011945
795 6845.491882251645
796 6845.195850531153
797 6844.8885016722115
798 6844.570770200144
799 6844.243793102038
800 6843.90885787377
801 6843.567373436447
802 6843.220886979857
803 6842.871035966035
804 6842.519518863379
805 6842.1680647889025
806 6841.818402588075
807 6841.472229869734
808 6841.131182594441
809 6840.796805731281
810 6840.470525524831
811 6840.153623868262
812 6839.847215254834
813 6839.552226717278
814 6839.269381106833
815 6838.999184031431
816 6838.741914701259
817 6838.497620831006
818 6838.266117693301
819 6838.046991359059
820 6837.839606036644
821 6837.643195072152
822 6837.456717347336
823 6837.278872917077
824 6837.108285605302
825 6836.943449016722
826 6836.782753544679
827 6836.624515248367
828 6836.467236196933
829 6836.309172073116
830 6836.148361973325
831 6835.9835029772685
832 6835.812987736925
833 6835.634958133697
834 6835.448041256435
835 6835.250995609592
836 6835.042789357534
837 6834.822726480052
838 6834.590189997604
839 6834.344677810135
840 6834.0861932109365
841 6833.814783880248
842 6833.530591349265
843 6833.234149836342
844 6832.926313266712
845 6832.608105449033
846 6832.280609507815
847 6831.9451098337095
848 6831.603067029493
849 6831.256084889321
850 6830.905801948439
851 6830.553914110128
852 6830.202224635924
853 6829.852469862604
854 6829.506361661219
855 6829.165568334494
856 6828.831617199434
857 6828.505952435403
858 6828.189896843374
859 6827.884554666456
860 6827.590819765121
861 6827.309408242547
862 6827.04081455707
863 6826.785302541407
864 6826.542900519157
865 6826.313400706688
866 6826.096362914875
867 6825.891122387023
868 6825.696801713024
869 6825.51232662061
870 6825.336445311302
871 6825.167750998573
872 6825.004707246751
873 6824.845675671227
874 6824.688945486645
875 6824.532764345214
876 6824.375369937656
877 6824.215021791308
878 6824.050032668399
879 6823.878799021193
880 6823.699855928134
881 6823.511859348083
882 6823.313598674817
883 6823.104070603221
884 6822.882475176683
885 6822.648230305874
886 6822.401015901749
887 6822.140726226798
888 6821.867451422193
889 6821.581543082984
890 6821.283581267024
891 6820.974401905915
892 6820.655019893449
893 6820.326620043034
894 6819.990559888808
895 6819.64830262888
896 6819.3014532908865
897 6818.951725909604
898 6818.600902960649
899 6818.250730047607
900 6817.902920416173
901 6817.559180270712
902 6817.2211430178695
903 6816.8903396486085
904 6816.56817095705
905 6816.255882106085
906 6815.954540007395
907 6815.665013903027
908 6815.387959474955
909 6815.123806898241
910 6814.872752957506
911 6814.634757363608
912 6814.409543423006
913 6814.196602965644
914 6813.995205503472
915 6813.804411387376
916 6813.623088779084
917 6813.449934163934
918 6813.283495947622
919 6813.122200818462
920 6812.965601392483
921 6812.817425243949
922 6812.6829766617975
923 6812.567651643387
924 6812.472866576166
925 6812.39647482917
926 6812.335226886625
927 6812.2855950121675
928 6812.243899916397
929 6812.206298366556
930 6812.16917111165
931 6812.128960788934
932 6812.082700469672
933 6812.030559183255
934 6811.972608823879
935 6811.909741267629
936 6811.843053055149
937 6811.773741142593
938 6811.703062225933
939 6811.632298404883
940 6811.562732127891
941 6811.495625451032
942 6811.432195514866
943 6811.37359285671
944 6811.320880533839
945 6811.275014426694
946 6811.236826457933
947 6811.20700929432
948 6811.186103692045
949 6811.17448862626
950 6811.172374417443
951 6811.179799061982
952 6811.196627472168
953 6811.222553939229
954 6811.257107753575
955 6811.299661723271
956 6811.349443401887
957 6811.405549296915
958 6811.4669615329985
959 6811.5325656528785
960 6811.6011712779855
961 6811.67153385773
962 6811.742377133186
963 6811.812416264832
964 6811.88038117287
965 6811.945039635982
966 6812.005219285227
967 6812.059829191344
968 6812.107941597724
969 6812.1487410622985
970 6812.181396156824
971 6812.205281440647
972 6812.219983059107
973 6812.225179338291
974 6812.220861535803
975 6812.207318755624
976 6812.185079992507
977 6812.154677737
978 6812.116578249163
979 6812.0713422919835
980 6812.019422350592
981 6811.961679843844
982 6811.899161962618
983 6811.833002566261
984 6811.764401296479
985 6811.694601743356
986 6811.624870151148
987 6811.556471712626
988 6811.490646750974
989 6811.428589028978
990 6811.371424519581
991 6811.32018964021
992 6811.275813586849
993 6811.239101360324
994 6811.210718692067
995 6811.191180182153
996 6811.1808400627715
997 6811.179885678013
998 6811.1883340007025
999 6811.206031250481
1000 6811.232655923279
1001 6811.267724405226
1002 6811.310600216217
1003 6811.360505284813
1004 6811.416533803763
1005 6811.477669103896
1006 6811.5428019914725
1007 6811.61075074012
1008 6811.680282798873
1009 6811.750137123542
1010 6811.819047329598
1011 6811.88576511154
1012 6811.949079887083
1013 6812.007842799548
1014 6812.061063692002
1015 6812.10786384724
1016 6812.147317568619
1017 6812.178636633479
1018 6812.201243742437
1019 6812.214730679592
1020 6812.218928920927
1021 6812.213882404799
1022 6812.199716470766
1023 6812.176672499712
1024 6812.14499251648
1025 6812.10521390826
1026 6812.058458760761
1027 6812.00603894345
1028 6811.948580123628
1029 6811.887522818968
1030 6811.8232200222365
1031 6811.756652427009
1032 6811.689027260673
1033 6811.62157080231
1034 6811.555506645456
1035 6811.492033050268
1036 6811.432301083902
1037 6811.377394509125
1038 6811.328309100618
1039 6811.2859351807765
1040 6811.25104135817
1041 6811.224260338146
1042 6811.206077701557
1043 6811.196823053664
1044 6811.196664010335
1045 6811.205603011817
1046 6811.2234776563455
1047 6811.249963348263
1048 6811.284579565613
1049 6811.326697557093
1050 6811.375552866973
1051 6811.430258956484
1052 6811.489823232551
1053 6811.553164834346
1054 6811.61913456037
1055 6811.686535618764
1056 6811.754145554965
1057 6811.820826823919
1058 6811.885446190849
1059 6811.9466928825
1060 6812.003430969103
1061 6812.054631991184
1062 6812.0993680391975
1063 6812.136851018533
1064 6812.1663649017955
1065 6812.187414600243
1066 6812.199733988508
1067 6812.203144601812
1068 6812.19765945053
1069 6812.183390545671
1070 6812.1605855584485
1071 6812.1296906859225
1072 6812.091516911467
1073 6812.046980599418
1074 6811.996653970759
1075 6811.941786805464
1076 6811.8829591397525
1077 6811.821450607036
1078 6811.757834222863
1079 6811.693138894964
1080 6811.6285378490975
1081 6811.565202676637
1082 6811.504282195131
1083 6811.446881635389
1084 6811.394041972361
1085 6811.346721422801
1086 6811.305778295515
1087 6811.271955251851
1088 6811.245865555824
1089 6811.227982262564
1090 6811.218629584416
1091 6811.217976818693
1092 6811.226035478929
1093 6811.242659009341
1094 6811.267545609934
1095 6811.30024367403
1096 6811.340159294097
1097 6811.386567879889
1098 6811.438627210853
1099 6811.495392704001
1100 6811.555834348232
1101 6811.618855248548
1102 6811.683437945146
1103 6811.748724316787
1104 6811.813528033714
1105 6811.876497131272
1106 6811.936353891621
1107 6811.991913540143
1108 6812.042140631238
1109 6812.086163093675
1110 6812.123177830878
1111 6812.152483791233
1112 6812.173551914515
1113 6812.186000711371
1114 6812.189605007343
1115 6812.184421067259
1116 6812.170891797789
1117 6812.149322707153
1118 6812.119939941429
1119 6812.083947405602
1120 6812.042239645569
1121 6811.995226781823
1122 6811.943267384076
1123 6811.88764646133
1124 6811.828760216326
1125 6811.767508828849
1126 6811.705149690422
1127 6811.643072480517
1128 6811.582084483023
1129 6811.5232079771085
1130 6811.467517536612
1131 6811.416016411725
1132 6811.369636182
1133 6811.329217726086
1134 6811.29549421659
1135 6811.269077277412
1136 6811.250445768784
1137 6811.239937565787
1138 6811.237742837618
1139 6811.243901094238
1140 6811.258300347603
1141 6811.28067907067
1142 6811.310630920258
1143 6811.347612389615
1144 6811.390952607529
1145 6811.439865100763
1146 6811.4934635384025
1147 6811.550773943841
1148 6811.610756213473
1149 6811.672322430651
1150 6811.7343556141695
1151 6811.795730651119
1152 6811.855428459444
1153 6811.912616506727
1154 6811.966287912185
1155 6812.015493128429
1156 6812.059287096599
1157 6812.096916650578
1158 6812.127667655445
1159 6812.15094593701
1160 6812.166308172085
1161 6812.17349501426
1162 6812.172484005621
1163 6812.163383927831
1164 6812.146354595517
1165 6812.121751962392
1166 6812.090176576771
1167 6812.052366000711
1168 6812.009174083693
1169 6811.9611162697165
1170 6811.908427061255
1171 6811.8519281034805
1172 6811.79264385093
1173 6811.7316493440785
1174 6811.670050891815
1175 6811.608965742432
1176 6811.549501701219
1177 6811.4927371722715
1178 6811.43970189668
1179 6811.3913575467295
1180 6811.348580969006
1181 6811.312148072185
1182 6811.282719630197
1183 6811.260829381518
1184 6811.246873936377
1185 6811.241106281184
1186 6811.243631176474
1187 6811.254402470649
1188 6811.273224396506
1189 6811.29975510424
1190 6811.333512558142
1191 6811.373884038311
1192 6811.420137006346
1193 6811.471431918848
1194 6811.526838082471
1195 6811.585350550481
1196 6811.645907975834
1197 6811.707411662827
1198 6811.768799320817
1199 6811.829182804435
1200 6811.887564804062
1201 6811.942585959846
1202 6811.993243138654
1203 6812.038716281927
1204 6812.078046056082
1205 6812.110516188212
1206 6812.1356223883695
1207 6812.152921597656
1208 6812.162070474105
1209 6812.162948608626
1210 6812.155605483896
1211 6812.140029361787
1212 6812.116735110467
1213 6812.086679326886
1214 6812.050593436136
1215 6812.009302324756
1216 6811.963626118487
1217 6811.914384644996
1218 6811.862505711081
1219 6811.809008552684
1220 6811.754897299513
1221 6811.701103119405
1222 6811.64844721191
1223 6811.597687990075
1224 6811.549696794589
1225 6811.505317114861
1226 6811.465081999753
1227 6811.429335950465
1228 6811.399028518269
1229 6811.374645465446
1230 6811.356220930731
1231 6811.344000558335
1232 6811.338205723942
1233 6811.338941308071
1234 6811.346293928832
1235 6811.360313400285
1236 6811.380522828462
1237 6811.406580539101
1238 6811.43832521781
1239 6811.475340198855
1240 6811.516929462465
1241 6811.562211646486
1242 6811.610319250935
1243 6811.660379389449
1244 6811.7114794712925
1245 6811.7627057580075
1246 6811.8131038490355
1247 6811.861783317405
1248 6811.907914945659
1249 6811.950732732205
1250 6811.989506989177
1251 6812.023390942161
1252 6812.051446865128
1253 6812.073096765092
1254 6812.088180378572
1255 6812.096963264452
1256 6812.098891359688
1257 6812.093980976695
1258 6812.082172705909
1259 6812.063552190566
1260 6812.038716156245
1261 6812.008099157742
1262 6811.97213876502
1263 6811.931261168884
1264 6811.886160015351
1265 6811.8376526492875
1266 6811.786678381209
1267 6811.734281084371
1268 6811.681271682545
1269 6811.628571900376
1270 6811.577137938849
1271 6811.527902487137
1272 6811.482152678209
1273 6811.441402732787
1274 6811.405881524782
1275 6811.376620026934
1276 6811.353398842286
1277 6811.3366937645005
1278 6811.327231120799
1279 6811.324881324736
1280 6811.329964771896
1281 6811.34186808771
1282 6811.360234934874
1283 6811.384731799593
1284 6811.415049325798
1285 6811.45108849506
1286 6811.4923175419735
1287 6811.537877532408
1288 6811.586994706906
1289 6811.638751083375
1290 6811.692132350848
1291 6811.746120704897
1292 6811.799709425439
1293 6811.85187511571
1294 6811.901623126194
1295 6811.947998495207
1296 6811.990101760919
1297 6812.027193954078
1298 6812.058638568304
1299 6812.083884540416
1300 6812.102505945699
1301 6812.114197509104
1302 6812.118750348717
1303 6812.1160828172815
1304 6812.10625512635
1305 6812.089509134315
1306 6812.066347761615
1307 6812.037356662961
1308 6812.003161355336
1309 6811.964456871683
1310 6811.922078985217
1311 6811.876595723622
1312 6811.828042142487
1313 6811.777391647986
1314 6811.725916274329
1315 6811.67405880605
1316 6811.6226414787825
1317 6811.572597057484
1318 6811.52483349266
1319 6811.480216577128
1320 6811.439555368553
1321 6811.403587408269
1322 6811.372965049007
1323 6811.348243524097
1324 6811.329871185118
1325 6811.318180974937
1326 6811.313384694987
1327 6811.315569239886
1328 6811.324799461859
1329 6811.341217436328
1330 6811.364617319187
1331 6811.394467969164
1332 6811.430208825644
1333 6811.471067012069
1334 6811.516146158732
1335 6811.564712096914
1336 6811.615927785596
1337 6811.669197090193
1338 6811.723116401488
1339 6811.776582053932
1340 6811.828624531109
1341 6811.878346538735
1342 6811.924971472593
1343 6811.96765778231
1344 6812.0058241498855
1345 6812.038706820296
1346 6812.065466623794
1347 6812.085566399611
1348 6812.098642247848
1349 6812.104485404668
1350 6812.103372035706
1351 6812.0962683723255
1352 6812.0827765128115
1353 6812.062859686437
1354 6812.038039750277
1355 6812.008063378466
1356 6811.972652909928
1357 6811.932386966775
1358 6811.8879043184315
1359 6811.83998493867
1360 6811.7896336289095
1361 6811.738176771912
1362 6811.686538037175
1363 6811.635214333354
1364 6811.585035342378
1365 6811.536911349528
1366 6811.491715420737
1367 6811.450267058235
1368 6811.413318258974
1369 6811.381539856126
1370 6811.355507046427
1371 6811.335691859822
1372 6811.322454117018
1373 6811.316033024599
1374 6811.31654469748
1375 6811.323979914892
1376 6811.338203819862
1377 6811.3589576163695
1378 6811.3858644248785
1379 6811.4184357524755
1380 6811.456080500656
1381 6811.498115643445
1382 6811.543942353024
1383 6811.593070218675
1384 6811.644217197839
1385 6811.696341821451
1386 6811.748608226429
1387 6811.800434104666
1388 6811.851004589082
1389 6811.899304315788
1390 6811.944050209009
1391 6811.984371522103
1392 6812.019625681894
1393 6812.049080120396
1394 6812.072192640202
1395 6812.088593428981
1396 6812.097931890013
1397 6812.1000227266395
1398 6812.094886990345
1399 6812.082767887788
1400 6812.063789426794
1401 6812.03880025523
1402 6812.009259477816
1403 6811.975901654022
1404 6811.939362050367
1405 6811.900287824189
1406 6811.859396903124
1407 6811.817522935691
1408 6811.7755442906455
1409 6811.734293797334
1410 6811.694512929164
1411 6811.656804718429
1412 6811.621287605453
1413 6811.587680604363
1414 6811.5568883166625
1415 6811.529030799507
1416 6811.504792970068
1417 6811.484186320028
1418 6811.467462963837
1419 6811.454926503432
1420 6811.446803577144
1421 6811.443422301182
1422 6811.445389119838
1423 6811.452703126782
1424 6811.465300914809
1425 6811.482722293919
1426 6811.504322339575
1427 6811.529971820851
1428 6811.558795101794
1429 6811.590146330464
1430 6811.623456616501
1431 6811.658122100926
1432 6811.693514138007
1433 6811.729667604135
1434 6811.7670015981885
1435 6811.803674046192
1436 6811.839531053576
1437 6811.87432347837
1438 6811.90826208842
1439 6811.940962247176
1440 6811.971851496141
1441 6812.000398632498
1442 6812.026112362571
1443 6812.048558833178
1444 6812.0673652595015
1445 6812.082229716492
1446 6812.092971024687
1447 6812.099527442184
1448 6812.10191241877
1449 6812.100250465984
1450 6812.094721832712
1451 6812.085576329679
1452 6812.073134551773
1453 6812.057742260223
1454 6812.039795537338
1455 6812.019702712721
1456 6811.9977550893445
1457 6811.974045048695
1458 6811.948998985827
1459 6811.923156085086
1460 6811.896764056506
1461 6811.869753971342
1462 6811.842496504402
1463 6811.815425929866
1464 6811.789119564071
1465 6811.764191569396
1466 6811.741284805572
1467 6811.721039343611
1468 6811.704031342986
1469 6811.690815491726
1470 6811.681787121967
1471 6811.677191955861
1472 6811.677291068972
1473 6811.682323147647
1474 6811.692299716787
1475 6811.70707650366
1476 6811.726469796511
1477 6811.75023445387
1478 6811.778061044284
1479 6811.809532432035
1480 6811.844165045919
1481 6811.8815598343535
1482 6811.92139808994
1483 6811.9644985046925
1484 6812.010822487792
1485 6812.059279298612
1486 6812.108352036956
1487 6812.155371621122
1488 6812.196722310712
1489 6812.232066655998
1490 6812.258444702419
1491 6812.274979261859
1492 6812.281274369021
1493 6812.27869228842
1494 6812.269456378417
1495 6812.2533665784495
1496 6812.231282313302
1497 6812.204226937234
1498 6812.171902303639
1499 6812.133453955045
1500 6812.090440455711
1501 6812.042841798449
1502 6811.992296883927
1503 6811.9396964150355
1504 6811.886705749132
1505 6811.8310205979205
1506 6811.773152042097
1507 6811.714566519806
1508 6811.657126486796
1509 6811.602669536279
1510 6811.554417577905
1511 6811.513633100973
1512 6811.479235795158
1513 6811.454398056148
1514 6811.44356971992
1515 6811.451250317201
1516 6811.481465549719
1517 6811.53805194041
1518 6811.624381060825
1519 6811.743379021926
1520 6811.8974294679065
1521 6812.088277790865
1522 6812.317018374977
1523 6812.584050620743
1524 6812.889089550252
1525 6813.231151183942
1526 6813.6085598717555
1527 6814.019019171681
1528 6814.459645783175
1529 6814.927010796744
1530 6815.4171871113895
1531 6815.925834758465
1532 6816.448294881405
1533 6816.979630048685
1534 6817.514736773706
1535 6818.048470400756
1536 6818.575687022449
1537 6819.091390425563
1538 6819.5908177103765
1539 6820.069493519139
1540 6820.523325767962
1541 6820.94866805129
1542 6821.342390977595
1543 6821.701878094191
1544 6822.025189226274
1545 6822.3110726176565
1546 6822.558922849604
1547 6822.768849377461
1548 6822.941701278287
1549 6823.078881004737
1550 6823.182397568612
1551 6823.254833907453
1552 6823.299430145008
1553 6823.320122991742
1554 6823.32107745396
1555 6823.306865714126
1556 6823.282156982879
1557 6823.266805891781
1558 6823.281076177077
1559 6823.314479863748
1560 6823.371944380395
1561 6823.47306937058
1562 6823.620542728099
1563 6823.816140514716
1564 6824.060775520737
1565 6824.354443783197
1566 6824.696181137941
1567 6825.084195029632
1568 6825.513959712154
1569 6825.980239974474
1570 6826.47851174466
1571 6826.994905136083
1572 6827.514004148177
1573 6828.028386442995
1574 6828.532181521477
1575 6829.02117408934
1576 6829.489754635945
1577 6829.932634957801
1578 6830.350034519674
1579 6830.742863541745
1580 6831.120941840225
1581 6831.49377556724
1582 6831.8595669586
1583 6832.216305692468
1584 6832.562073340992
1585 6832.895282626402
1586 6833.21462876817
1587 6833.518962476015
1588 6833.807359216541
1589 6834.079190783737
1590 6834.334117014355
1591 6834.572110420589
1592 6834.793527030797
1593 6834.998990724429
1594 6835.189415356778
1595 6835.36599652701
1596 6835.530165999009
1597 6835.683580091272
1598 6835.828108590619
1599 6835.965728155063
1600 6836.098481450422
1601 6836.228537361351
1602 6836.358120785316
1603 6836.489447673515
1604 6836.624830834805
1605 6836.76652399252
1606 6836.915774127111
1607 6837.073800686591
1608 6837.242173729976
1609 6837.422085201719
1610 6837.614815654629
1611 6837.8214913848105
1612 6838.042932124683
1613 6838.279632623951
1614 6838.531868436517
1615 6838.799489045503
1616 6839.081862558097
1617 6839.378362671233
1618 6839.688305488346
1619 6840.010584558147
1620 6840.344182621896
1621 6840.687888630671
1622 6841.039924445543
1623 6841.398391340604
1624 6841.761246357592
1625 6842.126337327433
1626 6842.491420995811
1627 6842.854234550694
1628 6843.2125084563995
1629 6843.564038334867
1630 6843.904857588463
1631 6844.231286897695
1632 6844.541833738092
1633 6844.834929469281
1634 6845.109134584491
1635 6845.363315885395
1636 6845.596661980284
1637 6845.808588701121
1638 6845.999023813266
1639 6846.168459563294
1640 6846.31765540899
1641 6846.447398479595
1642 6846.558624347445
1643 6846.652632504333
1644 6846.732963148022
1645 6846.803654719161
1646 6846.8652571260955
1647 6846.917869147096
1648 6846.963358977035
1649 6847.004007719215
1650 6847.042450264151
1651 6847.081709203641
1652 6847.124658591822
1653 6847.173263565427
1654 6847.228618746467
1655 6847.291636412723
1656 6847.362727222084
1657 6847.440749290762
1658 6847.525351508786
1659 6847.615725133035
1660 6847.710759148966
1661 6847.8074251289045
1662 6847.902645603392
1663 6847.996371591864
1664 6848.0867552423915
1665 6848.171146726922
1666 6848.248933280377
1667 6848.319856372597
1668 6848.3839404103255
1669 6848.441387954226
1670 6848.492634532703
1671 6848.537797638517
1672 6848.576466433018
1673 6848.608264568793
1674 6848.633103516085
1675 6848.651218189311
1676 6848.663113985968
1677 6848.669692089842
1678 6848.6718704864525
1679 6848.67029125135
1680 6848.6655982336215
1681 6848.658431542313
1682 6848.6494056335005
1683 6848.63906627019
1684 6848.627889972609
1685 6848.616298294818
1686 6848.604648630471
1687 6848.593234608354
1688 6848.58228705929
1689 6848.571968895531
1690 6848.562459385193
1691 6848.553763519259
1692 6848.545396467164
1693 6848.536804329096
1694 6848.5276781390785
1695 6848.517848910956
1696 6848.507201001521
1697 6848.495729339208
1698 6848.483564903924
1699 6848.470842792991
1700 6848.457726291652
1701 6848.444392114765
1702 6848.431005799423
1703 6848.417734169001
1704 6848.404763380374
1705 6848.392310215809
1706 6848.38055294256
1707 6848.369246414728
1708 6848.3581424557315
1709 6848.347328971268
1710 6848.336808901035
1711 6848.326534162158
1712 6848.316435938191
1713 6848.306447387008
1714 6848.296510410356
1715 6848.286593182509
1716 6848.276724692202
1717 6848.266992944819
1718 6848.257496376381
1719 6848.248316672777
1720 6848.23954417569
1721 6848.231278815101
1722 6848.2236173030415
1723 6848.216644024961
1724 6848.210429684029
1725 6848.205037118901
1726 6848.200368391516
1727 6848.196148127217
1728 6848.192338392129
1729 6848.188229167171
1730 6848.183388848018
1731 6848.17796109109
1732 6848.172098180141
1733 6848.166167950809
1734 6848.160567001749
1735 6848.1555258268
1736 6848.151195674725
1737 6848.14937574108
1738 6848.1490823691465
1739 6848.148164622437
1740 6848.147126264256
1741 6848.146265431389
1742 6848.145837077039
1743 6848.146027298337
1744 6848.146901983204
1745 6848.148427653348
1746 6848.150602804207
1747 6848.153447590883
1748 6848.156915360905
1749 6848.160964777347
1750 6848.165522201813
1751 6848.170452751968
1752 6848.17561888183
1753 6848.180913668458
1754 6848.186281818472
1755 6848.191714340214
1756 6848.197245879093
1757 6848.207534223564
1758 6848.226024421546
1759 6848.25063754117
1760 6848.278888563699
1761 6848.308715843982
1762 6848.33884074902
1763 6848.36814815476
1764 6848.39557543476
1765 6848.426229958789
1766 6848.459957638221
1767 6848.495522798672
1768 6848.536413416081
1769 6848.5797963299765
1770 6848.626571884427
1771 6848.672557551757
1772 6848.709764890702
1773 6848.737001090648
1774 6848.754123431205
1775 6848.761291548627
1776 6848.7588888839155
1777 6848.747568499734
1778 6848.728543313099
1779 6848.70359394732
1780 6848.674521365008
1781 6848.6429061413355
1782 6848.610140576971
1783 6848.5773916063345
1784 6848.545566326646
1785 6848.5151638457155
1786 6848.486473654712
1787 6848.458867518604
1788 6848.432377320605
1789 6848.408376597292
1790 6848.387851642029
1791 6848.371160098129
1792 6848.358193111087
1793 6848.348564211871
1794 6848.341774199359
1795 6848.337305573896
1796 6848.334642399933
1797 6848.328674073934
1798 6848.315261182319
1799 6848.298231996138
1800 6848.285073819808
1801 6848.279673975303
1802 6848.274171147401
1803 6848.265712522122
1804 6848.2565151380195
1805 6848.247504745849
1806 6848.238240961582
1807 6848.227376073021
1808 6848.216258899334
1809 6848.204605279782
1810 6848.192711573641
1811 6848.181125863226
1812 6848.169842831314
1813 6848.158573442895
1814 6848.147051946643
1815 6848.135339944424
1816 6848.124415317389
1817 6848.115219339056
1818 6848.108636918151
1819 6848.105558887973
1820 6848.11050882699
1821 6848.126695348029
1822 6848.150903314007
1823 6848.1764722797425
1824 6848.197453169158
1825 6848.211732012936
1826 6848.219200702833
1827 6848.218990444239
1828 6848.210212357321
1829 6848.193428258477
1830 6848.169513753513
1831 6848.139515899552
1832 6848.104586551902
1833 6848.065949936431
1834 6848.024853818109
1835 6847.982531643823
1836 6847.940170609995
1837 6847.898920868014
1838 6847.859810878006
1839 6847.823711251462
1840 6847.791381884561
1841 6847.763454804938
1842 6847.74042556408
1843 6847.722631956853
1844 6847.7102352223465
1845 6847.703863319584
1846 6847.703934058976
1847 6847.7099928800635
1848 6847.722291478456
1849 6847.741361552907
1850 6847.7676617158395
1851 6847.800749368662
1852 6847.840603882221
1853 6847.887454496137
1854 6847.938764252986
1855 6847.99196190928
1856 6848.046095381628
1857 6848.10017595321
1858 6848.153209049941
1859 6848.204229108633
1860 6848.252327960193
1861 6848.296702304146
1862 6848.336695287177
1863 6848.3718126266585
1864 6848.401735257496
1865 6848.426312186343
1866 6848.44555391529
1867 6848.459020403315
1868 6848.466594279775
1869 6848.469030768312
1870 6848.4671621708385
1871 6848.461860791481
1872 6848.454003737297
1873 6848.444431615566
1874 6848.433896765738
1875 6848.423013977183
1876 6848.412289382459
1877 6848.402196809316
1878 6848.393188882244
1879 6848.385627452248
1880 6848.379742225924
1881 6848.375660844456
1882 6848.373386000647
1883 6848.372825113161
1884 6848.373853467413
1885 6848.376287157181
1886 6848.379897364673
1887 6848.384433324183
1888 6848.38964318513
1889 6848.395286984945
1890 6848.401145105329
1891 6848.407028022362
1892 6848.412776938011
1893 6848.4184628956145
1894 6848.424145013369
1895 6848.429668625782
1896 6848.434910363517
1897 6848.440515218948
1898 6848.447085350295
1899 6848.454344899994
1900 6848.461820383779
1901 6848.468922083382
1902 6848.475115892846
1903 6848.479856867515
1904 6848.482570965702
1905 6848.4829152155735
1906 6848.480798410694
1907 6848.476069674346
1908 6848.468667555492
1909 6848.459063122851
1910 6848.443618065576
1911 6848.417075641686
1912 6848.378955810041
1913 6848.339820752561
1914 6848.31116698035
1915 6848.285681727968
1916 6848.2561926936805
1917 6848.225470998926
1918 6848.195569633455
1919 6848.168303378697
1920 6848.144904018685
1921 6848.125774191191
1922 6848.110930721746
1923 6848.1002564880955
1924 6848.093573040371
1925 6848.090572752316
1926 6848.0907269595355
1927 6848.09336126735
1928 6848.097767802686
1929 6848.105124729924
1930 6848.114745978524
1931 6848.123489595892
1932 6848.130354486795
1933 6848.13475804505
1934 6848.143463735676
1935 6848.162282481002
1936 6848.189984652862
1937 6848.223583439504
1938 6848.258530676763
1939 6848.292332372423
1940 6848.322633129048
1941 6848.347474415942
1942 6848.366390420308
1943 6848.379512591207
1944 6848.3869586861865
1945 6848.38896378694
1946 6848.386047659554
1947 6848.3786972530925
1948 6848.3676732927415
1949 6848.350041909887
1950 6848.326212935276
1951 6848.301387365659
1952 6848.273798288904
1953 6848.240149168057
1954 6848.202062778699
1955 6848.16229273752
1956 6848.1227618554285
1957 6848.085211809433
1958 6848.050739882633
1959 6848.019993479389
1960 6847.993420911389
1961 6847.971261705146
1962 6847.953569541972
1963 6847.940204888788
1964 6847.9308650330295
1965 6847.925182213731
1966 6847.922958930785
1967 6847.924219366034
1968 6847.925107565798
1969 6847.9221358264895
1970 6847.914598353115
1971 6847.903532170826
1972 6847.891438316119
1973 6847.877965127561
1974 6847.866265045659
1975 6847.857896819162
1976 6847.851016134558
1977 6847.845880793012
1978 6847.842227153145
1979 6847.838040948557
1980 6847.831857886773
1981 6847.822657244444
1982 6847.807784150044
1983 6847.784368370762
1984 6847.7515233889135
1985 6847.709413853254
1986 6847.658635337905
1987 6847.5999257191625
1988 6847.538699391965
1989 6847.481362172664
1990 6847.430016836548
1991 6847.385183990789
1992 6847.346548514017
1993 6847.314640477175
1994 6847.289829533152
1995 6847.272345082204
1996 6847.262310234522
1997 6847.259899522813
1998 6847.265471608318
1999 6847.279615336831
2000 6847.303514838543


==> plotdata/satellite_constellation/sat_A2_dtheta.tex <==
t dtheta
0 -25.0
1 -24.99995660733824
2 -24.999803185502145
3 -24.99959153421935
4 -24.99939620297594
5 -24.999324761867292
6 -24.999474914269797
7 -24.99987176066242
8 -25.00051195648052
9 -25.00141169080175
10 -25.002767208060334
11 -25.004751234269968
12 -25.00743156538338
13 -25.01082499930613
14 -25.014957979114783
15 -25.019868556354897
16 -25.025597855612634
17 -25.03222594632757
18 -25.03984090690771
19 -25.04849998491162
20 -25.05821822989433
21 -25.069034315178737
22 -25.081004136365713
23 -25.094111345457485
24 -25.108292520079296
25 -25.123488813108057
26 -25.13957423817414
27 -25.156460519574047
28 -25.174074842095962
29 -25.192354165253384
30 -25.21128300663084
31 -25.230798575404485
32 -25.250763442509804
33 -25.27112461333895
34 -25.29184875275545
35 -25.312884346763774
36 -25.33417415111209
37 -25.35565750192227
38 -25.377271942864922
39 -25.398955510847628
40 -25.42071331450199
41 -25.44255721400309
42 -25.464374630776597
43 -25.48604764800856
44 -25.50750661253051
45 -25.52873960110124
46 -25.54975379311167
47 -25.570569534057597
48 -25.59125873613462
49 -25.611811077184626
50 -25.632239256549756
51 -25.652673200881534
52 -25.673268863474977
53 -25.694011693287578
54 -25.71491928876405
55 -25.73615047252775
56 -25.757762194436246
57 -25.77978299522999
58 -25.802269437540524
59 -25.82523623281575
60 -25.84870746176043
61 -25.872775573542224
62 -25.89752839853339
63 -25.92302771665978
64 -25.94931420272504
65 -25.976430135835937
66 -26.00448405457998
67 -26.03357442805787
68 -26.063756483999306
69 -26.095056458404844
70 -26.127477069838594
71 -26.16098169019837
72 -26.19553004789028
73 -26.231095595932263
74 -26.26765176906478
75 -26.305126680632245
76 -26.343411580886194
77 -26.382418110645066
78 -26.422067876607525
79 -26.46226646827346
80 -26.502935723203283
81 -26.544027087772978
82 -26.585456221608503
83 -26.627090679815186
84 -26.6688395943137
85 -26.71068409873508
86 -26.752559426633685
87 -26.794362229359322
88 -26.83602475095462
89 -26.877491354675442
90 -26.9187130853422
91 -26.95966199284878
92 -27.000338450267424
93 -27.040742676153744
94 -27.08090112558613
95 -27.12087624835577
96 -27.16069505879117
97 -27.200417213227777
98 -27.24015287884784
99 -27.280007947575466
100 -27.320079758505766
101 -27.360463580451587
102 -27.401255624098745
103 -27.44254509359908
104 -27.484414962900075
105 -27.52695630255466
106 -27.57026593066304
107 -27.61442945922675
108 -27.659520273963867
109 -27.705610477436625
110 -27.752762552511644
111 -27.801050386962498
112 -27.85048386445466
113 -27.9011269439573
114 -27.953059698448943
115 -28.006181838377497
116 -28.060339326672203
117 -28.115418419837727
118 -28.171264252527532
119 -28.227740992496866
120 -28.284818198972793
121 -28.342470072698436
122 -28.400638754154393
123 -28.459249355965053
124 -28.518127880395657
125 -28.577140382365513
126 -28.636220704685798
127 -28.69522185388851
128 -28.753956048399658
129 -28.812258758868552
130 -28.870013763639182
131 -28.927110848206308
132 -28.983434389580616
133 -29.038891867028003
134 -29.093356499915625
135 -29.146720672050723
136 -29.198918435153885
137 -29.249871381492916
138 -29.29951292606843
139 -29.347797294863852
140 -29.394701208200324
141 -29.440222939208446
142 -29.484382722919694
143 -29.527200383904216
144 -29.568719698185685
145 -29.60899831747513
146 -29.648111609321532
147 -29.686145800538423
148 -29.723200170065954
149 -29.759381686738905
150 -29.794812449332607
151 -29.829624390048842
152 -29.86396334809476
153 -29.897987045167312
154 -29.931821275026046
155 -29.96560746554667
156 -29.999481927668086
157 -30.03358194766352
158 -30.06803381032131
159 -30.10291637693826
160 -30.138315589148686
161 -30.174309149657077
162 -30.210897638046
163 -30.24811532021438
164 -30.28603284535498
165 -30.324646832885236
166 -30.36392731025871
167 -30.403818486172288
168 -30.44425838366612
169 -30.485184865210083
170 -30.526493826051254
171 -30.568089683272234
172 -30.609904423571724
173 -30.651857588711987
174 -30.69388616662272
175 -30.73603453182229
176 -30.77832492726004
177 -30.82065830818315
178 -30.86301464804598
179 -30.905331873469112
180 -30.947514837324682
181 -30.989535708390925
182 -31.03135925448321
183 -31.072899119672353
184 -31.114077248119052
185 -31.15485459645217
186 -31.195146686997354
187 -31.234924842363007
188 -31.274158578468743
189 -31.312801201673114
190 -31.350825034758337
191 -31.388209235879756
192 -31.424926501776895
193 -31.46094214323151
194 -31.496280586329323
195 -31.53098975282278
196 -31.565090041317283
197 -31.59860475803065
198 -31.63156068641467
199 -31.6640046801966
200 -31.696024296776912
201 -31.7276439939567
202 -31.758906236354356
203 -31.78986834015711
204 -31.820566373545518
205 -31.851066102606215
206 -31.881418533081636
207 -31.911679824374477
208 -31.941908461111893
209 -31.972151871423616
210 -32.00244880997314
211 -32.03284151751401
212 -32.0633599489613
213 -32.09404036773256
214 -32.124911824836744
215 -32.155977555604515
216 -32.18724230572409
217 -32.21871639637471
218 -32.25039544138745
219 -32.28225944474488
220 -32.314290319905574
221 -32.34646210059517
222 -32.37874342359519
223 -32.41110450912442
224 -32.44358983815222
225 -32.4761822649725
226 -32.50886336063884
227 -32.54152411071967
228 -32.573963495819655
229 -32.606134732575164
230 -32.6380240351678
231 -32.66964215642376
232 -32.70101854563521
233 -32.73220969735407
234 -32.76327209606121
235 -32.79421660687968
236 -32.825030567932345
237 -32.855732296983824
238 -32.88633162436549
239 -32.916825261789704
240 -32.94728102525711
241 -32.9777353471518
242 -33.00818932242282
243 -33.03865097703432
244 -33.06909413793578
245 -33.099523083913056
246 -33.12996329131215
247 -33.160407665767934
248 -33.19086144319441
249 -33.22133377457806
250 -33.25181965195774
251 -33.28231271027796
252 -33.31281388514493
253 -33.343333679600654
254 -33.3738570535314
255 -33.404349674460924
256 -33.434805904698194
257 -33.465261240621295
258 -33.495751958267
259 -33.52612462120726
260 -33.556260314378356
261 -33.586222410558484
262 -33.61593404746701
263 -33.64529491571799
264 -33.67429497164208
265 -33.70293996322603
266 -33.731218547077056
267 -33.75919321469892
268 -33.78693436703542
269 -33.8144255387965
270 -33.841714499048614
271 -33.868857689391604
272 -33.895893978164324
273 -33.92283139269352
274 -33.94971687164671
275 -33.97658356152349
276 -34.003439975715104
277 -34.030347708512515
278 -34.05731326112421
279 -34.084316420276956
280 -34.11138183073392
281 -34.138529219072815
282 -34.165766515441774
283 -34.193090598244744
284 -34.220511255142185
285 -34.24807719747892
286 -34.275853135066676
287 -34.303807342059976
288 -34.331752449850484
289 -34.359570552224476
290 -34.38730392953476
291 -34.41509449014494
292 -34.44293404370148
293 -34.470689468521144
294 -34.498358184571366
295 -34.525991226764276
296 -34.55367034784658
297 -34.58148209319615
298 -34.60936972507981
299 -34.63729367448892
300 -34.66525368337944
301 -34.693162730553524
302 -34.72099006528857
303 -34.74875195575556
304 -34.7764245038948
305 -34.80396538425981
306 -34.831439882490685
307 -34.85893867121998
308 -34.8864398983976
309 -34.913916693054496
310 -34.941448129586675
311 -34.969069869024196
312 -34.996797232992364
313 -35.024661176292845
314 -35.05266280401746
315 -35.08081624987173
316 -35.109141259441806
317 -35.1376161416908
318 -35.16619321288026
319 -35.19488132784052
320 -35.22365077452224
321 -35.25239828656081
322 -35.281068277650206
323 -35.309529615463624
324 -35.337681918610656
325 -35.365570281314746
326 -35.393255621777634
327 -35.420788744677566
328 -35.448224382098694
329 -35.475611480820994
330 -35.5029779634883
331 -35.530344131314685
332 -35.55771503292599
333 -35.58509698328596
334 -35.612495675998645
335 -35.639919214533585
336 -35.66737183982631
337 -35.69486117429544
338 -35.72239846906697
339 -35.74999342643341
340 -35.77765407611983
341 -35.80538750624097
342 -35.83319810415918
343 -35.86108085681182
344 -35.889028327950484
345 -35.917022463153785
346 -35.945030688719136
347 -35.973021773804895
348 -36.00096649000552
349 -36.02883523140591
350 -36.05659907672954
351 -36.0842377587158
352 -36.11174105954953
353 -36.13910328808032
354 -36.16632325096976
355 -36.193411732220596
356 -36.220384020206936
357 -36.24724767481229
358 -36.2740111675765
359 -36.300688622865536
360 -36.32730215664491
361 -36.35386633788696
362 -36.38039132387758
363 -36.40689645990003
364 -36.433401699943
365 -36.45992356815627
366 -36.48647532511645
367 -36.51306645278436
368 -36.539702860316694
369 -36.566392395303964
370 -36.59311509270522
371 -36.619820300387524
372 -36.6464846558233
373 -36.6731006205451
374 -36.69966715591587
375 -36.72618213161005
376 -36.75264279340083
377 -36.77900356506447
378 -36.80522237091098
379 -36.83132280234737
380 -36.85731963379209
381 -36.88321424228222
382 -36.90898578011946
383 -36.93466218472535
384 -36.9602353557122
385 -36.985757211339134
386 -37.01126362993946
387 -37.036781768706895
388 -37.06233956867895
389 -37.08792312745428
390 -37.11354523855506
391 -37.139128891496796
392 -37.16471663001277
393 -37.19040753078041
394 -37.216112837957304
395 -37.24186285905938
396 -37.26774685041057
397 -37.293650590484276
398 -37.31959323947644
399 -37.34568672234474
400 -37.37182620663083
401 -37.3979587077338
402 -37.42412196726886
403 -37.450321222112414
404 -37.476585763779134
405 -37.5029264809404
406 -37.52939995431484
407 -37.555894833260346
408 -37.58238438615991
409 -37.60891467878663
410 -37.63539499391505
411 -37.661813023335924
412 -37.688253758599274
413 -37.7147283163102
414 -37.74113550762368
415 -37.7674521751163
416 -37.79378857563038
417 -37.82023422959579
418 -37.846763618362814
419 -37.8733955715667
420 -37.90013291045571
421 -37.92689372506462
422 -37.953599654906476
423 -37.9803446926146
424 -38.00721289467384
425 -38.03414845761255
426 -38.061112488149796
427 -38.08812024393462
428 -38.11513416298996
429 -38.14214113548833
430 -38.1690775193285
431 -38.195934185678155
432 -38.22270460176712
433 -38.249280986184175
434 -38.275708694535524
435 -38.302076934251474
436 -38.328439047861664
437 -38.35483565414546
438 -38.381268594226526
439 -38.407748309184576
440 -38.434325224628665
441 -38.461026104015524
442 -38.48782687859154
443 -38.51467437318797
444 -38.54152030181159
445 -38.56822230799579
446 -38.59474068135695
447 -38.62111307321061
448 -38.64727070353883
449 -38.67303498497099
450 -38.698378026117986
451 -38.72324672984773
452 -38.74744899009483
453 -38.77092318929704
454 -38.79367636926063
455 -38.81583413513815
456 -38.83740677948912
457 -38.8583535931763
458 -38.878764132691444
459 -38.89871469998266
460 -38.91828120717504
461 -38.93769279131412
462 -38.957097210960356
463 -38.97663255099017
464 -38.99651694862784
465 -39.01683930278113
466 -39.03772975227738
467 -39.05930166852417
468 -39.08153426429791
469 -39.1044212325556
470 -39.12803753319094
471 -39.15242800887552
472 -39.177479883077226
473 -39.20302208856353
474 -39.22906960497388
475 -39.25563664605752
476 -39.28263165586258
477 -39.309997826141405
478 -39.33771891372367
479 -39.365709168430826
480 -39.393913608234946
481 -39.422341617516814
482 -39.45093370346474
483 -39.479640467622545
484 -39.50846958703458
485 -39.5373860180469
486 -39.5663818216791
487 -39.59547341972957
488 -39.62465504095535
489 -39.65389665689473
490 -39.68320717236475
491 -39.7124754884095
492 -39.741630960468335
493 -39.7707067324329
494 -39.799697451996984
495 -39.82853521518407
496 -39.857061312943294
497 -39.88523325077861
498 -39.91305225902668
499 -39.940583704624004
500 -39.96788467963241
501 -39.994978189813054
502 -40.02189337722731
503 -40.04863905346949
504 -40.07521201554986
505 -40.101652760298485
506 -40.127920451043686
507 -40.15402954938105
508 -40.18011389312159
509 -40.206267974385995
510 -40.23256061076974
511 -40.25890482922361
512 -40.285280612536205
513 -40.311711138440494
514 -40.338199427279136
515 -40.36479642720077
516 -40.39150324490571
517 -40.41832130383964
518 -40.445250309003434
519 -40.4723159782462
520 -40.499553525650796
521 -40.52695708062612
522 -40.554566748010544
523 -40.582433626100126
524 -40.61044297116617
525 -40.63849687678893
526 -40.6666478633797
527 -40.69501314920752
528 -40.72354642972788
529 -40.752094014878935
530 -40.78073137595538
531 -40.809365714041306
532 -40.837815075339186
533 -40.86619876539975
534 -40.89451818084497
535 -40.922754892739405
536 -40.950926596060064
537 -40.97904537951209
538 -41.00709597468081
539 -41.035041477344976
540 -41.06289084928216
541 -41.09062479809568
542 -41.11830383315014
543 -41.14592419208688
544 -41.17348176221116
545 -41.200978040461166
546 -41.22842607299955
547 -41.2558418010375
548 -41.283297128254276
549 -41.31083972510144
550 -41.33844433306588
551 -41.36600294484065
552 -41.39343452821218
553 -41.42066697135026
554 -41.44762111418359
555 -41.47432371453368
556 -41.50081177700558
557 -41.52715789991168
558 -41.55342407893324
559 -41.57964484044898
560 -41.605851420264464
561 -41.63207290171855
562 -41.65833340015831
563 -41.684654997664566
564 -41.71108801118072
565 -41.73769426815591
566 -41.76451903233095
567 -41.79165479531563
568 -41.81915614416082
569 -41.846903333279265
570 -41.87479173549022
571 -41.90276070720459
572 -41.930792951262035
573 -41.95892796332772
574 -41.98715268809608
575 -42.015449683033154
576 -42.04383255610255
577 -42.0723261818881
578 -42.10087171896223
579 -42.12937891585727
580 -42.15779221542894
581 -42.186192709156394
582 -42.21463239987528
583 -42.24297533850262
584 -42.27115776302875
585 -42.29923252980808
586 -42.327237054446215
587 -42.355158670323576
588 -42.38297413054799
589 -42.410689982894915
590 -42.4383181344353
591 -42.465874224247806
592 -42.49337531429497
593 -42.520851555852495
594 -42.548326646187235
595 -42.57580272065989
596 -42.60328848893886
597 -42.63080161325311
598 -42.65833397236029
599 -42.68580390195733
600 -42.71311831662397
601 -42.74024089979634
602 -42.76715337823212
603 -42.7938553572722
604 -42.820343249285095
605 -42.84661550215687
606 -42.87267395573611
607 -42.89859369181979
608 -42.92447238176829
609 -42.95029565059238
610 -42.97604266035546
611 -43.00181412447426
612 -43.02762502056243
613 -43.05345600534256
614 -43.0793594960502
615 -43.10528899522315
616 -43.13127667420072
617 -43.157334806239625
618 -43.18341771969501
619 -43.20958797148484
620 -43.2359294211711
621 -43.26243532772277
622 -43.28912944069765
623 -43.31607679226081
624 -43.343268416731284
625 -43.37069406992045
626 -43.39832919164
627 -43.42613898895042
628 -43.45406052973209
629 -43.48199768765157
630 -43.509901980075746
631 -43.53772389500516
632 -43.565389461609676
633 -43.59283088947884
634 -43.620041147824416
635 -43.647021721252386
636 -43.67378369614434
637 -43.7003602997984
638 -43.72673162127785
639 -43.75298422345862
640 -43.77922754710746
641 -43.8055027628883
642 -43.83184615695462
643 -43.85826753325822
644 -43.88474616107276
645 -43.91127837684543
646 -43.937892787136015
647 -43.964565012706466
648 -43.991202122039134
649 -44.01769686750271
650 -44.043947734482764
651 -44.06986210029441
652 -44.095354907182035
653 -44.120289993210385
654 -44.1445373811646
655 -44.16788858742977
656 -44.19015225431882
657 -44.21142106368045
658 -44.231827730923904
659 -44.25134144921893
660 -44.26991299402715
661 -44.28754679082101
662 -44.304255522020874
663 -44.31998888758579
664 -44.33479769391648
665 -44.348818425214
666 -44.36211931904082
667 -44.3747840894705
668 -44.3868935278852
669 -44.39852478856673
670 -44.40978170103513
671 -44.42075949995303
672 -44.43152368068499
673 -44.44213276454964
674 -44.45265057837525
675 -44.46314012013162
676 -44.473659975109996
677 -44.48421934839297
678 -44.494842458623054
679 -44.505583872846486
680 -44.51646372913535
681 -44.527484999101134
682 -44.53863857591096
683 -44.54992664115544
684 -44.56133466117626
685 -44.57281348031335
686 -44.584285506111335
687 -44.595644952745026
688 -44.60684823671925
689 -44.61789579479733
690 -44.62873055116197
691 -44.639320522033174
692 -44.64970021506662
693 -44.65981833219933
694 -44.66953207175993
695 -44.678869924878384
696 -44.68797097763715
697 -44.69685281207005
698 -44.70553313491225
699 -44.71406555759997
700 -44.722483286757424
701 -44.73077836173287
702 -44.73894295320288
703 -44.7469892773008
704 -44.75492214976055
705 -44.7627167728633
706 -44.77038756819947
707 -44.777949742045564
708 -44.78538784519706
709 -44.79274630178775
710 -44.800028513041966
711 -44.80720007974779
712 -44.81422143776237
713 -44.821054986274746
714 -44.82766696242902
715 -44.833999960095944
716 -44.84001514525694
717 -44.84566902622198
718 -44.85097424919971
719 -44.85600761134523
720 -44.86080163306946
721 -44.865386406170806
722 -44.869771857395556
723 -44.873965329529575
724 -44.87797339229242
725 -44.88179193744232
726 -44.88540742649324
727 -44.88882901217082
728 -44.892092211555166
729 -44.895206765938816
730 -44.89816312885058
731 -44.90096042088263
732 -44.90362190092718
733 -44.90617230659716
734 -44.90862876961767
735 -44.91099822788642
736 -44.91329910615943
737 -44.91556251766114
738 -44.917827821573546
739 -44.92011705482155
740 -44.92241826237245
741 -44.92472666083567
742 -44.92701632920309
743 -44.92925464579576
744 -44.931432504378435
745 -44.93353627850305
746 -44.935597218788295
747 -44.9376728969493
748 -44.93982646149251
749 -44.942097317921
750 -44.94448839996701


==> plotdata/satellite_constellation/sat_A2_r.tex <==
t r
0 6848.233953273979
1 6848.243232922559
2 6848.273941049351
3 6848.3300852569655
4 6848.415218697253
5 6848.53237744675
6 6848.684026254294
7 6848.872013732672
8 6849.097539818919
9 6849.3611345252775
10 6849.662648658263
11 6850.0012566695
12 6850.375471774052
13 6850.783173017481
14 6851.221639204449
15 6851.6876059832475
16 6852.177324844016
17 6852.686621886233
18 6853.21097677725
19 6853.74560352904
20 6854.285535973849
21 6854.8257162111595
22 6855.361084880686
23 6855.88667113598
24 6856.397680527242
25 6856.889580229434
26 6857.358176434201
27 6857.799687013188
28 6858.21079959682
29 6858.588756504944
30 6858.931415915483
31 6859.237240285948
32 6859.505346646394
33 6859.735529601368
34 6859.928243114704
35 6860.084620016849
36 6860.206435067487
37 6860.296070516472
38 6860.356483145281
39 6860.391143907988
40 6860.403981067133
41 6860.399310806552
42 6860.381756064951
43 6860.356171091885
44 6860.327542728973
45 6860.300919793009
46 6860.28132730299
47 6860.273656402803
48 6860.282588452254
49 6860.312508860303
50 6860.367427864421
51 6860.450499908191
52 6860.564678821328
53 6860.71273902511
54 6860.896078714745
55 6861.116137350357
56 6861.373662143775
57 6861.667471511422
58 6861.9970566586035
59 6862.361495250681
60 6862.7583497286305
61 6863.185025647268
62 6863.638833522515
63 6864.116578013472
64 6864.614241653642
65 6865.1280014223075
66 6865.653821532361
67 6866.1869192176955
68 6866.722367272062
69 6867.255215876553
70 6867.780585487904
71 6868.293715515767
72 6868.790043930226
73 6869.265325457041
74 6869.715702004345
75 6870.137706921089
76 6870.528420937599
77 6870.885536621028
78 6871.207279213313
79 6871.492499776259
80 6871.740687079369
81 6871.951982841126
82 6872.127179403905
83 6872.267726028532
84 6872.375681690292
85 6872.453670667039
86 6872.504838136849
87 6872.532808371423
88 6872.5416309788625
89 6872.535673806246
90 6872.519571471474
91 6872.498115785977
92 6872.476180130882
93 6872.4586895795865
94 6872.450509211555
95 6872.45631016
96 6872.480494152868
97 6872.527157973872
98 6872.600006670274
99 6872.702273356722
100 6872.83667512879
101 6873.005363742709
102 6873.209875260652
103 6873.451106642968
104 6873.72932922363
105 6874.04414864914
106 6874.394510269136
107 6874.778726992795
108 6875.194499005813
109 6875.638976095186
110 6876.10872850774
111 6876.599857902336
112 6877.1080521154045
113 6877.627617785989
114 6878.147492573662
115 6878.655212508168
116 6879.14062172419
117 6879.595855098301
118 6880.014361635967
119 6880.392447995837
120 6880.726548787831
121 6881.012754608046
122 6881.246277948368
123 6881.421911263097
124 6881.535567426365
125 6881.586442109401
126 6881.572321753985
127 6881.490255869566
128 6881.3390681701585
129 6881.120865085953
130 6880.837551657683
131 6880.491163755253
132 6880.084908387448
133 6879.62273630356
134 6879.109070081334
135 6878.549950420444
136 6877.951478614264
137 6877.320262557723
138 6876.663763625231
139 6875.990331550879
140 6875.3089233027185
141 6874.627844693001
142 6873.955213660332
143 6873.299182332171
144 6872.667670117028
145 6872.0681650625265
146 6871.507687707792
147 6870.992464494464
148 6870.528054725247
149 6870.1193913897205
150 6869.77053669377
151 6869.4845614647575
152 6869.263387510689
153 6869.107638081011
154 6869.016625613875
155 6868.9884619052855
156 6869.0201455319
157 6869.107365763503
158 6869.244537679954
159 6869.425296461379
160 6869.6426578096425
161 6869.88913044265
162 6870.157530746656
163 6870.441841713941
164 6870.733967186957
165 6871.02551633683
166 6871.308700008971
167 6871.576735066831
168 6871.824294034919
169 6872.046881334256
170 6872.241452984832
171 6872.407170498674
172 6872.5440584755515
173 6872.653085197386
174 6872.736176636909
175 6872.794483689509
176 6872.825797601568
177 6872.828791719898
178 6872.803233027613
179 6872.747510244056
180 6872.662266321313
181 6872.547843269061
182 6872.404162803711
183 6872.231162269522
184 6872.03086926751
185 6871.805110986391
186 6871.5557687913615
187 6871.2857916868115
188 6870.997545125393
189 6870.694075692081
190 6870.37836775645
191 6870.053844658545
192 6869.724171108313
193 6869.393295646525
194 6869.065446635784
195 6868.744155411834
196 6868.432659464737
197 6868.134159996536
198 6867.8516347682435
199 6867.588153509293
200 6867.345521239687
201 6867.124582044398
202 6866.927154485294
203 6866.753951626807
204 6866.606054816869
205 6866.48381082651
206 6866.387393802473
207 6866.316592271356
208 6866.270378312425
209 6866.247138108017
210 6866.2450999449975
211 6866.262243858604
212 6866.296241517693
213 6866.344618977359
214 6866.404236302627
215 6866.472079856756
216 6866.54540917263
217 6866.621411916211
218 6866.69699593853
219 6866.769351921658
220 6866.836028544119
221 6866.895073760888
222 6866.94504944325
223 6866.984986081968
224 6867.010030611557
225 6867.0168122688865
226 6867.005869272751
227 6866.974604385776
228 6866.926189371007
229 6866.865619413375
230 6866.797673704331
231 6866.726566493728
232 6866.655510681801
233 6866.586884162612
234 6866.5214225583595
235 6866.45921368786
236 6866.400918103144
237 6866.346551118055
238 6866.294636416345
239 6866.2452161319825
240 6866.198517867752
241 6866.153829512993
242 6866.110561916287
243 6866.0682818723535
244 6866.026859765952
245 6865.987288312617
246 6865.950064929184
247 6865.914918622854
248 6865.881514176323
249 6865.849357030732
250 6865.818029162208
251 6865.787319886539
252 6865.75695254784
253 6865.726509274689
254 6865.695689837177
255 6865.6642175010475
256 6865.632250459609
257 6865.600147323245
258 6865.567263827597
259 6865.532389877649
260 6865.496594060644
261 6865.45996806749
262 6865.421411180589
263 6865.382033199775
264 6865.342768123604
265 6865.3044622942025
266 6865.2677549498185
267 6865.23249977545
268 6865.1965814636515
269 6865.161124037158
270 6865.127452210803
271 6865.095718327025
272 6865.065671880413
273 6865.037138670046
274 6865.010687272197
275 6864.985730256218
276 6864.962741752404
277 6864.941041946689
278 6864.919511060322
279 6864.898282094963
280 6864.8780347350785
281 6864.858466002451
282 6864.8392717468605
283 6864.820107012789
284 6864.801458596773
285 6864.782107005925
286 6864.744214121888
287 6864.6805024910645
288 6864.6032213779135
289 6864.520800781813
290 6864.439561560021
291 6864.362234089637
292 6864.288465505106
293 6864.221690045796
294 6864.164708960445
295 6864.118714047856
296 6864.083549266688
297 6864.058639447834
298 6864.04332059619
299 6864.037070291753
300 6864.039086444127
301 6864.048720720919
302 6864.065753994042
303 6864.089527540724
304 6864.1183260334565
305 6864.150684315656
306 6864.185611237485
307 6864.221941548268
308 6864.257474632176
309 6864.29170192751
310 6864.324200848452
311 6864.353952995448
312 6864.38069351122
313 6864.403294027319
314 6864.420938794586
315 6864.433157458829
316 6864.439802011283
317 6864.44098505403
318 6864.437013031442
319 6864.428386580251
320 6864.415412341337
321 6864.399207992398
322 6864.3822137952675
323 6864.364578431643
324 6864.347746277866
325 6864.332170892883
326 6864.317760349454
327 6864.30435424936
328 6864.2918845946715
329 6864.280221437653
330 6864.269321035303
331 6864.258969196712
332 6864.24903727275
333 6864.239432876266
334 6864.230189627769
335 6864.221345460517
336 6864.21309963899
337 6864.205736392032
338 6864.199330422792
339 6864.193811707649
340 6864.188980166058
341 6864.184601353306
342 6864.180527499549
343 6864.176594143263
344 6864.172586724974
345 6864.168131706989
346 6864.163085877106
347 6864.157434877315
348 6864.151145310844
349 6864.144087263433
350 6864.13614318703
351 6864.12738937853
352 6864.117930249603
353 6864.107723023279
354 6864.096776007234
355 6864.085321307661
356 6864.07357380227
357 6864.0616238225575
358 6864.049599468058
359 6864.037611710773
360 6864.025763876783
361 6864.014159857466
362 6864.002911613291
363 6863.992110271071
364 6863.981789229063
365 6863.97196476204
366 6863.962654667432
367 6863.9538809444575
368 6863.945674802027
369 6863.938089881422
370 6863.931134958775
371 6863.924794475557
372 6863.918947987014
373 6863.9133522416505
374 6863.9083480333675
375 6863.903657272674
376 6863.899233682869
377 6863.894674777799
378 6863.890308939432
379 6863.886201872405
380 6863.882366502243
381 6863.878536537862
382 6863.874593129888
383 6863.869330674743
384 6863.861781513083
385 6863.853584236286
386 6863.843848977777
387 6863.834131894352
388 6863.824040678375
389 6863.812918550139
390 6863.7993444109
391 6863.784380745839
392 6863.769621072186
393 6863.7531059052835
394 6863.734935975327
395 6863.718424124365
396 6863.701319624135
397 6863.683011628631
398 6863.666026400388
399 6863.648836111236
400 6863.630802253764
401 6863.615176470901
402 6863.604148519572
403 6863.599910757898
404 6863.602785308905
405 6863.612268152872
406 6863.625025257108
407 6863.6357620863655
408 6863.645685916966
409 6863.654857668261
410 6863.664464270572
411 6863.675849807963
412 6863.688941827668
413 6863.700975014319
414 6863.710634083736
415 6863.7163680662725
416 6863.720907423235
417 6863.725265300882
418 6863.729032590296
419 6863.730424734516
420 6863.726888046155
421 6863.717884486638
422 6863.706231677912
423 6863.694951288664
424 6863.683674245155
425 6863.6716579020285
426 6863.660131603742
427 6863.648717954418
428 6863.635889287855
429 6863.620416866955
430 6863.60085235306
431 6863.579444617683
432 6863.556843598144
433 6863.536208361152
434 6863.522560139827
435 6863.518323123449
436 6863.522986155703
437 6863.535136023493
438 6863.553338144873
439 6863.57660209897
440 6863.602385716973
441 6863.623875403065
442 6863.625166306038
443 6863.601105047502
444 6863.558694627548
445 6863.497863216683
446 6863.408846418923
447 6863.281151402147
448 6863.120480704597
449 6862.9354644888745
450 6862.7221047084595
451 6862.482281787353
452 6862.224747181977
453 6861.9584975805
454 6861.697070751942
455 6861.447773733253
456 6861.216051197939
457 6861.010327101109
458 6860.841205671993
459 6860.715034721165
460 6860.638816610883
461 6860.617924805454
462 6860.649566779879
463 6860.733584428729
464 6860.867847321653
465 6861.046369566759
466 6861.26358400313
467 6861.511281192708
468 6861.7813068999185
469 6862.0674094295
470 6862.361851136019
471 6862.655751768926
472 6862.941972289143
473 6863.218120874164
474 6863.482463300054
475 6863.731745587817
476 6863.963296392763
477 6864.175208464298
478 6864.366490047573
479 6864.535285684961
480 6864.682529050736
481 6864.807469648467
482 6864.91066452644
483 6864.9962082473985
484 6865.065046285016
485 6865.117057322096
486 6865.152650808054
487 6865.170713275681
488 6865.168715501335
489 6865.145442713934
490 6865.101925139244
491 6865.036941636612
492 6864.953889016284
493 6864.851880677914
494 6864.732378564479
495 6864.594255524616
496 6864.4413527370325
497 6864.285906727349
498 6864.135257140208
499 6863.996030719819
500 6863.872458831186
501 6863.7674671541945
502 6863.682126547326
503 6863.61680325418
504 6863.57114537398
505 6863.543643577838
506 6863.529341976803
507 6863.529824626697
508 6863.547229842626
509 6863.5773229153965
510 6863.615061458163
511 6863.659102936235
512 6863.709964338664
513 6863.766761258505
514 6863.830063019985
515 6863.898981885929
516 6863.972036656287
517 6864.047928459474
518 6864.125324695909
519 6864.203116529286
520 6864.2792475033
521 6864.351950489117
522 6864.418968844375
523 6864.476643274065
524 6864.522922478833
525 6864.560336200622
526 6864.59131169699
527 6864.612963203153
528 6864.622636767012
529 6864.625336690318
530 6864.608281322487
531 6864.569847810566
532 6864.527151177054
533 6864.482928210925
534 6864.436303792501
535 6864.389770106578
536 6864.342860705377
537 6864.297138005951
538 6864.252322849976
539 6864.21081362709
540 6864.173699700022
541 6864.14379292489
542 6864.121485164373
543 6864.1064990988725
544 6864.098650028997
545 6864.097953487898
546 6864.1042048945
547 6864.117002162878
548 6864.132677996891
549 6864.147125197185
550 6864.157978949603
551 6864.161460273154
552 6864.15689431053
553 6864.136763407367
554 6864.104674601431
555 6864.072341408554
556 6864.043126473122
557 6864.0191583044925
558 6864.0010243838315
559 6863.988672478286
560 6863.981853866577
561 6863.980095869691
562 6863.982749929899
563 6863.989114478332
564 6863.998470538063
565 6864.01043794136
566 6864.024964894307
567 6864.040748573136
568 6864.054360745242
569 6864.063807254289
570 6864.069175103035
571 6864.071266138619
572 6864.071673990229
573 6864.070313770489
574 6864.067161694936
575 6864.062262063563
576 6864.055683346686
577 6864.047680353925
578 6864.037408067696
579 6864.023940603238
580 6864.009669665419
581 6863.996749529123
582 6863.98372614786
583 6863.970316422867
584 6863.959364821033
585 6863.952195862715
586 6863.948084962336
587 6863.946191844256
588 6863.946435514573
589 6863.9490490698945
590 6863.954119931322
591 6863.961588923044
592 6863.971270879435
593 6863.98285799743
594 6863.995890396992
595 6864.009758343259
596 6864.023601873175
597 6864.035847327139
598 6864.044265344825
599 6864.047032568116
600 6864.043304428031
601 6864.033042790535
602 6864.016725309906
603 6863.995187118846
604 6863.969456132955
605 6863.940586859935
606 6863.909541139216
607 6863.877215281184
608 6863.844378721603
609 6863.811649842721
610 6863.778975239882
611 6863.7452615177535
612 6863.710144751261
613 6863.672619290273
614 6863.632411108944
615 6863.589167396684
616 6863.543933339532
617 6863.497020829286
618 6863.451296367009
619 6863.41087263727
620 6863.378586054711
621 6863.356321132494
622 6863.346880889198
623 6863.350255740628
624 6863.365717301832
625 6863.391279684246
626 6863.425339233953
627 6863.466673999779
628 6863.514110258932
629 6863.5667251574205
630 6863.623421645788
631 6863.682253760526
632 6863.741661844904
633 6863.800416071699
634 6863.8581457632445
635 6863.913109080913
636 6863.965484908332
637 6864.013991372028
638 6864.057378351361
639 6864.0942720666135
640 6864.121154712928
641 6864.133903148635
642 6864.1282697754295
643 6864.100922222278
644 6864.04924150967
645 6863.97127218454
646 6863.864009155455
647 6863.7159464089145
648 6863.518734783789
649 6863.275805276249
650 6862.991632497217
651 6862.666613248818
652 6862.294985763852
653 6861.88443893984
654 6861.44706423912
655 6860.986866708579
656 6860.515829296922
657 6860.044905795183
658 6859.573268521477
659 6859.099268155835
660 6858.632927733502
661 6858.1798850092855
662 6857.738868888932
663 6857.31826242189
664 6856.928066883138
665 6856.571688158668
666 6856.251434892763
667 6855.968763498676
668 6855.724575492046
669 6855.518855363152
670 6855.3506419309615
671 6855.217952046743
672 6855.1177771895045
673 6855.0466273604
674 6855.000997617551
675 6854.977283202488
676 6854.971961533079
677 6854.980051783564
678 6854.996393853837
679 6855.01521956595
680 6855.030466301554
681 6855.036870109581
682 6855.032902966852
683 6855.017980812053
684 6854.984580837973
685 6854.927658380607
686 6854.848236405886
687 6854.746808031519
688 6854.621475781399
689 6854.474172536849
690 6854.309547205297
691 6854.130084244669
692 6853.9357785554785
693 6853.727413548466
694 6853.511668811207
695 6853.295002130481
696 6853.080785106848
697 6852.8729286992075
698 6852.675245677729
699 6852.488962755621
700 6852.315174035673
701 6852.1551530806455
702 6852.009100593845
703 6851.87475994148
704 6851.74818715304
705 6851.628855367989
706 6851.523494652223
707 6851.435431802893
708 6851.362777463985
709 6851.303300845206
710 6851.254037064783
711 6851.211786850495
712 6851.173452185405
713 6851.13628208953
714 6851.098996532439
715 6851.055102824473
716 6851.0040083701215
717 6850.951915884324
718 6850.900068648398
719 6850.846918689633
720 6850.79152553667
721 6850.733333223427
722 6850.672014107442
723 6850.608512608797
724 6850.542634600273
725 6850.473306684718
726 6850.402017182359
727 6850.329519095122
728 6850.256778066449
729 6850.183998672327
730 6850.109906315286
731 6850.035341884341
732 6849.960063112776
733 6849.883436224012
734 6849.80579484687
735 6849.727340517852
736 6849.648261618504
737 6849.568762531649
738 6849.489362765715
739 6849.407508957441
740 6849.320651256552
741 6849.2288808171725
742 6849.138162294914
743 6849.056059658692
744 6848.984868733341
745 6848.927442302173
746 6848.8851825589345
747 6848.859677014746
748 6848.85158654417
749 6848.857619125335
750 6848.874622910209


==> plotdata/satellite_constellation/sat_A3_dtheta.tex <==
t dtheta
0 0.0
1 0.0
2 0.0
3 0.0
4 0.0
5 0.0
6 0.0
7 0.0
8 0.0
9 0.0
10 0.0
11 0.0
12 0.0
13 0.0
14 0.0
15 0.0
16 0.0
17 0.0
18 0.0
19 0.0
20 0.0
21 0.0
22 0.0
23 0.0
24 0.0
25 0.0
26 0.0
27 0.0
28 0.0
29 0.0
30 0.0
31 0.0
32 0.0
33 0.0
34 0.0
35 0.0
36 0.0
37 0.0
38 0.0
39 0.0
40 0.0
41 0.0
42 0.0
43 0.0
44 0.0
45 0.0
46 0.0
47 0.0
48 0.0
49 0.0
50 0.0
51 0.0
52 0.0
53 0.0
54 0.0
55 0.0
56 0.0
57 0.0
58 0.0
59 0.0
60 0.0
61 0.0
62 0.0
63 0.0
64 0.0
65 0.0
66 0.0
67 0.0
68 0.0
69 0.0
70 0.0
71 0.0
72 0.0
73 0.0
74 0.0
75 0.0
76 0.0
77 0.0
78 0.0
79 0.0
80 0.0
81 0.0
82 0.0
83 0.0
84 0.0
85 0.0
86 0.0
87 0.0
88 0.0
89 0.0
90 0.0
91 0.0
92 0.0
93 0.0
94 0.0
95 0.0
96 0.0
97 0.0
98 0.0
99 0.0
100 0.0
101 0.0
102 0.0
103 0.0
104 0.0
105 0.0
106 0.0
107 0.0
108 0.0
109 0.0
110 0.0
111 0.0
112 0.0
113 0.0
114 0.0
115 0.0
116 0.0
117 0.0
118 0.0
119 0.0
120 0.0
121 0.0
122 0.0
123 0.0
124 0.0
125 0.0
126 0.0
127 0.0
128 0.0
129 0.0
130 0.0
131 0.0
132 0.0
133 0.0
134 0.0
135 0.0
136 0.0
137 0.0
138 0.0
139 0.0
140 0.0
141 0.0
142 0.0
143 0.0
144 0.0
145 0.0
146 0.0
147 0.0
148 0.0
149 0.0
150 0.0
151 0.0
152 0.0
153 0.0
154 0.0
155 0.0
156 0.0
157 0.0
158 0.0
159 0.0
160 0.0
161 0.0
162 0.0
163 0.0
164 0.0
165 0.0
166 0.0
167 0.0
168 0.0
169 0.0
170 0.0
171 0.0
172 0.0
173 0.0
174 0.0
175 0.0
176 0.0
177 0.0
178 0.0
179 0.0
180 0.0
181 0.0
182 0.0
183 0.0
184 0.0
185 0.0
186 0.0
187 0.0
188 0.0
189 0.0
190 0.0
191 0.0
192 0.0
193 0.0
194 0.0
195 0.0
196 0.0
197 0.0
198 0.0
199 0.0
200 0.0
201 0.0
202 0.0
203 0.0
204 0.0
205 0.0
206 0.0
207 0.0
208 0.0
209 0.0
210 0.0
211 0.0
212 0.0
213 0.0
214 0.0
215 0.0
216 0.0
217 0.0
218 0.0
219 0.0
220 0.0
221 0.0
222 0.0
223 0.0
224 0.0
225 0.0
226 0.0
227 0.0
228 0.0
229 0.0
230 0.0
231 0.0
232 0.0
233 0.0
234 0.0
235 0.0
236 0.0
237 0.0
238 0.0
239 0.0
240 0.0
241 0.0
242 0.0
243 0.0
244 0.0
245 0.0
246 0.0
247 0.0
248 0.0
249 0.0
250 0.0
251 0.0
252 0.0
253 0.0
254 0.0
255 0.0
256 0.0
257 0.0
258 0.0
259 0.0
260 0.0
261 0.0
262 0.0
263 0.0
264 0.0
265 0.0
266 0.0
267 0.0
268 0.0
269 0.0
270 0.0
271 0.0
272 0.0
273 0.0
274 0.0
275 0.0
276 0.0
277 0.0
278 0.0
279 0.0
280 0.0
281 0.0
282 0.0
283 0.0
284 0.0
285 0.0
286 0.0
287 0.0
288 0.0
289 0.0
290 0.0
291 0.0
292 0.0
293 0.0
294 0.0
295 0.0
296 0.0
297 0.0
298 0.0
299 0.0
300 0.0
301 0.0
302 0.0
303 0.0
304 0.0
305 0.0
306 0.0
307 0.0
308 0.0
309 0.0
310 0.0
311 0.0
312 0.0
313 0.0
314 0.0
315 0.0
316 0.0
317 0.0
318 0.0
319 0.0
320 0.0
321 0.0
322 0.0
323 0.0
324 0.0
325 0.0
326 0.0
327 0.0
328 0.0
329 0.0
330 0.0
331 0.0
332 0.0
333 0.0
334 0.0
335 0.0
336 0.0
337 0.0
338 0.0
339 0.0
340 0.0
341 0.0
342 0.0
343 0.0
344 0.0
345 0.0
346 0.0
347 0.0
348 0.0
349 0.0
350 0.0
351 0.0
352 0.0
353 0.0
354 0.0
355 0.0
356 0.0
357 0.0
358 0.0
359 0.0
360 0.0
361 0.0
362 0.0
363 0.0
364 0.0
365 0.0
366 0.0
367 0.0
368 0.0
369 0.0
370 0.0
371 0.0
372 0.0
373 0.0
374 0.0
375 0.0
376 0.0
377 0.0
378 0.0
379 0.0
380 0.0
381 0.0
382 0.0
383 0.0
384 0.0
385 0.0
386 0.0
387 0.0
388 0.0
389 0.0
390 0.0
391 0.0
392 0.0
393 0.0
394 0.0
395 0.0
396 0.0
397 0.0
398 0.0
399 0.0
400 0.0
401 0.0
402 0.0
403 0.0
404 0.0
405 0.0
406 0.0
407 0.0
408 0.0
409 0.0
410 0.0
411 0.0
412 0.0
413 0.0
414 0.0
415 0.0
416 0.0
417 0.0
418 0.0
419 0.0
420 0.0
421 0.0
422 0.0
423 0.0
424 0.0
425 0.0
426 0.0
427 0.0
428 0.0
429 0.0
430 0.0
431 0.0
432 0.0
433 0.0
434 0.0
435 0.0
436 0.0
437 0.0
438 0.0
439 0.0
440 0.0
441 0.0
442 0.0
443 0.0
444 0.0
445 0.0
446 0.0
447 0.0
448 0.0
449 0.0
450 0.0
451 0.0
452 0.0
453 0.0
454 0.0
455 0.0
456 0.0
457 0.0
458 0.0
459 0.0
460 0.0
461 0.0
462 0.0
463 0.0
464 0.0
465 0.0
466 0.0
467 0.0
468 0.0
469 0.0
470 0.0
471 0.0
472 0.0
473 0.0
474 0.0
475 0.0
476 0.0
477 0.0
478 0.0
479 0.0
480 0.0
481 0.0
482 0.0
483 0.0
484 0.0
485 0.0
486 0.0
487 0.0
488 0.0
489 0.0
490 0.0
491 0.0
492 0.0
493 0.0
494 0.0
495 0.0
496 0.0
497 0.0
498 0.0
499 0.0
500 0.0
501 0.0
502 0.0
503 0.0
504 0.0
505 0.0
506 0.0
507 0.0
508 0.0
509 0.0
510 0.0
511 0.0
512 0.0
513 0.0
514 0.0
515 0.0
516 0.0
517 0.0
518 0.0
519 0.0
520 0.0
521 0.0
522 0.0
523 0.0
524 0.0
525 0.0
526 0.0
527 0.0
528 0.0
529 0.0
530 0.0
531 0.0
532 0.0
533 0.0
534 0.0
535 0.0
536 0.0
537 0.0
538 0.0
539 0.0
540 0.0
541 0.0
542 0.0
543 0.0
544 0.0
545 0.0
546 0.0
547 0.0
548 0.0
549 0.0
550 0.0
551 0.0
552 0.0
553 0.0
554 0.0
555 0.0
556 0.0
557 0.0
558 0.0
559 0.0
560 0.0
561 0.0
562 0.0
563 0.0
564 0.0
565 0.0
566 0.0
567 0.0
568 0.0
569 0.0
570 0.0
571 0.0
572 0.0
573 0.0
574 0.0
575 0.0
576 0.0
577 0.0
578 0.0
579 0.0
580 0.0
581 0.0
582 0.0
583 0.0
584 0.0
585 0.0
586 0.0
587 0.0
588 0.0
589 0.0
590 0.0
591 0.0
592 0.0
593 0.0
594 0.0
595 0.0
596 0.0
597 0.0
598 0.0
599 0.0
600 0.0
601 0.0
602 0.0
603 0.0
604 0.0
605 0.0
606 0.0
607 0.0
608 0.0
609 0.0
610 0.0
611 0.0
612 0.0
613 0.0
614 0.0
615 0.0
616 0.0
617 0.0
618 0.0
619 0.0
620 0.0
621 0.0
622 0.0
623 0.0
624 0.0
625 0.0
626 0.0
627 0.0
628 0.0
629 0.0
630 0.0
631 0.0
632 0.0
633 0.0
634 0.0
635 0.0
636 0.0
637 0.0
638 0.0
639 0.0
640 0.0
641 0.0
642 0.0
643 0.0
644 0.0
645 0.0
646 0.0
647 0.0
648 0.0
649 0.0
650 0.0
651 0.0
652 0.0
653 0.0
654 0.0
655 0.0
656 0.0
657 0.0
658 0.0
659 0.0
660 0.0
661 0.0
662 0.0
663 0.0
664 0.0
665 0.0
666 0.0
667 0.0
668 0.0
669 0.0
670 0.0
671 0.0
672 0.0
673 0.0
674 0.0
675 0.0
676 0.0
677 0.0
678 0.0
679 0.0
680 0.0
681 0.0
682 0.0
683 0.0
684 0.0
685 0.0
686 0.0
687 0.0
688 0.0
689 0.0
690 0.0
691 0.0
692 0.0
693 0.0
694 0.0
695 0.0
696 0.0
697 0.0
698 0.0
699 0.0
700 0.0
701 0.0
702 0.0
703 0.0
704 0.0
705 0.0
706 0.0
707 0.0
708 0.0
709 0.0
710 0.0
711 0.0
712 0.0
713 0.0
714 0.0
715 0.0
716 0.0
717 0.0
718 0.0
719 0.0
720 0.0
721 0.0
722 0.0
723 0.0
724 0.0
725 0.0
726 0.0
727 0.0
728 0.0
729 0.0
730 0.0
731 0.0
732 0.0
733 0.0
734 0.0
735 0.0
736 0.0
737 0.0
738 0.0
739 0.0
740 0.0
741 0.0
742 0.0
743 0.0
744 0.0
745 0.0
746 0.0
747 0.0
748 0.0
749 0.0
750 0.0
751 0.0
752 0.0
753 0.0
754 0.0
755 0.0
756 0.0
757 0.0
758 0.0
759 0.0
760 0.0
761 0.0
762 0.0
763 0.0
764 0.0
765 0.0
766 0.0
767 0.0
768 0.0
769 0.0
770 0.0
771 0.0
772 0.0
773 0.0
774 0.0
775 0.0
776 0.0
777 0.0
778 0.0
779 0.0
780 0.0
781 0.0
782 0.0
783 0.0
784 0.0
785 0.0
786 0.0
787 0.0
788 0.0
789 0.0
790 0.0
791 0.0
792 0.0
793 0.0
794 0.0
795 0.0
796 0.0
797 0.0
798 0.0
799 0.0
800 0.0
801 0.0
802 0.0
803 0.0
804 0.0
805 0.0
806 0.0
807 0.0
808 0.0
809 0.0
810 0.0
811 0.0
812 0.0
813 0.0
814 0.0
815 0.0
816 0.0
817 0.0
818 0.0
819 0.0
820 0.0
821 0.0
822 0.0
823 0.0
824 0.0
825 0.0
826 0.0
827 0.0
828 0.0
829 0.0
830 0.0
831 0.0
832 0.0
833 0.0
834 0.0
835 0.0
836 0.0
837 0.0
838 0.0
839 0.0
840 0.0
841 0.0
842 0.0
843 0.0
844 0.0
845 0.0
846 0.0
847 0.0
848 0.0
849 0.0
850 0.0
851 0.0
852 0.0
853 0.0
854 0.0
855 0.0
856 0.0
857 0.0
858 0.0
859 0.0
860 0.0
861 0.0
862 0.0
863 0.0
864 0.0
865 0.0
866 0.0
867 0.0
868 0.0
869 0.0
870 0.0
871 0.0
872 0.0
873 0.0
874 0.0
875 0.0
876 0.0
877 0.0
878 0.0
879 0.0
880 0.0
881 0.0
882 0.0
883 0.0
884 0.0
885 0.0
886 0.0
887 0.0
888 0.0
889 0.0
890 0.0
891 0.0
892 0.0
893 0.0
894 0.0
895 0.0
896 0.0
897 0.0
898 0.0
899 0.0
900 0.0
901 0.0
902 0.0
903 0.0
904 0.0
905 0.0
906 0.0
907 0.0
908 0.0
909 0.0
910 0.0
911 0.0
912 0.0
913 0.0
914 0.0
915 0.0
916 0.0
917 0.0
918 0.0
919 0.0
920 0.0
921 0.0
922 0.0
923 0.0
924 0.0
925 0.0
926 0.0
927 0.0
928 0.0
929 0.0
930 0.0
931 0.0
932 0.0
933 0.0
934 0.0
935 0.0
936 0.0
937 0.0
938 0.0
939 0.0
940 0.0
941 0.0
942 0.0
943 0.0
944 0.0
945 0.0
946 0.0
947 0.0
948 0.0
949 0.0
950 0.0
951 0.0
952 0.0
953 0.0
954 0.0
955 0.0
956 0.0
957 0.0
958 0.0
959 0.0
960 0.0
961 0.0
962 0.0
963 0.0
964 0.0
965 0.0
966 0.0
967 0.0
968 0.0
969 0.0
970 0.0
971 0.0
972 0.0
973 0.0
974 0.0
975 0.0
976 0.0
977 0.0
978 0.0
979 0.0
980 0.0
981 0.0
982 0.0
983 0.0
984 0.0
985 0.0
986 0.0
987 0.0
988 0.0
989 0.0
990 0.0
991 0.0
992 0.0
993 0.0
994 0.0
995 0.0
996 0.0
997 0.0
998 0.0
999 0.0
1000 0.0
1001 0.0
1002 0.0
1003 0.0
1004 0.0
1005 0.0
1006 0.0
1007 0.0
1008 0.0
1009 0.0
1010 0.0
1011 0.0
1012 0.0
1013 0.0
1014 0.0
1015 0.0
1016 0.0
1017 0.0
1018 0.0
1019 0.0
1020 0.0
1021 0.0
1022 0.0
1023 0.0
1024 0.0
1025 0.0
1026 0.0
1027 0.0
1028 0.0
1029 0.0
1030 0.0
1031 0.0
1032 0.0
1033 0.0
1034 0.0
1035 0.0
1036 0.0
1037 0.0
1038 0.0
1039 0.0
1040 0.0
1041 0.0
1042 0.0
1043 0.0
1044 0.0
1045 0.0
1046 0.0
1047 0.0
1048 0.0
1049 0.0
1050 0.0
1051 0.0
1052 0.0
1053 0.0
1054 0.0
1055 0.0
1056 0.0
1057 0.0
1058 0.0
1059 0.0
1060 0.0
1061 0.0
1062 0.0
1063 0.0
1064 0.0
1065 0.0
1066 0.0
1067 0.0
1068 0.0
1069 0.0
1070 0.0
1071 0.0
1072 0.0
1073 0.0
1074 0.0
1075 0.0
1076 0.0
1077 0.0
1078 0.0
1079 0.0
1080 0.0
1081 0.0
1082 0.0
1083 0.0
1084 0.0
1085 0.0
1086 0.0
1087 0.0
1088 0.0
1089 0.0
1090 0.0
1091 0.0
1092 0.0
1093 0.0
1094 0.0
1095 0.0
1096 0.0
1097 0.0
1098 0.0
1099 0.0
1100 0.0
1101 0.0
1102 0.0
1103 0.0
1104 0.0
1105 0.0
1106 0.0
1107 0.0
1108 0.0
1109 0.0
1110 0.0
1111 0.0
1112 0.0
1113 0.0
1114 0.0
1115 0.0
1116 0.0
1117 0.0
1118 0.0
1119 0.0
1120 0.0
1121 0.0
1122 0.0
1123 0.0
1124 0.0
1125 0.0
1126 0.0
1127 0.0
1128 0.0
1129 0.0
1130 0.0
1131 0.0
1132 0.0
1133 0.0
1134 0.0
1135 0.0
1136 0.0
1137 0.0
1138 0.0
1139 0.0
1140 0.0
1141 0.0
1142 0.0
1143 0.0
1144 0.0
1145 0.0
1146 0.0
1147 0.0
1148 0.0
1149 0.0
1150 0.0
1151 0.0
1152 0.0
1153 0.0
1154 0.0
1155 0.0
1156 0.0
1157 0.0
1158 0.0
1159 0.0
1160 0.0
1161 0.0
1162 0.0
1163 0.0
1164 0.0
1165 0.0
1166 0.0
1167 0.0
1168 0.0
1169 0.0
1170 0.0
1171 0.0
1172 0.0
1173 0.0
1174 0.0
1175 0.0
1176 0.0
1177 0.0
1178 0.0
1179 0.0
1180 0.0
1181 0.0
1182 0.0
1183 0.0
1184 0.0
1185 0.0
1186 0.0
1187 0.0
1188 0.0
1189 0.0
1190 0.0
1191 0.0
1192 0.0
1193 0.0
1194 0.0
1195 0.0
1196 0.0
1197 0.0
1198 0.0
1199 0.0
1200 0.0
1201 0.0
1202 0.0
1203 0.0
1204 0.0
1205 0.0
1206 0.0
1207 0.0
1208 0.0
1209 0.0
1210 0.0
1211 0.0
1212 0.0
1213 0.0
1214 0.0
1215 0.0
1216 0.0
1217 0.0
1218 0.0
1219 0.0
1220 0.0
1221 0.0
1222 0.0
1223 0.0
1224 0.0
1225 0.0
1226 0.0
1227 0.0
1228 0.0
1229 0.0
1230 0.0
1231 0.0
1232 0.0
1233 0.0
1234 0.0
1235 0.0
1236 0.0
1237 0.0
1238 0.0
1239 0.0
1240 0.0
1241 0.0
1242 0.0
1243 0.0
1244 0.0
1245 0.0
1246 0.0
1247 0.0
1248 0.0
1249 0.0
1250 0.0
1251 0.0
1252 0.0
1253 0.0
1254 0.0
1255 0.0
1256 0.0
1257 0.0
1258 0.0
1259 0.0
1260 0.0
1261 0.0
1262 0.0
1263 0.0
1264 0.0
1265 0.0
1266 0.0
1267 0.0
1268 0.0
1269 0.0
1270 0.0
1271 0.0
1272 0.0
1273 0.0
1274 0.0
1275 0.0
1276 0.0
1277 0.0
1278 0.0
1279 0.0
1280 0.0
1281 0.0
1282 0.0
1283 0.0
1284 0.0
1285 0.0
1286 0.0
1287 0.0
1288 0.0
1289 0.0
1290 0.0
1291 0.0
1292 0.0
1293 0.0
1294 0.0
1295 0.0
1296 0.0
1297 0.0
1298 0.0
1299 0.0
1300 0.0
1301 0.0
1302 0.0
1303 0.0
1304 0.0
1305 0.0
1306 0.0
1307 0.0
1308 0.0
1309 0.0
1310 0.0
1311 0.0
1312 0.0
1313 0.0
1314 0.0
1315 0.0
1316 0.0
1317 0.0
1318 0.0
1319 0.0
1320 0.0
1321 0.0
1322 0.0
1323 0.0
1324 0.0
1325 0.0
1326 0.0
1327 0.0
1328 0.0
1329 0.0
1330 0.0
1331 0.0
1332 0.0
1333 0.0
1334 0.0
1335 0.0
1336 0.0
1337 0.0
1338 0.0
1339 0.0
1340 0.0
1341 0.0
1342 0.0
1343 0.0
1344 0.0
1345 0.0
1346 0.0
1347 0.0
1348 0.0
1349 0.0
1350 0.0
1351 0.0
1352 0.0
1353 0.0
1354 0.0
1355 0.0
1356 0.0
1357 0.0
1358 0.0
1359 0.0
1360 0.0
1361 0.0
1362 0.0
1363 0.0
1364 0.0
1365 0.0
1366 0.0
1367 0.0
1368 0.0
1369 0.0
1370 0.0
1371 0.0
1372 0.0
1373 0.0
1374 0.0
1375 0.0
1376 0.0
1377 0.0
1378 0.0
1379 0.0
1380 0.0
1381 0.0
1382 0.0
1383 0.0
1384 0.0
1385 0.0
1386 0.0
1387 0.0
1388 0.0
1389 0.0
1390 0.0
1391 0.0
1392 0.0
1393 0.0
1394 0.0
1395 0.0
1396 0.0
1397 0.0
1398 0.0
1399 0.0
1400 0.0
1401 0.0
1402 0.0
1403 0.0
1404 0.0
1405 0.0
1406 0.0
1407 0.0
1408 0.0
1409 0.0
1410 0.0
1411 0.0
1412 0.0
1413 0.0
1414 0.0
1415 0.0
1416 0.0
1417 0.0
1418 0.0
1419 0.0
1420 0.0
1421 0.0
1422 0.0
1423 0.0
1424 0.0
1425 0.0
1426 0.0
1427 0.0
1428 0.0
1429 0.0
1430 0.0
1431 0.0
1432 0.0
1433 0.0
1434 0.0
1435 0.0
1436 0.0
1437 0.0
1438 0.0
1439 0.0
1440 0.0
1441 0.0
1442 0.0
1443 0.0
1444 0.0
1445 0.0
1446 0.0
1447 0.0
1448 0.0
1449 0.0
1450 0.0
1451 0.0
1452 0.0
1453 0.0
1454 0.0
1455 0.0
1456 0.0
1457 0.0
1458 0.0
1459 0.0
1460 0.0
1461 0.0
1462 0.0
1463 0.0
1464 0.0
1465 0.0
1466 0.0
1467 0.0
1468 0.0
1469 0.0
1470 0.0
1471 0.0
1472 0.0
1473 0.0
1474 0.0
1475 0.0
1476 0.0
1477 0.0
1478 0.0
1479 0.0
1480 0.0
1481 0.0
1482 0.0
1483 0.0
1484 0.0
1485 0.0
1486 0.0
1487 0.0
1488 0.0
1489 0.0
1490 0.0
1491 0.0
1492 0.0
1493 0.0
1494 0.0
1495 0.0
1496 0.0
1497 0.0
1498 0.0
1499 0.0
1500 0.0
1501 0.0
1502 0.0
1503 0.0
1504 0.0
1505 0.0
1506 0.0
1507 0.0
1508 0.0
1509 0.0
1510 0.0
1511 0.0
1512 0.0
1513 0.0
1514 0.0
1515 0.0
1516 0.0
1517 0.0
1518 0.0
1519 0.0
1520 0.0
1521 0.0
1522 0.0
1523 0.0
1524 0.0
1525 0.0
1526 0.0
1527 0.0
1528 0.0
1529 0.0
1530 0.0
1531 0.0
1532 0.0
1533 0.0
1534 0.0
1535 0.0
1536 0.0
1537 0.0
1538 0.0
1539 0.0
1540 0.0
1541 0.0
1542 0.0
1543 0.0
1544 0.0
1545 0.0
1546 0.0
1547 0.0
1548 0.0
1549 0.0
1550 0.0
1551 0.0
1552 0.0
1553 0.0
1554 0.0
1555 0.0
1556 0.0
1557 0.0
1558 0.0
1559 0.0
1560 0.0
1561 0.0
1562 0.0
1563 0.0
1564 0.0
1565 0.0
1566 0.0
1567 0.0
1568 0.0
1569 0.0
1570 0.0
1571 0.0
1572 0.0
1573 0.0
1574 0.0
1575 0.0
1576 0.0
1577 0.0
1578 0.0
1579 0.0
1580 0.0
1581 0.0
1582 0.0
1583 0.0
1584 0.0
1585 0.0
1586 0.0
1587 0.0
1588 0.0
1589 0.0
1590 0.0
1591 0.0
1592 0.0
1593 0.0
1594 0.0
1595 0.0
1596 0.0
1597 0.0
1598 0.0
1599 0.0
1600 0.0
1601 0.0
1602 0.0
1603 0.0
1604 0.0
1605 0.0
1606 0.0
1607 0.0
1608 0.0
1609 0.0
1610 0.0
1611 0.0
1612 0.0
1613 0.0
1614 0.0
1615 0.0
1616 0.0
1617 0.0
1618 0.0
1619 0.0
1620 0.0
1621 0.0
1622 0.0
1623 0.0
1624 0.0
1625 0.0
1626 0.0
1627 0.0
1628 0.0
1629 0.0
1630 0.0
1631 0.0
1632 0.0
1633 0.0
1634 0.0
1635 0.0
1636 0.0
1637 0.0
1638 0.0
1639 0.0
1640 0.0
1641 0.0
1642 0.0
1643 0.0
1644 0.0
1645 0.0
1646 0.0
1647 0.0
1648 0.0
1649 0.0
1650 0.0
1651 0.0
1652 0.0
1653 0.0
1654 0.0
1655 0.0
1656 0.0
1657 0.0
1658 0.0
1659 0.0
1660 0.0
1661 0.0
1662 0.0
1663 0.0
1664 0.0
1665 0.0
1666 0.0
1667 0.0
1668 0.0
1669 0.0
1670 0.0
1671 0.0
1672 0.0
1673 0.0
1674 0.0
1675 0.0
1676 0.0
1677 0.0
1678 0.0
1679 0.0
1680 0.0
1681 0.0
1682 0.0
1683 0.0
1684 0.0
1685 0.0
1686 0.0
1687 0.0
1688 0.0
1689 0.0
1690 0.0
1691 0.0
1692 0.0
1693 0.0
1694 0.0
1695 0.0
1696 0.0
1697 0.0
1698 0.0
1699 0.0
1700 0.0
1701 0.0
1702 0.0
1703 0.0
1704 0.0
1705 0.0
1706 0.0
1707 0.0
1708 0.0
1709 0.0
1710 0.0
1711 0.0
1712 0.0
1713 0.0
1714 0.0
1715 0.0
1716 0.0
1717 0.0
1718 0.0
1719 0.0
1720 0.0
1721 0.0
1722 0.0
1723 0.0
1724 0.0
1725 0.0
1726 0.0
1727 0.0
1728 0.0
1729 0.0
1730 0.0
1731 0.0
1732 0.0
1733 0.0
1734 0.0
1735 0.0
1736 0.0
1737 0.0
1738 0.0
1739 0.0
1740 0.0
1741 0.0
1742 0.0
1743 0.0
1744 0.0
1745 0.0
1746 0.0
1747 0.0
1748 0.0
1749 0.0
1750 0.0
1751 0.0
1752 0.0
1753 0.0
1754 0.0
1755 0.0
1756 0.0
1757 0.0
1758 0.0
1759 0.0
1760 0.0
1761 0.0
1762 0.0
1763 0.0
1764 0.0
1765 0.0
1766 0.0
1767 0.0
1768 0.0
1769 0.0
1770 0.0
1771 0.0
1772 0.0
1773 0.0
1774 0.0
1775 0.0
1776 0.0
1777 0.0
1778 0.0
1779 0.0
1780 0.0
1781 0.0
1782 0.0
1783 0.0
1784 0.0
1785 0.0
1786 0.0
1787 0.0
1788 0.0
1789 0.0
1790 0.0
1791 0.0
1792 0.0
1793 0.0
1794 0.0
1795 0.0
1796 0.0
1797 0.0
1798 0.0
1799 0.0
1800 0.0
1801 0.0
1802 0.0
1803 0.0
1804 0.0
1805 0.0
1806 0.0
1807 0.0
1808 0.0
1809 0.0
1810 0.0
1811 0.0
1812 0.0
1813 0.0
1814 0.0
1815 0.0
1816 0.0
1817 0.0
1818 0.0
1819 0.0
1820 0.0
1821 0.0
1822 0.0
1823 0.0
1824 0.0
1825 0.0
1826 0.0
1827 0.0
1828 0.0
1829 0.0
1830 0.0
1831 0.0
1832 0.0
1833 0.0
1834 0.0
1835 0.0
1836 0.0
1837 0.0
1838 0.0
1839 0.0
1840 0.0
1841 0.0
1842 0.0
1843 0.0
1844 0.0
1845 0.0
1846 0.0
1847 0.0
1848 0.0
1849 0.0
1850 0.0
1851 0.0
1852 0.0
1853 0.0
1854 0.0
1855 0.0
1856 0.0
1857 0.0
1858 0.0
1859 0.0
1860 0.0
1861 0.0
1862 0.0
1863 0.0
1864 0.0
1865 0.0
1866 0.0
1867 0.0
1868 0.0
1869 0.0
1870 0.0
1871 0.0
1872 0.0
1873 0.0
1874 0.0
1875 0.0
1876 0.0
1877 0.0
1878 0.0
1879 0.0
1880 0.0
1881 0.0
1882 0.0
1883 0.0
1884 0.0
1885 0.0
1886 0.0
1887 0.0
1888 0.0
1889 0.0
1890 0.0
1891 0.0
1892 0.0
1893 0.0
1894 0.0
1895 0.0
1896 0.0
1897 0.0
1898 0.0
1899 0.0
1900 0.0
1901 0.0
1902 0.0
1903 0.0
1904 0.0
1905 0.0
1906 0.0
1907 0.0
1908 0.0
1909 0.0
1910 0.0
1911 0.0
1912 0.0
1913 0.0
1914 0.0
1915 0.0
1916 0.0
1917 0.0
1918 0.0
1919 0.0
1920 0.0
1921 0.0
1922 0.0
1923 0.0
1924 0.0
1925 0.0
1926 0.0
1927 0.0
1928 0.0
1929 0.0
1930 0.0
1931 0.0
1932 0.0
1933 0.0
1934 0.0
1935 0.0
1936 0.0
1937 0.0
1938 0.0
1939 0.0
1940 0.0
1941 0.0
1942 0.0
1943 0.0
1944 0.0
1945 0.0
1946 0.0
1947 0.0
1948 0.0
1949 0.0
1950 0.0
1951 0.0
1952 0.0
1953 0.0
1954 0.0
1955 0.0
1956 0.0
1957 0.0
1958 0.0
1959 0.0
1960 0.0
1961 0.0
1962 0.0
1963 0.0
1964 0.0
1965 0.0
1966 0.0
1967 0.0
1968 0.0
1969 0.0
1970 0.0
1971 0.0
1972 0.0
1973 0.0
1974 0.0
1975 0.0
1976 0.0
1977 0.0
1978 0.0
1979 0.0
1980 0.0
1981 0.0
1982 0.0
1983 0.0
1984 0.0
1985 0.0
1986 0.0
1987 0.0
1988 0.0
1989 0.0
1990 0.0
1991 0.0
1992 0.0
1993 0.0
1994 0.0
1995 0.0
1996 0.0
1997 0.0
1998 0.0
1999 0.0
2000 0.0


==> plotdata/satellite_constellation/sat_A3_r.tex <==
t r
0 6848.233953273979
1 6848.239649633966
2 6848.250201788705
3 6848.26184780429
4 6848.276071752278
5 6848.290224839802
6 6848.306840287588
7 6848.325708002467
8 6848.348440454378
9 6848.371452084686
10 6848.389049005952
11 6848.403474040428
12 6848.4160835157245
13 6848.429041170457
14 6848.441641791679
15 6848.450892404702
16 6848.453022261856
17 6848.453077556001
18 6848.450024940183
19 6848.437036176914
20 6848.413655536227
21 6848.383810270993
22 6848.349468043186
23 6848.319067156967
24 6848.300492077785
25 6848.292839929526
26 6848.295583465893
27 6848.307312130521
28 6848.323502576015
29 6848.345211303949
30 6848.362286475197
31 6848.368926286701
32 6848.372292366753
33 6848.36639211231
34 6848.348646895617
35 6848.3226142751755
36 6848.290830222773
37 6848.255034075534
38 6848.217414394959
39 6848.180001266171
40 6848.143627179525
41 6848.110818699686
42 6848.083271978857
43 6848.063538836861
44 6848.052088255454
45 6848.044056934775
46 6848.038182649674
47 6848.034694103468
48 6848.036934287983
49 6848.043291318252
50 6848.049656223658
51 6848.05637777899
52 6848.06384024307
53 6848.072233425754
54 6848.080662303999
55 6848.094679688349
56 6848.118031196442
57 6848.149782814868
58 6848.188371904453
59 6848.234191079994
60 6848.284475893557
61 6848.328861706816
62 6848.3705502058665
63 6848.420492915232
64 6848.476332115532
65 6848.520556067315
66 6848.540341559415
67 6848.539679355342
68 6848.523244048211
69 6848.496693174734
70 6848.46633967385
71 6848.432323473986
72 6848.392101409637
73 6848.346743891048
74 6848.301007780513
75 6848.262073880517
76 6848.232335069896
77 6848.210950722471
78 6848.1971260687305
79 6848.191002671028
80 6848.183801352594
81 6848.1678458810875
82 6848.154153103839
83 6848.152264298782
84 6848.153111213684
85 6848.145402819074
86 6848.137271379572
87 6848.139026235145
88 6848.1498367478125
89 6848.168521414158
90 6848.193883128915
91 6848.224516937833
92 6848.2583836835
93 6848.2942946945495
94 6848.327231603495
95 6848.35416751114
96 6848.36959308007
97 6848.3662514426105
98 6848.346954516393
99 6848.315400098897
100 6848.273135277112
101 6848.220953702722
102 6848.159941894786
103 6848.091549129985
104 6848.01749125184
105 6847.939612623243
106 6847.859402018018
107 6847.77791284341
108 6847.696526170791
109 6847.616597277138
110 6847.539529654664
111 6847.474561726552
112 6847.430996064854
113 6847.409813380732
114 6847.407001395937
115 6847.417295467183
116 6847.439171091643
117 6847.468920699995
118 6847.499574897218
119 6847.527132868609
120 6847.55379481434
121 6847.581697393925
122 6847.609649214485
123 6847.635701792668
124 6847.660040152139
125 6847.684367991004
126 6847.708042608513
127 6847.73447318871
128 6847.764064563723
129 6847.797021185019
130 6847.8291066099455
131 6847.852340983106
132 6847.8666689286365
133 6847.875271183429
134 6847.881161386529
135 6847.884222067641
136 6847.884374851017
137 6847.881738750296
138 6847.876581028716
139 6847.871117903628
140 6847.865856642934
141 6847.858938556596
142 6847.852262504307
143 6847.846339709992
144 6847.841252962035
145 6847.837356464841
146 6847.834835395604
147 6847.833857513101
148 6847.83444539804
149 6847.836674754681
150 6847.840296312814
151 6847.845398034238
152 6847.85148690935
153 6847.860910772907
154 6847.872178590351
155 6847.884645193672
156 6847.898248785195
157 6847.912810229983
158 6847.930311774394
159 6847.948363414362
160 6847.965958680281
161 6847.984680499574
162 6848.004940358987
163 6848.025958084046
164 6848.046376358285
165 6848.065973007145
166 6848.084568439006
167 6848.101865821755
168 6848.117642158099
169 6848.131866284249
170 6848.144793876562
171 6848.156830215379
172 6848.168077475837
173 6848.178512954532
174 6848.188238596047
175 6848.196084347203
176 6848.201217331416
177 6848.204436476522
178 6848.206283915192
179 6848.207050614145
180 6848.206906700754
181 6848.206142988555
182 6848.205173762673
183 6848.2046442435885
184 6848.204611764458
185 6848.205212174897
186 6848.20642597414
187 6848.2080044848435
188 6848.209880137776
189 6848.211950925241
190 6848.214070643451
191 6848.216189497186
192 6848.216487347495
193 6848.21393909353
194 6848.209248438674
195 6848.201609306145
196 6848.191720671673
197 6848.180431742848
198 6848.167869470154
199 6848.154254853514
200 6848.139847074088
201 6848.12492369839
202 6848.109781257495
203 6848.09473993958
204 6848.080092292639
205 6848.066071833312
206 6848.052920657618
207 6848.040905925886
208 6848.03026000987
209 6848.021120367897
210 6848.013541499442
211 6848.007564721866
212 6848.003222831441
213 6848.000511678908
214 6847.999397297896
215 6847.999755482795
216 6848.0015051324735
217 6848.004576337977
218 6848.008847448175
219 6848.01417821347
220 6848.020342597636
221 6848.027196226068
222 6848.034630625949
223 6848.04249287712
224 6848.050631028581
225 6848.058927660434
226 6848.0663948971915
227 6848.074553596017
228 6848.084385873513
229 6848.094841094121
230 6848.1054854509
231 6848.116034189011
232 6848.126254258948
233 6848.135904923424
234 6848.1453557022805
235 6848.154992704704
236 6848.165225314493
237 6848.171408149025
238 6848.168050515742
239 6848.155948810272
240 6848.138938329396
241 6848.117624726173
242 6848.091290413947
243 6848.063364281103
244 6848.035516952583
245 6848.007738006499
246 6847.980625360943
247 6847.953430843488
248 6847.925813218697
249 6847.898847266784
250 6847.873093565578
251 6847.848987905187
252 6847.826900561645
253 6847.808406048834
254 6847.795259091436
255 6847.790196615455
256 6847.796360165137
257 6847.815108537366
258 6847.849543740017
259 6847.90199480143
260 6847.970422716984
261 6848.05307289454
262 6848.147789079231
263 6848.250148363182
264 6848.355777472547
265 6848.461461290965
266 6848.563702264417
267 6848.6557581907955
268 6848.734424404609
269 6848.801685833189
270 6848.857073571209
271 6848.900397231775
272 6848.931642526865
273 6848.951143471584
274 6848.959020535469
275 6848.955615828736
276 6848.9414910462765
277 6848.917439736833
278 6848.884931867844
279 6848.8454341296965
280 6848.800112928953
281 6848.749871396609
282 6848.695667434618
283 6848.638598159752
284 6848.579755930104
285 6848.520064463349
286 6848.456028267135
287 6848.383827776134
288 6848.305422399675
289 6848.225204533323
290 6848.145741701775
291 6848.069537217319
292 6847.999328502126
293 6847.937719970319
294 6847.884711341901
295 6847.839831783454
296 6847.803336375539
297 6847.776382054587
298 6847.761225186137
299 6847.758071260116
300 6847.767828078855
301 6847.789870187594
302 6847.822043076619
303 6847.861867942678
304 6847.906673190897
305 6847.94816790474
306 6847.982419644409
307 6848.01260479595
308 6848.0358746128495
309 6848.048086573752
310 6848.048948043796
311 6848.039658031313
312 6848.020701514398
313 6847.992862280023
314 6847.957618579399
315 6847.917503369856
316 6847.876143259353
317 6847.836454316287
318 6847.800271936643
319 6847.770196316789
320 6847.752788190842
321 6847.752358920771
322 6847.774073133814
323 6847.820856491479
324 6847.877116980877
325 6847.9267439937175
326 6847.969708066178
327 6848.00455650705
328 6848.027985392695
329 6848.040747646259
330 6848.043134611009
331 6848.038858061108
332 6848.031403047389
333 6848.0208814813095
334 6848.007450981909
335 6847.99136177723
336 6847.972951993632
337 6847.952613642517
338 6847.930830284987
339 6847.908161932947
340 6847.885201386506
341 6847.862726785199
342 6847.8421456607
343 6847.825326726071
344 6847.814321910747
345 6847.810787112605
346 6847.815750026481
347 6847.829736653863
348 6847.85257435131
349 6847.883358423428
350 6847.920753129548
351 6847.9632669569755
352 6848.008941676826
353 6848.055522987423
354 6848.101077876032
355 6848.144528986837
356 6848.1851057383055
357 6848.221568115452
358 6848.252679822552
359 6848.277355303961
360 6848.296503185739
361 6848.310446935147
362 6848.317686664966
363 6848.3181093050425
364 6848.312304131912
365 6848.301182220911
366 6848.285877178936
367 6848.267628677418
368 6848.247817037441
369 6848.232969607351
370 6848.231132507605
371 6848.244863310504
372 6848.266948744544
373 6848.289894552969
374 6848.313673957667
375 6848.338328793104
376 6848.364161066747
377 6848.392450392566
378 6848.4217473072395
379 6848.449284693735
380 6848.479151733928
381 6848.51494987979
382 6848.555041751278
383 6848.592437547346
384 6848.616105836126
385 6848.625716706958
386 6848.621076035087
387 6848.606463239525
388 6848.591902009644
389 6848.579632525947
390 6848.5653729643045
391 6848.544145324003
392 6848.516309098161
393 6848.482455157376
394 6848.443371627174
395 6848.400222023365
396 6848.354228357015
397 6848.30662125573
398 6848.258600034855
399 6848.211290749905
400 6848.165701423829
401 6848.1220030454715
402 6848.080888399068
403 6848.045388220368
404 6848.017715679977
405 6848.001255489375
406 6847.999691492849
407 6848.011048270893
408 6848.027616530552
409 6848.044006332421
410 6848.059944083072
411 6848.075455095505
412 6848.086838479305
413 6848.09140683911
414 6848.09002230672
415 6848.08811035559
416 6848.085142408862
417 6848.074951374355
418 6848.057663565465
419 6848.033259494272
420 6848.001621735296
421 6847.963384066398
422 6847.928101258694
423 6847.900330141054
424 6847.876819916449
425 6847.858800508316
426 6847.843931925393
427 6847.835845297586
428 6847.833601420252
429 6847.830296931041
430 6847.8274868179005
431 6847.8268250733845
432 6847.830203894479
433 6847.837937641461
434 6847.8487004349045
435 6847.861060504574
436 6847.873415547479
437 6847.884428159893
438 6847.893168868698
439 6847.904579071022
440 6847.922708886366
441 6847.945255172805
442 6847.970143243965
443 6847.9956224491925
444 6848.020295922625
445 6848.043048352908
446 6848.063108024766
447 6848.079972022845
448 6848.093258955482
449 6848.102791020635
450 6848.107480527607
451 6848.111880178013
452 6848.1144244626885
453 6848.11295140837
454 6848.111354923593
455 6848.111710890701
456 6848.108264208322
457 6848.1027449912
458 6848.102590082593
459 6848.105434943136
460 6848.110480029735
461 6848.117586106818
462 6848.125884743929
463 6848.134212434031
464 6848.142626211407
465 6848.147383969195
466 6848.1465746149215
467 6848.143189429888
468 6848.140070631022
469 6848.139186788903
470 6848.1391269177
471 6848.138843553589
472 6848.140567282077
473 6848.144618506975
474 6848.152450032158
475 6848.166760806986
476 6848.183843487003
477 6848.1955728070125
478 6848.202892131492
479 6848.20855505438
480 6848.213100051413
481 6848.214632527696
482 6848.211934839264
483 6848.20624243376
484 6848.198721014875
485 6848.1916874063045
486 6848.186357606849
487 6848.175153804171
488 6848.152468748741
489 6848.123157428292
490 6848.087805492046
491 6848.047100636598
492 6848.0016174761295
493 6847.951905054825
494 6847.899189350035
495 6847.844755202013
496 6847.78990526833
497 6847.736282356611
498 6847.685736045998
499 6847.639816298759
500 6847.605702271675
501 6847.589692831103
502 6847.591534236585
503 6847.610608013294
504 6847.640476650683
505 6847.674733935466
506 6847.709209068322
507 6847.7413399778015
508 6847.773175198833
509 6847.804214167146
510 6847.832511900229
511 6847.856406761208
512 6847.879920759417
513 6847.906859920886
514 6847.935401004919
515 6847.965010883152
516 6847.994992531398
517 6848.023798937508
518 6848.051686456154
519 6848.074892163823
520 6848.0890451635705
521 6848.094551898228
522 6848.091645803392
523 6848.080433734237
524 6848.061460605122
525 6848.035534444096
526 6848.006271254846
527 6847.977918661928
528 6847.952052184046
529 6847.929955046778
530 6847.912929624458
531 6847.898238101758
532 6847.8823562986845
533 6847.865673399012
534 6847.8484925258335
535 6847.830972962903
536 6847.813153755847
537 6847.794926499773
538 6847.776090982706
539 6847.756652900712
540 6847.741414893154
541 6847.735046598668
542 6847.73716934156
543 6847.746025455085
544 6847.759833861161
545 6847.777645961049
546 6847.798418676708
547 6847.821697549971
548 6847.849565952902
549 6847.884989010428
550 6847.923212831126
551 6847.959712701698
552 6847.9960986456435
553 6848.029980780583
554 6848.058968983033
555 6848.083879259634
556 6848.104695397295
557 6848.120766645942
558 6848.1314237945035
559 6848.136413698359
560 6848.135635790332
561 6848.129100392985
562 6848.116842880809
563 6848.099129287361
564 6848.070836404667
565 6848.028325742963
566 6847.975522025699
567 6847.916579421535
568 6847.854462329872
569 6847.792760998242
570 6847.733004792755
571 6847.675823658047
572 6847.621894401299
573 6847.571415037573
574 6847.524042961926
575 6847.480793621502
576 6847.44655204666
577 6847.426135753948
578 6847.413165638133
579 6847.403214844619
580 6847.399450363935
581 6847.402004098763
582 6847.412377736865
583 6847.4308090858485
584 6847.455601927846
585 6847.485147349687
586 6847.519616479119
587 6847.55822827401
588 6847.598521805071
589 6847.6389383397
590 6847.678022537305
591 6847.714456157367
592 6847.747854911822
593 6847.77981797009
594 6847.812220595037
595 6847.845508257088
596 6847.880020458594
597 6847.915858215651
598 6847.952915693643
599 6847.996074072182
600 6848.047611100234
601 6848.103307000439
602 6848.159693011172
603 6848.216526223216
604 6848.274199998834
605 6848.329420571474
606 6848.376673892609
607 6848.408417352601
608 6848.422568950758
609 6848.42723930222
610 6848.424454667188
611 6848.407725178176
612 6848.378586561554
613 6848.337351955073
614 6848.2912409136325
615 6848.236619749916
616 6848.162226491462
617 6848.070402754853
618 6847.9631096204685
619 6847.848308281222
620 6847.735792698044
621 6847.628538664135
622 6847.5299214280885
623 6847.4429395035795
624 6847.369854459157
625 6847.314201735203
626 6847.283573125136
627 6847.280898460382
628 6847.3077017667065
629 6847.362602180947
630 6847.442169315561
631 6847.544022573254
632 6847.661619238318
633 6847.789729266238
634 6847.9220390034625
635 6848.053208210547
636 6848.179956939724
637 6848.301904379679
638 6848.418789603093
639 6848.521944700539
640 6848.604131010938
641 6848.657347862805
642 6848.679777941427
643 6848.677552119226
644 6848.652876425491
645 6848.606777501449
646 6848.544402150335
647 6848.471358267904
648 6848.390136178131
649 6848.302192666009
650 6848.209401740285
651 6848.1147568986535
652 6848.026205728334
653 6847.951711511692
654 6847.892494530375
655 6847.845767101219
656 6847.8104989477815
657 6847.785983891974
658 6847.77031509372
659 6847.764402805703
660 6847.7679874101095
661 6847.780913039771
662 6847.800073815295
663 6847.824289577847
664 6847.853930191331
665 6847.887729313352
666 6847.924855940756
667 6847.965473943278
668 6848.011776531973
669 6848.059450717428
670 6848.103452721257
671 6848.146059864401
672 6848.190376732475
673 6848.236372882148
674 6848.282150528805
675 6848.323461973136
676 6848.359017177473
677 6848.392643899469
678 6848.424286022952
679 6848.447687738822
680 6848.459837110196
681 6848.462013334687
682 6848.4545930836675
683 6848.438374109565
684 6848.413607220975
685 6848.381326377546
686 6848.34376133678
687 6848.302569453242
688 6848.258535693093
689 6848.212683635468
690 6848.164978720774
691 6848.115156576781
692 6848.056838699069
693 6847.989864369653
694 6847.915414450758
695 6847.828156123553
696 6847.736838932911
697 6847.646676543918
698 6847.556185290119
699 6847.46799766898
700 6847.385071533349
701 6847.309307191872
702 6847.238972684868
703 6847.1727295476285
704 6847.119080712409
705 6847.085374762677
706 6847.07105348676
707 6847.0711494436955
708 6847.079545566725
709 6847.100967027665
710 6847.138987741202
711 6847.192417240332
712 6847.260818223876
713 6847.342059126295
714 6847.432876813361
715 6847.529026562143
716 6847.624543497949
717 6847.716308539856
718 6847.802644508609
719 6847.879279105236
720 6847.9448741054575
721 6847.999672902321
722 6848.046737703009
723 6848.088215198559
724 6848.124011228854
725 6848.1541260345175
726 6848.178638961425
727 6848.197698749246
728 6848.211504471146
729 6848.220714754997
730 6848.226758015015
731 6848.229936259714
732 6848.229114499896
733 6848.220954594379
734 6848.201319332452
735 6848.167012351772
736 6848.116336412192
737 6848.049195116482
738 6847.975245281812
739 6847.904330338162
740 6847.835986326387
741 6847.76755445937
742 6847.698206799848
743 6847.628754830187
744 6847.566888915041
745 6847.520168446262
746 6847.48190781756
747 6847.450086502887
748 6847.431191517919
749 6847.423301631768
750 6847.421338453895
751 6847.4258109510665
752 6847.437304257401
753 6847.456524815491
754 6847.483524874469
755 6847.518096499276
756 6847.55979192584
757 6847.608056601825
758 6847.664728435873
759 6847.731430903229
760 6847.806403045349
761 6847.887930135026
762 6847.975059812432
763 6848.066508937992
764 6848.16026077822
765 6848.25460225151
766 6848.348624009367
767 6848.440597400502
768 6848.527260533473
769 6848.607801575358
770 6848.678826728165
771 6848.735746634482
772 6848.77958193415
773 6848.8105019752265
774 6848.829067511508
775 6848.836109400707
776 6848.832335544534
777 6848.8184299757495
778 6848.79530802728
779 6848.763553377878
780 6848.723837419394
781 6848.676917470781
782 6848.623678775052
783 6848.565062413106
784 6848.508366656246
785 6848.454648032556
786 6848.405294546698
787 6848.369494784683
788 6848.342957383684
789 6848.318696620886
790 6848.295222179036
791 6848.271885791614
792 6848.2492109721925
793 6848.2293067031305
794 6848.212307806303
795 6848.197725311828
796 6848.185556801496
797 6848.174214157082
798 6848.163506116835
799 6848.156919794494
800 6848.154263954059
801 6848.151259536167
802 6848.147499506493
803 6848.1432122931865
804 6848.13859378866
805 6848.136805343793
806 6848.137986476313
807 6848.139022774038
808 6848.142872284428
809 6848.152130048494
810 6848.166471348361
811 6848.185400145787
812 6848.208271126516
813 6848.234210503929
814 6848.261880579293
815 6848.2900187194045
816 6848.315135054459
817 6848.334146057609
818 6848.347002974338
819 6848.354697382147
820 6848.3555090693635
821 6848.348201459426
822 6848.332357284253
823 6848.313701011112
824 6848.291096416934
825 6848.25890195184
826 6848.21904385829
827 6848.1729625365115
828 6848.122120812484
829 6848.067773748622
830 6848.010916254011
831 6847.952697950274
832 6847.894218063334
833 6847.836469713139
834 6847.780282097924
835 6847.726403826683
836 6847.6756382284575
837 6847.628904199406
838 6847.587021023386
839 6847.55057926898
840 6847.520336613886
841 6847.496739786866
842 6847.479738990628
843 6847.469437892303
844 6847.466175368951
845 6847.470011782508
846 6847.4806886893375
847 6847.497892347683
848 6847.521226293674
849 6847.550080279307
850 6847.583848518761
851 6847.621959946503
852 6847.663956672993
853 6847.70937777165
854 6847.757352949912
855 6847.807596821993
856 6847.859411484702
857 6847.912150166452
858 6847.965112584923
859 6848.017412610354
860 6848.068079002493
861 6848.116289718507
862 6848.161391574571
863 6848.203005723888
864 6848.240338897271
865 6848.272910298849
866 6848.300283446571
867 6848.322480507109
868 6848.339598925801
869 6848.351316582858
870 6848.357235175308
871 6848.357324024784
872 6848.351577983868
873 6848.339622906931
874 6848.320977432828
875 6848.295519796706
876 6848.271111437315
877 6848.250612705109
878 6848.234701993825
879 6848.228057486896
880 6848.229925995391
881 6848.239545589637
882 6848.255987170523
883 6848.277927132155
884 6848.303163368996
885 6848.328748919096
886 6848.350434797078
887 6848.368593124356
888 6848.386756468914
889 6848.400795598768
890 6848.407232620882
891 6848.408023367826
892 6848.400412213879
893 6848.388326482695
894 6848.37911396918
895 6848.372612008468
896 6848.368480560591
897 6848.366439114816
898 6848.366408950992
899 6848.368184331151
900 6848.371434269206
901 6848.375853898752
902 6848.381110292455
903 6848.386455245429
904 6848.390582469976
905 6848.391869707203
906 6848.388631171293
907 6848.3792165676205
908 6848.362159257441
909 6848.336578422982
910 6848.302340714858
911 6848.259910033054
912 6848.210290915827
913 6848.154942320855
914 6848.09571177227
915 6848.034333808267
916 6847.972192716007
917 6847.910610688639
918 6847.850916009423
919 6847.794391364752
920 6847.737987730741
921 6847.680054818577
922 6847.623694152894
923 6847.568193177828
924 6847.5125056285715
925 6847.457268928695
926 6847.404672781147
927 6847.35876360412
928 6847.319062777737
929 6847.286246898795
930 6847.260520503994
931 6847.242310888383
932 6847.234194152205
933 6847.2367940010245
934 6847.250873306981
935 6847.276808672435
936 6847.314194085325
937 6847.360861830423
938 6847.414458200304
939 6847.473524801716
940 6847.536898297874
941 6847.603502990176
942 6847.672157047211
943 6847.741785663883
944 6847.8114557977815
945 6847.884948758527
946 6847.960055065983
947 6848.032603993208
948 6848.101259941632
949 6848.172330425258
950 6848.244202286564
951 6848.307039831221
952 6848.367658881059
953 6848.432694365673
954 6848.503064423725
955 6848.573231600824
956 6848.6267056130955
957 6848.667578457072
958 6848.708558215352
959 6848.750943016406
960 6848.794971036587
961 6848.8401499618485
962 6848.885419753615
963 6848.929513610185
964 6848.97104816288
965 6849.008214420159
966 6849.0397779690775
967 6849.065015992191
968 6849.082962048561
969 6849.092688878459
970 6849.093160005807
971 6849.083705140524
972 6849.062622438459
973 6849.026191746656
974 6848.9755886845105
975 6848.9133438287745
976 6848.840429721374
977 6848.759124560327
978 6848.671797463157
979 6848.581372061166
980 6848.489904438838
981 6848.405220384435
982 6848.333727566646
983 6848.274397683734
984 6848.2286156296495
985 6848.1976254882165
986 6848.1793839122365
987 6848.171734754266
988 6848.172537660336
989 6848.179751678397
990 6848.1914583656335
991 6848.205888746906
992 6848.221717077306
993 6848.237837573054
994 6848.252730672562
995 6848.265779855766
996 6848.277070205374
997 6848.285841097368
998 6848.2927971090885
999 6848.298364801203
1000 6848.301469826736
1001 6848.302857594544
1002 6848.303080519942
1003 6848.301600518859
1004 6848.298763177753
1005 6848.2950565931515
1006 6848.291391699666
1007 6848.288136221551
1008 6848.2848031488475
1009 6848.281249673933
1010 6848.277365839446
1011 6848.273049639132
1012 6848.268244683916
1013 6848.263246424564
1014 6848.258653852112
1015 6848.2547860052955
1016 6848.25051923954
1017 6848.2459789308405
1018 6848.242451252794
1019 6848.240043138468
1020 6848.241147689657
1021 6848.246196934635
1022 6848.251091692239
1023 6848.261657708553
1024 6848.286512002643
1025 6848.321624094263
1026 6848.355780330549
1027 6848.383042683996
1028 6848.403940656416
1029 6848.417229747204
1030 6848.423750046242
1031 6848.426260113297
1032 6848.436611384202
1033 6848.452598311448
1034 6848.460407154325
1035 6848.4681443292175
1036 6848.477972324747
1037 6848.485921672477
1038 6848.492742107418
1039 6848.499633287162
1040 6848.508155224371
1041 6848.514620137793
1042 6848.5211108810045
1043 6848.5278624194
1044 6848.5355409348
1045 6848.546043029544
1046 6848.553908238788
1047 6848.563758038398
1048 6848.572773751778
1049 6848.571564984836
1050 6848.5615187965195
1051 6848.545170763674
1052 6848.52600124586
1053 6848.506270215886
1054 6848.486576971889
1055 6848.46772061545
1056 6848.449966644813
1057 6848.433303344314
1058 6848.418442245371
1059 6848.40312366645
1060 6848.384711849705
1061 6848.365309830098
1062 6848.346611837586
1063 6848.3284281637225
1064 6848.309134036343
1065 6848.288661667705
1066 6848.268931244465
1067 6848.249828708211
1068 6848.231253960278
1069 6848.21415863443
1070 6848.212054062617
1071 6848.223629633138
1072 6848.232208625175
1073 6848.237647259994
1074 6848.241625475011
1075 6848.245835319567
1076 6848.2485972515315
1077 6848.247145998036
1078 6848.248327102104
1079 6848.2519372912775
1080 6848.264034971393
1081 6848.282127438031
1082 6848.291861131395
1083 6848.294531953693
1084 6848.298200803197
1085 6848.303210004024
1086 6848.305655884147
1087 6848.308856434897
1088 6848.308252820973
1089 6848.30612243385
1090 6848.313118419583
1091 6848.320947433198
1092 6848.319718579068
1093 6848.314141103586
1094 6848.308158116918
1095 6848.303050305627
1096 6848.299752383413
1097 6848.3012112017495
1098 6848.301286341342
1099 6848.296175738274
1100 6848.288880137063
1101 6848.279054364098
1102 6848.269512023444
1103 6848.260746829341
1104 6848.252249634845
1105 6848.2476948564145
1106 6848.246203119778
1107 6848.243993037043
1108 6848.241097939485
1109 6848.239647838973
1110 6848.236036564123
1111 6848.227043119803
1112 6848.215320280022
1113 6848.202663159732
1114 6848.190508156416
1115 6848.180176793559
1116 6848.173010112789
1117 6848.168062815023
1118 6848.165167071366
1119 6848.165038684418
1120 6848.167131017864
1121 6848.1699032055385
1122 6848.176127095113
1123 6848.183883888698
1124 6848.190943619229
1125 6848.199194854491
1126 6848.208527251947
1127 6848.217933825545
1128 6848.226230079734
1129 6848.234452031329
1130 6848.234282059584
1131 6848.219855825498
1132 6848.194704679146
1133 6848.159865125452
1134 6848.116601710841
1135 6848.068415455162
1136 6848.018587835555
1137 6847.970288526744
1138 6847.925981653363
1139 6847.883850864796
1140 6847.843844440512
1141 6847.812569495786
1142 6847.796513243505
1143 6847.799827780193
1144 6847.823814480001
1145 6847.867451245306
1146 6847.918548490674
1147 6847.9702894563525
1148 6848.023960778115
1149 6848.075050737811
1150 6848.11401807137
1151 6848.133877261234
1152 6848.1371105289945
1153 6848.126670246839
1154 6848.106299559103
1155 6848.081211185426
1156 6848.054793040727
1157 6848.027922159122
1158 6848.001430063857
1159 6847.9760138617
1160 6847.952212779711
1161 6847.9304391361175
1162 6847.911012072007
1163 6847.894179540886
1164 6847.880122798797
1165 6847.868974833798
1166 6847.860825836628
1167 6847.855731852168
1168 6847.853705218897
1169 6847.854621594749
1170 6847.858273710561
1171 6847.86446405871
1172 6847.872964351277
1173 6847.883519456251
1174 6847.895838826131
1175 6847.9096205787955
1176 6847.924548113787
1177 6847.940315695268
1178 6847.956619884096
1179 6847.973153609258
1180 6847.989618619565
1181 6848.005766623546
1182 6848.021382873988
1183 6848.036124990113
1184 6848.049668321834
1185 6848.06184618352
1186 6848.072491190149
1187 6848.081566951251
1188 6848.089162476562
1189 6848.095329879153
1190 6848.100067180843
1191 6848.103418734197
1192 6848.105463835677
1193 6848.106283454646
1194 6848.105867812126
1195 6848.104208469465
1196 6848.101489987842
1197 6848.097926158239
1198 6848.093711386001
1199 6848.089174827581
1200 6848.084366319195
1201 6848.079153849391
1202 6848.073634228747
1203 6848.067798804861
1204 6848.061605752671
1205 6848.055192464731
1206 6848.048739841335
1207 6848.042380653921
1208 6848.036248427979
1209 6848.03058363494
1210 6848.025533349776
1211 6848.0211395453725
1212 6848.017804957879
1213 6848.0158887530315
1214 6848.015458760874
1215 6848.016559804927
1216 6848.019180196464
1217 6848.0232540572115
1218 6848.02870746674
1219 6848.035471673252
1220 6848.043397040376
1221 6848.052299656781
1222 6848.061943485714
1223 6848.07208866113
1224 6848.082561273789
1225 6848.093182653644
1226 6848.103699582743
1227 6848.114081664473
1228 6848.124364984216
1229 6848.134128952027
1230 6848.143007589572
1231 6848.15092028599
1232 6848.157790977873
1233 6848.163565558327
1234 6848.168354417544
1235 6848.172192632993
1236 6848.174874583929
1237 6848.176494097075
1238 6848.17729528091
1239 6848.177318493012
1240 6848.176576047954
1241 6848.175135695683
1242 6848.173032560105
1243 6848.1702429886745
1244 6848.166813167144
1245 6848.162872699145
1246 6848.158492637998
1247 6848.153699988598
1248 6848.148602686812
1249 6848.143316605837
1250 6848.137970088458
1251 6848.132406598354
1252 6848.126390415876
1253 6848.120023814196
1254 6848.113842187247
1255 6848.108087235168
1256 6848.102569660622
1257 6848.09746891601
1258 6848.092798271545
1259 6848.088678218632
1260 6848.085314873136
1261 6848.082828437657
1262 6848.081284131928
1263 6848.0806419920045
1264 6848.080887613452
1265 6848.082054928249
1266 6848.084167637498
1267 6848.087207577665
1268 6848.091103433597
1269 6848.0957926911715
1270 6848.101179100237
1271 6848.1071276334815
1272 6848.113869602617
1273 6848.121335849041
1274 6848.129232689192
1275 6848.1367549820525
1276 6848.142890059668
1277 6848.1487314350015
1278 6848.154056631605
1279 6848.157912432169
1280 6848.160392749435
1281 6848.161117957006
1282 6848.160217326258
1283 6848.157800211435
1284 6848.154175033575
1285 6848.149814791856
1286 6848.144917304661
1287 6848.13940850234
1288 6848.13342248789
1289 6848.127265577365
1290 6848.121169412834
1291 6848.115327046769
1292 6848.109943826485
1293 6848.105115322435
1294 6848.101002191698
1295 6848.097720255021
1296 6848.095181554494
1297 6848.09337644925
1298 6848.092323910267
1299 6848.092012641716
1300 6848.092413471946
1301 6848.0934997667
1302 6848.095224124559
1303 6848.097533600278
1304 6848.100394503308
1305 6848.103797495812
1306 6848.107762277662
1307 6848.112288003562
1308 6848.117343458418
1309 6848.1228894414235
1310 6848.1289019635
1311 6848.135334586519
1312 6848.142090706826
1313 6848.149164511029
1314 6848.156948680441
1315 6848.165468130427
1316 6848.174344985749
1317 6848.183290887665
1318 6848.19207474822
1319 6848.201657604386
1320 6848.212769987286
1321 6848.224888111005
1322 6848.237588173629
1323 6848.250464387053
1324 6848.263111227849
1325 6848.27521244352
1326 6848.2865227352295
1327 6848.296824827557
1328 6848.306043078939
1329 6848.314156738772
1330 6848.321001578147
1331 6848.326515849081
1332 6848.330731103497
1333 6848.332174703045
1334 6848.3297800014425
1335 6848.324142279083
1336 6848.315636356336
1337 6848.304699220964
1338 6848.291793513058
1339 6848.277355579729
1340 6848.261796987594
1341 6848.245590029051
1342 6848.2291364908215
1343 6848.2128251910435
1344 6848.19706611824
1345 6848.182070193664
1346 6848.167953152024
1347 6848.154835458414
1348 6848.1428988305215
1349 6848.13230862014
1350 6848.1232574832
1351 6848.11589964851
1352 6848.110241563501
1353 6848.106325417358
1354 6848.104258213553
1355 6848.103955984452
1356 6848.105292540469
1357 6848.108194866516
1358 6848.112547193629
1359 6848.118225717759
1360 6848.125130092655
1361 6848.133156271354
1362 6848.1420801288095
1363 6848.151734759817
1364 6848.162011006218
1365 6848.172700555352
1366 6848.183613919418
1367 6848.194571010456
1368 6848.205319002651
1369 6848.215581736631
1370 6848.225180604222
1371 6848.233999040694
1372 6848.241944881349
1373 6848.2489487950925
1374 6848.254961666768
1375 6848.259955855777
1376 6848.264913480018
1377 6848.271906490332
1378 6848.2822855525255
1379 6848.294623689632
1380 6848.308216292087
1381 6848.3228711908205
1382 6848.336135965692
1383 6848.349114869493
1384 6848.361755251385
1385 6848.372068180937
1386 6848.379685289023
1387 6848.3840626227
1388 6848.3867873779345
1389 6848.388765351786
1390 6848.388013503328
1391 6848.3854796100095
1392 6848.381268301783
1393 6848.37356700839
1394 6848.362489335528
1395 6848.348215982628
1396 6848.330766364795
1397 6848.314765306656
1398 6848.305013516413
1399 6848.301236557823
1400 6848.302743722522
1401 6848.310480981468
1402 6848.323869798689
1403 6848.340628659981
1404 6848.359290474211
1405 6848.378543625545
1406 6848.39721433563
1407 6848.414350801067
1408 6848.429312061707
1409 6848.441750195853
1410 6848.45150845184
1411 6848.458448343759
1412 6848.462366150248
1413 6848.46329765602
1414 6848.461615601976
1415 6848.457694490642
1416 6848.450761308733
1417 6848.439556705079
1418 6848.424019040822
1419 6848.398751989563
1420 6848.363428198263
1421 6848.322806260577
1422 6848.275931516595
1423 6848.22436331953
1424 6848.169697719137
1425 6848.110925075333
1426 6848.049874599638
1427 6847.99071318801
1428 6847.934164210462
1429 6847.8811643223125
1430 6847.8328696558465
1431 6847.78976189707
1432 6847.752450704674
1433 6847.721606010565
1434 6847.697728902298
1435 6847.680100122647
1436 6847.668671706596
1437 6847.665818516413
1438 6847.6743201300305
1439 6847.692642683926
1440 6847.719563824197
1441 6847.7530129271245
1442 6847.791733528317
1443 6847.834233678281
1444 6847.87188041058
1445 6847.904162067888
1446 6847.9341001640405
1447 6847.960588173261
1448 6847.986512929629
1449 6848.014705490305
1450 6848.048776170356
1451 6848.088221343508
1452 6848.130724145145
1453 6848.176799757045
1454 6848.227207741904
1455 6848.282001448752
1456 6848.339659950414
1457 6848.3983310888525
1458 6848.456429582733
1459 6848.514387459593
1460 6848.572155670141
1461 6848.625890103041
1462 6848.672430210848
1463 6848.710118115125
1464 6848.738438626481
1465 6848.758978332324
1466 6848.771207082465
1467 6848.773575168787
1468 6848.767181412739
1469 6848.752618893237
1470 6848.7315225756765
1471 6848.706493516287
1472 6848.679196883202
1473 6848.65088621886
1474 6848.622399536264
1475 6848.593994031072
1476 6848.566392393717
1477 6848.540278035054
1478 6848.516164588904
1479 6848.49454444342
1480 6848.475563840979
1481 6848.459471564839
1482 6848.446283589365
1483 6848.436771126663
1484 6848.43180093619
1485 6848.431670518066
1486 6848.435310258801
1487 6848.440306780627
1488 6848.446002183616
1489 6848.452030672418
1490 6848.455441240073
1491 6848.45531100005
1492 6848.451484916782
1493 6848.445614189019
1494 6848.438241691257
1495 6848.429449487022
1496 6848.420330338913
1497 6848.412022058564
1498 6848.406208931939
1499 6848.4030006143685
1500 6848.402571124644
1501 6848.404421313895
1502 6848.407501813885
1503 6848.414214043738
1504 6848.42414278862
1505 6848.432134761653
1506 6848.438671540317
1507 6848.446002086529
1508 6848.454012919617
1509 6848.46277590708
1510 6848.471706833902
1511 6848.479431069247
1512 6848.487313826299
1513 6848.4947784072865
1514 6848.49917214662
1515 6848.500871890219
1516 6848.498165914015
1517 6848.488352585909
1518 6848.473501136179
1519 6848.457072001252
1520 6848.440312953728
1521 6848.424361948747
1522 6848.409833503545
1523 6848.396772611739
1524 6848.384967850731
1525 6848.374329653748
1526 6848.363924842203
1527 6848.353920692585
1528 6848.345879350246
1529 6848.341537387277
1530 6848.340245360042
1531 6848.3398702690365
1532 6848.339655477005
1533 6848.339062256827
1534 6848.338419960445
1535 6848.336914646268
1536 6848.33360846435
1537 6848.329519647748
1538 6848.32491786455
1539 6848.3198475816225
1540 6848.314400171742
1541 6848.308070999388
1542 6848.302813487727
1543 6848.30138028449
1544 6848.308392461283
1545 6848.32796301842
1546 6848.357214129594
1547 6848.386703996786
1548 6848.407576611171
1549 6848.419758188773
1550 6848.42293902851
1551 6848.413772261539
1552 6848.391265583647
1553 6848.360291172124
1554 6848.327017586873
1555 6848.2949586298855
1556 6848.2661551552865
1557 6848.240812975072
1558 6848.218416273804
1559 6848.198686344347
1560 6848.181537130095
1561 6848.167005860598
1562 6848.154965332707
1563 6848.145307495548
1564 6848.137951028198
1565 6848.132679666461
1566 6848.128908878467
1567 6848.125857356637
1568 6848.123094846903
1569 6848.1202516886015
1570 6848.116940697804
1571 6848.112884583121
1572 6848.107831269161
1573 6848.101639912709
1574 6848.09418158901
1575 6848.085664830085
1576 6848.07645788381
1577 6848.066811607226
1578 6848.057145599288
1579 6848.047831212127
1580 6848.039274565706
1581 6848.032347813213
1582 6848.027771488535
1583 6848.025722605394
1584 6848.026046467941
1585 6848.028688403989
1586 6848.033379054219
1587 6848.03929989182
1588 6848.0453708498835
1589 6848.05083445492
1590 6848.05524225298
1591 6848.058303672256
1592 6848.0607762842355
1593 6848.0632782660305
1594 6848.065186267101
1595 6848.066192962558
1596 6848.066101889964
1597 6848.063975128215
1598 6848.059537262702
1599 6848.052706070246
1600 6848.043488996214
1601 6848.032039534488
1602 6848.018664854742
1603 6848.0037387078955
1604 6847.9877171685
1605 6847.971030174491
1606 6847.9540220835015
1607 6847.936975123133
1608 6847.920093524756
1609 6847.903623143253
1610 6847.887864595155
1611 6847.873105298727
1612 6847.859607088163
1613 6847.847690282691
1614 6847.837789236965
1615 6847.830221406265
1616 6847.824998905621
1617 6847.822099523433
1618 6847.821611677429
1619 6847.823598425317
1620 6847.828183233454
1621 6847.835413825847
1622 6847.845161715145
1623 6847.857213253426
1624 6847.871282765912
1625 6847.88703399033
1626 6847.904103645075
1627 6847.922131623662
1628 6847.940731777539
1629 6847.9595012835225
1630 6847.978016812025
1631 6847.996024063581
1632 6848.013429192356
1633 6848.030071296261
1634 6848.0457486990645
1635 6848.060249412853
1636 6848.073392137715
1637 6848.084979479237
1638 6848.094853157631
1639 6848.102951602736
1640 6848.109291437763
1641 6848.1139285118015
1642 6848.116934886891
1643 6848.118409893294
1644 6848.118534215324
1645 6848.1175550342205
1646 6848.115662273838
1647 6848.11305384167
1648 6848.110023095966
1649 6848.1068550205055
1650 6848.103734701038
1651 6848.100773440587
1652 6848.098054738069
1653 6848.0956210585055
1654 6848.093473415337
1655 6848.092895620071
1656 6848.0957427087
1657 6848.102341814774
1658 6848.108738105373
1659 6848.110124659694
1660 6848.10458445044
1661 6848.091329295517
1662 6848.070035196039
1663 6848.044617301774
1664 6848.021886410768
1665 6848.005231287067
1666 6847.996648920647
1667 6847.996373822572
1668 6848.003098917835
1669 6848.015771043396
1670 6848.033572347282
1671 6848.058481751274
1672 6848.090138780671
1673 6848.1265158295455
1674 6848.168350693807
1675 6848.213860214095
1676 6848.260722810725
1677 6848.3067990156405
1678 6848.350351317924
1679 6848.390491343811
1680 6848.427661493858
1681 6848.461302818836
1682 6848.490081352322
1683 6848.514293369852
1684 6848.534281855107
1685 6848.550366577384
1686 6848.562854269475
1687 6848.572017195526
1688 6848.578100171942
1689 6848.580825202411
1690 6848.582808814225
1691 6848.584548913793
1692 6848.5821744873165
1693 6848.574555541951
1694 6848.562304260077
1695 6848.547170160378
1696 6848.529298100222
1697 6848.5090881890765
1698 6848.487785893225
1699 6848.466130579919
1700 6848.444735894942
1701 6848.425914986854
1702 6848.411029265778
1703 6848.399202388988
1704 6848.389722498107
1705 6848.38222148324
1706 6848.37644068555
1707 6848.372162544459
1708 6848.369229334795
1709 6848.367527355627
1710 6848.366974710373
1711 6848.367553839253
1712 6848.369195736934
1713 6848.371730176388
1714 6848.374947056486
1715 6848.378609882982
1716 6848.382471704954
1717 6848.386312245593
1718 6848.389891305818
1719 6848.39295081468
1720 6848.395238596356
1721 6848.396529427305
1722 6848.396716906439
1723 6848.395788851504
1724 6848.393801848765
1725 6848.390869023569
1726 6848.387127943475
1727 6848.382707509586
1728 6848.377736152566
1729 6848.372336345912
1730 6848.3666138214985
1731 6848.3606661498125
1732 6848.354590917749
1733 6848.348477116153
1734 6848.342402790382
1735 6848.33643814226
1736 6848.330647333246
1737 6848.325097690717
1738 6848.32023211395
1739 6848.317600322292
1740 6848.317785650393
1741 6848.31928630722
1742 6848.320789310231
1743 6848.319783961086
1744 6848.315121464856
1745 6848.309737562178
1746 6848.303642705885
1747 6848.295386888169
1748 6848.287911043624
1749 6848.281120760581
1750 6848.273291491499
1751 6848.2651667437985
1752 6848.257346951112
1753 6848.250296703378
1754 6848.244371054466
1755 6848.2398252221965
1756 6848.23682408425
1757 6848.235462289372
1758 6848.235774661669
1759 6848.237718674673
1760 6848.2411698185615
1761 6848.245940542667
1762 6848.251815451958
1763 6848.258591211928
1764 6848.2660866167025
1765 6848.274145115422
1766 6848.282525997397
1767 6848.291254450523
1768 6848.300556096937
1769 6848.31057968127
1770 6848.321390997427
1771 6848.332984887098
1772 6848.345306793987
1773 6848.358266795416
1774 6848.371651548128
1775 6848.384522877119
1776 6848.395543592937
1777 6848.403842965983
1778 6848.408485767671
1779 6848.409180168103
1780 6848.405101755144
1781 6848.395691972054
1782 6848.381610212544
1783 6848.363572630038
1784 6848.342296332522
1785 6848.32469408288
1786 6848.316129426341
1787 6848.315861837846
1788 6848.324070453956
1789 6848.339337791352
1790 6848.359546170769
1791 6848.378485782937
1792 6848.395898235872
1793 6848.4157740039045
1794 6848.436316409949
1795 6848.45619886797
1796 6848.474585641482
1797 6848.490976640835
1798 6848.505063311949
1799 6848.516648602395
1800 6848.5257759710275
1801 6848.532794994191
1802 6848.537787349596
1803 6848.540326181049
1804 6848.542104877962
1805 6848.544622411437
1806 6848.547114686433
1807 6848.548942754265
1808 6848.549644690968
1809 6848.548886851368
1810 6848.546476601345
1811 6848.542413926591
1812 6848.5368221010995
1813 6848.529866719594
1814 6848.52171268949
1815 6848.512506528515
1816 6848.502403627378
1817 6848.491563297603
1818 6848.480153032006
1819 6848.46829207883
1820 6848.456089013323
1821 6848.443731624666
1822 6848.431411277101
1823 6848.419205643688
1824 6848.407092131411
1825 6848.395031265991
1826 6848.3829821419
1827 6848.370904078105
1828 6848.357957969819
1829 6848.3436216965565
1830 6848.328424035082
1831 6848.313433143109
1832 6848.299333261386
1833 6848.285979427224
1834 6848.273258106504
1835 6848.2610766633
1836 6848.249353250076
1837 6848.238035802789
1838 6848.226865651094
1839 6848.216243032373
1840 6848.206860049364
1841 6848.199078480896
1842 6848.192982060788
1843 6848.188520883504
1844 6848.185705072008
1845 6848.184639190563
1846 6848.186129795626
1847 6848.196585308141
1848 6848.220604269475
1849 6848.254285491248
1850 6848.289588974667
1851 6848.326845477948
1852 6848.3701799093
1853 6848.406671920574
1854 6848.426465166936
1855 6848.432437505372
1856 6848.426131514089
1857 6848.408546764793
1858 6848.381703441493
1859 6848.348199420368
1860 6848.309934044156
1861 6848.2687795286065
1862 6848.226504298887
1863 6848.184774494575
1864 6848.14520320646
1865 6848.109270607098
1866 6848.078182816369
1867 6848.053144035212
1868 6848.03467015595
1869 6848.022629786224
1870 6848.015704943844
1871 6848.01300472981
1872 6848.014745899629
1873 6848.020224793781
1874 6848.028309664514
1875 6848.037626746769
1876 6848.0484605265565
1877 6848.061470181774
1878 6848.075870105499
1879 6848.090846430218
1880 6848.105629700729
1881 6848.119586636552
1882 6848.132253503863
1883 6848.143294107597
1884 6848.151589020229
1885 6848.156692892237
1886 6848.159480695093
1887 6848.160690274219
1888 6848.161047026517
1889 6848.161225964831
1890 6848.161706898209
1891 6848.162877965701
1892 6848.165007025075
1893 6848.168176095131
1894 6848.17244028278
1895 6848.177827194579
1896 6848.184310219
1897 6848.19181944244
1898 6848.200266890203
1899 6848.209397987696
1900 6848.218981577967
1901 6848.228953869199
1902 6848.2391679212
1903 6848.249373363293
1904 6848.259498473395
1905 6848.269633156752
1906 6848.27974114472
1907 6848.289660531004
1908 6848.299177316175
1909 6848.308192650593
1910 6848.3167050355405
1911 6848.324662705567
1912 6848.331952902243
1913 6848.338438346926
1914 6848.335062009501
1915 6848.313272132003
1916 6848.288120136525
1917 6848.275431457576
1918 6848.261136820684
1919 6848.230503016994
1920 6848.19942004457
1921 6848.172820080751
1922 6848.1407926928005
1923 6848.106275407103
1924 6848.073356909713
1925 6848.044875615181
1926 6848.024076613202
1927 6848.016770643865
1928 6848.0254285900355
1929 6848.050698719935
1930 6848.080098772667
1931 6848.099102187858
1932 6848.106867462568
1933 6848.102938306928
1934 6848.087369463309
1935 6848.06087916773
1936 6848.024851610808
1937 6847.994104160358
1938 6847.974463120239
1939 6847.958544741578
1940 6847.948002122413
1941 6847.944583105285
1942 6847.949632303939
1943 6847.965437227779
1944 6847.99560778057
1945 6848.039825908176
1946 6848.094181072842
1947 6848.155514458172
1948 6848.2184045536305
1949 6848.270685031423
1950 6848.303677441016
1951 6848.316820059097
1952 6848.322771991774
1953 6848.330145039857
1954 6848.338064977744
1955 6848.33814293775
1956 6848.331431008866
1957 6848.330223724321
1958 6848.322520536961
1959 6848.307271687925
1960 6848.29526017685
1961 6848.276171370795
1962 6848.253867519276
1963 6848.231073794973
1964 6848.199565553217
1965 6848.17343798668
1966 6848.15294511401
1967 6848.128530590392
1968 6848.102040973729
1969 6848.074868290057
1970 6848.048010775089
1971 6848.02202956278
1972 6847.997240089207
1973 6847.974035844758
1974 6847.952743539413
1975 6847.933600018016
1976 6847.916804522166
1977 6847.90245879515
1978 6847.890585827256
1979 6847.8811272765315
1980 6847.873954728011
1981 6847.868845818199
1982 6847.8654874448985
1983 6847.863534041498
1984 6847.862672786808
1985 6847.8626230442
1986 6847.863088670522
1987 6847.863717712684
1988 6847.864316227102
1989 6847.86488617608
1990 6847.865428923457
1991 6847.865934971124
1992 6847.86640528404
1993 6847.8668412105135
1994 6847.867214344184
1995 6847.867504641541
1996 6847.867752249739
1997 6847.868040336171
1998 6847.868445670021
1999 6847.870786207133
2000 6847.877165623115


==> plotdata/satellite_constellation/sat_A4_dtheta.tex <==
t dtheta
0 25.000000000000004
1 24.999914200920205
2 24.99974078207085
3 24.99953293344446
4 24.999338034797074
5 24.999185207332555
6 24.999125763750346
7 24.999293285573366
8 24.999856632956565
9 25.000969012311277
10 25.002604431791177
11 25.004758236926676
12 25.007525522818923
13 25.01104429530682
14 25.01543206711245
15 25.020781310424535
16 25.027165681272987
17 25.034602102612098
18 25.04307996147207
19 25.052598566527255
20 25.063177505816675
21 25.074790207024723
22 25.087370122501557
23 25.10090038490326
24 25.115389231363192
25 25.130819338212522
26 25.14722090092388
27 25.16456849050795
28 25.182805306829774
29 25.201851066351487
30 25.221566797738983
31 25.241852727717834
32 25.26267838850441
33 25.283926462582016
34 25.305460698577605
35 25.327166743106467
36 25.34894266144015
37 25.370699449513786
38 25.39236207536431
39 25.413869647518137
40 25.435111002485236
41 25.455986952625285
42 25.47654303581639
43 25.496851584945716
44 25.51695891334846
45 25.536876327041224
46 25.556618715302115
47 25.576210102060095
48 25.59564449071212
49 25.615018337124678
50 25.634423537896264
51 25.653851804869202
52 25.673282353606723
53 25.692876963794735
54 25.7127742835175
55 25.7329772322772
56 25.753595054201913
57 25.774765073359227
58 25.796592506629977
59 25.819220696432566
60 25.842776068662634
61 25.867305962893923
62 25.892850269601006
63 25.91946190725958
64 25.947197259904698
65 25.976092814724097
66 26.00610099774551
67 26.03716401308352
68 26.06924520416199
69 26.102314604238362
70 26.13634336259394
71 26.171318164499837
72 26.207206894864523
73 26.24394616065361
74 26.281455536887982
75 26.319683861657335
76 26.358602654673067
77 26.398151317687265
78 26.438250799114044
79 26.478832219074615
80 26.519807338362934
81 26.561058184354962
82 26.60250550394915
83 26.64412237822926
84 26.685849629892182
85 26.727567934850807
86 26.769217491126444
87 26.81079315333059
88 26.852271878009326
89 26.893638146633126
90 26.93489065134498
91 26.976029098392416
92 27.017046287216832
93 27.05795730619519
94 27.09877346803796
95 27.139491577680115
96 27.180164245785303
97 27.220830135030077
98 27.261494989588204
99 27.302183826291657
100 27.34294190299543
101 27.38382672069918
102 27.424903063993675
103 27.466247160791557
104 27.507943421502173
105 27.550066827242194
106 27.59268277512004
107 27.63585872374267
108 27.67966207272432
109 27.724155093821146
110 27.76939171607386
111 27.81539760201691
112 27.862239183603215
113 27.91003347914873
114 27.958963906224795
115 28.009171674703882
116 28.060619475904325
117 28.113225204000408
118 28.16690833564268
119 28.221574676832358
120 28.27710805315418
121 28.33342978315507
122 28.39047273397131
123 28.448104326444952
124 28.506162245298064
125 28.56447703445861
126 28.62286450468052
127 28.681199313085795
128 28.73938706463568
129 28.79723778192729
130 28.854606909840395
131 28.911345732703296
132 28.96726327835265
133 29.022183614486252
134 29.075980606120805
135 29.128545399871133
136 29.179792560581777
137 29.22964602392921
138 29.27803720939455
139 29.324933020140644
140 29.37032231186988
141 29.414209410417126
142 29.456570992121286
143 29.4974689119858
144 29.537006795418673
145 29.575270928439195
146 29.612356444985444
147 29.64837673613295
148 29.683453572463687
149 29.717726142830212
150 29.751350565197722
151 29.784477517706517
152 29.81725334475735
153 29.84983571413733
154 29.882407753439665
155 29.915114391767126
156 29.94809464438136
157 29.98147020022007
158 30.015343338712075
159 30.04983087211461
160 30.0850107174696
161 30.120912467343175
162 30.15759033064542
163 30.195113181537046
164 30.233495110650026
165 30.27271341417785
166 30.31271981872616
167 30.353447494450876
168 30.3948401229295
169 30.436827991294457
170 30.47929663117024
171 30.52213561484209
172 30.565256042853065
173 30.608570314696166
174 30.651994791927454
175 30.695480773407763
176 30.738963875256605
177 30.78238839866609
178 30.825690823878947
179 30.868792274628092
180 30.91162550700011
181 30.954085433930253
182 30.99613869615396
183 31.037738626744193
184 31.078822520859006
185 31.119387146269325
186 31.159387682654756
187 31.198754416818158
188 31.23744531036844
189 31.27543874470659
190 31.312713017444047
191 31.34924454219348
192 31.385043239963945
193 31.420123713819656
194 31.45449152139062
195 31.4881627175406
196 31.521164114948906
197 31.55353992713026
198 31.58533155974547
199 31.616588234875987
200 31.647365209285134
201 31.6776780507992
202 31.707595469054358
203 31.737236598756592
204 31.766680441774884
205 31.796002359372018
206 31.825267212128995
207 31.85453186060256
208 31.883847971891225
209 31.913257631338197
210 31.942800436344037
211 31.972526129840684
212 32.00248262044534
213 32.03271745815867
214 32.063259001958336
215 32.09410384491761
216 32.12524885826146
217 32.156723771636386
218 32.188540994925354
219 32.220663304288124
220 32.25306538292368
221 32.28569684718614
222 32.318502179604195
223 32.35147923736662
224 32.38460327125229
225 32.41781924105243
226 32.45105226359954
227 32.484251254875154
228 32.51742973953677
229 32.550600550697105
230 32.58368299891214
231 32.61665182448875
232 32.64956561129553
233 32.68240823242838
234 32.71515196598462
235 32.74778122491254
236 32.78029365220517
237 32.81270978758538
238 32.845026283580154
239 32.87719913625612
240 32.90917979488226
241 32.94095891845835
242 32.97253306747249
243 33.00387140590905
244 33.03496749767534
245 33.06583728509355
246 33.09648355243165
247 33.1269111861428
248 33.15712380107915
249 33.18712170219901
250 33.21693846771917
251 33.246574161554015
252 33.27600197647426
253 33.30521595963894
254 33.33423379075554
255 33.363090932375705
256 33.391795834521375
257 33.42031922975566
258 33.44867058838093
259 33.47698451195331
260 33.505314788177934
261 33.533684830695556
262 33.562191347972515
263 33.590868481410354
264 33.61973569511866
265 33.64881567600152
266 33.67811789204076
267 33.707647179745585
268 33.737346985638
269 33.767150587636806
270 33.7970448535503
271 33.82700943949916
272 33.8570163775615
273 33.88704067791582
274 33.91705972404592
275 33.947052964101054
276 33.97698899953996
277 34.006853140403855
278 34.03663918769658
279 34.06633073489455
280 34.09591649148582
281 34.12537882308904
282 34.15472790897612
283 34.18394454765786
284 34.21302519927319
285 34.24200317017994
286 34.27082974784861
287 34.29950175365828
288 34.32803187858353
289 34.35638624249934
290 34.38455400879038
291 34.41252432017596
292 34.440277863621304
293 34.46786066655737
294 34.49534013557569
295 34.52272414776844
296 34.54997759959972
297 34.57703572501339
298 34.60396705339965
299 34.63082514319459
300 34.657628010142425
301 34.684461206088635
302 34.711354280212504
303 34.73832739758247
304 34.765429253484044
305 34.79269091297718
306 34.82004135155186
307 34.847428050574614
308 34.874864699523684
309 34.90233006572438
310 34.92976906937456
311 34.95713854290602
312 34.98441694167941
313 35.01158555434355
314 35.03862438266491
315 35.065506400220336
316 35.09220001856024
317 35.11871625815943
318 35.14509102831605
319 35.17131106889195
320 35.19740663672142
321 35.223437013126045
322 35.2494847756411
323 35.27568905497777
324 35.30213016096331
325 35.32881153871594
326 35.355683940528586
327 35.38269908970238
328 35.409806265630344
329 35.436959592683024
330 35.46413286966918
331 35.49131111120624
332 35.51849143455465
333 35.545667711359776
334 35.57283404482805
335 35.59998435434836
336 35.62711072672549
337 35.6542038837577
338 35.68125919274002
339 35.70827261177349
340 35.735240813275695
341 35.76215564635193
342 35.789005398451316
343 35.81578320104663
344 35.842488574935665
345 35.86913130028233
346 35.89573027491541
347 35.92230890729355
348 35.94889330999582
349 35.975509576107996
350 36.00217800948183
351 36.02891217363582
352 36.05572272445812
353 36.08261439175416
354 36.10958219678033
355 36.13661195783147
356 36.16369123958528
357 36.19081338513125
358 36.217969681107256
359 36.24514828976684
360 36.27232962672963
361 36.29950197414988
362 36.326658627928005
363 36.3537857074203
364 36.380868743557855
365 36.40789550707962
366 36.43485710193568
367 36.46174854110625
368 36.488568776587904
369 36.51531454205986
370 36.54201112030517
371 36.5687146893311
372 36.5954590918394
373 36.62224774531522
374 36.649088907151466
375 36.67599103172739
376 36.70296175005656
377 36.73004230281987
378 36.757269457355235
379 36.78463107961755
380 36.812117596030554
381 36.839737665473514
382 36.86749902372023
383 36.89540033947457
384 36.92341118873597
385 36.95146113647851
386 36.97949916018049
387 37.00751838383524
388 37.0355292926183
389 37.06353930013781
390 37.09155528035144
391 37.11956414206844
392 37.147550042272385
393 37.17549671484898
394 37.203388021578704
395 37.23120858092986
396 37.25895622717737
397 37.28662677433877
398 37.3141867401806
399 37.3416182990868
400 37.368931951201965
401 37.39611441949488
402 37.423170484931774
403 37.45014079137697
404 37.477045167407816
405 37.503876168133345
406 37.53064856705847
407 37.557418581295906
408 37.58420111237719
409 37.610974022088605
410 37.63773635176518
411 37.66448140208397
412 37.69120653684494
413 37.71789746576317
414 37.744537764766555
415 37.77112696755829
416 37.797680973381716
417 37.82419539733465
418 37.85065623426092
419 37.877036105872136
420 37.90332176775522
421 37.929526103126655
422 37.95564952698112
423 37.98169057884497
424 38.00765921761605
425 38.03357810890085
426 38.05949081810781
427 38.085443638442605
428 38.111464314950545
429 38.1375575093522
430 38.163718986228396
431 38.189945260415854
432 38.216240325380774
433 38.242614155921956
434 38.26906792210816
435 38.29559586160562
436 38.322191185207004
437 38.34884238211261
438 38.37553487478083
439 38.40226802852399
440 38.42906886034796
441 38.45592854589873
442 38.48284203050894
443 38.50981663592334
444 38.5368200657418
445 38.563848663676005
446 38.59090782308159
447 38.617978054418764
448 38.64504485219236
449 38.67208950786963
450 38.69907519937942
451 38.726021447423435
452 38.75295897985971
453 38.779888038184055
454 38.80678649401204
455 38.83361023397764
456 38.86038531813729
457 38.887115757964544
458 38.91379690563472
459 38.94044837925816
460 38.967095288982456
461 38.99374640269412
462 39.020413334645845
463 39.04710400629191
464 39.073822450693314
465 39.10053241749546
466 39.12720506799047
467 39.15385892390126
468 39.180517374457835
469 39.20720867923194
470 39.23394282264525
471 39.26069287747167
472 39.28743678862142
473 39.31421667739802
474 39.34104731474687
475 39.36790965572717
476 39.39484664572102
477 39.42182871235234
478 39.448845347264694
479 39.47595392872302
480 39.50308753296336
481 39.53020567129867
482 39.55733787385827
483 39.584520406653446
484 39.61174726595884
485 39.63900058022934
486 39.66626821894463
487 39.69352122085108
488 39.72070706777894
489 39.74779482182205
490 39.774772345231405
491 39.80162572179768
492 39.82833857964404
493 39.85489736747346
494 39.881291547985555
495 39.9075131389981
496 39.933562648115824
497 39.95944028770736
498 39.98514760520162
499 40.01069590521205
500 40.03611478574479
501 40.06144264762546
502 40.086717380196
503 40.11199050276792
504 40.13732937284044
505 40.16277690197531
506 40.18834740361798
507 40.214041784124554
508 40.23984393698943
509 40.26574678889431
510 40.291748035593386
511 40.317839396173724
512 40.344019997262535
513 40.370299517615244
514 40.39664230604777
515 40.42305280375272
516 40.44955882474084
517 40.47616841228868
518 40.50286928191953
519 40.52968665586396
520 40.55659533444374
521 40.58354299258265
522 40.61058895269119
523 40.63775288793777
524 40.66503287098402
525 40.69240724174652
526 40.71980469362966
527 40.74717505960137
528 40.77450011251646
529 40.80177892930288
530 40.82902012243451
531 40.85625189948688
532 40.8834994592825
533 40.91075121025084
534 40.93798894066567
535 40.96519070723191
536 40.992324696704294
537 41.019364025889026
538 41.0462882765777
539 41.07307762665219
540 41.099728911962764
541 41.126261145026255
542 41.15269357157384
543 41.17904170719927
544 41.20531345291007
545 41.231514389178635
546 41.25764915051262
547 41.28367650449751
548 41.309606253868665
549 41.3355247421327
550 41.36148209043867
551 41.38751508801444
552 41.41364929414591
553 41.439885528349976
554 41.46621855111865
555 41.492646203398195
556 41.51916820395877
557 41.5457808547148
558 41.572476497829406
559 41.599247480863184
560 41.626078531870185
561 41.652948727554026
562 41.679841895558106
563 41.706745659984875
564 41.733613407809614
565 41.760375591422495
566 41.78699113312014
567 41.81342779724296
568 41.83964725944603
569 41.86571027504274
570 41.89170093371131
571 41.91762258065189
572 41.9434754978157
573 41.9692608341848
574 41.994979826262764
575 42.02063582419614
576 42.046205624152066
577 42.07168113909282
578 42.09715837049333
579 42.12265482861702
580 42.14813223366748
581 42.17359251585892
582 42.19903618280259
583 42.22449258569357
584 42.249991563260316
585 42.27555619771778
586 42.30118549895981
587 42.326873566719364
588 42.35263024977606
589 42.3784570835466
590 42.40435149126994
591 42.4303073901891
592 42.456317250629006
593 42.482360338193594
594 42.50842271968398
595 42.53451087422204
596 42.5606333737147
597 42.586799702376126
598 42.61301943032172
599 42.63934211361988
600 42.665825614630435
601 42.69247982537226
602 42.71930260052997
603 42.746278253861114
604 42.77340443958966
605 42.80067883691912
606 42.82809827679079
607 42.8555904938863
608 42.88305845768926
609 42.91052235533595
610 42.93801776215102
611 42.96548858751033
612 42.99289040337016
613 43.02024140104747
614 43.047542275736404
615 43.07480774800155
616 43.10198247462814
617 43.129035263759064
618 43.15593470492594
619 43.18260988631522
620 43.20907067621121
621 43.2353303144466
622 43.2613956112906
623 43.287273324690545
624 43.31297799546094
625 43.33853492334791
626 43.363988756742344
627 43.389373994208356
628 43.414729335655636
629 43.44015343912205
630 43.465718483991374
631 43.49148840962386
632 43.51748936484286
633 43.543768453496696
634 43.5703510497465
635 43.597221185664004
636 43.624356841041916
637 43.65173318196924
638 43.67938259079824
639 43.70727996218968
640 43.73538428868881
641 43.76363491885827
642 43.79195543551187
643 43.82027962235011
644 43.84854344203576
645 43.87668596065017
646 43.904631762097985
647 43.9322984063815
648 43.95962127679081
649 43.98657119619439
650 44.01311458892841
651 44.03919140833924
652 44.06474445919091
653 44.08978860447417
654 44.114361184220144
655 44.13846453029061
656 44.16208672702865
657 44.18520580675812
658 44.207788609155564
659 44.22983217443118
660 44.25135055180236
661 44.27234687258859
662 44.29283587573146
663 44.31282425915955
664 44.33231492943286
665 44.35131397343326
666 44.36982982608862
667 44.387863853416775
668 44.405431496281345
669 44.422559555489066
670 44.43925283018002
671 44.455514668851116
672 44.47137653449133
673 44.48688436342547
674 44.50207103734455
675 44.516960493153164
676 44.53157071280981
677 44.54592739962324
678 44.56005190759698
679 44.57394314261777
680 44.58759098952187
681 44.600984203550105
682 44.614108045227574
683 44.62694999464448
684 44.63949013961509
685 44.651714810005885
686 44.66359287917567
687 44.67508181083355
688 44.68616192450346
689 44.69682620407028
690 44.70707043432381
691 44.71688758875782
692 44.726289962464826
693 44.7352569476546
694 44.743788383782096
695 44.75189075532516
696 44.759533409900044
697 44.766721222976884
698 44.77347441554325
699 44.7798082378135
700 44.785749092568466
701 44.79131899527177
702 44.79653423175328
703 44.801408815722134
704 44.80592416469612
705 44.810099394471244
706 44.81400252379269
707 44.817713386331086
708 44.821290052120105
709 44.82473332489211
710 44.82807523878918
711 44.831366889600396
712 44.83464640209428
713 44.837944225515955
714 44.84131406615036
715 44.84479989152213
716 44.84840393686442
717 44.85212206879637
718 44.855945054401204
719 44.859855122710606
720 44.863826466471416
721 44.8678297659053
722 44.871846370307175
723 44.875868627162745
724 44.87988396942444
725 44.883882284089474
726 44.887856527489426
727 44.89180262727343
728 44.89571606553776
729 44.89959165235242
730 44.90338287285773
731 44.907041307561045
732 44.9105617642558
733 44.91394261554427
734 44.917167250980135
735 44.920236348449635
736 44.92314687377972
737 44.925870114246656
738 44.928365976450266
739 44.93062032391136
740 44.93264606996369
741 44.93444847069521
742 44.93602889197391
743 44.93740370935121
744 44.938604278390066
745 44.93967644569942
746 44.940631742950735
747 44.941479696592694
748 44.94222565367327
749 44.94287861656145
750 44.94346517249109


==> plotdata/satellite_constellation/sat_A4_r.tex <==
t r
0 6848.233953273979
1 6848.224673624644
2 6848.19396553725
3 6848.137821418625
4 6848.052687500491
5 6847.935527118705
6 6847.78387486914
7 6847.59588055978
8 6847.370342318111
9 6847.106728203247
10 6846.805185860743
11 6846.466540165534
12 6846.092278822882
13 6845.68452617258
14 6845.246005709108
15 6844.779991971008
16 6844.290252331415
17 6843.780980185085
18 6843.256720446393
19 6842.722288499946
20 6842.182684340964
21 6841.643003294697
22 6841.108345167479
23 6840.583722457299
24 6840.0739704326415
25 6839.583660628307
26 6839.1170184095245
27 6838.67784687449
28 6838.269471796856
29 6837.894703882677
30 6837.555699771238
31 6837.253932596585
32 6836.990270316276
33 6836.764881940988
34 6836.577221298802
35 6836.426087147185
36 6836.309625894562
37 6836.225361207189
38 6836.170237599563
39 6836.14068292617
40 6836.132659504041
41 6836.1417365927355
42 6836.163182660836
43 6836.1920566683775
44 6836.223272886514
45 6836.251696958567
46 6836.272252834058
47 6836.279999778631
48 6836.2702348044295
49 6836.238726921562
50 6836.1814702251095
51 6836.094829088669
52 6835.976059492203
53 6835.823035171848
54 6835.634124055334
55 6835.408424291596
56 6835.145720605968
57 6834.846364318538
58 6834.511145852194
59 6834.141350075714
60 6833.739055542674
61 6833.306702102627
62 6832.847031939623
63 6832.3638811265655
64 6831.861241543634
65 6831.343021924343
66 6830.8138653180795
67 6830.278737093755
68 6829.742695056054
69 6829.210826530305
70 6828.688684275053
71 6828.181873556811
72 6827.6944439716935
73 6827.229847613119
74 6826.791913292085
75 6826.383993250834
76 6826.0089054009895
77 6825.668811826649
78 6825.365203711076
79 6825.098988035538
80 6824.870384537286
81 6824.678943448953
82 6824.523964776883
83 6824.403680493355
84 6824.315304238392
85 6824.255866252431
86 6824.221849213304
87 6824.209323342107
88 6824.213929574221
89 6824.230968289134
90 6824.255551089404
91 6824.282824087157
92 6824.307734573746
93 6824.325097216434
94 6824.330025621255
95 6824.31785568442
96 6824.284229140534
97 6824.225176913658
98 6824.137218585837
99 6824.017414964679
100 6823.863360178269
101 6823.6732481950185
102 6823.445961580277
103 6823.181050674066
104 6822.878751865523
105 6822.540028306606
106 6822.166532431178
107 6821.760547744662
108 6821.324851397009
109 6820.862808689495
110 6820.378319655328
111 6819.875704963898
112 6819.359694208852
113 6818.835211176399
114 6818.308831569871
115 6817.791182096504
116 6817.293227151628
117 6816.823878988243
118 6816.390249828452
119 6815.997661011925
120 6815.65074328327
121 6815.354218415029
122 6815.114083893876
123 6814.935955802386
124 6814.824802452136
125 6814.784286727534
126 6814.816331395261
127 6814.92051386742
128 6815.0973939689065
129 6815.347298264195
130 6815.668123717583
131 6816.057739406835
132 6816.512580012411
133 6817.027419535173
134 6817.595378928176
135 6818.209230988424
136 6818.860806673277
137 6819.542057592519
138 6820.243991511167
139 6820.95782744645
140 6821.674871804421
141 6822.38621576332
142 6823.082363026892
143 6823.753370702854
144 6824.391041479626
145 6824.988100173367
146 6825.5378968495315
147 6826.034409067839
148 6826.472409048017
149 6826.847482298297
150 6827.156427167884
151 6827.397379494552
152 6827.56934406379
153 6827.6727038147665
154 6827.7094777958555
155 6827.682891946011
156 6827.59712334496
157 6827.457440973474
158 6827.269798051986
159 6827.040854389881
160 6826.777848147634
161 6826.488194384007
162 6826.178972186831
163 6825.858418430877
164 6825.53496298259
165 6825.21676668394
166 6824.911240183859
167 6824.624753475519
168 6824.3626955373375
169 6824.130202169139
170 6823.93114530775
171 6823.767627195183
172 6823.6405763652665
173 6823.550159678361
174 6823.495743500352
175 6823.476409598718
176 6823.491871411009
177 6823.541694224574
178 6823.626037118632
179 6823.744163477932
180 6823.895333445563
181 6824.077742379552
182 6824.2886285754175
183 6824.526412666549
184 6824.788423058926
185 6825.072914517458
186 6825.378062808666
187 6825.7014585153565
188 6826.039682095347
189 6826.389087105333
190 6826.745856765325
191 6827.105931359934
192 6827.465181957051
193 6827.819441696743
194 6828.164353281154
195 6828.496145738567
196 6828.8113970918075
197 6829.106954343572
198 6829.380062376347
199 6829.628387536625
200 6829.850016993331
201 6830.042860101016
202 6830.2039173673875
203 6830.332429202524
204 6830.428779595364
205 6830.494140236459
206 6830.530190067854
207 6830.538871470041
208 6830.52225587685
209 6830.482501890272
210 6830.421635264109
211 6830.341913726376
212 6830.246023407754
213 6830.137209981397
214 6830.019296384261
215 6829.895616965575
216 6829.768960716211
217 6829.64225807319
218 6829.519358035942
219 6829.40369757851
220 6829.298240542871
221 6829.20526348266
222 6829.125119876286
223 6829.058911035785
224 6829.00844118691
225 6828.974407951368
226 6828.9567065747315
227 6828.954214686219
228 6828.964845991214
229 6828.98748959257
230 6829.021014619128
231 6829.062109561118
232 6829.109486864231
233 6829.162824180874
234 6829.221924159544
235 6829.2862576498665
236 6829.355291278901
237 6829.428475285454
238 6829.505202833833
239 6829.584849013887
240 6829.666865822055
241 6829.75074196012
242 6829.83606867865
243 6829.922557476812
244 6830.009630872831
245 6830.096814599912
246 6830.183813461197
247 6830.270174878132
248 6830.3553779436115
249 6830.438930218838
250 6830.520981908434
251 6830.6024796754755
252 6830.682999222183
253 6830.761863039941
254 6830.838481549699
255 6830.912379174016
256 6830.983209979534
257 6831.050813165498
258 6831.115188433911
259 6831.176232951161
260 6831.2336735423005
261 6831.2870787975435
262 6831.336472122463
263 6831.381967422957
264 6831.423706649085
265 6831.461821176604
266 6831.496431448893
267 6831.527636186113
268 6831.555510567272
269 6831.580154626999
270 6831.6017577454195
271 6831.620780485468
272 6831.637506473399
273 6831.652236968977
274 6831.665154608096
275 6831.6766907953825
276 6831.68706429424
277 6831.696092420544
278 6831.704007801399
279 6831.711097242278
280 6831.717547353352
281 6831.723305735528
282 6831.727913469862
283 6831.731599703227
284 6831.73402691063
285 6831.735964358066
286 6831.738140474489
287 6831.740839759105
288 6831.744278298776
289 6831.74884509866
290 6831.75495401006
291 6831.762916610312
292 6831.773016726306
293 6831.785359623784
294 6831.799788867128
295 6831.816118745784
296 6831.834280806699
297 6831.854156827119
298 6831.875695927337
299 6831.898871399759
300 6831.92362507582
301 6831.949844471801
302 6831.977422491273
303 6832.006035831461
304 6832.035330134087
305 6832.064960244228
306 6832.094587878679
307 6832.123896258781
308 6832.152590204895
309 6832.180405380509
310 6832.207149742972
311 6832.2326339840665
312 6832.25661029783
313 6832.278847832731
314 6832.299195217538
315 6832.317526762075
316 6832.333752943789
317 6832.347813853264
318 6832.359686351805
319 6832.369420529798
320 6832.377048422353
321 6832.382568726776
322 6832.3861356583075
323 6832.387840657414
324 6832.387768059518
325 6832.386067836495
326 6832.382887407724
327 6832.378363215831
328 6832.37263647969
329 6832.365866720667
330 6832.358192401446
331 6832.349706941659
332 6832.340594098105
333 6832.331035111038
334 6832.321278079369
335 6832.311583033381
336 6832.302262452293
337 6832.293542158522
338 6832.285652626921
339 6832.278896482749
340 6832.27366516281
341 6832.270502616605
342 6832.26996087306
343 6832.272334519014
344 6832.277666794876
345 6832.285826404941
346 6832.296600948359
347 6832.3097627707675
348 6832.325054212297
349 6832.342181691541
350 6832.360808551238
351 6832.3806236633745
352 6832.401349353071
353 6832.422673926673
354 6832.444295939663
355 6832.465965011367
356 6832.48744159007
357 6832.508484647228
358 6832.528860427625
359 6832.548356417904
360 6832.566775932848
361 6832.583943321162
362 6832.599707142183
363 6832.613940966334
364 6832.6265431438205
365 6832.637431184843
366 6832.6465432172145
367 6832.653840051071
368 6832.659315132475
369 6832.663012567766
370 6832.664985220434
371 6832.665291215884
372 6832.663990416371
373 6832.661120136411
374 6832.6567748893185
375 6832.6510531982285
376 6832.644094416085
377 6832.635954323293
378 6832.626756205145
379 6832.616649849593
380 6832.605838596877
381 6832.594569812944
382 6832.583151409531
383 6832.571894578457
384 6832.5610821345035
385 6832.550544977812
386 6832.5391594654175
387 6832.526515920197
388 6832.513016417226
389 6832.499069514637
390 6832.485096656963
391 6832.471459772457
392 6832.458522544239
393 6832.446660929363
394 6832.436226081274
395 6832.42752306913
396 6832.420975680712
397 6832.417356064992
398 6832.416872069295
399 6832.418795510014
400 6832.4225746942375
401 6832.427864409053
402 6832.434573711763
403 6832.443204353006
404 6832.454154371997
405 6832.467498495432
406 6832.483104359225
407 6832.500917880187
408 6832.5208305748365
409 6832.542546486939
410 6832.565847457372
411 6832.590420329321
412 6832.615705299133
413 6832.640874309161
414 6832.664805466446
415 6832.686589546418
416 6832.705643621393
417 6832.721737862929
418 6832.734741990653
419 6832.744311493845
420 6832.749557585137
421 6832.750250439181
422 6832.7466507924
423 6832.73869332409
424 6832.726603254438
425 6832.710874852802
426 6832.691834049436
427 6832.669984451227
428 6832.64611001553
429 6832.621091856575
430 6832.595783632186
431 6832.570933225177
432 6832.547150344909
433 6832.524946859587
434 6832.504886140092
435 6832.4873947274955
436 6832.472737899654
437 6832.461073382501
438 6832.452434928001
439 6832.446780668124
440 6832.44425522009
441 6832.445124306858
442 6832.448928604872
443 6832.455842181457
444 6832.465515281089
445 6832.477156098173
446 6832.49076433144
447 6832.506217909704
448 6832.523243232725
449 6832.541542387495
450 6832.560576093889
451 6832.579760215252
452 6832.599012966372
453 6832.618379712681
454 6832.637649745924
455 6832.656429611994
456 6832.67423808492
457 6832.690752004688
458 6832.705549031435
459 6832.71833194383
460 6832.728974518681
461 6832.737445473792
462 6832.743774867475
463 6832.748073465284
464 6832.750526783796
465 6832.751301753255
466 6832.750369226979
467 6832.747812406233
468 6832.743789771319
469 6832.738398735241
470 6832.731750320116
471 6832.723942640532
472 6832.715101616795
473 6832.7053991267285
474 6832.695088249611
475 6832.684582346737
476 6832.674093275175
477 6832.663683920983
478 6832.652778977013
479 6832.641958299059
480 6832.631689326152
481 6832.621543088945
482 6832.611653481848
483 6832.603036339368
484 6832.59668082209
485 6832.593309420106
486 6832.593239344434
487 6832.596273478546
488 6832.602076906936
489 6832.6104451158535
490 6832.621226349626
491 6832.634203298027
492 6832.649094252447
493 6832.665582108124
494 6832.68332831509
495 6832.701936931079
496 6832.721073730125
497 6832.740526634924
498 6832.760039159773
499 6832.779345935016
500 6832.798161783625
501 6832.815934554535
502 6832.831650609335
503 6832.8445431403925
504 6832.85413669785
505 6832.860156316159
506 6832.862435634727
507 6832.860753498313
508 6832.855091891062
509 6832.845729146509
510 6832.83312080351
511 6832.817571634209
512 6832.799422162541
513 6832.779056937938
514 6832.756662189472
515 6832.731375479227
516 6832.703320925271
517 6832.672144339433
518 6832.637683464291
519 6832.5993938045285
520 6832.558294300537
521 6832.513057533185
522 6832.463657501009
523 6832.411831253838
524 6832.360015957213
525 6832.310975847683
526 6832.266551056042
527 6832.227694960769
528 6832.19470161588
529 6832.167391093468
530 6832.145906466715
531 6832.130401817495
532 6832.121152482689
533 6832.119125824383
534 6832.125134609782
535 6832.139443456582
536 6832.162087973038
537 6832.192673936544
538 6832.230513303753
539 6832.274657224276
540 6832.323725886045
541 6832.376450242618
542 6832.431919749963
543 6832.489236801603
544 6832.547456170834
545 6832.605599967437
546 6832.662690804846
547 6832.717195906676
548 6832.7660354237605
549 6832.807670070351
550 6832.841773741999
551 6832.868429895599
552 6832.887888262405
553 6832.900517182518
554 6832.906795629992
555 6832.907268279034
556 6832.902544652598
557 6832.893349668178
558 6832.880423527338
559 6832.864557920802
560 6832.846801518307
561 6832.827933330388
562 6832.8082311156295
563 6832.787895409644
564 6832.767082001841
565 6832.745937167073
566 6832.724675785744
567 6832.703537972324
568 6832.682767383834
569 6832.662599646944
570 6832.643286506597
571 6832.625119937107
572 6832.60846039216
573 6832.593547624257
574 6832.580627103017
575 6832.569693477689
576 6832.560565728586
577 6832.552873459217
578 6832.5464418106
579 6832.541877229047
580 6832.539552386921
581 6832.539418939343
582 6832.5414330006215
583 6832.545515865838
584 6832.5514143457885
585 6832.558812021229
586 6832.56741923048
587 6832.576941648678
588 6832.587084759353
589 6832.597555957812
590 6832.608091002042
591 6832.618450745649
592 6832.62841611263
593 6832.637787529249
594 6832.6463857049175
595 6832.65405086779
596 6832.6606433330735
597 6832.666047256366
598 6832.670177591873
599 6832.6729803029175
600 6832.674427820835
601 6832.674515096981
602 6832.673253491665
603 6832.670668613903
604 6832.666840875242
605 6832.661972034153
606 6832.656058450047
607 6832.649138883754
608 6832.641196620866
609 6832.632175960176
610 6832.621814144963
611 6832.608834797986
612 6832.5930151873
613 6832.573222088185
614 6832.550424848547
615 6832.525416218558
616 6832.499404904903
617 6832.472467771094
618 6832.445659439018
619 6832.418591451539
620 6832.39258353332
621 6832.369226052066
622 6832.349844393527
623 6832.335274963413
624 6832.325757353676
625 6832.321077912781
626 6832.320890284988
627 6832.324956566867
628 6832.33325641054
629 6832.345187968331
630 6832.360634748335
631 6832.379302497282
632 6832.401020320065
633 6832.424355520747
634 6832.449440946014
635 6832.474973956542
636 6832.501171016835
637 6832.526183212596
638 6832.549630206031
639 6832.572074260395
640 6832.5952007717215
641 6832.620819643412
642 6832.6505265035275
643 6832.68680206069
644 6832.732110596416
645 6832.788714847021
646 6832.858912734649
647 6832.944763685201
648 6833.047164478472
649 6833.166482424254
650 6833.30330521757
651 6833.4580978872755
652 6833.630990879005
653 6833.821759098941
654 6834.030057480813
655 6834.255332450161
656 6834.496750688833
657 6834.753246471808
658 6835.023514285458
659 6835.30600857678
660 6835.598993236962
661 6835.900531303456
662 6836.208016512899
663 6836.5189831287435
664 6836.831552722576
665 6837.143752840933
666 6837.453607073782
667 6837.7591796338065
668 6838.0586020492565
669 6838.350105899346
670 6838.632088188392
671 6838.903196660858
672 6839.1618062251955
673 6839.40642147345
674 6839.63616689265
675 6839.851328917364
676 6840.05392038095
677 6840.245762586626
678 6840.428992296847
679 6840.606179222135
680 6840.7787928937105
681 6840.948041718735
682 6841.114949652499
683 6841.2815208120455
684 6841.449105598789
685 6841.622224811785
686 6841.805582936309
687 6841.995077305252
688 6842.185164079121
689 6842.372962677821
690 6842.55676583018
691 6842.735741988608
692 6842.909359296116
693 6843.077161787103
694 6843.238741851473
695 6843.393775625854
696 6843.541979900258
697 6843.683319498217
698 6843.818102070538
699 6843.947055058752
700 6844.072639034903
701 6844.1956907541635
702 6844.314992521048
703 6844.430877186011
704 6844.543549754476
705 6844.6531320116865
706 6844.75971091704
707 6844.863345220951
708 6844.964008220963
709 6845.061606715794
710 6845.156017671321
711 6845.247147933013
712 6845.334950524655
713 6845.419361407356
714 6845.500325752399
715 6845.577771081243
716 6845.651696194401
717 6845.72217567636
718 6845.789335551553
719 6845.853272098727
720 6845.913970679122
721 6845.971575251515
722 6846.026452956541
723 6846.079069902219
724 6846.129782915336
725 6846.17871339188
726 6846.225966400905
727 6846.271850060298
728 6846.316958191461
729 6846.361808453881
730 6846.406809583422
731 6846.451001534708
732 6846.492970258963
733 6846.53466668175
734 6846.578722137209
735 6846.621921009788
736 6846.661704299223
737 6846.699226389126
738 6846.734499605858
739 6846.766407153991
740 6846.794561782319
741 6846.819004633448
742 6846.840479576695
743 6846.860159587164
744 6846.8785326638945
745 6846.895681462362
746 6846.913079460482
747 6846.933262720233
748 6846.956216173823
749 6846.98003976307
750 6847.004711647571


==> plotdata/satellite_constellation/sat_A5_dtheta.tex <==
t dtheta
0 50.0
1 49.99991420090425
2 49.999740782139575
3 49.999532933775846
4 49.999338035667854
5 49.99918520918779
6 49.99912576720124
7 49.9992932914062
8 49.99985664203094
9 50.00096902546719
10 50.00260444982644
11 50.00475826057318
12 50.00752555276483
13 50.01104433221052
14 50.01543211156472
15 50.02078136290157
16 50.027165742403476
17 50.03460217302927
18 50.04308004191239
19 50.05259865790161
20 50.06317760921658
21 50.07479032354826
22 50.08737025304437
23 50.100900530768605
24 50.11538939400833
25 50.13081951891746
26 50.14722110075154
27 50.16456871027779
28 50.182805532544904
29 50.20185135598971
30 50.221567390266316
31 50.24185393183296
32 50.26268053381381
33 50.283929956759565
34 50.30546597996455
35 50.327174228639585
36 50.34895274133478
37 50.37071248179392
38 50.392378376628876
39 50.41388948753069
40 50.43513461920129
41 50.4560145357808
42 50.476574716103976
43 50.49688742655833
44 50.51699895119546
45 50.53692052757234
46 50.5566669925207
47 50.57626234217363
48 50.595700531991994
49 50.615078093972755
50 50.63448736114548
51 50.65392014475308
52 50.67335592308797
53 50.69295749468853
54 50.71286506680209
55 50.73308347264066
56 50.753724500812396
57 50.77492808328309
58 50.79680217670441
59 50.81949316895412
60 50.84312977660711
61 50.86776103582304
62 50.893427420391546
63 50.92018099451079
64 50.94807782071129
65 50.97715301222453
66 51.007356312068254
67 51.03862673019723
68 51.070924248793084
69 51.10421533854066
70 51.13846739112206
71 51.17366532378763
72 51.20977681816817
73 51.246736048802674
74 51.28445915735249
75 51.322891744573774
76 51.36200225085914
77 51.401727420777505
78 51.44198572207379
79 51.482705939123385
80 51.52379789093563
81 51.565142023877954
82 51.606657824344595
83 51.648318972813115
84 51.69006666212828
85 51.731781844711236
86 51.77340561001043
87 51.814933920042996
88 51.8563454039676
89 51.897626559856455
90 51.93877827773716
91 51.97980253332152
92 52.0206952953606
93 52.06147499847239
94 52.10215601487135
95 52.142738321155925
96 52.18327774247461
97 52.22381607225572
98 52.26436159572992
99 52.30494180929623
100 52.34560526587224
101 52.38641251504041
102 52.42743035081061
103 52.46873684603256
104 52.51041737843037
105 52.552547630457546
106 52.59519271287478
107 52.63842166158084
108 52.6823047751065
109 52.72690276224516
110 52.77226849567081
111 52.81842577930432
112 52.865442675807785
113 52.91342853869338
114 52.96246252215647
115 53.01260261791966
116 53.06387288760101
117 53.11627692045984
118 53.16981305087457
119 53.22445257660845
120 53.28011378943215
121 53.33670366387739
122 53.394151928306954
123 53.452370948890184
124 53.511260244148616
125 53.570726788467795
126 53.63069867575249
127 53.69111027233927
128 53.75186483167699
129 53.81287465239566
130 53.874078661169385
131 53.93538301164041
132 53.99669850215536
133 54.05795276682048
134 54.11909464336344
135 54.18008132696334
136 54.24087983332072
137 54.301466092270715
138 54.36182689494348
139 54.42195113752207
140 54.48186166927051
141 54.54167240022193
142 54.60154604834689
143 54.661586774612815
144 54.721789048458504
145 54.78206874917654
146 54.84236975447401
147 54.90273275701767
148 54.96317009614364
149 55.023630508913875
150 55.084109770285025
151 55.14466921550639
152 55.2053639033056
153 55.26622696884669
154 55.32729574834063
155 55.38858565314939
156 55.45010754259204
157 55.511865168061505
158 55.57385455240696
159 55.63609353868001
160 55.69857473810731
161 55.76127752676217
162 55.82418909926571
163 55.88730280515218
164 55.950606341327294
165 56.01407425334701
166 56.07767914994303
167 56.1413911593008
168 56.20517782474811
169 56.269006217740774
170 56.332842901419674
171 56.396656598125
172 56.46041933755975
173 56.524104334255526
174 56.587686373214886
175 56.651141024725376
176 56.714441477695814
177 56.77756404195265
178 56.84049143157772
179 56.90321215224669
180 56.96571904571507
181 57.02800884858555
182 57.090082818338935
183 57.15194700405864
184 57.21360290134935
185 57.27507128440161
186 57.33637954536127
187 57.39754175420428
188 57.45858034255049
189 57.519519247203746
190 57.580385767715114
191 57.64119569021786
192 57.701989638409664
193 57.76281009873962
194 57.82366935666556
195 57.88457624056437
196 57.945551580957726
197 58.00662175695151
198 58.067802410107554
199 58.12911029168861
200 58.190560468053654
201 58.2521652919753
202 58.31393414562067
203 58.37587405277772
204 58.43799007405193
205 58.50028340100591
206 58.56275154838394
207 58.62538945979272
208 58.688189064446185
209 58.75113916302201
210 58.81422548276326
211 58.87743084908828
212 58.940735793953344
213 59.00411893873368
214 59.06755817028507
215 59.131028483193056
216 59.19450380755256
217 59.25795962512075
218 59.32137103805737
219 59.384714992739696
220 59.447967375002506
221 59.51110525321916
222 59.5741103848331
223 59.63696580258803
224 59.6996564592771
225 59.76217091173865
226 59.82446977522695
227 59.886556677236584
228 59.94847149209641
229 60.01021111943998
230 60.071778978688464
231 60.133188138419634
232 60.194456656308304
233 60.25558741272526
234 60.31658770396756
235 60.377480083263784
236 60.438294222507054
237 60.49908520081719
238 60.559883654669264
239 60.62068003329581
240 60.68145451925236
241 60.74222616155853
242 60.803027930201985
243 60.86384944301036
244 60.924703572474776
245 60.985630796167335
246 61.04665256367552
247 61.10779450989309
248 61.16907177035083
249 61.23048998615462
250 61.292056353805606
251 61.35377662171963
252 61.415653837919656
253 61.4776725310136
254 61.53983474575025
255 61.60215571095151
256 61.66461969202601
257 61.72716658855988
258 61.78977700854127
259 61.85256623350064
260 61.91555894745763
261 61.97873396329329
262 62.04214810709569
263 62.10580156296532
264 62.16967930728456
265 62.2337705224233
266 62.29805259936187
267 62.36250149590413
268 62.427032613786395
269 62.491553638130654
270 62.55602193652546
271 62.62039735776944
272 62.684640834604416
273 62.748719343293054
274 62.81260131999239
275 62.87626321463346
276 62.9396851528312
277 63.002852442664135
278 63.06576822752829
279 63.12843103795569
280 63.19084117260013
281 63.25301111043355
282 63.31495556939507
283 63.37669193791076
284 63.43824202954857
285 63.4996291870012
286 63.56085155851369
287 63.62194861973437
288 63.68294602411064
289 63.74384315639236
290 63.804648863186216
291 63.86540357686358
292 63.92613402142276
293 63.98683538538417
294 64.0475740084467
295 64.10844594391908
296 64.16944192854663
297 64.23044762706898
298 64.29149401519295
299 64.35264897613524
300 64.41396371187047
301 64.47553864988134
302 64.53738249301023
303 64.5994976715893
304 64.66192808374298
305 64.72468164591112
306 64.78767632411517
307 64.85083859855189
308 64.91415900264394
309 64.97759163855523
310 65.04105629241819
311 65.10448473880025
312 65.16783074545656
313 65.23104934801091
314 65.29409473932499
315 65.35691657701503
316 65.41946120533404
317 65.48172004823357
318 65.54371230507323
319 65.6054093997667
320 65.66682916481756
321 65.72802214337757
322 65.78906515831903
323 65.85009616008092
324 65.91119628228779
325 65.97237325628484
326 66.03358652126818
327 66.09479862500119
328 66.15597210351959
329 66.2170766502674
330 66.27810254272723
331 66.33905319749509
332 66.39994828475811
333 66.46080312060529
334 66.52163353107696
335 66.58245785803157
336 66.6432882368524
337 66.70413708450104
338 66.76502231632085
339 66.82595825622937
340 66.88695846132617
341 66.94802946610554
342 67.00917732211532
343 67.070415340008
344 67.13176013303124
345 67.19323294510004
346 67.2548576130149
347 67.31665854183242
348 67.37866260661028
349 67.44088774165013
350 67.5033419199164
351 67.56602726617794
352 67.62893911794802
353 67.692065007539
354 67.75537829062907
355 67.81884186908268
356 67.88242053028218
357 67.94608371616087
358 68.00979796979985
359 68.0735268149643
360 68.13722648629847
361 68.20086184855657
362 68.26440419860924
363 68.3278193649556
364 68.39107483779402
365 68.4541428146456
366 68.51700139968197
367 68.57963541003305
368 68.64203740464166
369 68.70419980236656
370 68.76614602791135
371 68.82793498226721
372 68.88960676719799
373 68.95117267216406
374 69.01265035428762
375 69.07406335427403
376 69.13543639459951
377 69.19682762465013
378 69.2582945089149
379 69.31984436629655
380 69.38148727293888
381 69.44326604911997
382 69.50519927168153
383 69.56729979686364
384 69.6295606270869
385 69.69195311517328
386 69.75446222345495
387 69.81706307030262
388 69.8797660549336
389 69.94259077291157
390 70.0055518781766
391 70.06864304779495
392 70.13185037417949
393 70.19515807277573
394 70.25854878403682
395 70.3220044756292
396 70.38550779981344
397 70.44904187200041
398 70.5125904170062
399 70.57613781099803
400 70.63966905567658
401 70.70314852235467
402 70.76654435984877
403 70.82986808380402
404 70.8931328899031
405 70.95632022894108
406 71.01942687331017
407 71.08248951962986
408 71.14551010828686
409 71.20845340977897
410 71.27130241112928
411 71.33404264653272
412 71.39666891805504
413 71.45916908792323
414 71.52152074458967
415 71.58370691335564
416 71.64572978934655
417 71.70757965461198
418 71.76924387729922
419 71.83071311299193
420 71.89198018003593
421 71.95304481492495
422 72.01391986594413
423 72.07460878132768
424 72.13513109897123
425 72.19551708322025
426 72.25581644811281
427 72.31610996145322
428 72.37642398598824
429 72.43676852689936
430 72.49717606966901
431 72.55766873043815
432 72.61827556627073
433 72.67902560949132
434 72.73994045571528
435 72.801037977006
436 72.86233001435458
437 72.92382125652355
438 72.98550999373506
439 73.04740396341009
440 73.10952250450943
441 73.1718705958443
442 73.23444476740977
443 73.29723431537914
444 73.36022295459594
445 73.42338919272477
446 73.48670711297767
447 73.55014793179316
448 73.61368098613261
449 73.6772738505034
450 73.74087307884189
451 73.80446507854678
452 73.8680479737304
453 73.93160119641755
454 73.99508605539685
455 74.0584434887189
456 74.12167960189083
457 74.18478134227085
458 74.24772667395794
459 74.31051332194701
460 74.37315075674117
461 74.43563645734463
462 74.49797368037098
463 74.56016498953049
464 74.62221292898357
465 74.6840898627027
466 74.74577679885272
467 74.8072993226081
468 74.8686926785492
469 74.93000093124327
470 74.99125103399514
471 75.05243382755478
472 75.11354747405905
473 75.17465441690995
474 75.23579587363882
475 75.29696651589224
476 75.35823529227564
477 75.41961060324763
478 75.48108122792452
479 75.54270677222966
480 75.6044786093141
481 75.66636790306688
482 75.72837106194338
483 75.79053422078631
484 75.8528694892646
485 75.91537621891966
486 75.97806322227727
487 76.04091629238896
488 76.10388178377752
489 76.16692154455758
490 76.23001735817782
491 76.2931482528362
492 76.35628762393885
493 76.4194077737712
494 76.48248134452047
495 76.5454826342841
496 76.60838839446818
497 76.67117392590974
498 76.73381873490328
499 76.79630975510403
500 76.85865256156491
501 76.92087620281761
502 76.98300459001861
503 77.04505811700176
504 77.10707565986627
505 77.16907568309568
506 77.2310553057454
507 77.29299870963561
508 77.3548699408431
509 77.41665058944777
510 77.4783284967564
511 77.53989179771514
512 77.60134518466907
513 77.66270377826136
514 77.72398249676272
515 77.78521043956847
516 77.8463777682901
517 77.90748555777148
518 77.96860455847829
519 78.02971389109844
520 78.09078349031364
521 78.15184759141745
522 78.21291367916675
523 78.273993659539
524 78.33509269263274
525 78.3962109076821
526 78.4573352393959
527 78.51846331239628
528 78.57961890353539
529 78.64081445818512
530 78.70207215051884
531 78.76344921071166
532 78.82497673117076
533 78.88665104474694
534 78.9484674344543
535 79.01042056538655
536 79.07250285804555
537 79.13470445725596
538 79.19701272399465
539 79.25941162522977
540 79.32189055944893
541 79.38445268262382
542 79.44710080125799
543 79.50983314518395
544 79.57263893473264
545 79.63550182893756
546 79.69840240541474
547 79.7613206569172
548 79.82424145873722
549 79.88716046854256
550 79.95007518752986
551 80.01298567945354
552 80.07588653404696
553 80.13875108512688
554 80.20155081977394
555 80.26426530260453
556 80.32688625960216
557 80.3893994316015
558 80.45177537104591
559 80.51400956555206
560 80.57610207951925
561 80.63803895466155
562 80.6998223408475
563 80.7614624895872
564 80.82293066054828
565 80.88417625636357
566 80.94517876026231
567 81.00592738393732
568 81.06640749889465
569 81.12670434187949
570 81.18692681994344
571 81.24713563631325
572 81.30731746084683
573 81.36749675930145
574 81.42769335786795
575 81.48793159072127
576 81.54820835467164
577 81.60849012263745
578 81.6689086113521
579 81.72948960937417
580 81.79020980930831
581 81.85109233660629
582 81.91214866058807
583 81.97336201881977
584 82.03474774500367
585 82.0963485385592
586 82.15815185585991
587 82.22013866628556
588 82.28230294413495
589 82.34462767825707
590 82.40708977784203
591 82.46966177731481
592 82.5323140009762
593 82.5950031265269
594 82.65769269609649
595 82.72036702145495
596 82.78301331406519
597 82.84562078501837
598 82.90818018996686
599 82.97072414142639
600 83.03329583390654
601 83.09589342581627
602 83.15850573478048
603 83.22111065897752
604 83.28371114756914
605 83.3462928035072
606 83.40884467174492
607 83.47131649081186
608 83.53361800028227
609 83.59577986316714
610 83.6578841497308
611 83.71986172979065
612 83.78169838111607
613 83.84341005494866
614 83.90496192215672
615 83.96639026675719
616 84.02767882013045
617 84.08882344391502
618 84.14980906395087
619 84.2105793938472
620 84.27114345345271
621 84.33153816197606
622 84.39178142878293
623 84.45191648068474
624 84.51199455492535
625 84.57204763731869
626 84.63212211753373
627 84.6922867128188
628 84.75257931964678
629 84.81310851261345
630 84.87393713973172
631 84.93512853963294
632 84.99672531201472
633 85.05875508346853
634 85.12122112637216
635 85.18408688706924
636 85.2473084702542
637 85.31082867935656
638 85.37466075225893
639 85.43873903640305
640 85.50298356193886
641 85.56732316598664
642 85.6316608975184
643 85.69590766294716
644 85.76005555984459
645 85.8240681377537
646 85.88788537317409
647 85.95149430737425
648 86.01485053805376
649 86.07792327384118
650 86.14066887940793
651 86.2030193815613
652 86.26491217761837
653 86.3263467483359
654 86.38733152426292
655 86.44784033181233
656 86.5078340456923
657 86.56726305561945
658 86.62606560508698
659 86.68420964666063
660 86.74168143266118
661 86.79845711171886
662 86.85451956668805
663 86.90984339669217
664 86.96440949782286
665 87.01820645833784
666 87.07122680306689
667 87.1234599694557
668 87.17491347837108
669 87.22560937776332
670 87.27555106511213
671 87.32475411029215
672 87.37326466414316
673 87.42113316313063
674 87.46840307228615
675 87.51511604024718
676 87.56131253762014
677 87.60704907583461
678 87.65238238093274
679 87.69735567766678
680 87.74200924487515
681 87.78638231600767
682 87.83050999286357
683 87.87442663402503
684 87.91815982183466
685 87.9617343353347
686 88.00517726034943
687 88.04851093759733
688 88.09175134854472
689 88.13490806850827
690 88.17797948877745
691 88.2209506417967
692 88.26381780877801
693 88.30653620244784
694 88.34906148765789
695 88.39131408131024
696 88.43315312607858
697 88.47446239183205
698 88.51513866894877
699 88.55507366577348
700 88.59416035639728
701 88.63232058200258
702 88.66949463219882
703 88.7056180856902
704 88.74062885630121
705 88.7745256320629
706 88.8073696100668
707 88.83924596522284
708 88.87022809350333
709 88.90034103536458
710 88.9296486892636
711 88.95823956275599
712 88.98619583203153
713 89.01359755401808
714 89.0405492220041
715 89.0671371440165
716 89.09337297764938
717 89.11925533316344
718 89.14477992475379
719 89.16993889262721
720 89.1947210398975
721 89.21911167364374
722 89.24310688701544
723 89.26671672335709
724 89.28994919746052
725 89.31281235785475
726 89.33531430436248
727 89.35746352021448
728 89.379268842693
729 89.40073952469089
730 89.42188586792324
731 89.44271840293561
732 89.46324357649274
733 89.48346021473485
734 89.5033567692476
735 89.52293239376532
736 89.54217224836088
737 89.56104428582884
738 89.57950229425387
739 89.59751989416141
740 89.61509437205896
741 89.63221153585597
742 89.64885517388764
743 89.66503017376415
744 89.68075188909303
745 89.69604580034921
746 89.71090016825579
747 89.72531307036051
748 89.73928376861433
749 89.75280169879781
750 89.76587628807505
751 89.77851151873988
752 89.7907142693316
753 89.80248836863227
754 89.81383730802175
755 89.82476487635103
756 89.83527441378263
757 89.8453680764318
758 89.8550297323721
759 89.8642598852544
760 89.8730820146226
761 89.88150934194621
762 89.88955005174081
763 89.89721011759576
764 89.90449492021814
765 89.91140765107404
766 89.91795109393716
767 89.9241315499307
768 89.92995319477508
769 89.93541974582524
770 89.94053362232854
771 89.94526703514629
772 89.94960275056964
773 89.9535155065078
774 89.9570123185442
775 89.96009989642586
776 89.96276099666596
777 89.96500556124975
778 89.96682641039696
779 89.9682201402794
780 89.96918397211532
781 89.9697150590223
782 89.96981026816398
783 89.96946666860086
784 89.968677969298
785 89.96746208315724
786 89.96583229023305
787 89.96381855402524
788 89.96148862308672
789 89.95887713557917
790 89.95596902009054
791 89.95274157028493
792 89.94917641023767
793 89.94524903704911
794 89.94095438362686
795 89.93628363437143
796 89.93122627390211
797 89.92577792827122
798 89.91992060541578
799 89.91363298697809
800 89.90690705642473
801 89.89973147654489
802 89.892086038798
803 89.88394979932288
804 89.87530436877647
805 89.86612853673272
806 89.85642201599677
807 89.84618664590836
808 89.83540978251095
809 89.82409240416719
810 89.81224610502215
811 89.79988226623188
812 89.7870152312084
813 89.77366209132806
814 89.75983479828606
815 89.74553930140144
816 89.73078325758853
817 89.715566226705
818 89.69988398887514
819 89.68373707977402
820 89.66706635858705
821 89.64983740670675
822 89.6320606733119
823 89.61376982482682
824 89.59501239578583
825 89.5757811038297
826 89.5560860447608
827 89.53593053922643
828 89.51531934447571
829 89.4942612804716
830 89.47276421544346
831 89.45083248904801
832 89.42847307960662
833 89.40569259534259
834 89.38249663188832
835 89.35888966889945
836 89.33487507789667
837 89.31045541371402
838 89.28563369353171
839 89.26041360343369
840 89.23479727889953
841 89.20878753113331
842 89.18238777602832
843 89.15559773524605
844 89.12841478672134
845 89.10083726971895
846 89.0728627409028
847 89.04448596480265
848 89.01570026683933
849 88.98649638123085
850 88.95686667475425
851 88.92680574882213
852 88.89630044991505
853 88.86535108845268
854 88.83394869507217
855 88.80208810189102
856 88.76977391706782
857 88.73699940271038
858 88.70376760554213
859 88.67008084292601
860 88.63594015334193
861 88.6013439594603
862 88.56628405203357
863 88.53077417436859
864 88.49482634460027
865 88.45843902652945
866 88.4216133076986
867 88.38434746350006
868 88.3466551478399
869 88.3085497687194
870 88.27003971645361
871 88.23112956596135
872 88.19182681375607
873 88.1521394088738
874 88.11207530562918
875 88.07163639353021
876 88.03084323357298
877 87.98972660961448
878 87.94829027511308
879 87.90655571914277
880 87.86454314210678
881 87.82227185511424
882 87.77975955049104
883 87.73701830469074
884 87.69405375289492
885 87.65086268613825
886 87.60742905196567
887 87.56371871085808
888 87.51970296114729
889 87.47536925193742
890 87.43069366950806
891 87.3856433260892
892 87.34017860946064
893 87.29426484801493
894 87.24790064545338
895 87.20108260513409
896 87.15379942848597
897 87.1060322254414
898 87.05776719232466
899 87.00899938602495
900 86.95972004321747
901 86.90991914184963
902 86.85959324156399
903 86.80873980508925
904 86.75735194755231
905 86.70542169955993
906 86.65293961367637
907 86.59989452348607
908 86.546273770668
909 86.49206394171024
910 86.4372526936839
911 86.38183043154537
912 86.32579157017223
913 86.2691354572831
914 86.21186713057125
915 86.15399704172083
916 86.09553974198548
917 86.03651346827044
918 85.97693990441569
919 85.91678167284061
920 85.85588570383582
921 85.79418881486775
922 85.73181607713153
923 85.6689976569486
924 85.60591239280546
925 85.54263308346617
926 85.47921526634397
927 85.41571180425902
928 85.3521889459372
929 85.28869275106693
930 85.22526513700906
931 85.16193478014209
932 85.09871608822931
933 85.03557179699644
934 84.97245160824511
935 84.90934936307066
936 84.84627600386766
937 84.78325651598833
938 84.72030299673357
939 84.657417536059
940 84.59459779941753
941 84.53183576944603
942 84.46912734052782
943 84.40647852492368
944 84.34387588109621
945 84.2813456998666
946 84.21889552255331
947 84.15650631403507
948 84.09415230434686
949 84.03185776866832
950 83.9696817636552
951 83.90757827112897
952 83.84554444847777
953 83.78360443290157
954 83.72177311567229
955 83.66009077127961
956 83.59850939041962
957 83.53698342921356
958 83.47555095608335
959 83.41422067601478
960 83.3530072823864
961 83.29191991292346
962 83.2309743152119
963 83.17018065598586
964 83.10953532406981
965 83.04903081589345
966 82.9886643739751
967 82.92842919876966
968 82.86830473817396
969 82.80827293287274
970 82.74831234808431
971 82.68839788642684
972 82.62852974370769
973 82.56867056446865
974 82.50874652190001
975 82.44871456617615
976 82.38853000848985
977 82.32818729273347
978 82.26766417547425
979 82.20691959436341
980 82.14592990856131
981 82.08470583203905
982 82.02328939533027
983 81.96169782689695
984 81.89996512735026
985 81.83812891593189
986 81.77621198297125
987 81.71423242584034
988 81.65220269964423
989 81.59013148453658
990 81.52802409427021
991 81.46588214341638
992 81.40370831950858
993 81.34149966209101
994 81.27924821808092
995 81.2169487471195
996 81.15459785250053
997 81.09218377372687
998 81.02971568858023
999 80.96720676166244
1000 80.90464981334955
1001 80.8420475697187
1002 80.7794061226828
1003 80.71672858961128
1004 80.65402510594934
1005 80.59130710239678
1006 80.5285827340269
1007 80.46586537362016
1008 80.4031642846812
1009 80.34048573134555
1010 80.27783764416641
1011 80.21522797619556
1012 80.15266278431322
1013 80.0901479888692
1014 80.02768902164269
1015 79.9652909184241
1016 79.90295665023463
1017 79.84068566642244
1018 79.77847843440144
1019 79.7163359602341
1020 79.65426578727525
1021 79.59227480834562
1022 79.5303612398659
1023 79.46852484389923
1024 79.40678497570431
1025 79.34517184429006
1026 79.28367278218768
1027 79.22225108095721
1028 79.16088941723096
1029 79.0995599690644
1030 79.03822964931554
1031 78.97687536412278
1032 78.9155000478787
1033 78.85412598811756
1034 78.79273074729447
1035 78.73129401759891
1036 78.66980897771839
1037 78.60826667363075
1038 78.54666963553251
1039 78.48501395766914
1040 78.423312570907
1041 78.36155964910337
1042 78.29974471723526
1043 78.23787982182948
1044 78.1759701485194
1045 78.11403265298145
1046 78.05206869494846
1047 77.99008116133083
1048 77.92809363990048
1049 77.86610981010219
1050 77.80410113752113
1051 77.74203517646102
1052 77.67991443278288
1053 77.61774269160773
1054 77.55552851803968
1055 77.49328913024078
1056 77.43103686544607
1057 77.36878302357663
1058 77.3065389976468
1059 77.24431239286459
1060 77.18209578368332
1061 77.11989538814706
1062 77.05772543726208
1063 76.99558936493962
1064 76.933472960783
1065 76.8713653348303
1066 76.80928351795623
1067 76.74722798180538
1068 76.68519244343862
1069 76.6231752327775
1070 76.56119845421824
1071 76.499315499818
1072 76.4375057011685
1073 76.37574716845687
1074 76.31402739720035
1075 76.25232917693941
1076 76.19065274018818
1077 76.12898400357346
1078 76.06732024110283
1079 76.00565989373492
1080 75.94400784142623
1081 75.88238233247297
1082 75.82074235099563
1083 75.7590574934693
1084 75.69732294201376
1085 75.63555491424414
1086 75.57374222719258
1087 75.5118756966206
1088 75.44994635712487
1089 75.38794877766391
1090 75.32592522905315
1091 75.26388828830136
1092 75.20180049759446
1093 75.13965098627575
1094 75.07744568262068
1095 75.01519549049647
1096 74.95291435340272
1097 74.89063010701175
1098 74.82835134579173
1099 74.76606438889806
1100 74.7037701722203
1101 74.64145902539195
1102 74.57913899733619
1103 74.51682212513977
1104 74.45451613603649
1105 74.39224524107709
1106 74.33002322961103
1107 74.26784327591923
1108 74.20570920368915
1109 74.14363407041334
1110 74.08162174313497
1111 74.01964633026377
1112 73.9576960541974
1113 73.89577002306802
1114 73.8338698542316
1115 73.77199966033804
1116 73.71016644326342
1117 73.648372349945
1118 73.58661693278708
1119 73.52490220835534
1120 73.46322703643122
1121 73.40158588387955
1122 73.33997828075746
1123 73.27840413811772
1124 73.2168504552451
1125 73.15531469301108
1126 73.09379014480099
1127 73.03227075302462
1128 72.970745472316
1129 72.90920878998018
1130 72.84763617361749
1131 72.78598929747926
1132 72.72423055816041
1133 72.66232100471521
1134 72.60023902782372
1135 72.5379726678268
1136 72.47552029586035
1137 72.41289238674055
1138 72.3500905203854
1139 72.28711172215856
1140 72.22396384455706
1141 72.16068559673855
1142 72.0973325723236
1143 72.03397433951942
1144 71.97066899672798
1145 71.90746965094077
1146 71.84443718397439
1147 71.7815693139994
1148 71.71885917968099
1149 71.6563042953476
1150 71.59387061198255
1151 71.5314996555214
1152 71.46915224492743
1153 71.40680329748292
1154 71.34444301160462
1155 71.28207139223325
1156 71.21968824797612
1157 71.15729365335413
1158 71.09489102318175
1159 71.03248443136175
1160 70.97007793623386
1161 70.90767498265413
1162 70.84527844330849
1163 70.78289058642564
1164 70.72051298615726
1165 70.65814665781863
1166 70.59579221866495
1167 70.53344982637844
1168 70.47111964914481
1169 70.40880210748529
1170 70.34649703858152
1171 70.28420211470309
1172 70.22191524998912
1173 70.15963394500281
1174 70.09735528851617
1175 70.0350766184076
1176 69.97279456697187
1177 69.91050650352445
1178 69.84820945280697
1179 69.7858996570693
1180 69.7235739452587
1181 69.66123074497575
1182 69.59886758754165
1183 69.53646725204064
1184 69.47403227021297
1185 69.41157553048126
1186 69.3490959443121
1187 69.28660528558196
1188 69.22411049494875
1189 69.1616058687483
1190 69.09909023703152
1191 69.03656971366765
1192 68.97404931468432
1193 68.9115318781598
1194 68.84901390605472
1195 68.78650178944667
1196 68.72401463597318
1197 68.6615539800144
1198 68.59911409100754
1199 68.53669816330833
1200 68.47431369716506
1201 68.4119660353657
1202 68.34964992522242
1203 68.28736439934997
1204 68.22511544703508
1205 68.16290397201531
1206 68.10072787507164
1207 68.03858566954871
1208 67.97647524436265
1209 67.91439267345875
1210 67.8523355288612
1211 67.7903012589139
1212 67.72828312131803
1213 67.66627899304184
1214 67.60428621804108
1215 67.5422996530822
1216 67.48031886675454
1217 67.41833897085517
1218 67.35635746958361
1219 67.29437448109485
1220 67.23238531716703
1221 67.17038669368131
1222 67.10837382385914
1223 67.04634312320866
1224 66.98429416039903
1225 66.92222612128153
1226 66.86014725647516
1227 66.79805236240925
1228 66.7359279028564
1229 66.67377415013316
1230 66.6115916021998
1231 66.5493785397321
1232 66.48713244549113
1233 66.42485297140674
1234 66.36253790034264
1235 66.30018898023482
1236 66.23781319307598
1237 66.17541290393352
1238 66.11298957501009
1239 66.05054857086594
1240 65.98809616032328
1241 65.9256390623925
1242 65.86318133381586
1243 65.80072749796783
1244 65.7382842898436
1245 65.67585771714441
1246 65.61345114437883
1247 65.55106767686907
1248 65.48871254321008
1249 65.4263894649631
1250 65.36410254840436
1251 65.30185546833432
1252 65.23964916898508
1253 65.17748262418938
1254 65.11535011814952
1255 65.0532519667657
1256 64.99119013504549
1257 64.92916108559977
1258 64.86716263298504
1259 64.80519030791235
1260 64.74323931083937
1261 64.68130608103654
1262 64.61938813511044
1263 64.55748062374053
1264 64.49557787530061
1265 64.43367590271004
1266 64.37176942028547
1267 64.30985416698829
1268 64.2479261061826
1269 64.18598229824369
1270 64.12401691003626
1271 64.06202583148985
1272 64.00000514746516
1273 63.937955355248285
1274 63.87587595087328
1275 63.81376200019064
1276 63.751610690436294
1277 63.68941617474557
1278 63.627157853787175
1279 63.56483793147117
1280 63.50248311786656
1281 63.44010100469296
1282 63.37769292492786
1283 63.31525306496918
1284 63.252782711610124
1285 63.190292678962955
1286 63.12778774831512
1287 63.06526665717471
1288 63.00273485217067
1289 62.94020450549359
1290 62.87767899741379
1291 62.81516117542193
1292 62.752660529651564
1293 62.690184713862756
1294 62.62774661086488
1295 62.56533984036061
1296 62.502961627354345
1297 62.44062525898182
1298 62.378332063846514
1299 62.316081867579534
1300 62.253875213107364
1301 62.191712830980926
1302 62.12958899333084
1303 62.067501537182885
1304 62.0054505479978
1305 61.94343215807616
1306 61.88144475733468
1307 61.81948005751939
1308 61.75753019956742
1309 61.69559530660704
1310 61.63366791808167
1311 61.571752126227096
1312 61.509844486840315
1313 61.44792608600188
1314 61.38599909042167
1315 61.32406590526751
1316 61.26211824616276
1317 61.200148665866614
1318 61.13815073429698
1319 61.07612459676805
1320 61.0140740239484
1321 60.95199837625854
1322 60.889896808067014
1323 60.827769603540574
1324 60.76561775749564
1325 60.70344207371428
1326 60.641243589516925
1327 60.579024359815904
1328 60.5167857958908
1329 60.454530792129816
1330 60.39226485157286
1331 60.32999210412325
1332 60.267716272081536
1333 60.20543406222262
1334 60.14314673184858
1335 60.0808584818401
1336 60.01856149793117
1337 59.956263304982365
1338 59.89397183228321
1339 59.83168521048424
1340 59.769406870169774
1341 59.70713978509026
1342 59.64488760779185
1343 59.582653426263576
1344 59.52044009686623
1345 59.458251296544944
1346 59.39609005779626
1347 59.33395770575508
1348 59.27185412552655
1349 59.20977859709578
1350 59.14772947566105
1351 59.085705035221544
1352 59.02370400021707
1353 58.96172343250802
1354 58.89975952926729
1355 58.837809725842135
1356 58.77587050240786
1357 58.71393725357339
1358 58.65200525815878
1359 58.59006975505301
1360 58.52812551827802
1361 58.46616737791983
1362 58.40419178558106
1363 58.34219499154144
1364 58.280172906327
1365 58.21812208460458
1366 58.15603961162065
1367 58.093923257812264
1368 58.03177155649041
1369 57.96958319801646
1370 57.90735707026249
1371 57.845092951221105
1372 57.78279144471608
1373 57.72045399209134
1374 57.65808287560139
1375 57.59568114028992
1376 57.53323465697074
1377 57.47074018988982
1378 57.408223792429816
1379 57.34572759466629
1380 57.283259707958585
1381 57.22082898460479
1382 57.15845621947487
1383 57.09612310470577
1384 57.03384124745709
1385 56.97162977945103
1386 56.90948287238229
1387 56.847395698919186
1388 56.785344535687635
1389 56.72333725333039
1390 56.66139354078246
1391 56.59949723397846
1392 56.53765057687513
1393 56.47585113158922
1394 56.41409802066788
1395 56.35239156866488
1396 56.29071431394297
1397 56.22905720665099
1398 56.167421048037134
1399 56.10580968272089
1400 56.0442270440931
1401 55.982695061094915
1402 55.92123836532598
1403 55.85985769354321
1404 55.79854744378689
1405 55.73730424951449
1406 55.67611495346195
1407 55.61496203876824
1408 55.55383304625231
1409 55.492712200115406
1410 55.431586712732354
1411 55.37044463306503
1412 55.30927480219278
1413 55.24806266596092
1414 55.18679783499281
1415 55.12547321764934
1416 55.06405099145901
1417 55.002508637254394
1418 54.94091607601251
1419 54.879283444647434
1420 54.81762432184986
1421 54.75593519115295
1422 54.694096238861405
1423 54.632128876185185
1424 54.57003100643099
1425 54.50774316237569
1426 54.44537590620993
1427 54.38298989754425
1428 54.3204993393233
1429 54.257934779970945
1430 54.19530329581404
1431 54.13262120023001
1432 54.06990537510561
1433 54.00715924113727
1434 53.944395923438684
1435 53.881634732437476
1436 53.818882420064675
1437 53.75615652434297
1438 53.693512337218806
1439 53.63088640259223
1440 53.56835020885345
1441 53.505946045483135
1442 53.44371624065214
1443 53.38163103302382
1444 53.31960158076294
1445 53.25755045811384
1446 53.195487710097495
1447 53.133427641224905
1448 53.07133767337958
1449 53.00922065217786
1450 52.947114417991095
1451 52.88503808833982
1452 52.822899187538795
1453 52.76070499536289
1454 52.69849804775289
1455 52.636326172630085
1456 52.57422419276466
1457 52.51220433254699
1458 52.45026114531393
1459 52.38838326886128
1460 52.32660190228868
1461 52.264949862825155
1462 52.20340645446034
1463 52.14194387795511
1464 52.08052329022534
1465 52.01908589171806
1466 51.95764934461017
1467 51.89620193053396
1468 51.83472773077846
1469 51.7732223384241
1470 51.711667250067514
1471 51.65007444155944
1472 51.5884249292407
1473 51.52672624121249
1474 51.4649886389925
1475 51.40320519987805
1476 51.341403489467254
1477 51.27958986373987
1478 51.21777637239983
1479 51.15597116139299
1480 51.09418597132182
1481 51.03242820827307
1482 50.97070604444963
1483 50.909020322680384
1484 50.84737356098268
1485 50.78577563681225
1486 50.7242452447436
1487 50.6628015965451
1488 50.601436247212035
1489 50.540174913568414
1490 50.47898783531005
1491 50.417847246398516
1492 50.35671382607822
1493 50.29554500276988
1494 50.23432841805078
1495 50.17305759468234
1496 50.11172056358652
1497 50.05030372998523
1498 49.98881527664995
1499 49.92726053598245
1500 49.865638749630996
1501 49.803954349117696
1502 49.74218408126215
1503 49.680284143425375
1504 49.61830349502367
1505 49.55630649604111
1506 49.49425804893364
1507 49.4321474597307
1508 49.36994228334992
1509 49.30766360195787
1510 49.24537776161822
1511 49.18307232967567
1512 49.120678293031865
1513 49.05818631607305
1514 48.99561360793482
1515 48.9329670868889
1516 48.870292072886706
1517 48.80762292633271
1518 48.74500696737005
1519 48.68246873773104
1520 48.6200520822965
1521 48.5578444289433
1522 48.49593651160555
1523 48.43441919894668
1524 48.37338141498789
1525 48.31290235648117
1526 48.25304225418308
1527 48.19387446959013
1528 48.13546498068229
1529 48.07786893390294
1530 48.02117275265584
1531 47.965439672204404
1532 47.910700350859905
1533 47.85695247369475
1534 47.804210216755244
1535 47.752501420494795
1536 47.70179207917754
1537 47.65205395801746
1538 47.60326951057772
1539 47.55539868660213
1540 47.50840219133646
1541 47.462230908849776
1542 47.41680485425738
1543 47.37206705451634
1544 47.327957515792434
1545 47.284416598037375
1546 47.241427554425925
1547 47.198971330777525
1548 47.156968787316174
1549 47.1153039740726
1550 47.0738838458084
1551 47.03259258395833
1552 46.99130711680084
1553 46.94994831404072
1554 46.908453018104375
1555 46.86676717138472
1556 46.82487441994143
1557 46.78278395852298
1558 46.74051798533861
1559 46.69814370077773
1560 46.655742751773566
1561 46.61340506022037
1562 46.57123009123483
1563 46.52932027470971
1564 46.48777948726373
1565 46.4467132577023
1566 46.406228686263
1567 46.36642861849732
1568 46.32740305387367
1569 46.28922912784008
1570 46.25197645515773
1571 46.21569828055679
1572 46.18041432223379
1573 46.14611321682671
1574 46.1127638920836
1575 46.08032465715444
1576 46.04875052107585
1577 46.017990010058625
1578 45.987984931151715
1579 45.95868262770493
1580 45.93006488379553
1581 45.902121201682085
1582 45.87484375395052
1583 45.848223160442615
1584 45.82224353428997
1585 45.79687990821365
1586 45.7721075492727
1587 45.74790221535058
1588 45.724228526728076
1589 45.701042162237094
1590 45.678301322110784
1591 45.6559697913033
1592 45.63401502069425
1593 45.61240412499865
1594 45.591095870232984
1595 45.570049526026324
1596 45.549258483055354
1597 45.52871304430247
1598 45.508376747760174
1599 45.488220112088094
1600 45.46822087063512
1601 45.44836305895541
1602 45.42863691622078
1603 45.40903936305178
1604 45.389573473826914
1605 45.370248599591086
1606 45.35108099392199
1607 45.332092698193435
1608 45.31330943833734
1609 45.29475952259719
1610 45.276473961697455
1611 45.25848674625879
1612 45.24083426992174
1613 45.223555247318785
1614 45.20668811606452
1615 45.19027163876537
1616 45.174346004437226
1617 45.15894915508103
1618 45.14411201568203
1619 45.12985741184011
1620 45.11620670604218
1621 45.10317935994456
1622 45.090790476414334
1623 45.079050761566975
1624 45.06796756031025
1625 45.05754495357203
1626 45.04778262228314
1627 45.038674583963726
1628 45.03020921178422
1629 45.02236919921664
1630 45.01513285342794
1631 45.00847403717546
1632 45.00236236913973
1633 44.99676332640084
1634 44.99163902755876
1635 44.9869497024041
1636 44.982655978229
1637 44.97872274032396
1638 44.97511622516625
1639 44.97180334549661
1640 44.96875204176191
1641 44.965932792917066
1642 44.96332037163855
1643 44.960894260953644
1644 44.95863792166208
1645 44.95653905109419
1646 44.954591203375216
1647 44.95279289762586
1648 44.951138687196014
1649 44.94962412667782
1650 44.94824994799173
1651 44.947020580023384
1652 44.94594416914042
1653 44.94503167840725
1654 44.94429478460924
1655 44.94378522912638
1656 44.94354615153433
1657 44.94356790158113
1658 44.94384633944787
1659 44.944369919992596
1660 44.94511001296817
1661 44.946017856421804
1662 44.94704392247021
1663 44.94809204083068
1664 44.949083650453424
1665 44.95000748880968
1666 44.950862826775065
1667 44.951667768556156
1668 44.952443944911366
1669 44.95319112894307
1670 44.95387376973375
1671 44.95447130102581
1672 44.955046237247046
1673 44.955663526041384
1674 44.95632813757134
1675 44.957040085823635
1676 44.95780135667594
1677 44.95858404431398
1678 44.95938625563417
1679 44.96020298117637
1680 44.96100777388319
1681 44.9618227423392
1682 44.9626437651155
1683 44.963447722204194
1684 44.96423750279876
1685 44.96501580224923
1686 44.965783826148055
1687 44.96654150779417
1688 44.96728673990939
1689 44.968016796970254
1690 44.96871174703883
1691 44.96939906805409
1692 44.97011824891989
1693 44.97086951509104
1694 44.97161175302862
1695 44.97230324042925
1696 44.9729715783846
1697 44.97362294292324
1698 44.97422520728941
1699 44.97475890503914
1700 44.975216989644466
1701 44.975627973835856
1702 44.97602506130306
1703 44.97641346933963
1704 44.97679734031139
1705 44.97718050685573
1706 44.97756649706334
1707 44.97795741290367
1708 44.97835391863205
1709 44.97875665794472
1710 44.97916667537125
1711 44.97958626576541
1712 44.98001786700393
1713 44.980462867283215
1714 44.98092188179194
1715 44.98139301185236
1716 44.98187343374258
1717 44.9823471539539
1718 44.982817183239916
1719 44.983302822646785
1720 44.98380263499939
1721 44.98431265091502
1722 44.98482878231041
1723 44.98534797856604
1724 44.98586679866088
1725 44.986380680761485
1726 44.98689548427315
1727 44.987416533354455
1728 44.98793826371321
1729 44.98845593684447
1730 44.98896497330314
1731 44.9894615130435
1732 44.989942559244945
1733 44.990404930390376
1734 44.99084581822325
1735 44.99126441344759
1736 44.99166106793271
1737 44.99203597743548
1738 44.99240845822801
1739 44.99279605747345
1740 44.99319932890137
1741 44.99361872618649
1742 44.994051545883806
1743 44.99447433275882
1744 44.99486216009878
1745 44.99523126036697
1746 44.99556264091684
1747 44.99580288551211
1748 44.995946191332656
1749 44.99597912976679
1750 44.9958953365362
1751 44.995706257646425
1752 44.99542547012878
1753 44.99507366469143
1754 44.99467527767055
1755 44.99422565244259
1756 44.993710985401044
1757 44.99311915854179
1758 44.992442105613385
1759 44.99167578829293
1760 44.9908291373223
1761 44.989922549863095
1762 44.988962695606666
1763 44.98793788134154
1764 44.986848761301594
1765 44.985697449995314
1766 44.9844810061353
1767 44.98320405397976
1768 44.98188006769773
1769 44.980522069591075
1770 44.979142449091334
1771 44.97775200066687
1772 44.97636040301038
1773 44.974977655603425
1774 44.973614840719016
1775 44.97229421520179
1776 44.97102788887783
1777 44.96981188391604
1778 44.968655393011424
1779 44.96755742656835
1780 44.96649059416855
1781 44.965459223483364
1782 44.96448571648926
1783 44.96357762148336
1784 44.96274057019009
1785 44.961988870162386
1786 44.96136148244721
1787 44.96089300213224
1788 44.96062382649344
1789 44.96060715974856
1790 44.96087936386491
1791 44.96141778088768
1792 44.96217439857525
1793 44.963128090980355
1794 44.96426401138203
1795 44.96556167487811
1796 44.966995876984015
1797 44.96854218684979
1798 44.97018369440357
1799 44.97188988507358
1800 44.97361476607765
1801 44.97532930457661
1802 44.97701831260742
1803 44.97867353223287
1804 44.98029544348242
1805 44.98188943546349
1806 44.98345426763072
1807 44.98498058733191
1808 44.986452870584394
1809 44.98786377860174
1810 44.98919799795909
1811 44.99041876866971
1812 44.991492916943734
1813 44.99239992726588
1814 44.99315429218194
1815 44.993790978805755
1816 44.994344441901966
1817 44.99484998092704
1818 44.99534982075639
1819 44.99585843581284
1820 44.9963775306213
1821 44.996925533992616
1822 44.99751727582593
1823 44.99816415671923
1824 44.99887391420464
1825 44.99965054394471
1826 45.00049493443314
1827 45.00140554625786
1828 45.00237398554239
1829 45.003387722787856
1830 45.004436668051014
1831 45.00551413576319
1832 45.0066150676093
1833 45.007730318850385
1834 45.00884996921893
1835 45.009964050815455
1836 45.01106273609442
1837 45.01214617978733
1838 45.01318378819467
1839 45.01412492689569
1840 45.01494646275724
1841 45.015636061998215
1842 45.01618719583165
1843 45.01659694975314
1844 45.016869166916585
1845 45.01701328814463
1846 45.017039962897584
1847 45.01699001176867
1848 45.01692295600303
1849 45.01687447591434
1850 45.016856781570816
1851 45.01688929410496
1852 45.01700994865382
1853 45.01720657332968
1854 45.01743412439778
1855 45.01766734423414
1856 45.01788501122365
1857 45.018067139070915
1858 45.01819549434579
1859 45.018256425756654
1860 45.018240537846054
1861 45.01814192616755
1862 45.017957898339766
1863 45.01768894191396
1864 45.017339658047234
1865 45.01691855420165
1866 45.01643643077474
1867 45.015908163810835
1868 45.01534822402644
1869 45.014767598541354
1870 45.01417571186935
1871 45.01357890927178
1872 45.01298540039272
1873 45.01240216303328
1874 45.011833670462345
1875 45.01128150338609
1876 45.01074742022438
1877 45.01023665217281
1878 45.00975274369117
1879 45.00929717700224
1880 45.00886903048323
1881 45.008465690025574
1882 45.00808294680502
1883 45.00771524444201
1884 45.00735458844411
1885 45.00699092486973
1886 45.00661650050649
1887 45.0062235940953
1888 45.0058069832521
1889 45.0053641620377
1890 45.00489575372112
1891 45.004406621979314
1892 45.0039043511876
1893 45.003396991392776
1894 45.002893333573894
1895 45.002402387828525
1896 45.001952426484834
1897 45.00156591266083
1898 45.0012286435044
1899 45.00094316959037
1900 45.0007362380886
1901 45.00062941092804
1902 45.00060536156716
1903 45.00065791427541
1904 45.00080918302588
1905 45.00106097752467
1906 45.00140903496625
1907 45.001844283116505
1908 45.002352827112546
1909 45.00291892090079
1910 45.00352841986391
1911 45.00416929369275
1912 45.00483014945438
1913 45.005499846644256
1914 45.00616328032067
1915 45.00677339582246
1916 45.007267287771505
1917 45.00764546986047
1918 45.007946301761734
1919 45.00817954219628
1920 45.008352484277566
1921 45.00846423241675
1922 45.008488010444665
1923 45.008403035631396
1924 45.00817787031191
1925 45.007795887327184
1926 45.00723529146876
1927 45.00651303810206
1928 45.00569088567578
1929 45.004831449698514
1930 45.00399297067512
1931 45.00317967916956
1932 45.00238082858487
1933 45.00158283840484
1934 45.00076754745015
1935 44.999913277190366
1936 44.998999161629975
1937 44.99803097198428
1938 44.99705900861177
1939 44.99610527744482
1940 44.99518224164927
1941 44.99431208166153
1942 44.993536975539264
1943 44.992895376505686
1944 44.992428984745054
1945 44.99218018288339
1946 44.99217080748185
1947 44.99241093430968
1948 44.99289263637834
1949 44.99359526022381
1950 44.994470048213564
1951 44.99544300493365
1952 44.99645303566633
1953 44.997482029147335
1954 44.99849766218659
1955 44.99947244233729
1956 45.00037494395886
1957 45.001219397795396
1958 45.0021064542412
1959 45.00305943311914
1960 45.00395415441635
1961 45.00471376160467
1962 45.00533293830624
1963 45.00581845728153
1964 45.00617353886648
1965 45.00644382663645
1966 45.0066843226651
1967 45.00689148079742
1968 45.00708122085501
1969 45.00729312085991
1970 45.007510880387386
1971 45.007722698217755
1972 45.0079545891803
1973 45.00822842304992
1974 45.00856493171649
1975 45.00900612025783
1976 45.00957539412362
1977 45.01024638592647
1978 45.0109910716336
1979 45.01179301814762
1980 45.01263393278585
1981 45.01349264675014
1982 45.01434734897424
1983 45.015178118552925
1984 45.015968088248925
1985 45.016700843545415
1986 45.01735103744778
1987 45.017888930149034
1988 45.018288613785884
1989 45.01853218305639
1990 45.01861610420125
1991 45.01854581521705
1992 45.018330480628336
1993 45.01797653597088
1994 45.01749656405557
1995 45.016908432736635
1996 45.01623518841468
1997 45.015501047015974
1998 45.01472352992374
1999 45.01395071077519
2000 45.01324859877898


==> plotdata/satellite_constellation/sat_A5_r.tex <==
t r
0 6848.233953273979
1 6848.224673585111
2 6848.193965412004
3 6848.137821166771
4 6848.05268705065
5 6847.935526395055
6 6847.783873794677
7 6847.5958790961495
8 6847.370340470728
9 6847.106725987859
10 6846.805183301199
11 6846.4665372805175
12 6846.09227562513
13 6845.684522688492
14 6845.246001974229
15 6844.779987943627
16 6844.290247976487
17 6843.780975474641
18 6843.256715301564
19 6842.722282851925
20 6842.182678171488
21 6841.642996668688
22 6841.108337968222
23 6840.583714567482
24 6840.073961929346
25 6839.583651599335
26 6839.117008959724
27 6838.677837112748
28 6838.2694482515735
29 6837.894603797524
30 6837.555464431435
31 6837.253550854327
32 6836.989716095226
33 6836.764129902211
34 6836.57627582429
35 6836.424959479519
36 6836.308329847997
37 6836.2239132572995
38 6836.168657393956
39 6836.138986197147
40 6836.130864115186
41 6836.139868664489
42 6836.161270574277
43 6836.19011757104
44 6836.22132327922
45 6836.249760979304
46 6836.270352674306
47 6836.278160094777
48 6836.26847571598
49 6836.236905789237
50 6836.179449137424
51 6836.092568839063
52 6835.973255529543
53 6835.819081443255
54 6835.62824391568
55 6835.399597774734
56 6835.1326759936255
57 6834.827698324793
58 6834.485567643705
59 6834.107854025363
60 6833.696766981628
61 6833.255116261838
62 6832.786261851447
63 6832.294054509602
64 6831.782766189667
65 6831.257013669295
66 6830.721676695519
67 6830.181810120541
68 6829.6425531162295
69 6829.10903674556
70 6828.586291588352
71 6828.079156979144
72 6827.592193585808
73 6827.129600932397
74 6826.69514131268
75 6826.292071511553
76 6825.923083651125
77 6825.5902562008305
78 6825.295016042983
79 6825.038112349851
80 6824.819602693799
81 6824.638851764481
82 6824.494542661146
83 6824.384700536247
84 6824.306728208375
85 6824.257453024843
86 6824.233184203729
87 6824.229779544544
88 6824.2427202827885
89 6824.267192774619
90 6824.298175423632
91 6824.330529314214
92 6824.359091434883
93 6824.378767009271
94 6824.384621261474
95 6824.371969190805
96 6824.33645955842
97 6824.274153271178
98 6824.181594297046
99 6824.055871918835
100 6823.894673174058
101 6823.696324562699
102 6823.4598223215135
103 6823.184850650583
104 6822.871787634445
105 6822.521698735607
106 6822.136317910624
107 6821.718016779142
108 6821.269762240176
109 6820.795063387465
110 6820.297908638632
111 6819.782694141617
112 6819.254144720192
113 6818.7172287989215
114 6818.177068854481
115 6817.6388489045285
116 6817.107720764462
117 6816.588710748114
118 6816.086628500572
119 6815.6059796185955
120 6815.150883698752
121 6814.7249993022615
122 6814.331457194206
123 6813.9728031425975
124 6813.650951302033
125 6813.367149086506
126 6813.121954175591
127 6812.915226135332
128 6812.74612500469
129 6812.613127513428
130 6812.514059169539
131 6812.446125086223
132 6812.405962863257
133 6812.389709082235
134 6812.393066517482
135 6812.411382158311
136 6812.439731729578
137 6812.4730091417405
138 6812.506019626148
139 6812.53357332065
140 6812.5505798556205
141 6812.552910910261
142 6812.540530925284
143 6812.517489947357
144 6812.488510401116
145 6812.4565220319
146 6812.4212657443
147 6812.382266390757
148 6812.339856854333
149 6812.2933701790325
150 6812.2402848330075
151 6812.179046090628
152 6812.109352580388
153 6812.032210759689
154 6811.949016957003
155 6811.861278927849
156 6811.770586677114
157 6811.678584719076
158 6811.586941728121
159 6811.497320206428
160 6811.411345599093
161 6811.330577877576
162 6811.2564815185515
163 6811.1904006233
164 6811.133534565972
165 6811.086914750152
166 6811.051386096347
167 6811.027592834965
168 6811.015966428717
169 6811.016717783955
170 6811.029832707523
171 6811.055072339131
172 6811.091978199053
173 6811.139880304481
174 6811.197908679526
175 6811.265009982365
176 6811.339966665088
177 6811.42141902406
178 6811.507888804041
179 6811.597806640601
180 6811.689541336274
181 6811.781429228664
182 6811.871803593408
183 6811.959025490176
184 6812.041513231734
185 6812.117771659371
186 6812.186418603415
187 6812.2462099978175
188 6812.296062485969
189 6812.335073022981
190 6812.36253520056
191 6812.377952040089
192 6812.38106297025
193 6812.371851845281
194 6812.350441613809
195 6812.31720804382
196 6812.272758527393
197 6812.217908029997
198 6812.15364055664
199 6812.081118294733
200 6812.00165757481
201 6811.916697882205
202 6811.827778882855
203 6811.736512951661
204 6811.644555247377
205 6811.553573544717
206 6811.465218132063
207 6811.381091707874
208 6811.302720562529
209 6811.231526095159
210 6811.168799722812
211 6811.115679383094
212 6811.073128578056
213 6811.041919323044
214 6811.022617585958
215 6811.01557277832
216 6811.020912237691
217 6811.038538642854
218 6811.068131651553
219 6811.109153836704
220 6811.160860184398
221 6811.222312098795
222 6811.292394117479
223 6811.369834164783
224 6811.453226886599
225 6811.541059104371
226 6811.631737376198
227 6811.723616889914
228 6811.815031202867
229 6811.904322650121
230 6811.989872469841
231 6812.070129322067
232 6812.143638142815
233 6812.209066727089
234 6812.265229452287
235 6812.3111087435655
236 6812.345885479896
237 6812.3689611483105
238 6812.37988566329
239 6812.378472222954
240 6812.364800050362
241 6812.339061595702
242 6812.3018584836345
243 6812.254202626208
244 6812.19658452274
245 6812.1299471224975
246 6812.055487627914
247 6811.974552457985
248 6811.88860963305
249 6811.79921702539
250 6811.707995787516
251 6811.616599978459
252 6811.526687219409
253 6811.439888359067
254 6811.357778223606
255 6811.281847323041
256 6811.213472712211
257 6811.153894085736
258 6811.104191686006
259 6811.065353175013
260 6811.038271806662
261 6811.023226624354
262 6811.020427282792
263 6811.029924542447
264 6811.051545042715
265 6811.084895834916
266 6811.129371469797
267 6811.1841646525045
268 6811.248280564063
269 6811.320555093468
270 6811.399676533312
271 6811.484209190525
272 6811.572619366704
273 6811.663303276275
274 6811.754616171512
275 6811.844972782136
276 6811.932894508456
277 6812.016609616322
278 6812.094626878298
279 6812.165812903996
280 6812.228909246147
281 6812.28268801717
282 6812.326125703031
283 6812.358410070528
284 6812.378956246788
285 6812.387344914019
286 6812.383346890776
287 6812.367237423555
288 6812.339408102352
289 6812.300447343212
290 6812.251408533284
291 6812.193218841858
292 6812.12892884774
293 6812.059979610271
294 6811.985718556144
295 6811.907247446264
296 6811.827934828255
297 6811.749469985896
298 6811.672076191398
299 6811.595497142236
300 6811.520784479875
301 6811.4495507793035
302 6811.383637195704
303 6811.3237505943225
304 6811.271052212094
305 6811.226190922767
306 6811.189893834622
307 6811.162819380653
308 6811.145458779577
309 6811.138126175858
310 6811.140954466076
311 6811.153892715553
312 6811.17670507019
313 6811.208977287889
314 6811.250123024099
315 6811.299395349124
316 6811.355900379615
317 6811.41861264084
318 6811.4864216390215
319 6811.558183718028
320 6811.632596282672
321 6811.7082504809305
322 6811.783844214997
323 6811.858002664714
324 6811.9293633137795
325 6811.996637588544
326 6812.058628996176
327 6812.114228235548
328 6812.16244491967
329 6812.20243219547
330 6812.2334397131835
331 6812.254772310906
332 6812.266013582641
333 6812.26696016935
334 6812.257599734332
335 6812.238186581958
336 6812.209159759433
337 6812.170902418714
338 6812.124076463963
339 6812.069531883137
340 6812.008258516364
341 6811.94136906626
342 6811.870075798838
343 6811.795668996565
344 6811.719497953831
345 6811.642944508136
346 6811.567396935809
347 6811.494224900845
348 6811.424803100256
349 6811.360481666584
350 6811.302319358777
351 6811.251340423643
352 6811.208469459823
353 6811.174484325928
354 6811.150001303787
355 6811.135463968082
356 6811.131135657146
357 6811.137094692447
358 6811.153232971928
359 6811.179256993492
360 6811.214694030864
361 6811.258901054865
362 6811.311075376414
363 6811.370270012955
364 6811.435410720472
365 6811.5053156833155
366 6811.578716518887
367 6811.65428200141
368 6811.730664216734
369 6811.8065522151155
370 6811.880591015778
371 6811.9514439034965
372 6812.017836613776
373 6812.078550601433
374 6812.132461013662
375 6812.178545865147
376 6812.216019911877
377 6812.244127404475
378 6812.262348069481
379 6812.270375062846
380 6812.268036193378
381 6812.255527940048
382 6812.2335619523255
383 6812.20232599593
384 6812.162369507272
385 6812.114086928851
386 6812.05826839865
387 6811.995929905949
388 6811.92820207103
389 6811.856309618135
390 6811.781553985829
391 6811.705289886758
392 6811.62890000241
393 6811.553770080202
394 6811.481263665498
395 6811.412695687316
396 6811.349309452281
397 6811.292255012095
398 6811.242567354545
399 6811.201147852576
400 6811.16874701446
401 6811.145952474751
402 6811.133178220455
403 6811.1306553562
404 6811.138429378524
405 6811.156357994023
406 6811.184115247071
407 6811.221197242266
408 6811.2669311565805
409 6811.320486412499
410 6811.380890901985
411 6811.44704855132
412 6811.517759208788
413 6811.591740135212
414 6811.667649117065
415 6811.744109368336
416 6811.819733876772
417 6811.893151380105
418 6811.963030688536
419 6812.028104981312
420 6812.08719434232
421 6812.139290736823
422 6812.1836561146365
423 6812.219479415014
424 6812.246045604482
425 6812.263218054484
426 6812.270277931895
427 6812.267128673476
428 6812.254259834558
429 6812.231455934416
430 6812.198986678571
431 6812.157439599001
432 6812.107568318727
433 6812.0502771404
434 6811.98660633694
435 6811.917714363495
436 6811.844848728088
437 6811.769328739317
438 6811.692524146391
439 6811.615828329224
440 6811.54063075884
441 6811.468294241969
442 6811.40013096193
443 6811.337377215814
444 6811.281171606088
445 6811.232533330228
446 6811.192344208706
447 6811.161333259533
448 6811.140062977937
449 6811.128919028278
450 6811.128103502055
451 6811.137630403337
452 6811.157327388238
453 6811.186839130097
454 6811.225628226988
455 6811.272988801727
456 6811.328060892858
457 6811.38984482564
458 6811.457219683728
459 6811.528963365453
460 6811.603773909986
461 6811.680294321756
462 6811.757136530652
463 6811.832906789288
464 6811.906231283924
465 6811.975781155946
466 6812.040294991516
467 6812.098623713815
468 6812.149753737886
469 6812.1927264615615
470 6812.226787408521
471 6812.251276361836
472 6812.265737034164
473 6812.269907770255
474 6812.2639004973635
475 6812.248153313052
476 6812.222830485609
477 6812.188698369331
478 6812.1458147493395
479 6812.0948189223245
480 6812.036945910652
481 6811.973660566126
482 6811.905524654568
483 6811.833632700769
484 6811.7592886746725
485 6811.683840545438
486 6811.608656037637
487 6811.535099266821
488 6811.4645052497
489 6811.398154097991
490 6811.337248429751
491 6811.2828932893
492 6811.2360743749705
493 6811.197641285391
494 6811.1682910256495
495 6811.148555188601
496 6811.138791667979
497 6811.139177063539
498 6811.149704058629
499 6811.1701811807125
500 6811.200236528416
501 6811.239324066855
502 6811.286734327891
503 6811.341607063942
504 6811.4029464509995
505 6811.469639110986
506 6811.540475511144
507 6811.614170446696
508 6811.689387093776
509 6811.7648439400355
510 6811.839345841781
511 6811.911343140992
512 6811.979472855701
513 6812.042500457345
514 6812.09939182646
515 6812.149892577026
516 6812.193806169196
517 6812.229196666702
518 6812.255786587308
519 6812.274073098614
520 6812.28234784041
521 6812.280053705294
522 6812.267212684176
523 6812.244238189921
524 6812.211889026204
525 6812.170890392053
526 6812.122132757869
527 6812.066575846229
528 6812.005268792796
529 6811.939047909275
530 6811.868551206526
531 6811.79496864406
532 6811.719635129105
533 6811.643916705769
534 6811.569185727184
535 6811.4967974712945
536 6811.428065009663
537 6811.364235550741
538 6811.306468474339
539 6811.255812403089
540 6811.213185794343
541 6811.179361222298
542 6811.154950415707
543 6811.140395819463
544 6811.13596176311
545 6811.141729856093
546 6811.157593300459
547 6811.183263472832
548 6811.218274888591
549 6811.261991807432
550 6811.313622543833
551 6811.372230034119
552 6811.436749125642
553 6811.506008829564
554 6811.578755006522
555 6811.6536675357165
556 6811.7294898268765
557 6811.805214559366
558 6811.879466295597
559 6811.950608562607
560 6812.017529651451
561 6812.078956795766
562 6812.133532710092
563 6812.180226642481
564 6812.218221397715
565 6812.2468166958015
566 6812.265552145263
567 6812.274084746164
568 6812.272232718254
569 6812.259984664336
570 6812.237552705043
571 6812.205898866526
572 6812.166747954004
573 6812.120075765965
574 6812.067546206733
575 6812.0092697181835
576 6811.9470247774625
577 6811.8806481161455
578 6811.810967533848
579 6811.73924541805
580 6811.6667821458705
581 6811.595166380292
582 6811.5266275061485
583 6811.462690779342
584 6811.403335414502
585 6811.349335256215
586 6811.301666098483
587 6811.26119370766
588 6811.22865796793
589 6811.204648162617
590 6811.189595605337
591 6811.183770919571
592 6811.187279468144
593 6811.200057606189
594 6811.22187302452
595 6811.252330896096
596 6811.290876624113
597 6811.336810786525
598 6811.389300288296
599 6811.44739630813
600 6811.5100419064565
601 6811.576099153095
602 6811.644373347028
603 6811.713627399251
604 6811.782819898503
605 6811.851112457716
606 6811.916770071086
607 6811.978532377965
608 6812.035417616083
609 6812.086317945573
610 6812.130509133953
611 6812.167206132332
612 6812.195684194923
613 6812.215309451258
614 6812.225594300229
615 6812.226327793741
616 6812.2174946729665
617 6812.199422522909
618 6812.172902548229
619 6812.13839038496
620 6812.096338661218
621 6812.048178230231
622 6811.994956190695
623 6811.937869156682
624 6811.878315424765
625 6811.817280764382
626 6811.754931635128
627 6811.692487702003
628 6811.631645982464
629 6811.573242218431
630 6811.518904351477
631 6811.469444977945
632 6811.426627317185
633 6811.3908304827255
634 6811.363704594339
635 6811.344777686485
636 6811.335212447241
637 6811.332738690446
638 6811.336989041921
639 6811.348040634709
640 6811.36581906998
641 6811.39041298461
642 6811.421440153488
643 6811.458349231281
644 6811.501023099417
645 6811.551317300269
646 6811.610415648434
647 6811.681207390853
648 6811.766913572081
649 6811.870486695147
650 6811.994544625142
651 6812.141334162697
652 6812.312695340149
653 6812.510040123029
654 6812.7343301323435
655 6812.986043831338
656 6813.265153505299
657 6813.571117058118
658 6813.9029084089625
659 6814.259044338306
660 6814.637601730628
661 6815.036250703468
662 6815.452324833409
663 6815.882845961747
664 6816.324543604402
665 6816.7739603923965
666 6817.227509236317
667 6817.681536582233
668 6818.132400159532
669 6818.576516541242
670 6819.0104250277045
671 6819.430851822397
672 6819.834775096731
673 6820.219475460538
674 6820.582576739795
675 6820.922092500781
676 6821.23646342274
677 6821.524586971945
678 6821.785837790472
679 6822.020075245677
680 6822.227646234278
681 6822.40937967412
682 6822.56657010919
683 6822.700960672658
684 6822.814698288287
685 6822.910299508215
686 6822.990610292305
687 6823.05875181079
688 6823.118088621707
689 6823.172153814915
690 6823.224634179404
691 6823.279499964843
692 6823.340694285138
693 6823.411853571094
694 6823.506226749348
695 6823.638772900428
696 6823.814716679909
697 6824.0369355078965
698 6824.306580278157
699 6824.623820576727
700 6824.987724215357
701 6825.395067795627
702 6825.841485429554
703 6826.314985741027
704 6826.801012050165
705 6827.291879286152
706 6827.7818619597865
707 6828.265928222016
708 6828.739761733666
709 6829.199445657939
710 6829.6420818734405
711 6830.064947263985
712 6830.464939953026
713 6830.840299159586
714 6831.190188266014
715 6831.52485921447
716 6831.855014249017
717 6832.17976628961
718 6832.497782161249
719 6832.808032138551
720 6833.109614267952
721 6833.401817976393
722 6833.684193801111
723 6833.9565527235445
724 6834.2188900007295
725 6834.471343657084
726 6834.714067842195
727 6834.9471761601835
728 6835.170852058641
729 6835.3854067803995
730 6835.591368312994
731 6835.789467257055
732 6835.980579500077
733 6836.1657322971105
734 6836.346120586278
735 6836.5230591435875
736 6836.697905188687
737 6836.872149815626
738 6837.046917796827
739 6837.22315866888
740 6837.401967192157
741 6837.584839381197
742 6837.773186249379
743 6837.968143166051
744 6838.170809170306
745 6838.381603680846
746 6838.599432975115
747 6838.8226004980215
748 6839.052769769384
749 6839.29121977264
750 6839.536652306038
751 6839.787378514852
752 6840.0441904656755
753 6840.309139530591
754 6840.582045442942
755 6840.862588449179
756 6841.150309872603
757 6841.444603324652
758 6841.744764449365
759 6842.050004221385
760 6842.359423857027
761 6842.672048939126
762 6842.986849660983
763 6843.302755214299
764 6843.618677356655
765 6843.933533154835
766 6844.246248049116
767 6844.5557933177215
768 6844.861205688953
769 6845.1615882653
770 6845.456134501216
771 6845.744137478101
772 6846.025010199825
773 6846.298274923359
774 6846.563612978659
775 6846.820866663837
776 6847.070001569363
777 6847.311133002306
778 6847.544510263567
779 6847.770520017792
780 6847.989682076463
781 6848.202648007546
782 6848.410182966322
783 6848.613140723768
784 6848.812446954854
785 6849.00910199955
786 6849.204163443907
787 6849.398707679706
788 6849.593820350305
789 6849.790566632413
790 6849.989992392955
791 6850.193106424889
792 6850.400841756389
793 6850.614049102336
794 6850.8334817305185
795 6851.059782065864
796 6851.293470263688
797 6851.534934984752
798 6851.784405641221
799 6852.041988671436
800 6852.307667834392
801 6852.581246667055
802 6852.862379488198
803 6853.1506248527285
804 6853.445418888187
805 6853.746063925256
806 6854.05175962295
807 6854.361592744398
808 6854.674581272537
809 6854.98972683986
810 6855.305994032309
811 6855.622286450772
812 6855.937527260175
813 6856.250679700838
814 6856.560724851103
815 6856.866699581191
816 6857.167713611175
817 6857.462965351824
818 6857.751756065639
819 6858.033482861333
820 6858.307687391393
821 6858.574064922926
822 6858.832431010412
823 6859.0827437142925
824 6859.325104312253
825 6859.559755396583
826 6859.78707660914
827 6860.007577871835
828 6860.2218901902115
829 6860.4307544819685
830 6860.635008404249
831 6860.835279096567
832 6861.032557188874
833 6861.228178563773
834 6861.423215982057
835 6861.618749078707
836 6861.815800752495
837 6862.015421678596
838 6862.218629730678
839 6862.42631514252
840 6862.639372089235
841 6862.858536085189
842 6863.084387532426
843 6863.317515690946
844 6863.5583601788985
845 6863.8071624278955
846 6864.064046133085
847 6864.3290150746625
848 6864.601937102938
849 6864.882539005585
850 6865.17039204474
851 6865.464920430423
852 6865.765449284827
853 6866.071191778682
854 6866.3812637778
855 6866.694719881299
856 6867.01058014535
857 6867.3278215741675
858 6867.645345918431
859 6867.9620718183805
860 6868.2769282712015
861 6868.588882822775
862 6868.896982617124
863 6869.20029171518
864 6869.497982858734
865 6869.789353818058
866 6870.073790411274
867 6870.350801387098
868 6870.620027047007
869 6870.88124553009
870 6871.134376682181
871 6871.379483404716
872 6871.616770512489
873 6871.846581065231
874 6872.069390253952
875 6872.28579696873
876 6872.496513218294
877 6872.702351548215
878 6872.9042106374145
879 6873.103059433002
880 6873.299920037378
881 6873.495849671266
882 6873.691922011479
883 6873.889208249645
884 6874.088758202344
885 6874.291576096728
886 6874.498606860311
887 6874.710732749227
888 6874.928747987359
889 6875.153336980699
890 6875.385068414825
891 6875.624385291231
892 6875.871596934687
893 6876.126873693907
894 6876.390243989157
895 6876.661578345932
896 6876.940586162527
897 6877.226885063516
898 6877.519969061283
899 6877.819197302985
900 6878.123842093717
901 6878.433064702475
902 6878.745946318745
903 6879.061504260725
904 6879.378709298941
905 6879.6965037942755
906 6880.01382030568
907 6880.329600396105
908 6880.642813260383
909 6880.95247380183
910 6881.2576599338645
911 6881.557528769013
912 6881.851331393422
913 6882.138425977072
914 6882.418289004901
915 6882.690524404998
916 6882.954870472526
917 6883.211204369541
918 6883.459544134126
919 6883.699385243968
920 6883.927000297226
921 6884.135200032459
922 6884.315981728067
923 6884.464636774256
924 6884.582183034984
925 6884.671183351031
926 6884.734635026438
927 6884.775987560422
928 6884.799034153186
929 6884.80787740919
930 6884.8068737002395
931 6884.800567777216
932 6884.793556879411
933 6884.7898763763105
934 6884.791170170685
935 6884.797676833755
936 6884.809354842073
937 6884.825910760682
938 6884.846865487985
939 6884.871832319261
940 6884.900533320537
941 6884.932323908267
942 6884.966168542354
943 6885.001341897483
944 6885.037233239852
945 6885.073649281476
946 6885.110293425735
947 6885.14635570788
948 6885.180892582577
949 6885.213409925174
950 6885.2435114692935
951 6885.270629530885
952 6885.2945380551255
953 6885.314851967335
954 6885.331214473648
955 6885.343215461207
956 6885.350296027838
957 6885.352351870245
958 6885.349720076175
959 6885.342523683598
960 6885.330888971398
961 6885.314932683013
962 6885.294756926389
963 6885.270921341816
964 6885.243903642642
965 6885.214091808162
966 6885.181829585731
967 6885.147888800536
968 6885.112925175823
969 6885.0775524659875
970 6885.04239173721
971 6885.008060193655
972 6884.975091867049
973 6884.943996514099
974 6884.9154172047
975 6884.889913451202
976 6884.867982403599
977 6884.849921117542
978 6884.836035233522
979 6884.826620229653
980 6884.821978654639
981 6884.822087360799
982 6884.826875082379
983 6884.836204982739
984 6884.849844349828
985 6884.867476605589
986 6884.888747769282
987 6884.9132744586495
988 6884.940602773546
989 6884.970214387523
990 6885.001568139081
991 6885.034115675691
992 6885.067381470827
993 6885.100998440965
994 6885.134419033888
995 6885.167056342471
996 6885.198337315407
997 6885.227423440286
998 6885.253492618482
999 6885.276583632458
1000 6885.296395088364
1001 6885.312579104345
1002 6885.324851301139
1003 6885.3329166633475
1004 6885.336524420137
1005 6885.335763514564
1006 6885.330684042397
1007 6885.321374355237
1008 6885.307997146465
1009 6885.290732058467
1010 6885.269752932739
1011 6885.245407501129
1012 6885.218124780226
1013 6885.188424951183
1014 6885.156887850427
1015 6885.124154733699
1016 6885.0907618654
1017 6885.057151645866
1018 6885.023898418601
1019 6884.991591610677
1020 6884.960827300476
1021 6884.93226078102
1022 6884.906361997275
1023 6884.883604982228
1024 6884.864419075818
1025 6884.849147068582
1026 6884.838080360908
1027 6884.831412893199
1028 6884.829247734572
1029 6884.831596582914
1030 6884.83841712897
1031 6884.849586270898
1032 6884.864891509677
1033 6884.884050598892
1034 6884.906703987449
1035 6884.932472074688
1036 6884.960744626581
1037 6884.99060624524
1038 6885.021472485925
1039 6885.052774316213
1040 6885.084168076648
1041 6885.115433593513
1042 6885.145772499749
1043 6885.174535662831
1044 6885.201194784752
1045 6885.225382207827
1046 6885.246775034779
1047 6885.264944659612
1048 6885.279590335839
1049 6885.290505976398
1050 6885.297512495945
1051 6885.300488873796
1052 6885.29949153803
1053 6885.294671284211
1054 6885.285972465293
1055 6885.273579612231
1056 6885.257753687467
1057 6885.238774528816
1058 6885.2169843863385
1059 6885.192792743516
1060 6885.166652693543
1061 6885.139010034901
1062 6885.110343389614
1063 6885.081188153459
1064 6885.052157922864
1065 6885.023786044904
1066 6884.996513906717
1067 6884.970710646039
1068 6884.946828123708
1069 6884.925268795657
1070 6884.906376056419
1071 6884.890481784033
1072 6884.877924228493
1073 6884.869057875677
1074 6884.864028813559
1075 6884.862772970299
1076 6884.86521588048
1077 6884.871328093605
1078 6884.8809933305765
1079 6884.894017409539
1080 6884.9101371384295
1081 6884.928988961659
1082 6884.950227891442
1083 6884.973432923921
1084 6884.998144941384
1085 6885.023924002095
1086 6885.050354973868
1087 6885.076997102374
1088 6885.103412746673
1089 6885.129176926289
1090 6885.153881062352
1091 6885.177151364709
1092 6885.198615416047
1093 6885.217865002587
1094 6885.234577521374
1095 6885.24849954502
1096 6885.259423095824
1097 6885.26716890663
1098 6885.271607644042
1099 6885.2726834415525
1100 6885.270435258422
1101 6885.264995656278
1102 6885.256478882865
1103 6885.245034284333
1104 6885.230862729351
1105 6885.214212985451
1106 6885.195357572166
1107 6885.174586745256
1108 6885.152311534859
1109 6885.128917461271
1110 6885.104758465021
1111 6885.080246381079
1112 6885.055815653326
1113 6885.0319083872255
1114 6885.008955092671
1115 6884.987364912342
1116 6884.967520056155
1117 6884.9497666886155
1118 6884.934410856331
1119 6884.921719419678
1120 6884.911910054179
1121 6884.905153561051
1122 6884.901575454798
1123 6884.901229784234
1124 6884.904126845428
1125 6884.91021173602
1126 6884.919375445012
1127 6884.931447399817
1128 6884.946217740014
1129 6884.96341649189
1130 6884.982736113427
1131 6885.003851145055
1132 6885.026397340588
1133 6885.049964517728
1134 6885.074135865575
1135 6885.098495693391
1136 6885.1226260076655
1137 6885.146121485813
1138 6885.16861746344
1139 6885.189729217019
1140 6885.209086030554
1141 6885.226348231184
1142 6885.241100177512
1143 6885.252830577528
1144 6885.261417037154
1145 6885.2661881394315
1146 6885.267120530151
1147 6885.264784837012
1148 6885.259311016175
1149 6885.250777235561
1150 6885.239339062833
1151 6885.225212699069
1152 6885.208648568751
1153 6885.189927914679
1154 6885.169378980783
1155 6885.147375024335
1156 6885.124317286334
1157 6885.100580701635
1158 6885.076567471762
1159 6885.052695821039
1160 6885.029386454088
1161 6885.007050156731
1162 6884.986079310643
1163 6884.966844523475
1164 6884.94968090272
1165 6884.934883568325
1166 6884.922706945932
1167 6884.913360267286
1168 6884.90701278064
1169 6884.903782321476
1170 6884.9037188843095
1171 6884.9068353076755
1172 6884.913064762712
1173 6884.922314179116
1174 6884.9344053997875
1175 6884.949133072559
1176 6884.966230708797
1177 6884.985408553303
1178 6885.006354942252
1179 6885.028718973995
1180 6885.052092689565
1181 6885.076076796547
1182 6885.100292423457
1183 6885.124094859707
1184 6885.146351363619
1185 6885.166555113483
1186 6885.184207320408
1187 6885.199033666162
1188 6885.211144625886
1189 6885.220606654173
1190 6885.227227163193
1191 6885.230884461997
1192 6885.231564318132
1193 6885.2293197652625
1194 6885.22408930685
1195 6885.2156462990715
1196 6885.20420503467
1197 6885.1903535380925
1198 6885.174386625049
1199 6885.156570438472
1200 6885.1372359744655
1201 6885.1167862663
1202 6885.095572750494
1203 6885.07375216054
1204 6885.051560826285
1205 6885.029400338749
1206 6885.007698118021
1207 6884.986866311963
1208 6884.9672977426035
1209 6884.949358205629
1210 6884.933377514701
1211 6884.919642117413
1212 6884.9083939579605
1213 6884.899850278267
1214 6884.89422652947
1215 6884.891569898657
1216 6884.891882775698
1217 6884.895148693598
1218 6884.9012034665875
1219 6884.909982228459
1220 6884.9213621657245
1221 6884.935135382475
1222 6884.951031033758
1223 6884.968655011001
1224 6884.987644275027
1225 6885.007682035877
1226 6885.028593105629
1227 6885.050471277923
1228 6885.073039676435
1229 6885.095885137795
1230 6885.118570704668
1231 6885.14073872972
1232 6885.162011959227
1233 6885.182016621846
1234 6885.200376425956
1235 6885.216688097407
1236 6885.230637229616
1237 6885.242002871674
1238 6885.250595628795
1239 6885.256255115466
1240 6885.258882250992
1241 6885.258458690138
1242 6885.255037519049
1243 6885.248622634709
1244 6885.2393060472305
1245 6885.227275341947
1246 6885.212792270941
1247 6885.196054769289
1248 6885.177333197077
1249 6885.156959789968
1250 6885.135322554796
1251 6885.112853544191
1252 6885.089912570724
1253 6885.066889559641
1254 6885.044199223654
1255 6885.022247792214
1256 6885.001427084884
1257 6884.9821083746865
1258 6884.96463142893
1259 6884.949294566171
1260 6884.936357695446
1261 6884.926043024066
1262 6884.918546862455
1263 6884.914031055945
1264 6884.912532554899
1265 6884.91406784242
1266 6884.918608337198
1267 6884.926066917091
1268 6884.936313122169
1269 6884.949176018687
1270 6884.964463181277
1271 6884.981826203005
1272 6885.000967277516
1273 6885.021590532221
1274 6885.043396846548
1275 6885.066017694334
1276 6885.089056017135
1277 6885.112106948348
1278 6885.134450533426
1279 6885.154632452214
1280 6885.1721203502675
1281 6885.186698374685
1282 6885.198301320671
1283 6885.206810933733
1284 6885.211956022387
1285 6885.213722667402
1286 6885.212262278776
1287 6885.207596240571
1288 6885.199783956752
1289 6885.189080282013
1290 6885.175843741066
1291 6885.160264872849
1292 6885.1426187206325
1293 6885.1232953380095
1294 6885.102846930336
1295 6885.0819397527675
1296 6885.060605748297
1297 6885.039167660455
1298 6885.018024119262
1299 6884.997548104832
1300 6884.978051150266
1301 6884.959895175269
1302 6884.943378630872
1303 6884.928657068553
1304 6884.915973272708
1305 6884.905557565683
1306 6884.897649498834
1307 6884.892487855147
1308 6884.890066621815
1309 6884.8904200015195
1310 6884.893611625738
1311 6884.899655656952
1312 6884.908917833965
1313 6884.921355678449
1314 6884.936750849111
1315 6884.9548330846765
1316 6884.975285015143
1317 6884.99774743883
1318 6885.021826002572
1319 6885.047097920783
1320 6885.073119154716
1321 6885.099431928069
1322 6885.125574360705
1323 6885.151088225866
1324 6885.175525517798
1325 6885.198457472393
1326 6885.2194813491
1327 6885.238227954432
1328 6885.254368232721
1329 6885.26761875496
1330 6885.277746872333
1331 6885.284574635518
1332 6885.287981950919
1333 6885.287835860907
1334 6885.28398433404
1335 6885.27667031241
1336 6885.266000130046
1337 6885.252001126809
1338 6885.235099067463
1339 6885.215643786812
1340 6885.193976154175
1341 6885.170476219811
1342 6885.145557275353
1343 6885.119656858858
1344 6885.093229645382
1345 6885.0667394719
1346 6885.040651574676
1347 6885.015423609473
1348 6884.991499045778
1349 6884.969298166039
1350 6884.949210864716
1351 6884.931589998644
1352 6884.91674502374
1353 6884.904936605637
1354 6884.896372353305
1355 6884.891202528885
1356 6884.889518211735
1357 6884.891348802603
1358 6884.896660707829
1359 6884.905357629666
1360 6884.9172909418185
1361 6884.932250568062
1362 6884.949970926518
1363 6884.970144883585
1364 6884.99241952338
1365 6885.016403501998
1366 6885.041675098506
1367 6885.067790723578
1368 6885.0942921383685
1369 6885.120713787693
1370 6885.146591603567
1371 6885.171471743065
1372 6885.194917226924
1373 6885.216516371381
1374 6885.235889391619
1375 6885.252696644383
1376 6885.266642977989
1377 6885.277483563655
1378 6885.28502837437
1379 6885.28914467364
1380 6885.289759568501
1381 6885.286862262851
1382 6885.280483482229
1383 6885.270691009476
1384 6885.257706159629
1385 6885.241771229382
1386 6885.223166103902
1387 6885.202217440882
1388 6885.1792928596
1389 6885.154794691948
1390 6885.129084372109
1391 6885.102434340459
1392 6885.07549957757
1393 6885.048726176412
1394 6885.022349675129
1395 6884.99707572734
1396 6884.973371628639
1397 6884.951448429404
1398 6884.931638364076
1399 6884.914308111581
1400 6884.899722871579
1401 6884.888063915108
1402 6884.879472590204
1403 6884.874078963076
1404 6884.871996242895
1405 6884.873213899168
1406 6884.877817584913
1407 6884.885575282114
1408 6884.896333379904
1409 6884.909825156143
1410 6884.925801783263
1411 6884.9439797091745
1412 6884.964112107578
1413 6884.985826233431
1414 6885.0086909719075
1415 6885.032268338237
1416 6885.055030615799
1417 6885.073518632794
1418 6885.086510427632
1419 6885.093557523508
1420 6885.094181919701
1421 6885.093036044934
1422 6885.0905432200125
1423 6885.085684291393
1424 6885.079617206916
1425 6885.06857553247
1426 6885.051403800459
1427 6885.032860339394
1428 6885.014111066507
1429 6884.994387932906
1430 6884.975253757991
1431 6884.956031348698
1432 6884.937996261561
1433 6884.920603130057
1434 6884.905001163398
1435 6884.890499373992
1436 6884.878127559049
1437 6884.867071471931
1438 6884.859332327414
1439 6884.854380150568
1440 6884.851075232882
1441 6884.850462851784
1442 6884.85129831228
1443 6884.854305803083
1444 6884.858277376475
1445 6884.865081479245
1446 6884.873911283366
1447 6884.885465669149
1448 6884.898552853128
1449 6884.914035727992
1450 6884.931170631009
1451 6884.950693637492
1452 6884.972310481037
1453 6884.99545194117
1454 6885.019592853516
1455 6885.0443148355
1456 6885.069379203955
1457 6885.094720017784
1458 6885.119971191711
1459 6885.144689124332
1460 6885.168442559984
1461 6885.190815122453
1462 6885.211413256322
1463 6885.229873948706
1464 6885.245874228443
1465 6885.2587710050475
1466 6885.267556221292
1467 6885.272561240107
1468 6885.273076203362
1469 6885.269768209982
1470 6885.262321456327
1471 6885.251618054443
1472 6885.238070665623
1473 6885.221916188918
1474 6885.203439507836
1475 6885.18267575292
1476 6885.159344839113
1477 6885.134250829961
1478 6885.107299957357
1479 6885.079441586659
1480 6885.050594208548
1481 6885.0217981968
1482 6884.9929695896335
1483 6884.965183669468
1484 6884.938329803319
1485 6884.913415968491
1486 6884.890142672753
1487 6884.869584088927
1488 6884.851304390367
1489 6884.836731821023
1490 6884.826572411724
1491 6884.821031445542
1492 6884.820204269665
1493 6884.824104342865
1494 6884.832661761802
1495 6884.845725109088
1496 6884.863070253736
1497 6884.88434238135
1498 6884.9090575685395
1499 6884.936892754174
1500 6884.967399930226
1501 6885.000042928238
1502 6885.034247083331
1503 6885.0694089806275
1504 6885.10491071947
1505 6885.140044305728
1506 6885.1738828301795
1507 6885.20570706125
1508 6885.234568674057
1509 6885.2581910572735
1510 6885.276665883139
1511 6885.290505585147
1512 6885.298824138066
1513 6885.297855131329
1514 6885.283631598979
1515 6885.2521201738255
1516 6885.199423436583
1517 6885.121974057285
1518 6885.016656098951
1519 6884.880892055333
1520 6884.712623368511
1521 6884.510337088626
1522 6884.2731305195175
1523 6884.000703684413
1524 6883.6933477733055
1525 6883.351962136436
1526 6882.9780366963605
1527 6882.573621051719
1528 6882.141325731555
1529 6881.684251636053
1530 6881.205919204659
1531 6880.710229931347
1532 6880.201384360234
1533 6879.683812609717
1534 6879.162091205542
1535 6878.640881383126
1536 6878.124823342056
1537 6877.618458481716
1538 6877.126179762161
1539 6876.652138555168
1540 6876.200158848976
1541 6875.773707384683
1542 6875.375808011181
1543 6875.008759801336
1544 6874.674400963048
1545 6874.373933146293
1546 6874.108219829458
1547 6873.877736967066
1548 6873.68198082772
1549 6873.519770318456
1550 6873.389139988166
1551 6873.287942631379
1552 6873.213218090185
1553 6873.1613456574705
1554 6873.128699446926
1555 6873.111856807469
1556 6873.1072086352315
1557 6873.110350395008
1558 6873.100191127715
1559 6873.055837162557
1560 6872.973487881814
1561 6872.85001862532
1562 6872.683181559672
1563 6872.471621191568
1564 6872.214680337305
1565 6871.912384163563
1566 6871.565331972719
1567 6871.174941253723
1568 6870.745829709985
1569 6870.282605853083
1570 6869.788928753616
1571 6869.276113362625
1572 6868.760263928932
1573 6868.252254872778
1574 6867.759095116722
1575 6867.28522650728
1576 6866.832284426105
1577 6866.403698798499
1578 6866.003364150066
1579 6865.618968269972
1580 6865.23814501728
1581 6864.863221749439
1582 6864.496429873138
1583 6864.139847516198
1584 6863.795430723418
1585 6863.465062556679
1586 6863.14954937044
1587 6862.849292858767
1588 6862.5651854564085
1589 6862.297517138661
1590 6862.046213046743
1591 6861.811124576498
1592 6861.59185123878
1593 6861.3877142094225
1594 6861.197765623633
1595 6861.020808332665
1596 6860.855419107629
1597 6860.699978571987
1598 6860.552696186434
1599 6860.411635979036
1600 6860.274753898016
1601 6860.139936323534
1602 6860.00503320622
1603 6859.867900736235
1604 6859.726442502301
1605 6859.578640439315
1606 6859.422598595159
1607 6859.256584432155
1608 6859.079042476082
1609 6858.888614880748
1610 6858.684173239216
1611 6858.464844501353
1612 6858.230028175548
1613 6857.979656043669
1614 6857.714011987012
1615 6857.4334175372915
1616 6857.138473955643
1617 6856.830051456318
1618 6856.510926243784
1619 6856.184154044976
1620 6855.8511946084
1621 6855.513540984554
1622 6855.17272118127
1623 6854.8300548874495
1624 6854.486708162656
1625 6854.144035773766
1626 6853.8039703565455
1627 6853.468773705003
1628 6853.140682698986
1629 6852.82173617593
1630 6852.513711483039
1631 6852.218174102045
1632 6851.936726042057
1633 6851.670720093698
1634 6851.420851012788
1635 6851.187494045219
1636 6850.969462573215
1637 6850.765145070421
1638 6850.574009856977
1639 6850.395493541293
1640 6850.228861863937
1641 6850.072996129974
1642 6849.926293945403
1643 6849.786914126082
1644 6849.653236615015
1645 6849.523705228704
1646 6849.396542842292
1647 6849.272564717767
1648 6849.1526787898365
1649 6849.0352059605075
1650 6848.91873627847
1651 6848.802230671577
1652 6848.685012408336
1653 6848.566988362917
1654 6848.448692935022
1655 6848.326065817761
1656 6848.201714557461
1657 6848.083215356216
1658 6847.972377205566
1659 6847.870794112816
1660 6847.779766708352
1661 6847.700383970998
1662 6847.633205880359
1663 6847.57823075805
1664 6847.535453883795
1665 6847.50448859512
1666 6847.484523376597
1667 6847.474704167183
1668 6847.474102867488
1669 6847.482201870537
1670 6847.496393816036
1671 6847.514217871934
1672 6847.53534772359
1673 6847.560371709208
1674 6847.589654455558
1675 6847.621704058859
1676 6847.655402272773
1677 6847.68978886954
1678 6847.72405183904
1679 6847.757711583711
1680 6847.790483067936
1681 6847.821895455758
1682 6847.851397626249
1683 6847.878586165863
1684 6847.90320950387
1685 6847.92516025826
1686 6847.944492060667
1687 6847.9614423829225
1688 6847.976654363025
1689 6847.990622446434
1690 6848.003416272491
1691 6848.015145776904
1692 6848.026087642187
1693 6848.036461916917
1694 6848.046323751965
1695 6848.05575801293
1696 6848.064841092509
1697 6848.073660622876
1698 6848.082094065964
1699 6848.089787295946
1700 6848.096419883985
1701 6848.1017830610435
1702 6848.105784691143
1703 6848.108425090321
1704 6848.109829483788
1705 6848.110223386743
1706 6848.109856096414
1707 6848.108984655386
1708 6848.107861942319
1709 6848.106712055581
1710 6848.105723102559
1711 6848.105045439383
1712 6848.1047984325105
1713 6848.105077646329
1714 6848.105933037049
1715 6848.107235618182
1716 6848.108716393265
1717 6848.11056648479
1718 6848.112032615288
1719 6848.112458477688
1720 6848.112011642505
1721 6848.110869891316
1722 6848.109184089603
1723 6848.1073633799915
1724 6848.1058834857395
1725 6848.104915118393
1726 6848.104243935769
1727 6848.103899131739
1728 6848.1041781044605
1729 6848.105260510544
1730 6848.107217967245
1731 6848.110039401467
1732 6848.113642603121
1733 6848.117938964012
1734 6848.122789797084
1735 6848.127882401595
1736 6848.132976991334
1737 6848.137988081609
1738 6848.142793791575
1739 6848.14732106658
1740 6848.151568570706
1741 6848.155507029029
1742 6848.159098945264
1743 6848.1623219759
1744 6848.16516711062
1745 6848.1676460372155
1746 6848.174534964221
1747 6848.189319930402
1748 6848.21440642253
1749 6848.245794395952
1750 6848.27600138195
1751 6848.304512232199
1752 6848.330608583518
1753 6848.349841364494
1754 6848.366628962069
1755 6848.389938082722
1756 6848.4202743575515
1757 6848.456529750935
1758 6848.497056749861
1759 6848.536473911618
1760 6848.569294094051
1761 6848.595178266286
1762 6848.619856242499
1763 6848.647587596347
1764 6848.677243177413
1765 6848.708275171935
1766 6848.738043417557
1767 6848.7647690649455
1768 6848.7886066933115
1769 6848.809206065121
1770 6848.826695587716
1771 6848.841248983357
1772 6848.852910990476
1773 6848.861710106493
1774 6848.867787045455
1775 6848.871285604104
1776 6848.8723142372955
1777 6848.871207154675
1778 6848.862443184849
1779 6848.846665989644
1780 6848.830205172636
1781 6848.807884553855
1782 6848.77538884572
1783 6848.734507967533
1784 6848.686520857602
1785 6848.625617181443
1786 6848.550896879872
1787 6848.468163521345
1788 6848.379758956657
1789 6848.289751248731
1790 6848.202594235269
1791 6848.121301163999
1792 6848.046441937634
1793 6847.978061635045
1794 6847.917092559449
1795 6847.864268582883
1796 6847.820144261293
1797 6847.7851489165805
1798 6847.760203550377
1799 6847.747239988809
1800 6847.743720132514
1801 6847.745976971112
1802 6847.753501866369
1803 6847.76542126371
1804 6847.780994541937
1805 6847.799510499399
1806 6847.8202597061045
1807 6847.842583906941
1808 6847.865608538656
1809 6847.888597539147
1810 6847.917252661357
1811 6847.956403842354
1812 6848.003268259775
1813 6848.051263746108
1814 6848.093082273722
1815 6848.124856935808
1816 6848.145005469009
1817 6848.154334395258
1818 6848.155111242225
1819 6848.148202078352
1820 6848.133423231198
1821 6848.111868835419
1822 6848.084713545351
1823 6848.053184084696
1824 6848.018529321301
1825 6847.981952722571
1826 6847.944590727757
1827 6847.907537347414
1828 6847.871920968072
1829 6847.83869174662
1830 6847.808588817195
1831 6847.78226601543
1832 6847.760222630424
1833 6847.742801111615
1834 6847.730182986442
1835 6847.722391608693
1836 6847.719279707902
1837 6847.7245271988295
1838 6847.742838056467
1839 6847.773001066889
1840 6847.812483742436
1841 6847.859740069519
1842 6847.912775790633
1843 6847.968728851653
1844 6848.024966812161
1845 6848.0800795230725
1846 6848.132806219268
1847 6848.182072153587
1848 6848.227006901527
1849 6848.266955792335
1850 6848.301520056876
1851 6848.330557920817
1852 6848.354132438191
1853 6848.372468733671
1854 6848.3859176522965
1855 6848.394302203688
1856 6848.397665465104
1857 6848.396849298442
1858 6848.39271419616
1859 6848.386115955468
1860 6848.377887669742
1861 6848.368811249441
1862 6848.359581263106
1863 6848.350776655223
1864 6848.342787962142
1865 6848.335846453464
1866 6848.330157239117
1867 6848.325924857197
1868 6848.32327673999
1869 6848.322221336902
1870 6848.322682948942
1871 6848.324532388138
1872 6848.327590895544
1873 6848.331643337442
1874 6848.336455047303
1875 6848.341786427837
1876 6848.347412928107
1877 6848.353139850833
1878 6848.3588045914685
1879 6848.364282320199
1880 6848.3694874884295
1881 6848.3743666619785
1882 6848.379087383683
1883 6848.383794353068
1884 6848.388425026243
1885 6848.3929456723345
1886 6848.398083024567
1887 6848.404486901466
1888 6848.411931640775
1889 6848.420025120691
1890 6848.42813625197
1891 6848.435503463915
1892 6848.441439919385
1893 6848.445475612298
1894 6848.4473943652665
1895 6848.447135022023
1896 6848.439026849145
1897 6848.4252627419955
1898 6848.41360268979
1899 6848.396789423769
1900 6848.368049858592
1901 6848.33795807924
1902 6848.317944058981
1903 6848.300232887178
1904 6848.277562494694
1905 6848.252918730671
1906 6848.228365182243
1907 6848.205514417659
1908 6848.185651859841
1909 6848.169548049856
1910 6848.157412501035
1911 6848.149097277658
1912 6848.144271276008
1913 6848.142599860886
1914 6848.1436541004105
1915 6848.146701867424
1916 6848.152838557697
1917 6848.161441941559
1918 6848.168133709153
1919 6848.170316347071
1920 6848.168942489778
1921 6848.165167516357
1922 6848.159140798473
1923 6848.159857204116
1924 6848.174914114921
1925 6848.201044792393
1926 6848.234152768349
1927 6848.270490040032
1928 6848.306452802888
1929 6848.338638857755
1930 6848.365315988968
1931 6848.386101518311
1932 6848.400715155027
1933 6848.409220621723
1934 6848.411948251526
1935 6848.409306752127
1936 6848.4020344761275
1937 6848.387036831892
1938 6848.36388074044
1939 6848.337917508161
1940 6848.312423205951
1941 6848.2870635461095
1942 6848.258680091573
1943 6848.225729498117
1944 6848.189673519328
1945 6848.152758981048
1946 6848.116825804666
1947 6848.083221180253
1948 6848.053079920282
1949 6848.026988261563
1950 6848.005058667691
1951 6847.987324633736
1952 6847.973729697185
1953 6847.964112733268
1954 6847.9586634743555
1955 6847.957000036059
1956 6847.9546801028755
1957 6847.9480171482155
1958 6847.9394697052
1959 6847.934267518238
1960 6847.9334287513575
1961 6847.934299496871
1962 6847.934144710529
1963 6847.929962880913
1964 6847.920543245645
1965 6847.90554018817
1966 6847.884564714685
1967 6847.857914818016
1968 6847.8259456820315
1969 6847.789648291762
1970 6847.749123089606
1971 6847.703212684566
1972 6847.651877498079
1973 6847.595400168032
1974 6847.534305411241
1975 6847.474142816961
1976 6847.421599245003
1977 6847.377522617893
1978 6847.341884077286
1979 6847.315460216234
1980 6847.298869679086
1981 6847.292298187578
1982 6847.295520731816
1983 6847.308291472453
1984 6847.3307245201495
1985 6847.3632231381835
1986 6847.405735931763
1987 6847.456890822788
1988 6847.514593637194
1989 6847.575752237188
1990 6847.637148373596
1991 6847.69699718814
1992 6847.754229326771
1993 6847.807643464848
1994 6847.855492465288
1995 6847.8962071946935
1996 6847.929530403577
1997 6847.955976000864
1998 6847.9755810650795
1999 6847.988032861582
2000 6847.992595363217

